Linear isoperimetric functions for surfaces in hyperbolic groups

We show that word-hyperbolic groups satisfy linear isoperimetric functions for all homotopy types of surface diagrams. This generalises the linear isoperimetric functions for disc and annular diagrams.

==> linearisopbob.tex <==
@article {OS20,
    AUTHOR = {Olshanskii, A. Yu. and Sapir, M. V.},
     TITLE = {Conjugacy problem in groups with quadratic {D}ehn function},
   JOURNAL = {Bull. Math. Sci.},
  FJOURNAL = {Bulletin of Mathematical Sciences},
    VOLUME = {10},
      YEAR = {2020},
    NUMBER = {1},
     PAGES = {1950023, 103},
      ISSN = {1664-3607},
   MRCLASS = {20F05 (03D35 20F06 20F65)},
  MRNUMBER = {4095947},
MRREVIEWER = {Jack O. Button},
       DOI = {10.1142/S1664360719500231},
       URL = {https://doi.org/10.1142/S1664360719500231},
}

@article {BH13,
    AUTHOR = {Buckley, D. J. and Holt, Derek F.},
     TITLE = {The conjugacy problem in hyperbolic groups for finite lists of
              group elements},
   JOURNAL = {Internat. J. Algebra Comput.},
  FJOURNAL = {International Journal of Algebra and Computation},
    VOLUME = {23},
      YEAR = {2013},
    NUMBER = {5},
     PAGES = {1127--1150},
      ISSN = {0218-1967},
   MRCLASS = {20F67 (20F10)},
  MRNUMBER = {3096315},
MRREVIEWER = {Richard Weidmann},
       DOI = {10.1142/S0218196713500203},
       URL = {https://doi.org/10.1142/S0218196713500203},
}
	

@book {Marden07,
    AUTHOR = {Marden, A.},
     TITLE = {Outer circles},
      NOTE = {An introduction to hyperbolic 3-manifolds},
 PUBLISHER = {Cambridge University Press, Cambridge},
      YEAR = {2007},
     PAGES = {xviii+427},
      ISBN = {978-0-521-83974-7},
   MRCLASS = {57-01 (20H10 30-02 30F40 57-02 57M50 57N10)},
  MRNUMBER = {2355387},
MRREVIEWER = {Bruno P. Zimmermann},
       DOI = {10.1017/CBO9780511618918},
       URL = {https://doi.org/10.1017/CBO9780511618918},
}
	

@article {ABDY13,
    AUTHOR = {Abrams, Aaron and Brady, Noel and Dani, Pallavi and Young,
              Robert},
     TITLE = {Homological and homotopical {D}ehn functions are different},
   JOURNAL = {Proc. Natl. Acad. Sci. USA},
  FJOURNAL = {Proceedings of the National Academy of Sciences of the United
              States of America},
    VOLUME = {110},
      YEAR = {2013},
    NUMBER = {48},
     PAGES = {19206--19212},
      ISSN = {0027-8424},
   MRCLASS = {20F65 (57M07)},
  MRNUMBER = {3153947},
MRREVIEWER = {Gilbert Levitt},
       DOI = {10.1073/pnas.1207377110},
       URL = {https://doi.org/10.1073/pnas.1207377110},
}
	

@article {MPE16,
    AUTHOR = {Mart\'{\i}nez-Pedroza, Eduardo},
     TITLE = {A note on fine graphs and homological isoperimetric
              inequalities},
   JOURNAL = {Canad. Math. Bull.},
  FJOURNAL = {Canadian Mathematical Bulletin. Bulletin Canadien de
              Math\'{e}matiques},
    VOLUME = {59},
      YEAR = {2016},
    NUMBER = {1},
     PAGES = {170--181},
      ISSN = {0008-4395},
   MRCLASS = {20F67 (05C10 20J05 55U15 57M20 57M60)},
  MRNUMBER = {3451908},
MRREVIEWER = {Stefan Witzel},
       DOI = {10.4153/CMB-2015-070-2},
       URL = {https://doi.org/10.4153/CMB-2015-070-2},
}

@article {Gersten1996,
    AUTHOR = {Gersten, S. M.},
     TITLE = {Subgroups of word hyperbolic groups in dimension {$2$}},
   JOURNAL = {J. London Math. Soc. (2)},
  FJOURNAL = {Journal of the London Mathematical Society. Second Series},
    VOLUME = {54},
      YEAR = {1996},
    NUMBER = {2},
     PAGES = {261--283},
      ISSN = {0024-6107},
   MRCLASS = {20F32 (20F06 57M07)},
  MRNUMBER = {1405055},
MRREVIEWER = {Athanase Papadopoulos},
       DOI = {10.1112/jlms/54.2.261},
       URL = {https://doi.org/10.1112/jlms/54.2.261},
}
	

@article {Mineyev2000,
    AUTHOR = {Mineyev, Igor},
     TITLE = {Higher dimensional isoperimetric functions in hyperbolic
              groups},
   JOURNAL = {Math. Z.},
  FJOURNAL = {Mathematische Zeitschrift},
    VOLUME = {233},
      YEAR = {2000},
    NUMBER = {2},
     PAGES = {327--345},
      ISSN = {0025-5874},
   MRCLASS = {20F67 (20F65 20J05 57M07)},
  MRNUMBER = {1743440},
MRREVIEWER = {Eric M. Freden},
       DOI = {10.1007/PL00004801},
       URL = {https://doi.org/10.1007/PL00004801},
}

@article {Gersten1998,
    AUTHOR = {Gersten, S. M.},
     TITLE = {Cohomological lower bounds for isoperimetric functions on
              groups},
   JOURNAL = {Topology},
  FJOURNAL = {Topology. An International Journal of Mathematics},
    VOLUME = {37},
      YEAR = {1998},
    NUMBER = {5},
     PAGES = {1031--1072},
      ISSN = {0040-9383},
   MRCLASS = {20F65 (20F06 57M05)},
  MRNUMBER = {1650363},
MRREVIEWER = {Jon M. Corson},
       DOI = {10.1016/S0040-9383(97)00070-0},
       URL = {https://doi.org/10.1016/S0040-9383(97)00070-0},
}

@article {Lang2000,
    AUTHOR = {Lang, Urs},
     TITLE = {Higher-dimensional linear isoperimetric inequalities in
              hyperbolic groups},
   JOURNAL = {Internat. Math. Res. Notices},
  FJOURNAL = {International Mathematics Research Notices},
      YEAR = {2000},
    NUMBER = {13},
     PAGES = {709--717},
      ISSN = {1073-7928},
   MRCLASS = {20F67},
  MRNUMBER = {1772520},
MRREVIEWER = {Stephen G. Brick},
       DOI = {10.1155/S1073792800000398},
       URL = {https://doi.org/10.1155/S1073792800000398},
}

@article {BridsonHowie05,
    AUTHOR = {Bridson, Martin R. and Howie, James},
     TITLE = {Conjugacy of finite subsets in hyperbolic groups},
   JOURNAL = {Internat. J. Algebra Comput.},
  FJOURNAL = {International Journal of Algebra and Computation},
    VOLUME = {15},
      YEAR = {2005},
    NUMBER = {4},
     PAGES = {725--756},
      ISSN = {0218-1967},
   MRCLASS = {20F67 (20F10 57M07 94A60)},
  MRNUMBER = {2160576},
MRREVIEWER = {Goulnara N. Arzhantseva},
       DOI = {10.1142/S0218196705002529},
       URL = {https://doi.org/10.1142/S0218196705002529},
}

@article {JMM1996,
    AUTHOR = {Juvan, M. and Malni\v{c}, A. and Mohar, B.},
     TITLE = {Systems of curves on surfaces},
   JOURNAL = {J. Combin. Theory Ser. B},
  FJOURNAL = {Journal of Combinatorial Theory. Series B},
    VOLUME = {68},
      YEAR = {1996},
    NUMBER = {1},
     PAGES = {7--22},
      ISSN = {0095-8956},
   MRCLASS = {57M15 (05C10)},
  MRNUMBER = {1405702},
       DOI = {10.1006/jctb.1996.0053},
       URL = {https://doi.org/10.1006/jctb.1996.0053},
}

@incollection {Bridson2002,
    AUTHOR = {Bridson, Martin R.},
     TITLE = {The geometry of the word problem},
 BOOKTITLE = {Invitations to geometry and topology},
    SERIES = {Oxf. Grad. Texts Math.},
    VOLUME = {7},
     PAGES = {29--91},
 PUBLISHER = {Oxford Univ. Press, Oxford},
      YEAR = {2002},
   MRCLASS = {20F65 (20F10 49J05 57M07)},
  MRNUMBER = {1967746},
MRREVIEWER = {Ross Geoghegan},
}

@article {BurilloTaback2002,
    AUTHOR = {Burillo, Jos\'{e} and Taback, Jennifer},
     TITLE = {Equivalence of geometric and combinatorial {D}ehn functions},
   JOURNAL = {New York J. Math.},
  FJOURNAL = {New York Journal of Mathematics},
    VOLUME = {8},
      YEAR = {2002},
     PAGES = {169--179},
   MRCLASS = {20F65 (49Q15 53C20 57M07)},
  MRNUMBER = {1934388},
MRREVIEWER = {Stephen G. Brick},
       URL = {http://nyjm.albany.edu:8000/j/2002/8_169.html},
}

@article {WiseVanishingL2B2,
    AUTHOR = {Wise, Daniel T.},
     TITLE = {A note on the vanishing of the 2nd {$L^2$}-{B}etti number},
      JOURNAL = {Proc. Amer. Math. Soc.},
  FJOURNAL = {Proceedings of the American Mathematical Society},
     PAGES = {1--6},
Note={To appear},
}


@article {Magnus1935,
    AUTHOR = {Magnus, Wilhelm},
     TITLE = {Beziehungen zwischen {G}ruppen und {I}dealen in einem
              speziellen {R}ing},
   JOURNAL = {Math. Ann.},
  FJOURNAL = {Mathematische Annalen},
    VOLUME = {111},
      YEAR = {1935},
    NUMBER = {1},
     PAGES = {259--280},
      ISSN = {0025-5831},
   MRCLASS = {DML},
  MRNUMBER = {1512992},
       DOI = {10.1007/BF01472217},
       URL = {https://doi-org.proxy3.library.mcgill.ca/10.1007/BF01472217},
}

@article {Bahls2007,
    AUTHOR = {Bahls, Patrick},
     TITLE = {The group {$\rm BS(1,2)$} and a construction of {M}agnus},
   JOURNAL = {Comm. Algebra},
  FJOURNAL = {Communications in Algebra},
    VOLUME = {35},
      YEAR = {2007},
    NUMBER = {12},
     PAGES = {4088--4095},
      ISSN = {0092-7872},
   MRCLASS = {20F05 (20F60 20M05)},
  MRNUMBER = {2372320},
MRREVIEWER = {Carl Droms},
       DOI = {10.1080/00927870701544831},
       URL = {https://doi-org.proxy3.library.mcgill.ca/10.1080/00927870701544831},
}

@article {FujiwaraPapasoglu2006,
    AUTHOR = {Fujiwara, K. and Papasoglu, P.},
     TITLE = {J{SJ}-decompositions of finitely presented groups and
              complexes of groups},
   JOURNAL = {Geom. Funct. Anal.},
  FJOURNAL = {Geometric and Functional Analysis},
    VOLUME = {16},
      YEAR = {2006},
    NUMBER = {1},
     PAGES = {70--125},
      ISSN = {1016-443X},
   MRCLASS = {20F65 (20E08 57M07)},
  MRNUMBER = {2221253},
MRREVIEWER = {Matt T. Clay},
       DOI = {10.1007/s00039-006-0550-2},
       URL = {https://doi-org.proxy3.library.mcgill.ca/10.1007/s00039-006-0550-2},
}
	

@article {DunwoodySageev99,
    AUTHOR = {Dunwoody, M. J. and Sageev, M. E.},
     TITLE = {J{SJ}-splittings for finitely presented groups over slender
              groups},
   JOURNAL = {Invent. Math.},
  FJOURNAL = {Inventiones Mathematicae},
    VOLUME = {135},
      YEAR = {1999},
    NUMBER = {1},
     PAGES = {25--44},
      ISSN = {0020-9910},
   MRCLASS = {20F65 (20E06 20E08 57M05 57M07 57N10)},
  MRNUMBER = {1664694},
MRREVIEWER = {Thomas Delzant},
       DOI = {10.1007/s002220050278},
       URL = {https://doi-org.proxy3.library.mcgill.ca/10.1007/s002220050278},
}
	

@incollection {Stallings2002,
    AUTHOR = {Stallings, John R.},
     TITLE = {An extension theorem for {E}uler characteristics of groups},
      NOTE = {Dedicated to John Stallings on the occasion of his 65th
              birthday},
   JOURNAL = {Geom. Dedicata},
  FJOURNAL = {Geometriae Dedicata},
    VOLUME = {92},
      YEAR = {2002},
     PAGES = {3--39},
      ISSN = {0046-5755},
   MRCLASS = {20J05 (16E05)},
  MRNUMBER = {1934007},
MRREVIEWER = {Kenneth A. Brown},
       DOI = {10.1023/A:1019696726402},
       URL = {https://doi-org.proxy3.library.mcgill.ca/10.1023/A:1019696726402},
}
	

  @article{KielakVAF,
Author = {Dawid Kielak},
Title = {Residually finite rationally-solvable groups and virtual fibering},
Year = {2018},
Eprint = {arXiv:1809.09386},
}

@misc{LouderWiltonNegative2018,
Author = {Larsen Louder and Henry Wilton},
Title = {Negative immersions for one-relator groups},
Year = {2018},
Eprint = {arXiv:1803.02671},
}

@misc{LouderWilton2018,
Author = {Larsen Louder and Henry Wilton},
Title = {One-relator groups with torsion are coherent},
Year = {2018},
Eprint = {arXiv:1805.11976},
}

@book{BurilloThompsonBook,
    AUTHOR = {Jos{\'e} Burillo},
     TITLE = {Introduction to Thompson's group F},
 URL = {https://mat-web.upc.edu/people/pep.burillo/F%20book.pdf},
      YEAR = {2019},
     PAGES = {1--85},
     }


@article {Bagherzadeh1976,
    AUTHOR = {Bagherzadeh, G. H.},
     TITLE = {Commutativity in one-relator groups},
   JOURNAL = {J. London Math. Soc. (2)},
  FJOURNAL = {Journal of the London Mathematical Society. Second Series},
    VOLUME = {13},
      YEAR = {1976},
    NUMBER = {3},
     PAGES = {459--471},
      ISSN = {0024-6107},
   MRCLASS = {20F05},
  MRNUMBER = {0407158},
MRREVIEWER = {D. E. Cohen},
       DOI = {10.1112/jlms/s2-13.3.459},
       URL = {https://doi-org.proxy3.library.mcgill.ca/10.1112/jlms/s2-13.3.459},
}


@misc{Tran2017,
Author = {Hung Cong Tran},
Title = {Malnormality and join-free subgroups in right-angled Coxeter groups},
Year = {2017},
Eprint = {arXiv:1703.09032},
}

@article {BorisovSapir2005,
    AUTHOR = {Borisov, Alexander and Sapir, Mark},
     TITLE = {Polynomial maps over finite fields and residual finiteness of mapping tori of group endomorphisms},
   JOURNAL = {Invent. Math.},
  FJOURNAL = {Inventiones Mathematicae},
    VOLUME = {160},
      YEAR = {2005},
    NUMBER = {2},
     PAGES = {341--356},
      ISSN = {0020-9910},
   MRCLASS = {20E06 (20E26)},
  MRNUMBER = {2138070},
MRREVIEWER = {Martin Edjvet},
       DOI = {10.1007/s00222-004-0411-2},
       URL = {https://doi-org.proxy3.library.mcgill.ca/10.1007/s00222-004-0411-2},
}

@article {KoptevaHowie2006,
    AUTHOR = {Howie, James and Kopteva, Natalia},
     TITLE = {The {T}its alternative for generalized tetrahedron groups},
   JOURNAL = {J. Group Theory},
  FJOURNAL = {Journal of Group Theory},
    VOLUME = {9},
      YEAR = {2006},
    NUMBER = {2},
     PAGES = {173--189},
      ISSN = {1433-5883},
   MRCLASS = {20F05 (20F65)},
  MRNUMBER = {2220573},
MRREVIEWER = {Fabio Scarabotti},
       DOI = {10.1515/JGT.2006.012},
       URL = {https://doi-org.proxy3.library.mcgill.ca/10.1515/JGT.2006.012},
}

@article {Dehn1911,
    AUTHOR = {Dehn, M.},
     TITLE = {\"{U}ber unendliche diskontinuierliche {G}ruppen},
   JOURNAL = {Math. Ann.},
  FJOURNAL = {Mathematische Annalen},
    VOLUME = {71},
      YEAR = {1911},
    NUMBER = {1},
     PAGES = {116--144},
      ISSN = {0025-5831},
   MRCLASS = {DML},
  MRNUMBER = {1511645},
       DOI = {10.1007/BF01456932},
       URL = {https://doi-org.proxy3.library.mcgill.ca/10.1007/BF01456932},
}

@article{FuterWise2017,
Author = { David Futer and Daniel T. Wise},
Title = {Generic Curves and Sectional Curvature},
Pages = {1--17},
Note = {in preparation},
Year = {2016},
}


@MastersThesis{DellaVecciaMSc2016,
  author =   { Antony Della Veccia},
  title =    {Sectional Curvature of One-Relator Groups},
  school =   {McGill University},
  year =     {2016},
}


@article {Farrell76,
    AUTHOR = {Farrell, F. Thomas},
     TITLE = {Right-orderable deck transformation groups},
   JOURNAL = {Rocky Mountain J. Math.},
  FJOURNAL = {The Rocky Mountain Journal of Mathematics},
    VOLUME = {6},
      YEAR = {1976},
    NUMBER = {3},
     PAGES = {441--447},
      ISSN = {0035-7596},
   MRCLASS = {55A10 (06A55)},
  MRNUMBER = {0418078},
MRREVIEWER = {Leonard R. Rubin},
       DOI = {10.1216/RMJ-1976-6-3-441},
       URL = {https://doi-org.proxy3.library.mcgill.ca/10.1216/RMJ-1976-6-3-441},
}


@misc{Lueck2003v1,
Author = {Wolfgang Lueck},
Title = {{$L^2$}-Invariants from the Algebraic Point of View},
Year = {2003},
Eprint = {arXiv:math/0310489v1},
}

@article {GrigorchukWilson2003,
    AUTHOR = {Grigorchuk, R. I. and Wilson, J. S.},
     TITLE = {A structural property concerning abstract commensurability of
              subgroups},
   JOURNAL = {J. London Math. Soc. (2)},
  FJOURNAL = {Journal of the London Mathematical Society. Second Series},
    VOLUME = {68},
      YEAR = {2003},
    NUMBER = {3},
     PAGES = {671--682},
      ISSN = {0024-6107},
   MRCLASS = {20F10 (20E08 20E34)},
  MRNUMBER = {2009443},
MRREVIEWER = {Tullio G. Ceccherini-Silberstein},
       DOI = {10.1112/S0024610703004745},
       URL = {https://doi-org.proxy3.library.mcgill.ca/10.1112/S0024610703004745},
}

@article {McCammond2017,
    AUTHOR = {McCammond, Jonathan P.},
     TITLE = {The mysterious geometry of Artin groups},
      PAGES = {1--44},
      YEAR = {2017},
URL = { http://web.math.ucsb.edu/~jon.mccammond/papers/mysterious- geometry.pdf},
 }

@article {WiseLastArtin2013,
    AUTHOR = {Wise, Daniel T.},
     TITLE = {The last incoherent {A}rtin group},
   JOURNAL = {Proc. Amer. Math. Soc.},
  FJOURNAL = {Proceedings of the American Mathematical Society},
    VOLUME = {141},
      YEAR = {2013},
    NUMBER = {1},
     PAGES = {139--149},
      ISSN = {0002-9939},
   MRCLASS = {20F36 (20F05)},
  MRNUMBER = {2988718},
MRREVIEWER = {Luis Paris},
       DOI = {10.1090/S0002-9939-2012-11507-2},
       URL = {https://doi-org.proxy3.library.mcgill.ca/10.1090/S0002-9939-2012-11507-2},
}



@article {Dodziuk79,
    AUTHOR = {Dodziuk, Jozef},
     TITLE = {{$L^{2}$} harmonic forms on rotationally symmetric
              {R}iemannian manifolds},
   JOURNAL = {Proc. Amer. Math. Soc.},
  FJOURNAL = {Proceedings of the American Mathematical Society},
    VOLUME = {77},
      YEAR = {1979},
    NUMBER = {3},
     PAGES = {395--400},
      ISSN = {0002-9939},
   MRCLASS = {58A14 (53C99 58G99)},
  MRNUMBER = {545603},
MRREVIEWER = {H. Wu},
       DOI = {10.2307/2042193},
       URL = {https://doi-org.proxy3.library.mcgill.ca/10.2307/2042193},
}

@article {Luck1994,
    AUTHOR = {L\"{u}ck, W.},
     TITLE = {Approximating {$L^2$}-invariants by their finite-dimensional
              analogues},
   JOURNAL = {Geom. Funct. Anal.},
  FJOURNAL = {Geometric and Functional Analysis},
    VOLUME = {4},
      YEAR = {1994},
    NUMBER = {4},
     PAGES = {455--481},
      ISSN = {1016-443X},
   MRCLASS = {58G12 (46L85 57Q10)},
  MRNUMBER = {1280122},
MRREVIEWER = {Peter Haskell},
       DOI = {10.1007/BF01896404},
       URL = {https://doi-org.proxy3.library.mcgill.ca/10.1007/BF01896404},
}
	

@article{BambergerCarrierGasterWise2019,
Author={Jacob Bamberger and David Carrier and Jonah Gaster and Daniel T. Wise},
Title={Stackings and Bislim Structures},
Pages ={1--10},
Year={2019},
}

@article {Mineyev2012graphs,
    AUTHOR = {Mineyev, Igor},
     TITLE = {Groups, graphs, and the {H}anna {N}eumann conjecture},
   JOURNAL = {J. Topol. Anal.},
  FJOURNAL = {Journal of Topology and Analysis},
    VOLUME = {4},
      YEAR = {2012},
    NUMBER = {1},
     PAGES = {1--12},
      ISSN = {1793-5253},
   MRCLASS = {20E05 (05C10 20E07 20E08)},
  MRNUMBER = {2914871},
MRREVIEWER = {Gary L. Walls},
       DOI = {10.1142/S1793525312500045},
       URL = {https://doi-org.proxy3.library.mcgill.ca/10.1142/S1793525312500045},
}
	

@article {CullerShalen2012,
    AUTHOR = {Culler, Marc and Shalen, Peter B.},
     TITLE = {4-free groups and hyperbolic geometry},
   JOURNAL = {J. Topol.},
  FJOURNAL = {Journal of Topology},
    VOLUME = {5},
      YEAR = {2012},
    NUMBER = {1},
     PAGES = {81--136},
      ISSN = {1753-8416},
   MRCLASS = {57M50},
  MRNUMBER = {2897050},
MRREVIEWER = {Colin C. Adams},
       DOI = {10.1112/jtopol/jtr028},
       URL = {https://doi-org.proxy3.library.mcgill.ca/10.1112/jtopol/jtr028},
}


@article {Guba86,
    AUTHOR = {Guba, V. S.},
     TITLE = {Conditions under which {$2$}-generated subgroups in small
              cancellation groups are free},
   JOURNAL = {Izv. Vyssh. Uchebn. Zaved. Mat.},
  FJOURNAL = {Izvestiya Vysshikh Uchebnykh Zavedeni\u{\i}. Matematika},
      YEAR = {1986},
    NUMBER = {7},
     PAGES = {12--19, 87},
      ISSN = {0021-3446},
   MRCLASS = {20F05 (20F26)},
  MRNUMBER = {867603},
MRREVIEWER = {M. Greendlinger},
}
	
 
  
@article {Dymara2004,
    AUTHOR = {Dymara, Jan},
     TITLE = {{$L^2$}-cohomology of buildings with fundamental class},
   JOURNAL = {Proc. Amer. Math. Soc.},
  FJOURNAL = {Proceedings of the American Mathematical Society},
    VOLUME = {132},
      YEAR = {2004},
    NUMBER = {6},
     PAGES = {1839--1843},
      ISSN = {0002-9939},
   MRCLASS = {58J22 (20F55 20F65)},
  MRNUMBER = {2051148},
MRREVIEWER = {Alain Valette},
       DOI = {10.1090/S0002-9939-03-07234-4},
       URL = {https://doi-org.proxy3.library.mcgill.ca/10.1090/S0002-9939-03-07234-4},
}
	

@article {BourdonPajot2003,
    AUTHOR = {Bourdon, Marc and Pajot, Herv\'{e}},
     TITLE = {Cohomologie {$l_p$} et espaces de {B}esov},
   JOURNAL = {J. Reine Angew. Math.},
  FJOURNAL = {Journal f\"{u}r die Reine und Angewandte Mathematik. [Crelle's
              Journal]},
    VOLUME = {558},
      YEAR = {2003},
     PAGES = {85--108},
      ISSN = {0075-4102},
   MRCLASS = {20F67 (30F45 46E30)},
  MRNUMBER = {1979183},
MRREVIEWER = {Jeremy T. Tyson},
       DOI = {10.1515/crll.2003.043},
       URL = {https://doi-org.proxy3.library.mcgill.ca/10.1515/crll.2003.043},
}

@article{Wise2019CoherenceNote,
author={Wise, Daniel T.},
title={A Note on the Coherence of 3-manifold groups},
pages = {1--4},
year={2019},
}

@article {KleinerLott2008,
    AUTHOR = {Kleiner, Bruce and Lott, John},
     TITLE = {Notes on {P}erelman's papers},
   JOURNAL = {Geom. Topol.},
  FJOURNAL = {Geometry \& Topology},
    VOLUME = {12},
      YEAR = {2008},
    NUMBER = {5},
     PAGES = {2587--2855},
      ISSN = {1465-3060},
   MRCLASS = {53C44 (57M40)},
  MRNUMBER = {2460872},
MRREVIEWER = {G\'{e}rard Besson},
       DOI = {10.2140/gt.2008.12.2587},
       URL = {https://doi-org.proxy3.library.mcgill.ca/10.2140/gt.2008.12.2587},
}
	

@article {Scott83geometries,
    AUTHOR = {Scott, Peter},
     TITLE = {The geometries of {$3$}-manifolds},
   JOURNAL = {Bull. London Math. Soc.},
  FJOURNAL = {The Bulletin of the London Mathematical Society},
    VOLUME = {15},
      YEAR = {1983},
    NUMBER = {5},
     PAGES = {401--487},
      ISSN = {0024-6093},
   MRCLASS = {57N10 (22E10 53C20)},
  MRNUMBER = {705527},
MRREVIEWER = {John Hempel},
       DOI = {10.1112/blms/15.5.401},
       URL = {https://doi-org.proxy3.library.mcgill.ca/10.1112/blms/15.5.401},
}
	

@incollection{WiseCoherenceSurvey,
author={Wise, Daniel T.},
title={An Invitation to Coherent Groups},
booktitle = {What's Next?: The Mathematical Legacy of William P. Thurston},
   EDITOR = {Thurston, Dylan},
   publisher = {Princeton University Press},
pages = {1--89},
note={To appear.},
year={2020},
}


@misc{Swarup2004,
Author = {Gadde A. Swarup},
Title = {Delzant's variation on Scott complexity},
Year = {2004},
Eprint = {arXiv:math/0401308},
}

@article {Delzant1995,
    AUTHOR = {Delzant, T.},
     TITLE = {L'image d'un groupe dans un groupe hyperbolique},
   JOURNAL = {Comment. Math. Helv.},
  FJOURNAL = {Commentarii Mathematici Helvetici},
    VOLUME = {70},
      YEAR = {1995},
    NUMBER = {2},
     PAGES = {267--284},
      ISSN = {0010-2571},
   MRCLASS = {20F32 (57M07)},
  MRNUMBER = {1324630},
MRREVIEWER = {Tadeusz Januszkiewicz},
       DOI = {10.1007/BF02566008},
       URL = {https://doi-org.proxy3.library.mcgill.ca/10.1007/BF02566008},
}
	
@article {Baumslag1950,
    AUTHOR = {Baumslag, Gilbert},
     TITLE = {Some aspects of groups with unique roots},
   JOURNAL = {Acta Math.},
  FJOURNAL = {Acta Mathematica},
    VOLUME = {104},
      YEAR = {1960},
     PAGES = {217--303},
      ISSN = {0001-5962},
   MRCLASS = {20.08},
  MRNUMBER = {0122859},
MRREVIEWER = {B. H. Neumann},
       DOI = {10.1007/BF02546390},
       URL = {https://doi-org.proxy3.library.mcgill.ca/10.1007/BF02546390},
}

@article{DahmaniMj2016,
Author = {Francois Dahmani and Mahan Mj},
Title = {Height, Graded Relative Hyperbolicity and Quasiconvexity},
Year = {2017},
journal = {Journal d'Ecole Polytechnique},
pages={515--556},
volume={4},
}

@article {BurnsChauSolitar77,
    AUTHOR = {Burns, R. G. and Chau, T. C. and Solitar, D.},
     TITLE = {On the intersection of free factors of a free group},
   JOURNAL = {Proc. Amer. Math. Soc.},
  FJOURNAL = {Proceedings of the American Mathematical Society},
    VOLUME = {64},
      YEAR = {1977},
    NUMBER = {1},
     PAGES = {43--44},
      ISSN = {0002-9939},
   MRCLASS = {20E05},
  MRNUMBER = {0447405},
MRREVIEWER = {Peter M. Neumann},
       DOI = {10.2307/2040977},
       URL = {https://doi.org/10.2307/2040977},
}


@article {Hagen2013,
    AUTHOR = {Hagen, Mark F.},
     TITLE = {The simplicial boundary of a {CAT}(0) cube complex},
   JOURNAL = {Algebr. Geom. Topol.},
  FJOURNAL = {Algebraic \& Geometric Topology},
    VOLUME = {13},
      YEAR = {2013},
    NUMBER = {3},
     PAGES = {1299--1367},
      ISSN = {1472-2747},
   MRCLASS = {20F65 (05C25)},
  MRNUMBER = {3071129},
MRREVIEWER = {Tetsu Toyoda},
       DOI = {10.2140/agt.2013.13.1299},
       URL = {https://doi-org.proxy3.library.mcgill.ca/10.2140/agt.2013.13.1299},
}

@article {JacoShalen79,
    AUTHOR = {Jaco, William H. and Shalen, Peter B.},
     TITLE = {Seifert fibered spaces in {$3$}-manifolds},
   JOURNAL = {Mem. Amer. Math. Soc.},
  FJOURNAL = {Memoirs of the American Mathematical Society},
    VOLUME = {21},
      YEAR = {1979},
    NUMBER = {220},
     PAGES = {viii+192},
      ISSN = {0065-9266},
   MRCLASS = {57N10},
  MRNUMBER = {539411},
MRREVIEWER = {Hugh M. Hilden},
       DOI = {10.1090/memo/0220},
       URL = {https://doi-org.proxy3.library.mcgill.ca/10.1090/memo/0220},
}

@article{HuangWiseSeparability,
author={Huang, Jingyin and Wise, Daniel T.},
title={Stature and Separability in Graphs of Groups},
pages = {1--31},
journal={Preprint},
year={2018},
}

@article{HuangWiseSpecial,
author={Huang, Jingyin and Wise, Daniel T.},
title={Virtual Specialness of Certain Graphs of Special Cube Complexes},
pages = {1--27},
journal={Preprint},
year={2018},
}

@article {LyndonSchutzenberger62,
    AUTHOR = {Lyndon, R. C. and Sch\"{u}tzenberger, M. P.},
     TITLE = {The equation {$a^{M}=b^{N}c^{P}$} in a free group},
   JOURNAL = {Michigan Math. J.},
  FJOURNAL = {The Michigan Mathematical Journal},
    VOLUME = {9},
      YEAR = {1962},
     PAGES = {289--298},
      ISSN = {0026-2285},
   MRCLASS = {20.10},
  MRNUMBER = {0162838},
MRREVIEWER = {M. Greendlinger},
       URL = {http://projecteuclid.org.proxy3.library.mcgill.ca/euclid.mmj/1028998766},
}

@article {MR3856793,
    AUTHOR = {Coulon, R\'{e}mi and Dal'Bo, Fran\c{c}oise and Sambusetti, Andrea},
     TITLE = {Growth gap in hyperbolic groups and amenability},
   JOURNAL = {Geom. Funct. Anal.},
  FJOURNAL = {Geometric and Functional Analysis},
    VOLUME = {28},
      YEAR = {2018},
    NUMBER = {5},
     PAGES = {1260--1320},
      ISSN = {1016-443X},
   MRCLASS = {43A07},
  MRNUMBER = {3856793},
       DOI = {10.1007/s00039-018-0459-6},
       URL = {https://doi.org/10.1007/s00039-018-0459-6},
}


@article {Kim04,
    AUTHOR = {Kim, Goansu},
     TITLE = {On the residual finiteness of fundamental groups of graphs of
              certain groups},
   JOURNAL = {J. Korean Math. Soc.},
  FJOURNAL = {Journal of the Korean Mathematical Society},
    VOLUME = {41},
      YEAR = {2004},
    NUMBER = {5},
     PAGES = {913--920},
      ISSN = {0304-9914},
   MRCLASS = {20E26 (20E06 20E08)},
  MRNUMBER = {2081764},
MRREVIEWER = {Thomas Weigel},
       DOI = {10.4134/JKMS.2004.41.5.913},
       URL = {https://doi-org.proxy3.library.mcgill.ca/10.4134/JKMS.2004.41.5.913},
}


@article {CollinsEdjvetGill1994,
    AUTHOR = {Collins, D. J. and Edjvet, M. and Gill, C. P.},
     TITLE = {Growth series for the group {$\langle x,y|\
              x^{-1}yx=y^l\rangle$}},
   JOURNAL = {Arch. Math. (Basel)},
  FJOURNAL = {Archiv der Mathematik},
    VOLUME = {62},
      YEAR = {1994},
    NUMBER = {1},
     PAGES = {1--11},
      ISSN = {0003-889X},
   MRCLASS = {20F10 (20E06 20F05)},
  MRNUMBER = {1249578},
MRREVIEWER = {John S. Wilson},
       DOI = {10.1007/BF01200431},
       URL = {https://doi-org.proxy3.library.mcgill.ca/10.1007/BF01200431},
}

@article {BucherTalambutsa2017,
    AUTHOR = {Bucher, Michelle and Talambutsa, Alexey},
     TITLE = {Minimal exponential growth rates of metabelian
              {B}aumslag-{S}olitar groups and lamplighter groups},
   JOURNAL = {Groups Geom. Dyn.},
  FJOURNAL = {Groups, Geometry, and Dynamics},
    VOLUME = {11},
      YEAR = {2017},
    NUMBER = {1},
     PAGES = {189--209},
      ISSN = {1661-7207},
   MRCLASS = {20F69 (20F16)},
  MRNUMBER = {3641839},
MRREVIEWER = {Alla S. Detinko},
       DOI = {10.4171/GGD/394},
       URL = {https://doi-org.proxy3.library.mcgill.ca/10.4171/GGD/394},
}

@article{BambergerCarrierGasterWise2018,
    AUTHOR = {Bamberger, Jacob, and Carrier, David and Gaster, Jonah and Wise, Daniel T.},
  TITLE = {Good Stackings, Bislim Structures, and Equivariant Staggerings},
   NOTE = {Preprint 2018},
 PAGES = {1--7},
}

@book {CassonBleiler88,
    AUTHOR = {Casson, Andrew J. and Bleiler, Steven A.},
     TITLE = {Automorphisms of surfaces after {N}ielsen and {T}hurston},
    SERIES = {London Mathematical Society Student Texts},
    VOLUME = {9},
 PUBLISHER = {Cambridge University Press, Cambridge},
      YEAR = {1988},
     PAGES = {iv+105},
      ISBN = {0-521-34203-1},
   MRCLASS = {57N05 (32G15 57R30 58F15)},
  MRNUMBER = {964685},
MRREVIEWER = {William Dunbar},
       DOI = {10.1017/CBO9780511623912},
       URL = {https://doi-org.proxy3.library.mcgill.ca/10.1017/CBO9780511623912},
}

@book {minc:nonnegative,
    AUTHOR = {Minc, Henryk},
     TITLE = {Nonnegative matrices},
    SERIES = {Wiley-Interscience Series in Discrete Mathematics and  Optimization},
      NOTE = {A Wiley-Interscience Publication},
 PUBLISHER = {John Wiley \& Sons, Inc., New York},
      YEAR = {1988},
     PAGES = {xiv+206},
      ISBN = {0-471-83966-3},
   MRCLASS = {15-02 (15A48)},
  MRNUMBER = {932967 (89i:15001)},
MRREVIEWER = {Thomas L. Markham},
}

@incollection {BestvinaFeighn2009,
    AUTHOR = {Bestvina, Mladen and Feighn, Mark},
     TITLE = {Notes on {S}ela's work: limit groups and {M}akanin-{R}azborov diagrams},
 BOOKTITLE = {Geometric and cohomological methods in group theory},
    SERIES = {London Math. Soc. Lecture Note Ser.},
    VOLUME = {358},
     PAGES = {1--29},
 PUBLISHER = {Cambridge Univ. Press, Cambridge},
      YEAR = {2009},
   MRCLASS = {20F70 (20E08 20F65)},
  MRNUMBER = {2605174},
MRREVIEWER = {Henry Wilton},
}


@article {CoulonDalboSambusetti2018,
    AUTHOR = {Coulon, R\'{e}mi and Dal'Bo, Fran\c{c}oise and Sambusetti, Andrea},
     TITLE = {Growth gap in hyperbolic groups and amenability},
   JOURNAL = {Geom. Funct. Anal.},
  FJOURNAL = {Geometric and Functional Analysis},
    VOLUME = {28},
      YEAR = {2018},
    NUMBER = {5},
     PAGES = {1260--1320},
      ISSN = {1016-443X},
   MRCLASS = {43A07},
  MRNUMBER = {3856793},
       DOI = {10.1007/s00039-018-0459-6},
       URL = {https://doi.org/10.1007/s00039-018-0459-6},
}

@article{Dougall2017,
Author = {Rhiannon Dougall},
Title = {Critical exponents of normal subgroups, the spectrum of group extended transfer operators, and Kazhdan distance},
Year = {2017},
Note = {to appear.},
JOURNAL = {Adv. Math.},
Eprint = {arXiv:1702.06115},
}


	
@article {DougallSharp2016,
    AUTHOR = {Dougall, Rhiannon and Sharp, Richard},
     TITLE = {Amenability, critical exponents of subgroups and growth of closed geodesics},
   JOURNAL = {Math. Ann.},
  FJOURNAL = {Mathematische Annalen},
    VOLUME = {365},
      YEAR = {2016},
    NUMBER = {3-4},
     PAGES = {1359--1377},
      ISSN = {0025-5831},
   MRCLASS = {37D40 (53C22)},
  MRNUMBER = {3521093},
MRREVIEWER = {Thomas Barthelm\'e},
       DOI = {10.1007/s00208-015-1338-1},
       URL = {https://doi-org.proxy3.library.mcgill.ca/10.1007/s00208-015-1338-1},
}


@article {RipsSela97,
    AUTHOR = {Rips, E. and Sela, Z.},
     TITLE = {Cyclic splittings of finitely presented groups and the
              canonical {JSJ} decomposition},
   JOURNAL = {Ann. of Math. (2)},
  FJOURNAL = {Annals of Mathematics. Second Series},
    VOLUME = {146},
      YEAR = {1997},
    NUMBER = {1},
     PAGES = {53--109},
      ISSN = {0003-486X},
   MRCLASS = {20F32 (20E06 20F34 57M05 57M07)},
  MRNUMBER = {1469317},
MRREVIEWER = {Thomas Delzant},
       DOI = {10.2307/2951832},
       URL = {https://doi-org.proxy3.library.mcgill.ca/10.2307/2951832},
}

@article{LiWise2017,
    AUTHOR = {Li, Jiakai and Wise, Daniel T.},
     TITLE = {No Growth Gaps for Special Cube Complexes},
       NOTE = {Submitted},
          JOURNAL = {Math. Proc. Cambridge Philos. Soc.},
  FJOURNAL = {Mathematical Proceedings of the Cambridge Philosophical Society},
           PAGES = {1--13},
}

@article {HarlanderRosebrock2017,
    AUTHOR = {Harlander, Jens and Rosebrock, Stephan},
     TITLE = {Injective labeled oriented trees are aspherical},
   JOURNAL = {Math. Z.},
  FJOURNAL = {Mathematische Zeitschrift},
    VOLUME = {287},
      YEAR = {2017},
    NUMBER = {1-2},
     PAGES = {199--214},
      ISSN = {0025-5874},
   MRCLASS = {57M20 (20F05 57M05)},
  MRNUMBER = {3694674},
       DOI = {10.1007/s00209-016-1823-6},
       URL = {https://doi-org.proxy3.library.mcgill.ca/10.1007/s00209-016-1823-6},
}
	

@article{Woodhouse15VirtuallySpecial,
    AUTHOR = {Woodhouse, Daniel J.},
     TITLE = {Classifying virtually special tubular groups},
   JOURNAL = {Groups Geom. Dyn.},
  FJOURNAL = {Groups, Geometry, and Dynamics},
    VOLUME = {12},
      YEAR = {2018},
    NUMBER = {2},
     PAGES = {679--702},
      ISSN = {1661-7207},
   MRCLASS = {20F67 (20E06 20F65)},
  MRNUMBER = {3813206},
MRREVIEWER = {Christopher H. Cashen},
       DOI = {10.4171/GGD/452},
       URL = {https://doi-org.proxy3.library.mcgill.ca/10.4171/GGD/452},
}


@article {AndreadakisRaptisVarsos88,
    AUTHOR = {Andreadakis, S. and Raptis, E. and Varsos, D.},
     TITLE = {A characterization of residually finite {HNN}-extensions of
              finitely generated abelian groups},
   JOURNAL = {Arch. Math. (Basel)},
  FJOURNAL = {Archiv der Mathematik},
    VOLUME = {50},
      YEAR = {1988},
    NUMBER = {6},
     PAGES = {495--501},
      ISSN = {0003-889X},
   MRCLASS = {20E06 (20E26)},
  MRNUMBER = {948263},
MRREVIEWER = {David Meier},
       DOI = {10.1007/BF01193619},
       URL = {http://dx.doi.org/10.1007/BF01193619},
}

@article {Button17,
    AUTHOR = {Button, Jack},
     TITLE = {Tubular free by cyclic groups act freely on {CAT}(0) cube
              complexes},
   JOURNAL = {Canad. Math. Bull.},
  FJOURNAL = {Canadian Mathematical Bulletin. Bulletin Canadien de
              Math\'ematiques},
    VOLUME = {60},
      YEAR = {2017},
    NUMBER = {1},
     PAGES = {54--62},
      ISSN = {0008-4395},
   MRCLASS = {20F65 (20E08 20E22 20F67)},
  MRNUMBER = {3612098},
MRREVIEWER = {Mark F. Hagen},
       DOI = {10.4153/CMB-2016-074-0},
       URL = {http://dx.doi.org/10.4153/CMB-2016-074-0},
}
		
		@article {ManningMartinez2010,
    AUTHOR = {Manning, Jason Fox and Mart\'\i nez-Pedroza, Eduardo},
     TITLE = {Separation of relatively quasiconvex subgroups},
   JOURNAL = {Pacific J. Math.},
  FJOURNAL = {Pacific Journal of Mathematics},
    VOLUME = {244},
      YEAR = {2010},
    NUMBER = {2},
     PAGES = {309--334},
      ISSN = {0030-8730},
   MRCLASS = {20F67 (20E26 57M50)},
  MRNUMBER = {2587434},
MRREVIEWER = {Vassilis Metaftsis},
       DOI = {10.2140/pjm.2010.244.309},
       URL = {http://dx.doi.org/10.2140/pjm.2010.244.309},
}
	

@article {KarrassPietrowskiSolitar73,
    AUTHOR = {Karrass, A. and Pietrowski, A. and Solitar, D.},
     TITLE = {Finite and infinite cyclic extensions of free groups},
      NOTE = {Collection of articles dedicated to the memory of Hanna
              Neumann, IV},
   JOURNAL = {J. Austral. Math. Soc.},
  FJOURNAL = {Australian Mathematical Society. Journal. Series A. Pure
              Mathematics and Statistics},
    VOLUME = {16},
      YEAR = {1973},
     PAGES = {458--466},
      ISSN = {0263-6115},
   MRCLASS = {20F05},
  MRNUMBER = {0349850},
MRREVIEWER = {Stephen Meskin},
}

@article {CrokeKleiner2000,
    AUTHOR = {Croke, Christopher B. and Kleiner, Bruce},
     TITLE = {Spaces with nonpositive curvature and their ideal boundaries},
   JOURNAL = {Topology},
  FJOURNAL = {Topology. An International Journal of Mathematics},
    VOLUME = {39},
      YEAR = {2000},
    NUMBER = {3},
     PAGES = {549--556},
      ISSN = {0040-9383},
   MRCLASS = {53C21 (53C23 57M07)},
  MRNUMBER = {1746908},
MRREVIEWER = {Joseph E. Borzellino},
       DOI = {10.1016/S0040-9383(99)00016-6},
       URL = {http://dx.doi.org/10.1016/S0040-9383(99)00016-6},
}
	

@article {AgolGrovesManning2016,
    AUTHOR = {Agol, Ian and Groves, Daniel and Manning, Jason Fox},
     TITLE = {An alternate proof of {W}ise's malnormal special quotient
              theorem},
   JOURNAL = {Forum Math. Pi},
  FJOURNAL = {Forum of Mathematics. Pi},
    VOLUME = {4},
      YEAR = {2016},
     PAGES = {e1, 54},
      ISSN = {2050-5086},
   MRCLASS = {20F67 (20E08)},
  MRNUMBER = {3456181},
MRREVIEWER = {Fran\c{c}ois Dahmani},
       DOI = {10.1017/fmp.2015.8},
       URL = {http://dx.doi.org/10.1017/fmp.2015.8},
}

@article{JankiewiczNorineWise17,
Author={Janikiewicz, Kasia and  Norine, Sergei and 
Wise, Daniel T.},
Note={to appear},
Pages={1--30},
Journal= {Journal of the Institute of Mathematics of Jussieu},
}

@article {JanzenWise09smallest,
    AUTHOR = {Janzen, David and Wise, Daniel T.},
     TITLE = {A smallest irreducible lattice in the product of trees},
   JOURNAL = {Algebr. Geom. Topol.},
  FJOURNAL = {Algebraic \& Geometric Topology},
    VOLUME = {9},
      YEAR = {2009},
    NUMBER = {4},
     PAGES = {2191--2201},
      ISSN = {1472-2747},
   MRCLASS = {20F67 (20E08)},
  MRNUMBER = {2558308},
MRREVIEWER = {Matt T. Clay},
       DOI = {10.2140/agt.2009.9.2191},
       URL = {http://dx.doi.org/10.2140/agt.2009.9.2191},
}

@article{WiseSomeVirtualLimit,
author={Wise, Daniel T.},
title={Some Virtual Limit Groups},
pages = {1--6},
note={Submitted},
year={2017},
}

@article{LiWise17,
author={Li, Jiakai and Wise, Daniel T.},
title={Special groups have no growth-gap},
pages = {1--13},
note={Submitted},
year={2017},
}


@article{GromovSchoen1992,
author = { Michael Gromov and Richard Schoen},
journal = {Publications Mathématiques de l'IHÉS},       
language = {eng},
pages = {165-246},
publisher = {Institut des Hautes Études Scientifiques},
title = {Harmonic maps into singular spaces and $p$-adic superrigidity for lattices in groups of rank one},
url = {http://eudml.org/doc/104083},
volume = {76},
year = {1992}
}
 

@article{Corlette1992,
ISSN = {0003486X},
URL = {http://www.jstor.org/stable/2946567},
author = {Kevin Corlette},
journal = {Annals of Mathematics},
number = {1},
pages = {165-182},
publisher = {Annals of Mathematics},
title = {Archimedean Superrigidity and Hyperbolic Geometry},
volume = {135},
year = {1992}
}

@incollection {cannon:trieste-survey,
    AUTHOR = {Cannon, James W.},
     TITLE = {The theory of negatively curved spaces and groups},
 BOOKTITLE = {Ergodic theory, symbolic dynamics, and hyperbolic spaces
              ({T}rieste, 1989)},
    SERIES = {Oxford Sci. Publ.},
     PAGES = {315--369},
 PUBLISHER = {Oxford Univ. Press, New York},
      YEAR = {1991},
   MRCLASS = {57S30 (20F32 53C23 57M07)},
  MRNUMBER = {1130181},
}


@article {Cannon84,
    AUTHOR = {Cannon, James W.},
     TITLE = {The combinatorial structure of cocompact discrete hyperbolic
              groups},
   JOURNAL = {Geom. Dedicata},
  FJOURNAL = {Geometriae Dedicata},
    VOLUME = {16},
      YEAR = {1984},
    NUMBER = {2},
     PAGES = {123--148},
      ISSN = {0046-5755},
   MRCLASS = {20F10 (05C25 22E40 57M05)},
  MRNUMBER = {758901},
MRREVIEWER = {William Harvey},
       DOI = {10.1007/BF00146825},
       URL = {http://dx.doi.org/10.1007/BF00146825},
}

@article {Bowen2015,
    AUTHOR = {Bowen, Lewis},
     TITLE = {Cheeger constants and {$L^2$}-{B}etti numbers},
   JOURNAL = {Duke Math. J.},
  FJOURNAL = {Duke Mathematical Journal},
    VOLUME = {164},
      YEAR = {2015},
    NUMBER = {3},
     PAGES = {569--615},
      ISSN = {0012-7094},
   MRCLASS = {57S30 (20E26 58J50)},
  MRNUMBER = {3314481},
MRREVIEWER = {Shiping Liu},
       DOI = {10.1215/00127094-2871415},
       URL = {http://dx.doi.org/10.1215/00127094-2871415},
}

@article {Corlette90,
    AUTHOR = {Corlette, Kevin},
     TITLE = {Hausdorff dimensions of limit sets. {I}},
   JOURNAL = {Invent. Math.},
  FJOURNAL = {Inventiones Mathematicae},
    VOLUME = {102},
      YEAR = {1990},
    NUMBER = {3},
     PAGES = {521--541},
      ISSN = {0020-9910},
   MRCLASS = {58F11 (53C35 58F17 58G11)},
  MRNUMBER = {1074486},
MRREVIEWER = {William Goldman},
       DOI = {10.1007/BF01233439},
       URL = {http://dx.doi.org/10.1007/BF01233439},
}

@misc{YangContracting,
Author = {Wenyuan Yang},
Title = {Statistically convex-cocompact actions of groups with contracting elements},
Year = {2016},
Eprint = {arXiv:1612.03648},
}

@article{DahmaniFuterWise,
Author = {Fran\c{c}ois Dahmani and David Futer and Daniel T. Wise},
Title = {Growth of quasiconvex subgroups},
Pages={1--28},
Year = {2016},
howpublished = {arXiv:1602.08085},
}

@article{DahmaniMj2016,
Author = {Francois Dahmani and Mahan Mj},
Title = {Height, Graded Relative Hyperbolicity and Quasiconvexity},
Year = {2017},
journal = {Journal d'Ecole Polytechnique},
year = {2017},
pages={515--556},
volume={4},
}


 @misc{wiki:600cell,
   author = "Wikipedia",
   title = "600-cell --- {W}ikipedia{,} The Free Encyclopedia",
   year = "2017",
   url = "https://en.wikipedia.org/w/index.php?title=600-cell&oldid=757557549#Union_of_two_tori",
   note = "[Online; accessed 12-April-2017]"
 }


@article{JankiewiczSmallCancellation,
author={Jankiewicz, Kasia},
title={The fundamental theorem of cubical small cancellation theory},
journal={Trans. Amer. Math. Soc.},
year={2016},
doi={10.1090/tran/6852 },
url={https://doi.org/10.1090/tran/6852},
}


@article {AgolGrovesManning2009,
    AUTHOR = {Agol, Ian and Groves, Daniel and Manning, Jason Fox},
     TITLE = {Residual finiteness, {QCERF} and fillings of hyperbolic
              groups},
   JOURNAL = {Geom. Topol.},
  FJOURNAL = {Geometry \& Topology},
    VOLUME = {13},
      YEAR = {2009},
    NUMBER = {2},
     PAGES = {1043--1073},
      ISSN = {1465-3060},
   MRCLASS = {20E26 (20F67 57M07)},
  MRNUMBER = {2470970},
MRREVIEWER = {Zoran \AA ~uni\"A?},
       DOI = {10.2140/gt.2009.13.1043},
       URL = {http://dx.doi.org/10.2140/gt.2009.13.1043},
}

@article {BleilerHodgson1996,
    AUTHOR = {Bleiler, Steven A. and Hodgson, Craig D.},
     TITLE = {Spherical space forms and {D}ehn filling},
   JOURNAL = {Topology},
  FJOURNAL = {Topology. An International Journal of Mathematics},
    VOLUME = {35},
      YEAR = {1996},
    NUMBER = {3},
     PAGES = {809--833},
      ISSN = {0040-9383},
   MRCLASS = {57M25 (57M50)},
  MRNUMBER = {1396779},
MRREVIEWER = {Ying Qing Wu},
       DOI = {10.1016/0040-9383(95)00040-2},
       URL = {http://dx.doi.org/10.1016/0040-9383(95)00040-2},
}

@unpublished{Hatcher3Man,
    AUTHOR = {Hatcher, Allen},
     TITLE = {Notes on Basic 3-Manifold Topology},
 NOTE=  {\url{https://www.math.cornell.edu/~hatcher/3M/3M.pdf}},
     YEAR={2007},
     PAGES = {1--61},
}



@article{FuterWise2016,
Author = { David Futer and Daniel T. Wise},
Title = {Cubulating Random Quotients of Cubulated Hyperbolic Groups},
Pages = {1--20},
Year = {2016},
}


@article{MartinSteenbock2016,
Author = { Alexandre Martin and Markus Steenbock},
Title = {A combination theorem for cubulation in small cancellation theory over free products},
Journal = {Ann. Inst. Fourier},
Pages = {1--46},
Year = {2016},
Note = {To Appear},
}

@misc{FPGK,
Author = {Gonzalo Fiz Pontiveros and Roman Glebov and Ilan Karpas},
Title = {Virtually fibering random right-angled Coxeter groups},
Year = {2017},
Eprint = {arXiv:1703.01207},
}

@article {DavisOkun2001,
    AUTHOR = {Davis, Michael W. and Okun, Boris},
     TITLE = {Vanishing theorems and conjectures for the {$\ell^2$}-homology of right-angled {C}oxeter groups},
   JOURNAL = {Geom. Topol.},
  FJOURNAL = {Geometry and Topology},
    VOLUME = {5},
      YEAR = {2001},
     PAGES = {7--74},
      ISSN = {1465-3060},
   MRCLASS = {58J22 (20F55 20F65 20J05 57S30)},
  MRNUMBER = {1812434},
MRREVIEWER = {Daan Krammer},
       DOI = {10.2140/gt.2001.5.7},
       URL = {http://dx.doi.org/10.2140/gt.2001.5.7},
}

@misc{FisherLarsenSpatzierStover,
Author = {David Fisher and Michael Larsen and Ralf Spatzier and Matthew Stover},
Title = {Character varieties and actions on products of trees},
Year = {2016},
Eprint = {arXiv:1605.05163},
}

@article {BBaumslag67,
    AUTHOR = {Baumslag, Benjamin},
     TITLE = {Residually free groups},
   JOURNAL = {Proc. London Math. Soc. (3)},
  FJOURNAL = {Proceedings of the London Mathematical Society. Third Series},
    VOLUME = {17},
      YEAR = {1967},
     PAGES = {402--418},
      ISSN = {0024-6115},
   MRCLASS = {20.10},
  MRNUMBER = {0215903},
MRREVIEWER = {P. J. Higgins},
}

@article {Lyndon59,
    AUTHOR = {Lyndon, R. C.},
     TITLE = {The equation {$a^{2}b^{2}=c^{2}$} in free groups},
   JOURNAL = {Michigan Math. J},
  FJOURNAL = {The Michigan Mathematical Journal},
    VOLUME = {6},
      YEAR = {1959},
     PAGES = {89--95},
      ISSN = {0026-2285},
   MRCLASS = {20.00},
  MRNUMBER = {0103218},
MRREVIEWER = {P. M. Cohn},
}

@article {BaumslagLevinRosenberger93,
    AUTHOR = {Baumslag, Benjamin and Levin, Frank and Rosenberger, Gerhard},
     TITLE = {A cyclically pinched product of free groups which is not
              residually free},
   JOURNAL = {Math. Z.},
  FJOURNAL = {Mathematische Zeitschrift},
    VOLUME = {212},
      YEAR = {1993},
    NUMBER = {4},
     PAGES = {533--534},
      ISSN = {0025-5874},
     CODEN = {MAZEAX},
   MRCLASS = {20E06},
  MRNUMBER = {1214043},
MRREVIEWER = {D. E. Cohen},
       DOI = {10.1007/BF02571673},
       URL = {http://dx.doi.org/10.1007/BF02571673},
}
	

@article {Baumslag62,
    AUTHOR = {Baumslag, Gilbert},
     TITLE = {On generalised free products},
   JOURNAL = {Math. Z.},
  FJOURNAL = {Mathematische Zeitschrift},
    VOLUME = {78},
      YEAR = {1962},
     PAGES = {423--438},
      ISSN = {0025-5874},
   MRCLASS = {20.10},
  MRNUMBER = {0140562},
MRREVIEWER = {Hanna Neumann},
}

@article {BaumslagLevin76,
    AUTHOR = {Baumslag, Benjamin and Levin, Frank},
     TITLE = {A free product with a non-power amalgamated which is not
              residually free},
   JOURNAL = {Math. Z.},
  FJOURNAL = {Mathematische Zeitschrift},
    VOLUME = {151},
      YEAR = {1976},
    NUMBER = {3},
     PAGES = {235--237},
      ISSN = {0025-5874},
   MRCLASS = {20E30},
  MRNUMBER = {0422430},
MRREVIEWER = {R. C. Lyndon},
}

@article {Bollobas80,
    AUTHOR = {Bollob{\'a}s, B{\'e}la},
     TITLE = {The distribution of the maximum degree of a random graph},
   JOURNAL = {Discrete Math.},
  FJOURNAL = {Discrete Mathematics},
    VOLUME = {32},
      YEAR = {1980},
    NUMBER = {2},
     PAGES = {201--203},
      ISSN = {0012-365X},
     CODEN = {DSMHA4},
   MRCLASS = {05C99 (60C05)},
  MRNUMBER = {592855},
       DOI = {10.1016/0012-365X(80)90054-0},
       URL = {http://dx.doi.org/10.1016/0012-365X(80)90054-0},
}

@article {Palasti64,
    AUTHOR = {Pal{\'a}sti, Ilona},
     TITLE = {On the connectedness of bichromatic random graphs},
   JOURNAL = {Magyar Tud. Akad. Mat. Kutat\'o Int. K\"ozl.},
    VOLUME = {8},
      YEAR = {1964},
     PAGES = {431--441 (1964)},
   MRCLASS = {55.10 (05.65)},
  MRNUMBER = {0166778},
MRREVIEWER = {O. Ore},
}

@article {ERMatching66,
	AUTHOR = {Erd{\H{o}}s, P. and R{\'e}nyi, A.},
	TITLE = {On the existence of a factor of degree one of a connected
	random graph},
	JOURNAL = {Acta Math. Acad. Sci. Hungar.},
	FJOURNAL = {Acta Mathematica Academiae Scientiarum Hungaricae},
	VOLUME = {17},
	YEAR = {1966},
	PAGES = {359--368},
	ISSN = {0001-5954},
	MRCLASS = {05.40},
	MRNUMBER = {0200186},
	MRREVIEWER = {W. Moser},
}

@article{Caprace13,
    AUTHOR = {Caprace, Pierre-Emmanuel},
     TITLE = {Buildings with isolated subspaces and relatively hyperbolic
              {C}oxeter groups},
    pages={1--12},
journal={arXiv:0703799v3},
year={2013},
}

@article {Vesnin87,
    AUTHOR = {Vesnin, A. Yu.},
     TITLE = {Three-dimensional hyperbolic manifolds of {L}\"obell type},
   JOURNAL = {Sibirsk. Mat. Zh.},
  FJOURNAL = {Akademiya Nauk SSSR. Sibirskoe Otdelenie. Sibirski\u\i\
              Matematicheski\u\i\ Zhurnal},
    VOLUME = {28},
      YEAR = {1987},
    NUMBER = {5},
     PAGES = {50--53},
      ISSN = {0037-4474},
   MRCLASS = {57N10 (22E40 53A35)},
  MRNUMBER = {924975 (89f:57022)},
MRREVIEWER = {A. D. Mednykh},
}


@book {RivinPhD,
    AUTHOR = {Rivin, Igor},
     TITLE = {On Geometry of Convex Polyhedra in Hyperbolic 3-Space},
      NOTE = {Thesis (Ph.D.)--Princeton University},
 PUBLISHER = {ProQuest LLC, Ann Arbor, MI},
      YEAR = {1986},
     PAGES = {51},
   MRCLASS = {Thesis},
  MRNUMBER = {2635205},
       URL =
              {http://gateway.proquest.com/openurl?url_ver=Z39.88-2004&rft_val_fmt=info:ofi/fmt:kev:mtx:dissertation&res_dat=xri:pqdiss&rft_dat=xri:pqdiss:8626178},
}

@article{LutzNevo14,
    AUTHOR = {Lutz, Frank H. and Nevo, Eran},
     TITLE = {Stellar theory for flag complexes},
    pages={1--12},
journal={arXiv:1302.5197v3},
year={2014},
}

@incollection {Stallings62,
    AUTHOR = {Stallings, John},
     TITLE = {On fibering certain {$3$}-manifolds},
 BOOKTITLE = {Topology of 3-manifolds and related topics ({P}roc. {T}he
              {U}niv. of {G}eorgia {I}nstitute, 1961)},
     PAGES = {95--100},
 PUBLISHER = {Prentice-Hall, Englewood Cliffs, N.J.},
      YEAR = {1962},
   MRCLASS = {54.78},
  MRNUMBER = {0158375 (28 \#1600)},
MRREVIEWER = {O. G. Harrold},
}

@article {Kapovich2013,
    AUTHOR = {Kapovich, Michael},
     TITLE = {Noncoherence of arithmetic hyperbolic lattices},
   JOURNAL = {Geom. Topol.},
  FJOURNAL = {Geometry \& Topology},
    VOLUME = {17},
      YEAR = {2013},
    NUMBER = {1},
     PAGES = {39--71},
      ISSN = {1465-3060},
   MRCLASS = {11F06 (22E40)},
  MRNUMBER = {3035323},
MRREVIEWER = {O. V. Shvartsman},
       DOI = {10.2140/gt.2013.17.39},
       URL = {http://dx.doi.org/10.2140/gt.2013.17.39},
}


@article {gersten-short,
    AUTHOR = {Gersten, Steve and Short, Hamish},
     TITLE = {Rational subgroups of biautomatic groups},
   JOURNAL = {Ann. of Math. (2)},
  FJOURNAL = {Annals of Mathematics. Second Series},
    VOLUME = {134},
      YEAR = {1991},
    NUMBER = {1},
     PAGES = {125--158},
      ISSN = {0003-486X},
     CODEN = {ANMAAH},
   MRCLASS = {20M05 (20F10 20F32 57M05)},
  MRNUMBER = {1114609 (92g:20092)},
MRREVIEWER = {Athanase Papadopoulos},
       DOI = {10.2307/2944334},
       URL = {http://dx.doi.org/10.2307/2944334},
}

@INCOLLECTION{ABC91,
   author = {Alonso, Juan M. and  Brady, Thomas and Cooper, Daryl and Ferlini, Vincent and Lustig, Martin and Mihalik, Michael L. and Shapiro, Michael and Short, Hamish},
   title = {Notes on word hyperbolic groups},
   booktitle = {Group theory from a geometrical viewpoint ({T}rieste, 1990)},
   EDITOR = {Ghys, {\'E}. and Haefliger, A. and Verjovsky, A.},
   publisher = {World Sci. Publishing},
   year = {1991},
   pages = {3--63},
   address = {River Edge, NJ},
      note = {Edited by H. Short},
}


@article {Coornaert93,
    AUTHOR = {Coornaert, Michel},
     TITLE = {Mesures de {P}atterson-{S}ullivan sur le bord d'un espace
              hyperbolique au sens de {G}romov},
   JOURNAL = {Pacific J. Math.},
  FJOURNAL = {Pacific Journal of Mathematics},
    VOLUME = {159},
      YEAR = {1993},
    NUMBER = {2},
     PAGES = {241--270},
      ISSN = {0030-8730},
     CODEN = {PJMAAI},
   MRCLASS = {57S30 (20F32 30F35 30F40 53C23)},
  MRNUMBER = {1214072 (94m:57075)},
MRREVIEWER = {Christopher W. Stark},
       URL = {http://projecteuclid.org/euclid.pjm/1102634263},
}


@incollection {Hodgson90,
    AUTHOR = {Hodgson, Craig D.},
     TITLE = {Deduction of {A}ndreev's theorem from {R}ivin's
              characterization of convex hyperbolic polyhedra},
 BOOKTITLE = {Topology '90 ({C}olumbus, {OH}, 1990)},
    SERIES = {Ohio State Univ. Math. Res. Inst. Publ.},
    VOLUME = {1},
     PAGES = {185--193},
 PUBLISHER = {de Gruyter, Berlin},
      YEAR = {1992},
   MRCLASS = {57M50 (52A55)},
  MRNUMBER = {1184410 (93h:57022)},
MRREVIEWER = {B. N. Apanasov},
}

@article {Andreev70,
    AUTHOR = {Andreev, E. M.},
     TITLE = {Convex polyhedra of finite volume in {L}oba\v cevski\u\i\
              space},
   JOURNAL = {Mat. Sb. (N.S.)},
    VOLUME = {83 (125)},
      YEAR = {1970},
     PAGES = {256--260},
   MRCLASS = {50.40 (52.00)},
  MRNUMBER = {0273510 (42 \#8388)},
MRREVIEWER = {M. Decuyper},
}

@article {RoederHubbardDunbar2007,
    AUTHOR = {Roeder, Roland K. W. and Hubbard, John H. and Dunbar, William
              D.},
     TITLE = {Andreev's theorem on hyperbolic polyhedra},
   JOURNAL = {Ann. Inst. Fourier (Grenoble)},
  FJOURNAL = {Universit\'e de Grenoble. Annales de l'Institut Fourier},
    VOLUME = {57},
      YEAR = {2007},
    NUMBER = {3},
     PAGES = {825--882},
      ISSN = {0373-0956},
     CODEN = {AIFUA7},
   MRCLASS = {51M10 (51F15 52B10 57M50)},
  MRNUMBER = {2336832 (2008e:51011)},
MRREVIEWER = {Joan Porti},
       URL = {http://aif.cedram.org/item?id=AIF_2007__57_3_825_0},
}


@article {Davis85,
    AUTHOR = {Davis, Michael W.},
     TITLE = {A hyperbolic {$4$}-manifold},
   JOURNAL = {Proc. Amer. Math. Soc.},
  FJOURNAL = {Proceedings of the American Mathematical Society},
    VOLUME = {93},
      YEAR = {1985},
    NUMBER = {2},
     PAGES = {325--328},
      ISSN = {0002-9939},
     CODEN = {PAMYAR},
   MRCLASS = {57N13 (51M10 52A25)},
  MRNUMBER = {770546 (86h:57016)},
MRREVIEWER = {G. Peter Scott},
       DOI = {10.2307/2044771},
       URL = {http://dx.doi.org/10.2307/2044771},
}


@article {Caprace09,
    AUTHOR = {Caprace, Pierre-Emmanuel},
     TITLE = {Buildings with isolated subspaces and relatively hyperbolic
              {C}oxeter groups},
   JOURNAL = {Innov. Incidence Geom.},
  FJOURNAL = {Innovations in Incidence Geometry},
    VOLUME = {10},
      YEAR = {2009},
     PAGES = {15--31},
      ISSN = {1781-6475},
   MRCLASS = {20F67 (20E42 20F55)},
  MRNUMBER = {2665193 (2011f:20098)},
MRREVIEWER = {Jean L{\'e}cureux},
}


@article {Gould2014,
    AUTHOR = {Gould, Ronald J.},
     TITLE = {Recent advances on the {H}amiltonian problem: {S}urvey {III}},
   JOURNAL = {Graphs Combin.},
  FJOURNAL = {Graphs and Combinatorics},
    VOLUME = {30},
      YEAR = {2014},
    NUMBER = {1},
     PAGES = {1--46},
      ISSN = {0911-0119},
   MRCLASS = {05C45 (05-02 05C38)},
  MRNUMBER = {3143857},
MRREVIEWER = {Ralph Faudree},
       DOI = {10.1007/s00373-013-1377-x},
       URL = {http://dx.doi.org/10.1007/s00373-013-1377-x},
}

@incollection{Grinberg68,
    AUTHOR = {Grinberg, {\`E}. Ja.},
     TITLE = {Plane homogeneous graphs of degree three without {H}amiltonian
              circuits. },
 BOOKTITLE = {Latvian {M}ath. {Y}earbook, 4 ({R}ussian)},
     PAGES = {51--58},
 PUBLISHER = {Izdat. ``Zinatne'', Riga},
      YEAR = {1968},
   MRCLASS = {05.40},
  MRNUMBER = {0238732 (39 \#96)},
MRREVIEWER = {W. Imrich},
}

@article{HelferWise2015,
    AUTHOR = {Helfer, Joseph and Wise, Daniel T.},
     TITLE = {Counting cycles in labeled graphs: the nonpositive immersion property for one-relator groups},
   JOURNAL = {Int. Math. Res. Not. IMRN},
  FJOURNAL = {International Mathematics Research Notices. IMRN},
      YEAR = {2016},
    NUMBER = {9},
     PAGES = {2813--2827},
      ISSN = {1073-7928},
   MRCLASS = {05C20 (05C10 20E05 57M20)},
  MRNUMBER = {3519130},
MRREVIEWER = {Rafael Oswaldo Ruggiero},
       URL = {https://doi-org.proxy3.library.mcgill.ca/10.1093/imrn/rnv208},
}


@article{WiseWoodhouse15,
    AUTHOR = {Wise, Daniel T. and Woodhouse, Daniel J.},
     TITLE = {A cubical flat torus theorem and the bounded packing property},
   JOURNAL = {Israel J. Math.},
  FJOURNAL = {Israel Journal of Mathematics},
    VOLUME = {217},
      YEAR = {2017},
    NUMBER = {1},
     PAGES = {263--281},
      ISSN = {0021-2172},
   MRCLASS = {20F67 (20F06 20F65)},
  MRNUMBER = {3625111},
       DOI = {10.1007/s11856-017-1445-7},
       URL = {https://doi-org.proxy3.library.mcgill.ca/10.1007/s11856-017-1445-7},
}


@incollection {delaRue93,
    AUTHOR = {de la Rue, Thierry},
     TITLE = {Espaces de {L}ebesgue},
 BOOKTITLE = {S\'eminaire de {P}robabilit\'es, {XXVII}},
    SERIES = {Lecture Notes in Math.},
    VOLUME = {1557},
     PAGES = {15--21},
 PUBLISHER = {Springer, Berlin},
      YEAR = {1993},
   MRCLASS = {28A05 (28D05)},
  MRNUMBER = {1308547 (95j:28001)},
       DOI = {10.1007/BFb0087958},
       URL = {http://dx.doi.org/10.1007/BFb0087958},
}

@article {Robertson98,
    AUTHOR = {Robertson, Guyan},
     TITLE = {Crofton formulae and geodesic distance in hyperbolic spaces},
   JOURNAL = {J. Lie Theory},
  FJOURNAL = {Journal of Lie Theory},
    VOLUME = {8},
      YEAR = {1998},
    NUMBER = {1},
     PAGES = {163--172},
      ISSN = {0949-5932},
   MRCLASS = {53C65 (52A55)},
  MRNUMBER = {1616751 (99c:53083)},
MRREVIEWER = {Alan S. McRae},
}

@article {Robertson98b,
    AUTHOR = {Robertson, Guyan},
     TITLE = {Addendum to: ``{C}rofton formulae and geodesic distance in
              hyperbolic spaces'' [{J}. {L}ie {T}heory {\bf 8} (1998), no.\
              1, 163--172; {MR}1616751 (99c:53083)]},
   JOURNAL = {J. Lie Theory},
  FJOURNAL = {Journal of Lie Theory},
    VOLUME = {8},
      YEAR = {1998},
    NUMBER = {2},
     PAGES = {441},
      ISSN = {0949-5932},
   MRCLASS = {53C65 (52A55)},
  MRNUMBER = {1650402},
}


@article {ChatterjiDrtutuHaglund10,
    AUTHOR = {Chatterji, Indira and Dru{\c{t}}u, Cornelia and Haglund,
              Fr{\'e}d{\'e}ric},
     TITLE = {Kazhdan and {H}aagerup properties from the median viewpoint},
   JOURNAL = {Adv. Math.},
  FJOURNAL = {Advances in Mathematics},
    VOLUME = {225},
      YEAR = {2010},
    NUMBER = {2},
     PAGES = {882--921},
      ISSN = {0001-8708},
   MRCLASS = {20F65 (20F50 20F67 46B04)},
  MRNUMBER = {2671183 (2011g:20059)},
MRREVIEWER = {Alain Valette},
       DOI = {10.1016/j.aim.2010.03.012},
       URL = {http://dx.doi.org/10.1016/j.aim.2010.03.012},
}



@article {CoornaertKnieper2002,
    AUTHOR = {Coornaert, M. and Knieper, G.},
     TITLE = {Growth of conjugacy classes in {G}romov hyperbolic groups},
   JOURNAL = {Geom. Funct. Anal.},
  FJOURNAL = {Geometric and Functional Analysis},
    VOLUME = {12},
      YEAR = {2002},
    NUMBER = {3},
     PAGES = {464--478},
      ISSN = {1016-443X},
     CODEN = {GFANFB},
   MRCLASS = {20F67 (37C85 57M07)},
  MRNUMBER = {1924369 (2003f:20071)},
MRREVIEWER = {John Meier},
       DOI = {10.1007/s00039-002-8254-8},
       URL = {http://dx.doi.org/10.1007/s00039-002-8254-8},
}

@article{JankiewiczWise2015,
    AUTHOR = {Jankiewicz, Kasia and Wise, Daniel T.},
     TITLE = {Incoherent {C}oxeter groups},
   JOURNAL = {Proc. Amer. Math. Soc.},
  FJOURNAL = {Proceedings of the American Mathematical Society},
    VOLUME = {144},
      YEAR = {2016},
    NUMBER = {5},
     PAGES = {1857--1866},
      ISSN = {0002-9939},
   MRCLASS = {20F55 (20F67)},
  MRNUMBER = {3460148},
MRREVIEWER = {Jean Michel},
       DOI = {10.1090/proc/13013},
       URL = {http://dx.doi.org/10.1090/proc/13013},
}
	


@article {MihalikTschantz2009,
    AUTHOR = {Mihalik, Michael and Tschantz, Steven},
     TITLE = {Visual decompositions of {C}oxeter groups},
   JOURNAL = {Groups Geom. Dyn.},
  FJOURNAL = {Groups, Geometry, and Dynamics},
    VOLUME = {3},
      YEAR = {2009},
    NUMBER = {1},
     PAGES = {173--198},
      ISSN = {1661-7207},
   MRCLASS = {20F55 (20E06 20E08)},
  MRNUMBER = {2466022 (2009k:20090)},
MRREVIEWER = {Ian M. Chiswell},
       DOI = {10.4171/GGD/53},
       URL = {http://dx.doi.org/10.4171/GGD/53},
}

@article {Pogorelov67,
    AUTHOR = {Pogorelov, A. V.},
     TITLE = {Regular decomposition of the {L}oba\v cevski\u\i\ space},
   JOURNAL = {Mat. Zametki},
  FJOURNAL = {Akademiya Nauk SSSR. Matematicheskie Zametki},
    VOLUME = {1},
      YEAR = {1967},
     PAGES = {3--8},
      ISSN = {0025-567X},
   MRCLASS = {50.40 (50.90)},
  MRNUMBER = {0208458 (34 \#8268)},
MRREVIEWER = {Z. N{\'a}den{\'{\i}}k},
}

@article {Inoue08,
    AUTHOR = {Inoue, Taiyo},
     TITLE = {Organizing volumes of right-angled hyperbolic polyhedra},
   JOURNAL = {Algebr. Geom. Topol.},
  FJOURNAL = {Algebraic \& Geometric Topology},
    VOLUME = {8},
      YEAR = {2008},
    NUMBER = {3},
     PAGES = {1523--1565},
      ISSN = {1472-2747},
   MRCLASS = {57M50 (51M10 52B10)},
  MRNUMBER = {2443253 (2009k:57025)},
MRREVIEWER = {Ivan Izmestiev},
       DOI = {10.2140/agt.2008.8.1523},
       URL = {http://dx.doi.org/10.2140/agt.2008.8.1523},
}

@article {Deutsch99,
    AUTHOR = {Deutsch, Emeric},
     TITLE = {Dyck path enumeration},
   JOURNAL = {Discrete Math.},
  FJOURNAL = {Discrete Mathematics},
    VOLUME = {204},
      YEAR = {1999},
    NUMBER = {1-3},
     PAGES = {167--202},
      ISSN = {0012-365X},
     CODEN = {DSMHA4},
   MRCLASS = {05A15},
  MRNUMBER = {1691869 (2000d:05007)},
MRREVIEWER = {Ira Gessel},
       DOI = {10.1016/S0012-365X(98)00371-9},
       URL = {http://dx.doi.org/10.1016/S0012-365X(98)00371-9},
}

@article {Callan95,
    AUTHOR = {Callan, David},
     TITLE = {Pair Them Up! {A} Visual Approach to the {C}hung-{F}eller Theorem},
   JOURNAL = {Coll. Math. Jour.},
  FJOURNAL = {The College Mathematics Journal},
    VOLUME = {26},
      YEAR = {1995},
     PAGES = {196--198},
}


@article {Renault2008,
    AUTHOR = {Renault, Marc},
     TITLE = {Lost (and found) in translation: {A}ndr\'e's actual method and
              its application to the generalized ballot problem},
   JOURNAL = {Amer. Math. Monthly},
  FJOURNAL = {American Mathematical Monthly},
    VOLUME = {115},
      YEAR = {2008},
    NUMBER = {4},
     PAGES = {358--363},
      ISSN = {0002-9890},
     CODEN = {AMMYAE},
   MRCLASS = {05-03 (01A55 52B05 60-03)},
  MRNUMBER = {2398417 (2008m:05001)},
MRREVIEWER = {Toshihiro Watanabe},
}

@article {Dwass67,
    AUTHOR = {Dwass, Meyer},
     TITLE = {Simple random walk and rank order statistics},
   JOURNAL = {Ann. Math. Statist.},
  FJOURNAL = {Annals of Mathematical Statistics},
    VOLUME = {38},
      YEAR = {1967},
     PAGES = {1042--1053},
      ISSN = {0003-4851},
   MRCLASS = {62.75},
  MRNUMBER = {0215463 (35 \#6304)},
MRREVIEWER = {I. Vincze},
}

@article {DuncanHowie91,
    AUTHOR = {Duncan, Andrew J. and Howie, James},
     TITLE = {The genus problem for one-relator products of locally
              indicable groups},
   JOURNAL = {Math. Z.},
  FJOURNAL = {Mathematische Zeitschrift},
    VOLUME = {208},
      YEAR = {1991},
    NUMBER = {2},
     PAGES = {225--237},
      ISSN = {0025-5874},
     CODEN = {MAZEAX},
   MRCLASS = {20F32 (57M07)},
  MRNUMBER = {1128707 (92i:20040)},
MRREVIEWER = {Martin Edjvet},
       DOI = {10.1007/BF02571522},
       URL = {http://dx.doi.org/10.1007/BF02571522},
}

@article {Narayana67,
    AUTHOR = {Narayana, T. V.},
     TITLE = {Cyclic permutation of lattice paths and the {C}hung-{F}eller
              theorem},
   JOURNAL = {Skand. Aktuarietidskr},
    VOLUME = {1967},
      YEAR = {1967},
     PAGES = {23--30},
   MRCLASS = {05.04},
  MRNUMBER = {0224486 (37 \#85)},
MRREVIEWER = {M. Skalsky},
}


@article {BlackwellHodges67,
    AUTHOR = {Blackwell, David and Hodges, Jr., J. L.},
     TITLE = {Elementary {P}ath {C}ounts},
   JOURNAL = {Amer. Math. Monthly},
  FJOURNAL = {The American Mathematical Monthly},
    VOLUME = {74},
      YEAR = {1967},
    NUMBER = {7},
     PAGES = {801--804},
      ISSN = {0002-9890},
     CODEN = {AMMYAE},
   MRCLASS = {Contributed Item},
  MRNUMBER = {1534440},
       DOI = {10.2307/2315796},
       URL = {http://dx.doi.org/10.2307/2315796},
}

@article {DvoretzkyMotzkin47,
    AUTHOR = {Dvoretzky, A. and Motzkin, Th.},
     TITLE = {A problem of arrangements},
   JOURNAL = {Duke Math. J.},
  FJOURNAL = {Duke Mathematical Journal},
    VOLUME = {14},
      YEAR = {1947},
     PAGES = {305--313},
      ISSN = {0012-7094},
   MRCLASS = {09.0X},
  MRNUMBER = {0021531 (9,75i)},
MRREVIEWER = {H. B. Mann},
}



@article {Chen2008,
    AUTHOR = {Chen, Young-Ming},
     TITLE = {The {C}hung-{F}eller theorem revisited},
   JOURNAL = {Discrete Math.},
  FJOURNAL = {Discrete Mathematics},
    VOLUME = {308},
      YEAR = {2008},
    NUMBER = {7},
     PAGES = {1328--1329},
      ISSN = {0012-365X},
     CODEN = {DSMHA4},
   MRCLASS = {05A15},
  MRNUMBER = {2382368 (2008j:05019)},
MRREVIEWER = {Sen-Peng Eu},
       DOI = {10.1016/j.disc.2007.03.068},
       URL = {http://dx.doi.org/10.1016/j.disc.2007.03.068},
}

@article {ChungFeller49,
    AUTHOR = {Chung, Kai Lai and Feller, W.},
     TITLE = {On fluctuations in coin-tossing},
   JOURNAL = {Proc. Nat. Acad. Sci. U. S. A.},
  FJOURNAL = {Proceedings of the National Academy of Sciences of the United
              States of America},
    VOLUME = {35},
      YEAR = {1949},
     PAGES = {605--608},
      ISSN = {0027-8424},
   MRCLASS = {60.0X},
  MRNUMBER = {0033459 (11,444b)},
MRREVIEWER = {H. Cram{\'e}r},
}

@article {Rukavicka2011,
    AUTHOR = {Rukavicka, Josef},
     TITLE = {On generalized {D}yck paths},
   JOURNAL = {Electron. J. Combin.},
  FJOURNAL = {Electronic Journal of Combinatorics},
    VOLUME = {18},
      YEAR = {2011},
    NUMBER = {1},
     PAGES = {Paper 40, 3},
      ISSN = {1077-8926},
   MRCLASS = {05A15},
  MRNUMBER = {2776816 (2012b:05028)},
MRREVIEWER = {A. Sapounakis},
}

@article {HagenPrzytycki15,
    AUTHOR = {Hagen, Mark and Przytycki, Piotr},
     TITLE = {Cocompactly cubulated graph manifolds},
   JOURNAL = {Israel J. Math.},
   note = {to appear},
  }

@article {WoodhouseTubularAction,
    AUTHOR = {Woodhouse, Daniel J.},
     TITLE = {Classifying finite dimensional cubulations of tubular groups},
   JOURNAL = {Michigan Math. J.},
  FJOURNAL = {Michigan Mathematical Journal},
    VOLUME = {65},
      YEAR = {2016},
    NUMBER = {3},
     PAGES = {511--532},
      ISSN = {0026-2285},
   MRCLASS = {20E08 (20E26 20F67 57M07)},
  MRNUMBER = {3542763},
MRREVIEWER = {Christopher H. Cashen},
       DOI = {10.1307/mmj/1472066145},
       URL = {http://dx.doi.org/10.1307/mmj/1472066145},
}


@book {DavisCoxeterBook2008,
    AUTHOR = {Davis, Michael W.},
     TITLE = {The geometry and topology of {C}oxeter groups},
    SERIES = {London Mathematical Society Monographs Series},
    VOLUME = {32},
 PUBLISHER = {Princeton University Press, Princeton, NJ},
      YEAR = {2008},
     PAGES = {xvi+584},
      ISBN = {978-0-691-13138-2; 0-691-13138-4},
   MRCLASS = {20F55 (05B45 05C25 51-02 57M07)},
  MRNUMBER = {2360474 (2008k:20091)},
MRREVIEWER = {Ralf Gramlich},
}

@book {GrahamRothschildSpencer80,
    AUTHOR = {Graham, Ronald L. and Rothschild, Bruce L. and Spencer, Joel
              H.},
     TITLE = {Ramsey theory},
      NOTE = {Wiley-Interscience Series in Discrete Mathematics,
              A Wiley-Interscience Publication},
 PUBLISHER = {John Wiley \& Sons, Inc., New York},
      YEAR = {1980},
     PAGES = {ix+174},
      ISBN = {0-471-05997-8},
   MRCLASS = {05-02 (04A20 05C55 54H20)},
  MRNUMBER = {591457 (82b:05001)},
MRREVIEWER = {J. E. Graver},
}

@inproceedings {WiseICM,
    AUTHOR = {Wise, Daniel T.},
     TITLE = {The cubical route to understanding groups},
 BOOKTITLE = {Proceedings of the {I}nternational {C}ongress of
              {M}athematicians---{S}eoul 2014. {V}ol. {II}},
     PAGES = {1075--1099},
 PUBLISHER = {Kyung Moon Sa, Seoul},
      YEAR = {2014},
   MRCLASS = {20F67 (57M60)},
  MRNUMBER = {3728653},
MRREVIEWER = {Sebastian Wolfgang Hensel},
}



@article {LouderWilton2014,
   AUTHOR = {Louder, Larsen and Wilton, Henry},
     TITLE = {Stackings and the {$W$}-cycles conjecture},
   JOURNAL = {Canad. Math. Bull.},
  FJOURNAL = {Canadian Mathematical Bulletin. Bulletin Canadien de
              Math\'ematiques},
    VOLUME = {60},
      YEAR = {2017},
    NUMBER = {3},
     PAGES = {604--612},
      ISSN = {0008-4395},
   MRCLASS = {20F65 (05C25)},
  MRNUMBER = {3679733},
       URL = {https://doi-org.proxy3.library.mcgill.ca/10.4153/CMB-2016-078-3},
}



@misc{DicksOnePageProof2011,
Author = {Dicks, Warren},
Title = {Simplified {M}ineyev},
Year= {2011},
Pages = {1--2},
howpublished = {\url{http://mat.uab.es/~dicks/SimplifiedMineyev.pdf}}
}



@unpublished {CaretteQItoAmenable,
AUTHOR = {Carette, Mathieu},
TITLE = {The Haagerup property is not invariant under quasi-isometry},
NOTE = {With an appendix by Sylvain Arnt, Thibault Pillon, Alain Valette. Preprint, \url{http://arxiv.org/abs/1403.5446}},
YEAR = {2014},
}

@unpublished {Whyte10,
AUTHOR = {Whyte, Kevin},
TITLE = {Coarse bundles},
NOTE = {Preprint, \url{http://arxiv.org/abs/1006.3347}},
YEAR = {2010},
}


@book {CCJJV01,
    AUTHOR = {Cherix, Pierre-Alain and Cowling, Michael and Jolissaint, Paul
              and Julg, Pierre and Valette, Alain},
     TITLE = {Groups with the {H}aagerup property},
    SERIES = {Progress in Mathematics},
    VOLUME = {197},
      NOTE = {Gromov's a-T-menability},
 PUBLISHER = {Birkh\"auser Verlag},
   ADDRESS = {Basel},
      YEAR = {2001},
     PAGES = {viii+126},
      ISBN = {3-7643-6598-6},
   MRCLASS = {22D10 (22-02 22D25 22E30 43A07 46Lxx)},
  MRNUMBER = {1852148 (2002h:22007)},
MRREVIEWER = {Tullio G. Ceccherini-Silberstein},
       DOI = {10.1007/978-3-0348-8237-8},
       URL = {http://dx.doi.org/10.1007/978-3-0348-8237-8},
}


@article {Jolissaint00,
    AUTHOR = {Jolissaint, Paul},
     TITLE = {Borel cocycles, approximation properties and relative property
              {T}},
   JOURNAL = {Ergodic Theory Dynam. Systems},
  FJOURNAL = {Ergodic Theory and Dynamical Systems},
    VOLUME = {20},
      YEAR = {2000},
    NUMBER = {2},
     PAGES = {483--499},
      ISSN = {0143-3857},
   MRCLASS = {22D10 (28D15 37A20 46L55)},
  MRNUMBER = {1756981 (2001f:22015)},
MRREVIEWER = {Bachir Bekka},
       DOI = {10.1017/S0143385700000237},
       URL = {http://dx.doi.org/10.1017/S0143385700000237},
}

@article {CornulierValette12,
    AUTHOR = {Yves de Cornulier and Alain Valette},
     TITLE = {On equivariant embeddings of generalized Baumslag-Solitar groups},
    pages={1--22}, journal={http://arxiv.org/abs/1212.6765},
note={Submitted},
year={2012},
}

@article {DrummGoldman99,
    AUTHOR = {Drumm, Todd A. and Goldman, William M.},
     TITLE = {The geometry of crooked planes},
   JOURNAL = {Topology},
  FJOURNAL = {Topology. An International Journal of Mathematics},
    VOLUME = {38},
      YEAR = {1999},
    NUMBER = {2},
     PAGES = {323--351},
      ISSN = {0040-9383},
     CODEN = {TPLGAF},
   MRCLASS = {57S30 (22E40 57M60)},
  MRNUMBER = {1660333 (99m:57034)},
MRREVIEWER = {Allan Edmonds},
       DOI = {10.1016/S0040-9383(98)00016-0},
       URL = {http://dx.doi.org/10.1016/S0040-9383(98)00016-0},
}

@article{HagenWiseFreeByZirreducible,
author={Mark F. Hagen and Daniel T. Wise}, title={Cubulating
hyperbolic free-by-cyclic groups: the irreducible case},
pages={1--39},
journal = {Duke Math. J.},
note={To appear},
year={2013},
}

@article{HagenWiseFreeByZgeneral,
    AUTHOR = {Hagen, Mark F. and Wise, Daniel T.},
     TITLE = {Cubulating hyperbolic free-by-cyclic groups: the general case},
   JOURNAL = {Geom. Funct. Anal.},
  FJOURNAL = {Geometric and Functional Analysis},
    VOLUME = {25},
      YEAR = {2015},
    NUMBER = {1},
     PAGES = {134--179},
      ISSN = {1016-443X},
   MRCLASS = {20F65 (20F67 57M20)},
  MRNUMBER = {3320891},
       DOI = {10.1007/s00039-015-0314-y},
       URL = {http://dx.doi.org/10.1007/s00039-015-0314-y},
}

@article {Promislow88,
    AUTHOR = {Promislow, S. David},
     TITLE = {A simple example of a torsion-free, nonunique product group},
   JOURNAL = {Bull. London Math. Soc.},
  FJOURNAL = {The Bulletin of the London Mathematical Society},
    VOLUME = {20},
      YEAR = {1988},
    NUMBER = {4},
     PAGES = {302--304},
      ISSN = {0024-6093},
     CODEN = {LMSBBT},
   MRCLASS = {20F05 (20C07)},
  MRNUMBER = {940281 (89e:20064)},
MRREVIEWER = {Stephen J. Pride},
       DOI = {10.1112/blms/20.4.302},
       URL = {http://dx.doi.org/10.1112/blms/20.4.302},
}

@article {PolakWise2014,
    AUTHOR = {Pol{\'a}k, Jason K. C. and Wise, Daniel T.},
     TITLE = {Polygonal {$\scr{VH}$} complexes},
   JOURNAL = {Publ. Mat.},
  FJOURNAL = {Publicacions Matem\`atiques},
    VOLUME = {57},
      YEAR = {2013},
    NUMBER = {2},
     PAGES = {421--428},
      ISSN = {0214-1493},
   MRCLASS = {20F67},
  MRNUMBER = {3114776},
       DOI = {10.5565/PUBLMAT_57213_07},
       URL = {http://dx.doi.org/10.5565/PUBLMAT_57213_07},
}
	


@article {ScottSwarup90,
    AUTHOR = {Scott, G. P. and Swarup, G. A.},
     TITLE = {Geometric finiteness of certain {K}leinian groups},
   JOURNAL = {Proc. Amer. Math. Soc.},
  FJOURNAL = {Proceedings of the American Mathematical Society},
    VOLUME = {109},
      YEAR = {1990},
    NUMBER = {3},
     PAGES = {765--768},
      ISSN = {0002-9939},
     CODEN = {PAMYAR},
   MRCLASS = {57M05 (57N10)},
  MRNUMBER = {1013981 (90k:57002)},
MRREVIEWER = {Andrey V. Tetenov},
       DOI = {10.2307/2048217},
       URL = {http://dx.doi.org/10.2307/2048217},
}
		

@article {BigdelyWise2013,
    AUTHOR = {Bigdely, Hadi and Wise, Daniel T.},
     TITLE = {C(6) groups do not contain {$F_2\times F_2$}},
   JOURNAL = {J. Pure Appl. Algebra},
  FJOURNAL = {Journal of Pure and Applied Algebra},
    VOLUME = {217},
      YEAR = {2013},
    NUMBER = {1},
     PAGES = {22--30},
      ISSN = {0022-4049},
     CODEN = {JPAAA2},
   MRCLASS = {20F06},
  MRNUMBER = {2965900},
       DOI = {10.1016/j.jpaa.2012.04.016},
       URL = {http://dx.doi.org/10.1016/j.jpaa.2012.04.016},
}

@book {WiseCBMS2012,
    AUTHOR = {Wise, Daniel T.},
     TITLE = {From riches to raags: 3-manifolds, right-angled {A}rtin
              groups, and cubical geometry},
    SERIES = {CBMS Regional Conference Series in Mathematics},
    VOLUME = {117},
 PUBLISHER = {Published for the Conference Board of the Mathematical
              Sciences, Washington, DC},
      YEAR = {2012},
     PAGES = {xiv+141},
      ISBN = {978-0-8218-8800-1},
   MRCLASS = {20F67 (20F06 57M07)},
  MRNUMBER = {2986461},
}

@article {SilverWilliams2009,
    AUTHOR = {Silver, Daniel S. and Williams, Susan G.},
     TITLE = {Twisted {A}lexander polynomials and representation shifts},
   JOURNAL = {Bull. Lond. Math. Soc.},
  FJOURNAL = {Bulletin of the London Mathematical Society},
    VOLUME = {41},
      YEAR = {2009},
    NUMBER = {3},
     PAGES = {535--540},
      ISSN = {0024-6093},
   MRCLASS = {57M25 (37B10 57M27)},
  MRNUMBER = {2506837 (2010c:57015)},
MRREVIEWER = {Quach thi C{\^a}m V{\^a}n},
       DOI = {10.1112/blms/bdp029},
       URL = {http://dx.doi.org/10.1112/blms/bdp029},
}

@article{LiuGraphManifolds,
    AUTHOR = {Liu, Yi},
     TITLE = {Virtual cubulation of nonpositively curved graph manifolds},
   JOURNAL = {J. Topol.},
  FJOURNAL = {Journal of Topology},
    VOLUME = {6},
      YEAR = {2013},
    NUMBER = {4},
     PAGES = {793--822},
      ISSN = {1753-8416},
   MRCLASS = {57M05 (20F65)},
  MRNUMBER = {3145140},
       DOI = {10.1112/jtopol/jtt010},
       URL = {http://dx.doi.org/10.1112/jtopol/jtt010},
}


@article {PrzytyckiWiseGraphManifolds,
  AUTHOR = {Przytycki, Piotr and Wise, Daniel T.},
     TITLE = {Graph manifolds with boundary are virtually special},
   JOURNAL = {J. Topol.},
  FJOURNAL = {Journal of Topology},
    VOLUME = {7},
      YEAR = {2014},
    NUMBER = {2},
     PAGES = {419--435},
      ISSN = {1753-8416},
   MRCLASS = {20F65 (57M27)},
  MRNUMBER = {3217626},
MRREVIEWER = {Ian Agol},
       DOI = {10.1112/jtopol/jtt009},
       URL = {https://doi-org.proxy3.library.mcgill.ca/10.1112/jtopol/jtt009},
}




@article {AgolGrovesManning2012,
    AUTHOR = {Agol, Ian},
     TITLE = {The virtual {H}aken conjecture},
      NOTE = {With an appendix by Agol, Daniel Groves, and Jason Manning},
   JOURNAL = {Doc. Math.},
  FJOURNAL = {Documenta Mathematica},
    VOLUME = {18},
      YEAR = {2013},
     PAGES = {1045--1087},
      ISSN = {1431-0635},
   MRCLASS = {20F67 (57Mxx)},
  MRNUMBER = {3104553},
MRREVIEWER = {Thomas Koberda},
}
	

@article {MartinezPedrozaWiseSectional,
    AUTHOR = {Mart{\'{\i}}nez-Pedroza, Eduardo and Wise, Daniel T.},
     TITLE = {Coherence and negative sectional curvature in complexes of
              groups},
   JOURNAL = {Michigan Math. J.},
  FJOURNAL = {Michigan Mathematical Journal},
    VOLUME = {62},
      YEAR = {2013},
    NUMBER = {3},
     PAGES = {507--536},
      ISSN = {0026-2285},
   MRCLASS = {20F65 (20F67)},
  MRNUMBER = {3102528},
MRREVIEWER = {Mark F. Hagen},
       DOI = {10.1307/mmj/1378757886},
       URL = {http://dx.doi.org/10.1307/mmj/1378757886},
}

@article {Mitra99,
    AUTHOR = {Mitra, Mahan},
     TITLE = {On a theorem of {S}cott and {S}warup},
   JOURNAL = {Proc. Amer. Math. Soc.},
  FJOURNAL = {Proceedings of the American Mathematical Society},
    VOLUME = {127},
      YEAR = {1999},
    NUMBER = {6},
     PAGES = {1625--1631},
      ISSN = {0002-9939},
     CODEN = {PAMYAR},
   MRCLASS = {20F32 (57M50 57N10)},
  MRNUMBER = {1610757 (99i:20050)},
MRREVIEWER = {Dubravko Ivan{\v{s}}i{\'c}},
       DOI = {10.1090/S0002-9939-99-04935-7},
       URL = {http://dx.doi.org/10.1090/S0002-9939-99-04935-7},
}

@article {Friedman2015,
    AUTHOR = {Friedman, Joel},
     TITLE = {Sheaves on graphs, their homological invariants, and a proof
              of the {H}anna {N}eumann conjecture},
                   NOTE = {With an appendix by Warren Dicks},
   JOURNAL = {Mem. Amer. Math. Soc.},
  FJOURNAL = {Memoirs of the American Mathematical Society},
    VOLUME = {233},
      YEAR = {2015},
    NUMBER = {1100},
     PAGES = {xii+106},
      ISSN = {0065-9266},
      ISBN = {978-1-4704-0988-3},
   MRCLASS = {20E05 (05C10 18F20 55N30)},
  MRNUMBER = {3289057},
       DOI = {10.1090/memo/1100},
       URL = {http://dx.doi.org/10.1090/memo/1100},
}

@article {Mineyev2012,
    AUTHOR = {Mineyev, Igor},
     TITLE = {Submultiplicativity and the {H}anna {N}eumann conjecture},
   JOURNAL = {Ann. of Math. (2)},
  FJOURNAL = {Annals of Mathematics. Second Series},
    VOLUME = {175},
      YEAR = {2012},
    NUMBER = {1},
     PAGES = {393--414},
      ISSN = {0003-486X},
     CODEN = {ANMAAH},
   MRCLASS = {57Mxx (20E05)},
  MRNUMBER = {2874647},
       DOI = {10.4007/annals.2012.175.1.11},
       URL = {http://dx.doi.org/10.4007/annals.2012.175.1.11},
}
		




@article {DicksLinnell2007,
    AUTHOR = {Dicks, Warren and Linnell, Peter A.},
     TITLE = {{$L^2$}-{B}etti numbers of one-relator groups},
   JOURNAL = {Math. Ann.},
  FJOURNAL = {Mathematische Annalen},
    VOLUME = {337},
      YEAR = {2007},
    NUMBER = {4},
     PAGES = {855--874},
      ISSN = {0025-5831},
     CODEN = {MAANA},
   MRCLASS = {20J05 (16S34 20F05)},
  MRNUMBER = {2285740 (2007m:20076)},
MRREVIEWER = {E. F. Robertson},
       DOI = {10.1007/s00208-006-0058-y},
       URL = {http://dx.doi.org/10.1007/s00208-006-0058-y},
}

@article {PrzytyckiWiseMixed,
    AUTHOR = {Przytycki, Piotr and Wise, Daniel T.},
     TITLE = {Mixed 3-manifolds are virtually special},
   JOURNAL = {J. Amer. Math. Soc.},
  FJOURNAL = {Journal of the American Mathematical Society},
    VOLUME = {31},
      YEAR = {2018},
    NUMBER = {2},
     PAGES = {319--347},
      ISSN = {0894-0347},
   MRCLASS = {57M50 (20F65 57M27)},
  MRNUMBER = {3758147},
MRREVIEWER = {Bruno P. Zimmermann},
       DOI = {10.1090/jams/886},
       URL = {https://doi-org.proxy3.library.mcgill.ca/10.1090/jams/886},
}


@article {Gersten87b,
    AUTHOR = {Gersten, S. M.},
     TITLE = {Branched coverings of {$2$}-complexes and diagrammatic
              reducibility},
   JOURNAL = {Trans. Amer. Math. Soc.},
  FJOURNAL = {Transactions of the American Mathematical Society},
    VOLUME = {303},
      YEAR = {1987},
    NUMBER = {2},
     PAGES = {689--706},
      ISSN = {0002-9947},
     CODEN = {TAMTAM},
   MRCLASS = {57M12 (20F05 57M20)},
  MRNUMBER = {902792 (90a:57004)},
       DOI = {10.2307/2000691},
       URL = {http://dx.doi.org/10.2307/2000691},
}
		



@article {BekkaValette97,
    AUTHOR = {Bekka, Mohammed E. B. and Valette, Alain},
     TITLE = {Group cohomology, harmonic functions and the first {$L^2$}-{B}etti number},
   JOURNAL = {Potential Anal.},
  FJOURNAL = {Potential Analysis. An International Journal Devoted to the
              Interactions between Potential Theory, Probability Theory,
              Geometry and Functional Analysis},
    VOLUME = {6},
      YEAR = {1997},
    NUMBER = {4},
     PAGES = {313--326},
      ISSN = {0926-2601},
     CODEN = {POANE2},
   MRCLASS = {20J05 (31C05 58G12)},
  MRNUMBER = {1452785 (98e:20056)},
MRREVIEWER = {William Paschke},
       DOI = {10.1023/A:1017974406074},
       URL = {http://dx.doi.org/10.1023/A:1017974406074},
}

@article{ChesebroDeBloisWilton2009,
Title={
Some virtually special hyperbolic 3-manifold groups},
Author={Eric Chesebro, Jason DeBlois, and Henry Wilton},
Year={2009},
       URL = {arXiv:0903.5288v3 [math.GT]},
       Pages={1--51},
}



@article {KapovichLeeb1995,
    AUTHOR = {Kapovich, M. and Leeb, B.},
     TITLE = {On asymptotic cones and quasi-isometry classes of fundamental
              groups of {$3$}-manifolds},
   JOURNAL = {Geom. Funct. Anal.},
  FJOURNAL = {Geometric and Functional Analysis},
    VOLUME = {5},
      YEAR = {1995},
    NUMBER = {3},
     PAGES = {582--603},
      ISSN = {1016-443X},
     CODEN = {GFANFB},
   MRCLASS = {57M50 (20F32 53C23 57N10)},
  MRNUMBER = {1339818 (96e:57006)},
MRREVIEWER = {Fr{\'e}d{\'e}ric Paulin},
       DOI = {10.1007/BF01895833},
       URL = {http://dx.doi.org/10.1007/BF01895833},
}

@article {Sauer2006,
    AUTHOR = {Sauer, R.},
     TITLE = {Homological invariants and quasi-isometry},
   JOURNAL = {Geom. Funct. Anal.},
  FJOURNAL = {Geometric and Functional Analysis},
    VOLUME = {16},
      YEAR = {2006},
    NUMBER = {2},
     PAGES = {476--515},
      ISSN = {1016-443X},
     CODEN = {GFANFB},
   MRCLASS = {20F65 (20F16 20J06)},
  MRNUMBER = {2231471 (2007e:20090)},
MRREVIEWER = {Wolfgang Pitsch},
       DOI = {10.1007/s00039-006-0562-y},
       URL = {http://dx.doi.org/10.1007/s00039-006-0562-y},
}

@article {Dranishnikov2009,
    AUTHOR = {Dranishnikov, A.},
     TITLE = {Cohomological approach to asymptotic dimension},
   JOURNAL = {Geom. Dedicata},
  FJOURNAL = {Geometriae Dedicata},
    VOLUME = {141},
      YEAR = {2009},
     PAGES = {59--86},
      ISSN = {0046-5755},
     CODEN = {GEMDAT},
   MRCLASS = {20F69 (18G99)},
  MRNUMBER = {2520063 (2011a:20114)},
       DOI = {10.1007/s10711-008-9343-0},
       URL = {http://dx.doi.org/10.1007/s10711-008-9343-0},
}

@article {Gromov2004,
    AUTHOR = {Gromov, M.},
     TITLE = {{${\rm CAT}(\kappa)$}-spaces: construction and concentration},
   JOURNAL = {Zap. Nauchn. Sem. S.-Peterburg. Otdel. Mat. Inst. Steklov.
              (POMI)},
  FJOURNAL = {Rossi\u\i skaya Akademiya Nauk. Sankt-Peterburgskoe Otdelenie.
              Matematicheski\u\i\ Institut im. V. A. Steklova. Zapiski
              Nauchnykh Seminarov (POMI)},
    VOLUME = {280},
      YEAR = {2001},
    NUMBER = {Geom. i Topol. 7},
     PAGES = {100--140, 299--300},
      ISSN = {0373-2703},
   MRCLASS = {53C23 (20F67 53C45)},
  MRNUMBER = {1879258 (2002j:53045)},
MRREVIEWER = {Athanase Papadopoulos},
       DOI = {10.1023/B:JOTH.0000008756.15786.0f},
       URL = {http://dx.doi.org/10.1023/B:JOTH.0000008756.15786.0f},
}

@book {GuilleminPollack74,
    AUTHOR = {Guillemin, Victor and Pollack, Alan},
     TITLE = {Differential topology},
 PUBLISHER = {Prentice-Hall Inc.},
   ADDRESS = {Englewood Cliffs, N.J.},
      YEAR = {1974},
     PAGES = {xvi+222},
   MRCLASS = {58-01 (57-01)},
  MRNUMBER = {0348781 (50 \#1276)},
MRREVIEWER = {K. H. Mayer},
}
		



@article{HagenCrystallographicCubes,
   AUTHOR = {Hagen, Mark F.},
     TITLE = {Cocompactly cubulated crystallographic groups},
   JOURNAL = {J. Lond. Math. Soc. (2)},
  FJOURNAL = {Journal of the London Mathematical Society. Second Series},
    VOLUME = {90},
      YEAR = {2014},
    NUMBER = {1},
     PAGES = {140--166},
      ISSN = {0024-6107},
   MRCLASS = {20F65 (20H15)},
  MRNUMBER = {3245140},
MRREVIEWER = {Andrzej Szczepa\'{n}ski},
       DOI = {10.1112/jlms/jdu017},
       URL = {https://doi-org.proxy3.library.mcgill.ca/10.1112/jlms/jdu017},
}



		


@unpublished{KharlampovichMyasnikovSerbinLambdaTrees,
 Author = {O. Kharlampovich and A. Myasnikov and D. Serbin},
 Date-Added = {2009-11-01},
 Date-Modified = {2011-11-02},
 Note = {Preprint. arXiv:0911.0209v4 [math.GR]},
 Title = {Groups acting freely on $\Lambda$-trees},
 Year = {2011},
}

@ARTICLE{Osin2006,
AUTHOR = {Osin, D. V.},
TITLE = {Relative {D}ehn functions of amalgamated products and
{HNN}-extensions},
BOOKTITLE = {Topological and asymptotic aspects of group theory},
SERIES = {Contemp. Math.},
VOLUME = {394},
PAGES = {209--220},
PUBLISHER = {Amer. Math. Soc.},
ADDRESS = {Providence, RI},
YEAR = {2006},
MRCLASS = {20F65 (20E06 20F05 20F67 57M07)},
MRNUMBER = {2216718 (2007g:20042)},
MRREVIEWER = {Thomas Delzant},
}


@article {Mitra2004,
    AUTHOR = {Mitra, Mahan},
     TITLE = {Height in splittings of hyperbolic groups},
   JOURNAL = {Proc. Indian Acad. Sci. Math. Sci.},
  FJOURNAL = {Indian Academy of Sciences. Proceedings. Mathematical
              Sciences},
    VOLUME = {114},
      YEAR = {2004},
    NUMBER = {1},
     PAGES = {39--54},
      ISSN = {0253-4142},
   MRCLASS = {20F67 (20E06 20F34)},
  MRNUMBER = {2040599 (2005d:20073)},
MRREVIEWER = {Denis V. Osin},
       DOI = {10.1007/BF02829670},
       URL = {http://dx.doi.org/10.1007/BF02829670},
}

@article {CapracePrzytycki2011,
    AUTHOR = {Caprace, Pierre-Emmanuel and Przytycki, Piotr},
     TITLE = {Bipolar {C}oxeter groups},
   JOURNAL = {J. Algebra},
  FJOURNAL = {Journal of Algebra},
    VOLUME = {338},
      YEAR = {2011},
     PAGES = {35--55},
      ISSN = {0021-8693},
     CODEN = {JALGA4},
   MRCLASS = {20F65 (20F55)},
  MRNUMBER = {2805179},
       DOI = {10.1016/j.jalgebra.2011.05.007},
       URL = {http://dx.doi.org/10.1016/j.jalgebra.2011.05.007},
}
		



@article {Cashen2010,
    AUTHOR = {Cashen, Christopher H.},
     TITLE = {Quasi-isometries between tubular groups},
   JOURNAL = {Groups Geom. Dyn.},
  FJOURNAL = {Groups, Geometry, and Dynamics},
    VOLUME = {4},
      YEAR = {2010},
    NUMBER = {3},
     PAGES = {473--516},
      ISSN = {1661-7207},
   MRCLASS = {20F65 (20E08)},
  MRNUMBER = {2653972 (2011i:20062)},
MRREVIEWER = {Mihalis A. Sykiotis},
       DOI = {10.4171/GGD/92},
       URL = {http://dx.doi.org/10.4171/GGD/92},
}
		



@article {BradyBridson2000,
    AUTHOR = {Brady, N. and Bridson, M. R.},
     TITLE = {There is only one gap in the isoperimetric spectrum},
   JOURNAL = {Geom. Funct. Anal.},
  FJOURNAL = {Geometric and Functional Analysis},
    VOLUME = {10},
      YEAR = {2000},
    NUMBER = {5},
     PAGES = {1053--1070},
      ISSN = {1016-443X},
     CODEN = {GFANFB},
   MRCLASS = {20F10 (20F65)},
  MRNUMBER = {1800063 (2001j:20046)},
MRREVIEWER = {Eric M. Freden},
       DOI = {10.1007/PL00001646},
       URL = {http://dx.doi.org/10.1007/PL00001646},
}

@book {Grunbaum2003,
    AUTHOR = {Gr{\"u}nbaum, Branko},
     TITLE = {Convex polytopes},
    SERIES = {Graduate Texts in Mathematics},
    VOLUME = {221},
   EDITION = {2nd},
      NOTE = {Prepared and with a preface by Volker Kaibel, Victor Klee and
              G{\"u}nter M. Ziegler},
 PUBLISHER = {Springer-Verlag},
   ADDRESS = {New York},
      YEAR = {2003},
     PAGES = {xvi+468},
      ISBN = {0-387-00424-6; 0-387-40409-0},
   MRCLASS = {52-01 (52Bxx)},
  MRNUMBER = {1976856 (2004b:52001)},
MRREVIEWER = {Alexander Zvonkin},
}


@article{HaglundSemiSimple,
    AUTHOR = {Haglund, Fr{\'e}d{\'e}ric},
Title = {Isometries of {C}{A}{T}(0) cube complexes are semi-simple},
      YEAR = {2007},
     PAGES = {1-15},
     NOTE = {arXiv:0705.3386},
}


@article {MartinezPedrozaCombinations2009,
    AUTHOR = {Mart{\'{\i}}nez-Pedroza, Eduardo},
     TITLE = {Combination of quasiconvex subgroups of relatively hyperbolic
              groups},
   JOURNAL = {Groups Geom. Dyn.},
  FJOURNAL = {Groups, Geometry, and Dynamics},
    VOLUME = {3},
      YEAR = {2009},
    NUMBER = {2},
     PAGES = {317--342},
      ISSN = {1661-7207},
   MRCLASS = {20F67 (20F65)},
  MRNUMBER = {2486802 (2010c:20054)},
MRREVIEWER = {Goulnara N. Arzhantseva},
       DOI = {10.4171/GGD/59},
       URL = {http://dx.doi.org/10.4171/GGD/59},
}
		



@article {CapraceSageev2011,
   author = {Caprace, Pierre-Emmanuel and Sageev, Michah},
   title = {Rank Rigidity for Cat(0) Cube Complexes},
   journal = {Geometric And Functional Analysis},
   issn = {1016-443X},
   pages = {851-891},
   volume = {21},
   issue = {4},
   note = {10.1007/s00039-011-0126-7},
   year = {2011},
}

@article{WiseGerstenRevisited,
    AUTHOR = {Wise, Daniel T.},
     TITLE = {Cubular tubular groups},
   JOURNAL = {Trans. Amer. Math. Soc.},
  FJOURNAL = {Transactions of the American Mathematical Society},
    VOLUME = {366},
      YEAR = {2014},
    NUMBER = {10},
     PAGES = {5503--5521},
      ISSN = {0002-9947},
   MRCLASS = {20F67 (20E06 20F65)},
  MRNUMBER = {3240932},
       DOI = {10.1090/S0002-9947-2014-06065-0},
       URL = {http://dx.doi.org/10.1090/S0002-9947-2014-06065-0},
}

@article {BrinkHowlett93,
    AUTHOR = {Brink, Brigitte and Howlett, Robert B.},
    TITLE = {A finiteness property and an automatic structure for {C}oxeter
              groups},
   JOURNAL = {Math. Ann.},
  FJOURNAL = {Mathematische Annalen},
    VOLUME = {296},
      YEAR = {1993},
    NUMBER = {1},
     PAGES = {179--190},
      ISSN = {0025-5831},
     CODEN = {MAANA},
   MRCLASS = {20F55 (20F10)},
  MRNUMBER = {1213378 (94d:20045)},
MRREVIEWER = {D. F. Holt},
       DOI = {10.1007/BF01445101},
       URL = {http://dx.doi.org/10.1007/BF01445101},
}


@book {GeogheganBook2008,
    AUTHOR = {Geoghegan, Ross},
     TITLE = {Topological methods in group theory},
    SERIES = {Graduate Texts in Mathematics},
    VOLUME = {243},
 PUBLISHER = {Springer},
   ADDRESS = {New York},
      YEAR = {2008},
     PAGES = {xiv+473},
      ISBN = {978-0-387-74611-1},
   MRCLASS = {57M07 (20F65 20J05 55-02 55P57 57-02)},
  MRNUMBER = {2365352 (2008j:57002)},
MRREVIEWER = {John G. Ratcliffe},
       DOI = {10.1007/978-0-387-74614-2},
       URL = {http://dx.doi.org/10.1007/978-0-387-74614-2},
}


@article {KrophollerRoller89,
    AUTHOR = {Kropholler, P. H. and Roller, M. A.},
     TITLE = {Relative ends and duality groups},
   JOURNAL = {J. Pure Appl. Algebra},
  FJOURNAL = {Journal of Pure and Applied Algebra},
    VOLUME = {61},
      YEAR = {1989},
    NUMBER = {2},
     PAGES = {197--210},
      ISSN = {0022-4049},
     CODEN = {JPAAA2},
   MRCLASS = {20J05},
  MRNUMBER = {1025923 (91b:20069)},
MRREVIEWER = {M. J. Dunwoody},
       DOI = {10.1016/0022-4049(89)90014-5},
       URL = {http://dx.doi.org/10.1016/0022-4049(89)90014-5},
}


@article{Tukia94,
    AUTHOR = {Tukia, Pekka},
     TITLE = {Convergence groups and {G}romov's metric hyperbolic spaces},
   JOURNAL = {New Zealand J. Math.},
  FJOURNAL = {New Zealand Journal of Mathematics},
    VOLUME = {23},
      YEAR = {1994},
    NUMBER = {2},
     PAGES = {157--187},
      ISSN = {1171-6096},
   MRCLASS = {30F40 (20H10 57M07 57S05 57S30)},
  MRNUMBER = {1313451 (96c:30042)},
MRREVIEWER = {A. Hinkkanen},
}



@article {MjReeves2008,
    AUTHOR = {Mj, Mahan and Reeves, Lawrence},
     TITLE = {A combination theorem for strong relative hyperbolicity},
   JOURNAL = {Geom. Topol.},
  FJOURNAL = {Geometry \& Topology},
    VOLUME = {12},
      YEAR = {2008},
    NUMBER = {3},
     PAGES = {1777--1798},
      ISSN = {1465-3060},
   MRCLASS = {20F67 (57M50)},
  MRNUMBER = {2421140 (2010d:20052)},
       DOI = {10.2140/gt.2008.12.1777},
       URL = {http://dx.doi.org/10.2140/gt.2008.12.1777},
}



@ARTICLE{Yang11,
author = {{Yang}, W.},
title = "{Peripheral structures of relatively hyperbolic groups}",
journal = {ArXiv e-prints},
archivePrefix = "arXiv",
eprint = {1101.2990},
primaryClass = "math.GR",
keywords = {Mathematics - Group Theory, Primary 20F65, 20F67},
year = 2011,
month = jan,
adsurl = {http://adsabs.harvard.edu/abs/2011arXiv1101.2990Y},
adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{MartinezPedroza08,
author = {{Martinez-Pedroza}, E.},
title = "{On Quasiconvexity and Relative Hyperbolic Structures}",
journal = {ArXiv e-prints},
archivePrefix = "arXiv",
eprint = {0811.2384},
primaryClass = "math.GR",
keywords = {Mathematics - Group Theory, 20F65 20F67},
year = 2008,
month = nov,
adsurl = {http://adsabs.harvard.edu/abs/2008arXiv0811.2384M},
adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article {MartinezPedrozaWise2011,
    AUTHOR = {Mart{\'{\i}}nez-Pedroza, Eduardo and Wise, Daniel T.},
     TITLE = {Relative quasiconvexity using fine hyperbolic graphs},
   JOURNAL = {Algebr. Geom. Topol.},
  FJOURNAL = {Algebraic \& Geometric Topology},
    VOLUME = {11},
      YEAR = {2011},
    NUMBER = {1},
     PAGES = {477--501},
      ISSN = {1472-2747},
   MRCLASS = {20F67 (20F65 57M07)},

  MRNUMBER = {2783235},
       DOI = {10.2140/agt.2011.11.477},
       URL = {http://dx.doi.org/10.2140/agt.2011.11.477},
}

@article {Osin06,
    AUTHOR = {Osin, Denis V.},
     TITLE = {Elementary subgroups of relatively hyperbolic groups and
              bounded generation},
   JOURNAL = {Internat. J. Algebra Comput.},
  FJOURNAL = {International Journal of Algebra and Computation},
    VOLUME = {16},
      YEAR = {2006},
    NUMBER = {1},
     PAGES = {99--118},
      ISSN = {0218-1967},
   MRCLASS = {20F67 (20F65)},
  MRNUMBER = {2217644 (2007b:20092)},
MRREVIEWER = {Fran{\c{c}}ois Dahmani},
       DOI = {10.1142/S0218196706002901},
       URL = {http://dx.doi.org/10.1142/S0218196706002901},
}



@article {BigdelyWiseAmalgams,
    AUTHOR = {Bigdely, Hadi and Wise, Daniel T.},
     TITLE = {Quasiconvexity and relatively hyperbolic groups that split},
   JOURNAL = {Michigan Math. J.},
  FJOURNAL = {Michigan Mathematical Journal},
    VOLUME = {62},
      YEAR = {2013},
    NUMBER = {2},
     PAGES = {387--406},
      ISSN = {0026-2285},
   MRCLASS = {20F67 (57M50)},
  MRNUMBER = {3079269},
       DOI = {10.1307/mmj/1370870378},
       URL = {http://dx.doi.org/10.1307/mmj/1370870378},
}

@article{YangPacking,
   JOURNAL = {Proc. Amer. Math. Soc.},
  FJOURNAL = {Proceedings of the American Mathematical Society},
AUTHOR = {Yang, Wen-Yuan},
Note={To appear},
}


@article {DunfieldThurston2006,
    AUTHOR = {Dunfield, Nathan M. and Thurston, Dylan P.},
     TITLE = {A random tunnel number one 3-manifold does not fiber over the
              circle},
   JOURNAL = {Geom. Topol.},
  FJOURNAL = {Geometry and Topology},
    VOLUME = {10},
      YEAR = {2006},
     PAGES = {2431--2499},
      ISSN = {1465-3060},
   MRCLASS = {57M50 (20F05 57N10 57R22)},
  MRNUMBER = {2284062 (2007k:57033)},
MRREVIEWER = {Bruno Zimmermann},
       DOI = {10.2140/gt.2006.10.2431},
       URL = {http://dx.doi.org/10.2140/gt.2006.10.2431},
}
		



@article {Krammer2002,
    AUTHOR = {Krammer, Daan},
     TITLE = {Braid groups are linear},
   JOURNAL = {Ann. of Math. (2)},
  FJOURNAL = {Annals of Mathematics. Second Series},
    VOLUME = {155},
      YEAR = {2002},
    NUMBER = {1},
     PAGES = {131--156},
      ISSN = {0003-486X},
     CODEN = {ANMAAH},
   MRCLASS = {20F36 (57M07)},
  MRNUMBER = {1888796 (2003c:20040)},
MRREVIEWER = {Luis Paris},
       DOI = {10.2307/3062152},
       URL = {http://dx.doi.org/10.2307/3062152},
}
	

@article {Bigelow2001,
    AUTHOR = {Bigelow, Stephen J.},
     TITLE = {Braid groups are linear},
   JOURNAL = {J. Amer. Math. Soc.},
  FJOURNAL = {Journal of the American Mathematical Society},
    VOLUME = {14},
      YEAR = {2001},
    NUMBER = {2},
     PAGES = {471--486 (electronic)},
      ISSN = {0894-0347},
   MRCLASS = {20F36 (57M07)},
  MRNUMBER = {1815219 (2002a:20043)},
MRREVIEWER = {Darryl McCullough},
       DOI = {10.1090/S0894-0347-00-00361-1},
       URL = {http://dx.doi.org/10.1090/S0894-0347-00-00361-1},
}

@article {Krammer2000,
    AUTHOR = {Krammer, Daan},
     TITLE = {The braid group {$B_4$} is linear},
   JOURNAL = {Invent. Math.},
  FJOURNAL = {Inventiones Mathematicae},
    VOLUME = {142},
      YEAR = {2000},
    NUMBER = {3},
     PAGES = {451--486},
      ISSN = {0020-9910},
     CODEN = {INVMBH},
   MRCLASS = {20F36 (57M07)},
  MRNUMBER = {1804157 (2001k:20078)},
MRREVIEWER = {E. Formanek},
       DOI = {10.1007/s002220000088},
       URL = {http://dx.doi.org/10.1007/s002220000088},
}
	

@article {IvanovSchupp98,
    AUTHOR = {Ivanov, S. V. and Schupp, P. E.},
     TITLE = {On the hyperbolicity of small cancellation groups and
              one-relator groups},
   JOURNAL = {Trans. Amer. Math. Soc.},
  FJOURNAL = {Transactions of the American Mathematical Society},
    VOLUME = {350},
      YEAR = {1998},
    NUMBER = {5},
     PAGES = {1851--1894},
      ISSN = {0002-9947},
     CODEN = {TAMTAM},
   MRCLASS = {20F06},
  MRNUMBER = {1401522 (98h:20048)},
MRREVIEWER = {Martin Edjvet},
       DOI = {10.1090/S0002-9947-98-01818-2},
       URL = {http://dx.doi.org/10.1090/S0002-9947-98-01818-2},
}


@article {Leary_KanThurston,
    AUTHOR = {Leary, Ian J.},
     TITLE = {A metric {K}an-{T}hurston theorem},
   JOURNAL = {J. Topol.},
  FJOURNAL = {Journal of Topology},
    VOLUME = {6},
      YEAR = {2013},
    NUMBER = {1},
     PAGES = {251--284},
      ISSN = {1753-8416},
   MRCLASS = {20F67 (20J06 57S30)},
  MRNUMBER = {3029427},
MRREVIEWER = {Aditi Kar},
       URL = {https://doi.org/10.1112/jtopol/jts035},
}

@book{Serre77,
	Address = {Paris},
	Author = {Serre, J.-P.},
	Note = {Written in collaboration with H. Bass},
	Pages = {1--189},
	Publisher = {Soci\'et\'e Math\'ematique de France},
	Series = {Ast\'erisque},
	Title = {Arbres, amalgames, {${\rm SL}\sb{2}$}},
	Volume = {46},
	Year = {1977},
}

@article {BarrePichot2010,
    AUTHOR = {Barr{\'e}, Sylvain and Pichot, Mika{\"e}l},
     TITLE = {Random Groups and Nonarchimedean Lattices},
Note={Preprint 2010},
}


@article {BrewsterLennonx77,
    AUTHOR = {Brewster, D. C. and Lennox, J. C.},
     TITLE = {Maximal torsion free subgroups of polycyclic by finite groups},
   JOURNAL = {Arch. Math. (Basel)},
  FJOURNAL = {Archiv der Mathematik},
    VOLUME = {29},
      YEAR = {1977},
    NUMBER = {1},
     PAGES = {39--40},
      ISSN = {0003-889X},
   MRCLASS = {20E20},
  MRNUMBER = {0450414 (56 \#8708)},
MRREVIEWER = {H. Heineken},
}


@article {Papasoglu95,
    AUTHOR = {Papasoglu, P.},
     TITLE = {Strongly geodesically automatic groups are hyperbolic},
   JOURNAL = {Invent. Math.},
  FJOURNAL = {Inventiones Mathematicae},
    VOLUME = {121},
      YEAR = {1995},
    NUMBER = {2},
     PAGES = {323--334},
      ISSN = {0020-9910},
     CODEN = {INVMBH},
   MRCLASS = {20F32 (20F10 57M07)},
  MRNUMBER = {1346209 (96h:20073)},
MRREVIEWER = {Sarah E. Rees},
       DOI = {10.1007/BF01884301},
       URL = {http://dx.doi.org/10.1007/BF01884301},
}
		



@article {Minasyan2006,
    AUTHOR = {Minasyan, Ashot},
     TITLE = {Separable subsets of {GFERF} negatively curved groups},
   JOURNAL = {J. Algebra},
  FJOURNAL = {Journal of Algebra},
    VOLUME = {304},
      YEAR = {2006},
    NUMBER = {2},
     PAGES = {1090--1100},
      ISSN = {0021-8693},
     CODEN = {JALGA4},
   MRCLASS = {20F67},
  MRNUMBER = {2264291 (2007j:20064)},
MRREVIEWER = {Werner Nickel},
       DOI = {10.1016/j.jalgebra.2006.03.050},
       URL = {http://dx.doi.org/10.1016/j.jalgebra.2006.03.050},
}


@article {Penrose79,
    AUTHOR = {Penrose, R.},
     TITLE = {Pentaplexity: a class of nonperiodic tilings of the plane},
   JOURNAL = {Math. Intelligencer},
  FJOURNAL = {The Mathematical Intelligencer},
    VOLUME = {2},
      YEAR = {1979/80},
    NUMBER = {1},
     PAGES = {32--37},
      ISSN = {0343-6993},
     CODEN = {MAINDC},
   MRCLASS = {52A45 (05B45)},
  MRNUMBER = {558670 (81d:52012)},
MRREVIEWER = {Joshua Zak},
       DOI = {10.1007/BF03024384},
       URL = {http://dx.doi.org/10.1007/BF03024384},
}
		

@article {deBruijn81,
    AUTHOR = {de Bruijn, N. G.},
     TITLE = {Algebraic theory of {P}enrose's nonperiodic tilings of the
              plane. {I}, {II}},
   JOURNAL = {Nederl. Akad. Wetensch. Indag. Math.},
  FJOURNAL = {Koninklijke Nederlandse Akademie van Wetenschappen.
              Indagationes Mathematicae},
    VOLUME = {43},
      YEAR = {1981},
    NUMBER = {1},
     PAGES = {39--52, 53--66},
      ISSN = {0019-3577},
     CODEN = {IMTHBJ},
   MRCLASS = {05B45},
  MRNUMBER = {609465 (82e:05055)},
MRREVIEWER = {I. Debroey},
}
		



@article {Neumann2001,
    AUTHOR = {Neumann, Walter D.},
     TITLE = {Immersed and virtually embedded {$\pi_1$}-injective
              surfaces in graph manifolds},
   JOURNAL = {Algebr. Geom. Topol.},
  FJOURNAL = {Algebraic \& Geometric Topology},
    VOLUME = {1},
      YEAR = {2001},
     PAGES = {411--426 (electronic)},
      ISSN = {1472-2747},
   MRCLASS = {57N10 (57M10)},
  MRNUMBER = {1852764 (2002f:57047)},
MRREVIEWER = {Alberto Cavicchioli},
       DOI = {10.2140/agt.2001.1.411},
       URL = {http://dx.doi.org/10.2140/agt.2001.1.411},
}
		



@incollection {KapovichPotyagailoVinberg2008,
    AUTHOR = {Kapovich, Michael and Potyagailo, Leonid and Vinberg, Ernest},
     TITLE = {Noncoherence of some lattices in {${\rm Isom}(\Bbb H^n)$}},
 BOOKTITLE = {The {Z}ieschang {G}edenkschrift},
    SERIES = {Geom. Topol. Monogr.},
    VOLUME = {14},
     PAGES = {335--351},
 PUBLISHER = {Geom. Topol. Publ., Coventry},
      YEAR = {2008},
   MRCLASS = {22E40 (20F65)},
  MRNUMBER = {2484708 (2010g:22018)},
MRREVIEWER = {John R. Parker},
       DOI = {10.2140/gtm.2008.14.335},
       URL = {http://dx.doi.org/10.2140/gtm.2008.14.335},
}


@article {KapovichKleiner2005,
    AUTHOR = {Kapovich, Michael and Kleiner, Bruce},
     TITLE = {Coarse {A}lexander duality and duality groups},
   JOURNAL = {J. Differential Geom.},
  FJOURNAL = {Journal of Differential Geometry},
    VOLUME = {69},
      YEAR = {2005},
    NUMBER = {2},
     PAGES = {279--352},
      ISSN = {0022-040X},
     CODEN = {JDGEAS},
   MRCLASS = {57P10 (20F65 55M05)},
  MRNUMBER = {2168506 (2007c:57033)},
MRREVIEWER = {John Roe},
       URL = {http://projecteuclid.org/getRecord?id=euclid.jdg/1121449108},
}


@unpublished{GauteroFreeByFree,
Author = {Fran\c{c}ois Gautero},
Note = {Preprint.},
Title = {A non-trivial example of a free-by-free group with the Haagerup property}
}


@unpublished{WrightDimension,
 Author = {Nick Wright},
 Date-Added = {2010-09-06 22:03:34 -0500},
 Date-Modified = {2010-09-06 22:10:20 -0500},
 Note = {Preprint.},
 Title = {Finite asymptotic dimension for \textrm{CAT(0)} cube complexes},
 }

@article{HagenArboreal,
    author={Mark F. Hagen},
    title={Weak hyperbolicity of cube complexes and quasi-arboreal groups},
    Note={arXiv:1101.5191v4 [math.GR],},
}


@unpublished{LutowskiSzczepanski2010,
Author= {R.~Lutowski and A.~Szczepa\'{n}ski},
Note={Private communication},
Year=2010,
}

@article {AlibegovicBestvina2006,
    AUTHOR = {Alibegovi{\'c}, Emina and Bestvina, Mladen},
     TITLE = {Limit groups are {$\rm CAT(0)$}},
   JOURNAL = {J. London Math. Soc. (2)},
  FJOURNAL = {Journal of the London Mathematical Society. Second Series},
    VOLUME = {74},
      YEAR = {2006},
    NUMBER = {1},
     PAGES = {259--272},
      ISSN = {0024-6107},
     CODEN = {JLMSAK},
   MRCLASS = {57M07 (20F65)},
  MRNUMBER = {MR2254564 (2007m:57004)},
MRREVIEWER = {Vincent Guirardel},
       DOI = {10.1112/S0024610706023155},
       URL = {http://dx.doi.org/10.1112/S0024610706023155},
}



@article {Haglund1991,
    AUTHOR = {Haglund, Fr{\'e}d{\'e}ric},
     TITLE = {Les poly\`edres de {G}romov},
   JOURNAL = {C. R. Acad. Sci. Paris S\'er. I Math.},
  FJOURNAL = {Comptes Rendus de l'Acad\'emie des Sciences. S\'erie I.
              Math\'ematique},
    VOLUME = {313},
      YEAR = {1991},
    NUMBER = {9},
     PAGES = {603--606},
      ISSN = {0764-4442},
     CODEN = {CASMEI},
   MRCLASS = {57M20 (20F55 53C23)},
  MRNUMBER = {MR1133493 (92m:57005)},
MRREVIEWER = {Fr{\'e}d{\'e}ric Paulin},
}


@article {Deligne72,
    AUTHOR = {Deligne, Pierre},
     TITLE = {Les immeubles des groupes de tresses g\'en\'eralis\'es},
   JOURNAL = {Invent. Math.},
  FJOURNAL = {Inventiones Mathematicae},
    VOLUME = {17},
      YEAR = {1972},
     PAGES = {273--302},
      ISSN = {0020-9910},
   MRCLASS = {32C40 (55A25)},
  MRNUMBER = {MR0422673 (54 \#10659)},
MRREVIEWER = {Alan H. Durfee},
}


@article {Bieri76,
    AUTHOR = {Bieri, Robert},
     TITLE = {Normal subgroups in duality groups and in groups of
              cohomological dimension {$2$}},
   JOURNAL = {J. Pure Appl. Algebra},
  FJOURNAL = {Journal of Pure and Applied Algebra},
    VOLUME = {7},
      YEAR = {1976},
    NUMBER = {1},
     PAGES = {35--51},
      ISSN = {0022-4049},
   MRCLASS = {20J05 (55J30)},
  MRNUMBER = {MR0390078 (52 \#10904)},
MRREVIEWER = {Mauricio Gutierrez},
}


@article {Bestvina99,
    AUTHOR = {Bestvina, Mladen},
     TITLE = {Non-positively curved aspects of {A}rtin groups of finite
              type},
   JOURNAL = {Geom. Topol.},
  FJOURNAL = {Geometry and Topology},
    VOLUME = {3},
      YEAR = {1999},
     PAGES = {269--302 (electronic)},
      ISSN = {1465-3060},
   MRCLASS = {20F65 (20F36 57M07)},
  MRNUMBER = {MR1714913 (2000h:20079)},
MRREVIEWER = {Yoav Segev},
       DOI = {10.2140/gt.1999.3.269},
       URL = {http://dx.doi.org/10.2140/gt.1999.3.269},
}


@article {Squier87,
    AUTHOR = {Squier, Craig C.},
     TITLE = {On certain {$3$}-generator {A}rtin groups},
   JOURNAL = {Trans. Amer. Math. Soc.},
  FJOURNAL = {Transactions of the American Mathematical Society},
    VOLUME = {302},
      YEAR = {1987},
    NUMBER = {1},
     PAGES = {117--124},
      ISSN = {0002-9947},
     CODEN = {TAMTAM},
   MRCLASS = {20F05 (20E06 20F36)},
  MRNUMBER = {MR887500 (88g:20069)},
MRREVIEWER = {Stephen J. Pride},
       DOI = {10.2307/2000900},
       URL = {http://dx.doi.org/10.2307/2000900},
}


@article {KapovichILYA2001,
    AUTHOR = {Kapovich, Ilya},
     TITLE = {The combination theorem and quasiconvexity},
   JOURNAL = {Internat. J. Algebra Comput.},
  FJOURNAL = {International Journal of Algebra and Computation},
    VOLUME = {11},
      YEAR = {2001},
    NUMBER = {2},
     PAGES = {185--216},
      ISSN = {0218-1967},
   MRCLASS = {20F67 (20E06 20E08 20F65)},
  MRNUMBER = {MR1829050 (2002c:20067)},
MRREVIEWER = {Michel Coornaert},
       DOI = {10.1142/S0218196701000553},
       URL = {http://dx.doi.org/10.1142/S0218196701000553},
}
		



@article {Pride83b,
    AUTHOR = {Pride, Stephen J.},
     TITLE = {Small cancellation conditions satisfied by one-relator groups},
   JOURNAL = {Math. Z.},
  FJOURNAL = {Mathematische Zeitschrift},
    VOLUME = {184},
      YEAR = {1983},
    NUMBER = {2},
     PAGES = {283--286},
      ISSN = {0025-5874},
     CODEN = {MAZEAX},
   MRCLASS = {20F06 (20F10)},
  MRNUMBER = {MR716277 (85e:20028)},
MRREVIEWER = {N. D. Gupta},
       DOI = {10.1007/BF01252863},
       URL = {http://dx.doi.org/10.1007/BF01252863},
}


@unpublished{NevoSageevBoundary,
	Author = {Amos Nevo and Michah Sageev},
	Note = {In preparation, 2010},
Title = {Poisson Boundaries of \textrm{CAT(0)} Cube Complexes},
}


@article{LauerWise07,
    AUTHOR = {Lauer, Joseph and Wise, Daniel T.},
     TITLE = {Cubulating one-relator groups with torsion},
   JOURNAL = {Math. Proc. Cambridge Philos. Soc.},
  FJOURNAL = {Mathematical Proceedings of the Cambridge Philosophical
              Society},
    VOLUME = {155},
      YEAR = {2013},
    NUMBER = {3},
     PAGES = {411--429},
      ISSN = {0305-0041},
   MRCLASS = {20F65 (20F06)},
  MRNUMBER = {3118410},
MRREVIEWER = {Stephan Rosebrock},
       DOI = {10.1017/S0305004113000285},
       URL = {https://doi-org.proxy3.library.mcgill.ca/10.1017/S0305004113000285},
}


@unpublished{RollerPocSets,
	Author = {Roller, M.A.},
	Date-Added = {2008-09-16 15:55:38 -0500},
	Date-Modified = {2008-09-16 15:55:38 -0500},
	Note = {Preprint, Univ.\ of Southampton},
	Title = {Poc sets, median algebras and group actions. {A}n extended study of {D}unwoody's construction and {S}ageev's theorem},
	Year = {1998},
}

@article{RubinsteinSageev99,
	Author = {Rubinstein, Hyam and Sageev, Michah},
	Coden = {TPLGAF},
	Date-Added = {2008-08-27 14:32:38 -0500},
	Date-Modified = {2008-08-27 14:32:38 -0500},
	Fjournal = {Topology. An International Journal of Mathematics},
	Issn = {0040-9383},
	Journal = {Topology},
	Mrclass = {57N10 (57M50)},
	Mrnumber = {MR1690158 (2000c:57044)},
	Mrreviewer = {Joan Porti},
	Number = {6},
	Pages = {1281--1291},
	Title = {Intersection patterns of essential surfaces in {$3$}--manifolds},
	Volume = {38},
	Year = {1999},
}


@article{Scott83,
	Author = {Scott, Peter},
	Coden = {ANMAAH},
	Date-Added = {2009-07-15 16:40:14 -0500},
	Date-Modified = {2009-07-15 16:40:32 -0500},
	Fjournal = {Annals of Mathematics. Second Series},
	Issn = {0003-486X},
	Journal = {Ann. of Math. (2)},
	Mrclass = {57N10 (57N35)},
	Mrnumber = {MR683801 (84c:57008)},
	Mrreviewer = {John Hempel},
	Number = {1},
	Pages = {35--70},
	Title = {There are no fake {S}eifert fibre spaces with infinite {$\pi \sb{1}$}},
	Volume = {117},
	Year = {1983},
}


@unpublished{GuralnikLocalFiniteness,
	Author = {D. Guralnik},
	Date-Added = {2010-03-24 20:13:22 -0500},
	Date-Modified = {2010-03-24 20:23:15 -0500},
	Note = {Preprint. arXiv:math/0610950 [math.GR]},
	Title = {Local finiteness for cubulations of {CAT(0)} groups},
	Year = {2006},
}

@unpublished{GuralnikBoundaries,
	Author = {D. Guralnik},
	Date-Added = {2010-03-24 20:08:03 -0500},
	Date-Modified = {2010-03-24 20:23:01 -0500},
	Note = {Preprint. arXiv:math/0611006 [math.GR]},
	Title = {Coarse decompositions of boundaries for {CAT(0)} groups},
	Year = {2006},
}

@article{HassScott92,
	Author = {Hass, Joel and Scott, Peter},
	Coden = {TPLGAF},
	Date-Added = {2009-07-15 16:44:34 -0500},
	Date-Modified = {2009-07-15 16:44:45 -0500},
	Fjournal = {Topology. An International Journal of Mathematics},
	Issn = {0040-9383},
	Journal = {Topology},
	Mrclass = {57N10},
	Mrnumber = {MR1174254 (94g:57021)},
	Mrreviewer = {John Hempel},
	Number = {3},
	Pages = {493--517},
	Title = {Homotopy equivalence and homeomorphism of {$3$}-manifolds},
	Volume = {31},
	Year = {1992},
}

@article{HruskaRelQC,
    AUTHOR = {Hruska, G. Christopher},
     TITLE = {Relative hyperbolicity and relative quasiconvexity for
              countable groups},
   JOURNAL = {Algebr. Geom. Topol.},
  FJOURNAL = {Algebraic \& Geometric Topology},
    VOLUME = {10},
      YEAR = {2010},
    NUMBER = {3},
     PAGES = {1807--1856},
      ISSN = {1472-2747},
   MRCLASS = {20F65 (20F67)},
  MRNUMBER = {2684983},
       DOI = {10.2140/agt.2010.10.1807},
       URL = {http://dx.doi.org/10.2140/agt.2010.10.1807},
}


@article{WiseFreeCubulation,
    author={Wise, Daniel T.},
    title={Recubulating Free Groups},
     JOURNAL = {Israel J. Math.},
 FJOURNAL = {Israel Journal of Mathematics},
    PAGES={1--9},
Note={To appear},
 }


@article{WiseClean,
    author={Wise, Daniel T.},
    title={Virtual Cleanliness},
    PAGES={1--21},
    }


@article {AbramsGhrist2002,
    AUTHOR = {Abrams, Aaron and Ghrist, Robert},
     TITLE = {Finding topology in a factory: configuration spaces},
   JOURNAL = {Amer. Math. Monthly},
  FJOURNAL = {The American Mathematical Monthly},
    VOLUME = {109},
      YEAR = {2002},
    NUMBER = {2},
     PAGES = {140--150},
      ISSN = {0002-9890},
     CODEN = {AMMYAE},
   MRCLASS = {68T40 (52C99)},
  MRNUMBER = {MR1903151 (2003c:68222)},
MRREVIEWER = {Claudia Landi},
       DOI = {10.2307/2695326},
       URL = {http://dx.doi.org/10.2307/2695326},
}


@article {GubaSapir2005,
    AUTHOR = {Guba, V. S. and Sapir, M. V.},
     TITLE = {Diagram groups and directed 2-complexes: homotopy and
              homology},
   JOURNAL = {J. Pure Appl. Algebra},
  FJOURNAL = {Journal of Pure and Applied Algebra},
    VOLUME = {205},
      YEAR = {2006},
    NUMBER = {1},
     PAGES = {1--47},
      ISSN = {0022-4049},
     CODEN = {JPAAA2},
   MRCLASS = {20F65 (05E99 20F05 57M07)},
  MRNUMBER = {MR2193190 (2006j:20056)},
MRREVIEWER = {E. F. Robertson},
       DOI = {10.1016/j.jpaa.2005.06.012},
       URL = {http://dx.doi.org/10.1016/j.jpaa.2005.06.012},
}


@article {GubaSapir1997,
    AUTHOR = {Guba, Victor and Sapir, Mark},
     TITLE = {Diagram groups},
   JOURNAL = {Mem. Amer. Math. Soc.},
  FJOURNAL = {Memoirs of the American Mathematical Society},
    VOLUME = {130},
      YEAR = {1997},
    NUMBER = {620},
     PAGES = {viii+117},
      ISSN = {0065-9266},
     CODEN = {MAMCAU},
   MRCLASS = {20F05 (57M07)},
  MRNUMBER = {MR1396957 (98f:20013)},
MRREVIEWER = {Thomas Delzant},
}


@incollection {McCammond2009,
    AUTHOR = {McCammond, Jonathan P.},
     TITLE = {Constructing non-positively curved spaces and groups},
 BOOKTITLE ={Geometric and cohomological methods in group theory:
 LMS Lecture Note Series},
   Volume= {358},
      PAGES = {162-224},
      YEAR = {2009},
 }


@article {Elder2004,
    AUTHOR = {Elder, Murray J.},
     TITLE = {A non-{H}opfian almost convex group},
   JOURNAL = {J. Algebra},
  FJOURNAL = {Journal of Algebra},
    VOLUME = {271},
      YEAR = {2004},
    NUMBER = {1},
     PAGES = {11--21},
      ISSN = {0021-8693},
     CODEN = {JALGA4},
   MRCLASS = {20E06 (20F65)},
  MRNUMBER = {MR2022477 (2004k:20053)},
MRREVIEWER = {S. Andreadakis},
       DOI = {10.1016/j.jalgebra.2003.04.004},
       URL = {http://dx.doi.org/10.1016/j.jalgebra.2003.04.004},
}


@article{BergeronWiseBoundary,
   AUTHOR = {Bergeron, Nicolas and Wise, Daniel T.},
     TITLE = {A boundary criterion for cubulation},
   JOURNAL = {Amer. J. Math.},
  FJOURNAL = {American Journal of Mathematics},
    VOLUME = {134},
      YEAR = {2012},
    NUMBER = {3},
     PAGES = {843--859},
      ISSN = {0002-9327},
     CODEN = {AJMAAN},
   MRCLASS = {20F67 (57Mxx)},
  MRNUMBER = {2931226},
       DOI = {10.1353/ajm.2012.0020},
       URL = {http://dx.doi.org/10.1353/ajm.2012.0020},
}


@article {BehrstockJanuszkiewiczNeumann2009,
    AUTHOR = {Behrstock, Jason A. and Januszkiewicz, Tadeusz and Neumann,
              Walter D.},
     TITLE = {Commensurability and {QI} classification of free products of
              finitely generated abelian groups},
   JOURNAL = {Proc. Amer. Math. Soc.},
  FJOURNAL = {Proceedings of the American Mathematical Society},
    VOLUME = {137},
      YEAR = {2009},
    NUMBER = {3},
     PAGES = {811--813},
      ISSN = {0002-9939},
     CODEN = {PAMYAR},
   MRCLASS = {20E06 (20F36 20F65)},
  MRNUMBER = {MR2457418 (2009i:20051)},
MRREVIEWER = {Fran{\c{c}}ois Dahmani},
       DOI = {10.1090/S0002-9939-08-09559-2},
       URL = {http://dx.doi.org/10.1090/S0002-9939-08-09559-2},
}


@article{Charney2007,
    AUTHOR = {Charney, Ruth},
     TITLE = {An introduction to right-angled {A}rtin groups},
   JOURNAL = {Geom. Dedicata},
  FJOURNAL = {Geometriae Dedicata},
    VOLUME = {125},
      YEAR = {2007},
     PAGES = {141--158},
      ISSN = {0046-5755},
     CODEN = {GEMDAT},
   MRCLASS = {20F36 (20F65)},
  MRNUMBER = {MR2322545 (2008f:20076)},
MRREVIEWER = {Noelle C. Antony},
       DOI = {10.1007/s10711-007-9148-6},
       URL = {http://dx.doi.org/10.1007/s10711-007-9148-6},
}


@article{Champetier94,
    AUTHOR = {Champetier, Christophe},
     TITLE = {Petite simplification dans les groupes hyperboliques},
   JOURNAL = {Ann. Fac. Sci. Toulouse Math. (6)},
  FJOURNAL = {Toulouse. Facult\'e des Sciences. Annales. Math\'ematiques.
              S\'erie 6},
    VOLUME = {3},
      YEAR = {1994},
    NUMBER = {2},
     PAGES = {161--221},
      ISSN = {0240-2955},
   MRCLASS = {20F32 (20F06 53C23 57M07)},
  MRNUMBER = {MR1283206 (95e:20050)},
MRREVIEWER = {Michel Coornaert},
       URL = {http://www.numdam.org/item?id=AFST_1994_6_3_2_161_0},
}
		



@article {Gersten94,
    AUTHOR = {Gersten, S. M.},
     TITLE = {The automorphism group of a free group is not a {${\rm
              CAT}(0)$} group},
   JOURNAL = {Proc. Amer. Math. Soc.},
  FJOURNAL = {Proceedings of the American Mathematical Society},
    VOLUME = {121},
      YEAR = {1994},
    NUMBER = {4},
     PAGES = {999--1002},
      ISSN = {0002-9939},
     CODEN = {PAMYAR},
   MRCLASS = {20F32 (20E05 20F28 53C23 57M07)},
  MRNUMBER = {MR1195719 (94j:20043)},
MRREVIEWER = {S. Andreadakis},
       DOI = {10.2307/2161207},
       URL = {http://dx.doi.org/10.2307/2161207},
}


@article {Brady2000,
    AUTHOR = {Brady, Thomas},
     TITLE = {Artin groups of finite type with three generators},
   JOURNAL = {Michigan Math. J.},
  FJOURNAL = {The Michigan Mathematical Journal},
    VOLUME = {47},
      YEAR = {2000},
    NUMBER = {2},
     PAGES = {313--324},
      ISSN = {0026-2285},
   MRCLASS = {20F36 (20F05 20F55 20F65 57M07)},
  MRNUMBER = {MR1793627 (2001j:20056)},
MRREVIEWER = {Stephen P. Humphries},
       DOI = {10.1307/mmj/1030132536},
       URL = {http://dx.doi.org/10.1307/mmj/1030132536},
}


@article {Gordon2004,
    AUTHOR = {Gordon, C. McA.},
     TITLE = {Artin groups, 3-manifolds and coherence},
   JOURNAL = {Bol. Soc. Mat. Mexicana (3)},
  FJOURNAL = {Sociedad Matem\'atica Mexicana. Bolet\'\i n. Tercera Serie},
    VOLUME = {10},
      YEAR = {2004},
    NUMBER = {Special Issue},
     PAGES = {193--198},
      ISSN = {1405-213X},
   MRCLASS = {57M07 (20F36)},
  MRNUMBER = {MR2199348 (2006i:57003)},
MRREVIEWER = {Patrick Bahls},
}


@article {AppelSchupp83,
    AUTHOR = {Appel, K. I. and Schupp, P. E.},
     TITLE = {Artin groups and infinite {C}oxeter groups},
   JOURNAL = {Invent. Math.},
  FJOURNAL = {Inventiones Mathematicae},
    VOLUME = {72},
      YEAR = {1983},
    NUMBER = {2},
     PAGES = {201--220},
      ISSN = {0020-9910},
     CODEN = {INVMBH},
   MRCLASS = {20F36 (20F06 32C40)},
  MRNUMBER = {MR700768 (84h:20028)},
MRREVIEWER = {J. S. Birman},
       DOI = {10.1007/BF01389320},
       URL = {http://dx.doi.org/10.1007/BF01389320},
}
		



@article {Gitik99b,
    AUTHOR = {Gitik, Rita},
     TITLE = {On the profinite topology on negatively curved groups},
   JOURNAL = {J. Algebra},
  FJOURNAL = {Journal of Algebra},
    VOLUME = {219},
      YEAR = {1999},
    NUMBER = {1},
     PAGES = {80--86},
      ISSN = {0021-8693},
     CODEN = {JALGA4},
   MRCLASS = {20F65 (20E26 57M07)},
  MRNUMBER = {MR1707664 (2000g:20072)},
MRREVIEWER = {Michel Coornaert},
       DOI = {10.1006/jabr.1998.7847},
       URL = {http://dx.doi.org/10.1006/jabr.1998.7847},
}


@article {BFMT2009,
     AUTHOR = {Baumslag, Gilbert and Fine, Benjamin and Miller, III, Charles
               F. and Troeger, Douglas},
      TITLE = {Virtual properties of cyclically pinched one-relator groups},
    JOURNAL = {Internat. J. Algebra Comput.},
   FJOURNAL = {International Journal of Algebra and Computation},
     VOLUME = {19},
       YEAR = {2009},
     NUMBER = {2},
      PAGES = {213--227},
       ISSN = {0218-1967},
    MRCLASS = {20E06 (20F05)},
   MRNUMBER = {MR2512551},
MRREVIEWER = {David Meier},
        DOI = {10.1142/S0218196709005032},
        URL =
{http://dx.doi.org.lib-ezproxy.tamu.edu:2048/10.1142/S0218196709005032},
}


@article {WiseStructureAnnouncement09,
    AUTHOR = {Wise, Daniel T.},
     TITLE = {Research announcement: The structure of groups with a quasiconvex hierarchy},
   JOURNAL = {Electron. Res. Announc. Amer. Math. Soc.},
  FJOURNAL = {Electronic Research Announcements of the American Mathematical
              Society},
    VOLUME = {16},
      YEAR = {2009},
     PAGES = {44-55 (electronic)},
}


@article {Hruska2005,
    AUTHOR = {Hruska, G. Christopher},
     TITLE = {Geometric invariants of spaces with isolated flats},
   JOURNAL = {Topology},
  FJOURNAL = {Topology. An International Journal of Mathematics},
    VOLUME = {44},
      YEAR = {2005},
    NUMBER = {2},
     PAGES = {441--458},
      ISSN = {0040-9383},
     CODEN = {TPLGAF},
   MRCLASS = {20F67 (20F65)},
  MRNUMBER = {MR2114956 (2005k:20105)},
MRREVIEWER = {Murray J. Elder},
       DOI = {10.1016/j.top.2004.10.001},
       URL = {http://dx.doi.org/10.1016/j.top.2004.10.001},
}

@article {HruskaKleiner05,
    AUTHOR = {Hruska, G. Christopher and Kleiner, Bruce},
     TITLE = {Hadamard spaces with isolated flats},
      NOTE = {With an appendix by the authors and Mohamad Hindawi},
   JOURNAL = {Geom. Topol.},
  FJOURNAL = {Geometry and Topology},
    VOLUME = {9},
      YEAR = {2005},
     PAGES = {1501--1538 (electronic)},
      ISSN = {1465-3060},
   MRCLASS = {20F67 (20F69)},
  MRNUMBER = {MR2175151 (2007c:20105)},
MRREVIEWER = {Daniel P. Groves},
       DOI = {10.2140/gt.2005.9.1501},
       URL = {http://dx.doi.org/10.2140/gt.2005.9.1501},
}

@article {DrutuSapir2005,
    AUTHOR = {Dru{\c{t}}u, Cornelia and Sapir, Mark},
     TITLE = {Tree-graded spaces and asymptotic cones of groups},
      NOTE = {With an appendix by Denis Osin and Sapir},
   JOURNAL = {Topology},
  FJOURNAL = {Topology. An International Journal of Mathematics},
    VOLUME = {44},
      YEAR = {2005},
    NUMBER = {5},
     PAGES = {959--1058},
      ISSN = {0040-9383},
     CODEN = {TPLGAF},
   MRCLASS = {20F67 (57M07)},
  MRNUMBER = {MR2153979 (2006d:20078)},
MRREVIEWER = {Ilya Kapovich},
       DOI = {10.1016/j.top.2005.03.003},
       URL = {http://dx.doi.org/10.1016/j.top.2005.03.003},
}


@article {RequeimaWiseRelativeCoherence,
author={Requeima, James and Wise, Daniel T.},
title={Relative sectional curvature and coherent groups},
Note={Preprint 2009},
}

@article{WiseRandomMorse,
   AUTHOR = {Wise, Daniel T.},
     TITLE = {Morse theory, random subgraphs, and incoherent groups},
   JOURNAL = {Bull. Lond. Math. Soc.},
  FJOURNAL = {Bulletin of the London Mathematical Society},
    VOLUME = {43},
      YEAR = {2011},
    NUMBER = {5},
     PAGES = {840--848},
      ISSN = {0024-6093},
   MRCLASS = {53C23 (20F65 20H10)},
  MRNUMBER = {2854555},
       DOI = {10.1112/blms/bdr023},
       URL = {http://dx.doi.org/10.1112/blms/bdr023},
}


@article {BestvinaFeighn91,
    AUTHOR = {Bestvina, Mladen and Feighn, Mark},
     TITLE = {Bounding the complexity of simplicial group actions on trees},
   JOURNAL = {Invent. Math.},
  FJOURNAL = {Inventiones Mathematicae},
    VOLUME = {103},
      YEAR = {1991},
    NUMBER = {3},
     PAGES = {449--469},
      ISSN = {0020-9910},
     CODEN = {INVMBH},
   MRCLASS = {20E08 (57M07)},
  MRNUMBER = {MR1091614 (92c:20044)},
MRREVIEWER = {Roger C. Alperin},
}

@article {Lackenby10,
    AUTHOR = {Lackenby, Marc},
     TITLE = {Surface subgroups of {K}leinian groups with torsion},
   JOURNAL = {Invent. Math.},
  FJOURNAL = {Inventiones Mathematicae},
    VOLUME = {179},
      YEAR = {2010},
    NUMBER = {1},
     PAGES = {175--190},
      ISSN = {0020-9910},
     CODEN = {INVMBH},
   MRCLASS = {30F40 (20H10)},
  MRNUMBER = {2563763},
       DOI = {10.1007/s00222-009-0215-5},
       URL = {http://dx.doi.org/10.1007/s00222-009-0215-5},
}

@book {BorelWallach80,
    AUTHOR = {Borel, Armand and Wallach, Nolan R.},
     TITLE = {Continuous cohomology, discrete subgroups, and representations
              of reductive groups},
    SERIES = {Annals of Mathematics Studies},
    VOLUME = {94},
 PUBLISHER = {Princeton University Press},
   ADDRESS = {Princeton, N.J.},
      YEAR = {1980},
     PAGES = {xvii+388},
      ISBN = {0-691-08248-0; 0-691-08249-9},
   MRCLASS = {22E41 (22E40 22E45 57T15)},
  MRNUMBER = {MR554917 (83c:22018)},
MRREVIEWER = {Roger Howe},
}

@article {Lubotzky96,
    AUTHOR = {Lubotzky, Alexander},
     TITLE = {Eigenvalues of the {L}aplacian, the first {B}etti number and
              the congruence subgroup problem},
   JOURNAL = {Ann. of Math. (2)},
  FJOURNAL = {Annals of Mathematics. Second Series},
    VOLUME = {144},
      YEAR = {1996},
    NUMBER = {2},
     PAGES = {441--452},
      ISSN = {0003-486X},
     CODEN = {ANMAAH},
   MRCLASS = {22E40 (11R52 57R20)},
  MRNUMBER = {MR1418904 (98h:22013)},
}

 @article {Bergeron2002,
    AUTHOR = {Bergeron, N.},
     TITLE = {Cycles g\'eod\'esiques transverses dans les vari\'et\'es
              hyperboliques},
   JOURNAL = {Geom. Funct. Anal.},
  FJOURNAL = {Geometric and Functional Analysis},
    VOLUME = {12},
      YEAR = {2002},
    NUMBER = {3},
     PAGES = {437--463},
      ISSN = {1016-443X},
     CODEN = {GFANFB},
   MRCLASS = {57M50 (53C22 53C23)},
  MRNUMBER = {MR1924368 (2003g:57025)},
MRREVIEWER = {Athanase Papadopoulos},
}


@incollection {Bowditch99,
    AUTHOR = {Bowditch, B. H.},
     TITLE = {Convergence groups and configuration spaces},
 BOOKTITLE = {Geometric group theory down under ({C}anberra, 1996)},
     PAGES = {23--54},
 PUBLISHER = {de Gruyter},
   ADDRESS = {Berlin},
      YEAR = {1999},
   MRCLASS = {20F34 (20E08 57S30)},
  MRNUMBER = {MR1714838 (2001d:20035)},
MRREVIEWER = {Fr{\'e}d{\'e}ric Paulin},
}

@article {Bowditch98cb,
    AUTHOR = {Bowditch, Brian H.},
     TITLE = {A topological characterisation of hyperbolic groups},
   JOURNAL = {J. Amer. Math. Soc.},
  FJOURNAL = {Journal of the American Mathematical Society},
    VOLUME = {11},
      YEAR = {1998},
    NUMBER = {3},
     PAGES = {643--667},
      ISSN = {0894-0347},
   MRCLASS = {20F32 (53C23 54H15 57S30)},
  MRNUMBER = {MR1602069 (99c:20048)},
MRREVIEWER = {Jane Gilman},
}


@incollection {DelzantGromov05,
    AUTHOR = {Delzant, Thomas and Gromov, Misha},
     TITLE = {Cuts in {K}\"ahler groups},
 BOOKTITLE = {Infinite groups: geometric, combinatorial and dynamical
              aspects},
    SERIES = {Progr. Math.},
    VOLUME = {248},
     PAGES = {31--55},
 PUBLISHER = {Birkh\"auser},
   ADDRESS = {Basel},
      YEAR = {2005},
   MRCLASS = {32Q15 (20F65 57M07)},
  MRNUMBER = {MR2195452 (2006j:32023)},
MRREVIEWER = {Azniv Kasparian},
}



@article{KahnMarkovic09,
    AUTHOR = {Kahn, Jeremy and Markovic, Vladimir},
     TITLE = {Immersing almost geodesic surfaces in a closed hyperbolic
              three manifold},
   JOURNAL = {Ann. of Math. (2)},
  FJOURNAL = {Annals of Mathematics. Second Series},
    VOLUME = {175},
      YEAR = {2012},
    NUMBER = {3},
     PAGES = {1127--1190},
      ISSN = {0003-486X},
     CODEN = {ANMAAH},
   MRCLASS = {57M50 (30F40)},
  MRNUMBER = {2912704},
MRREVIEWER = {James W. Anderson},
       DOI = {10.4007/annals.2012.175.3.4},
       URL = {http://dx.doi.org/10.4007/annals.2012.175.3.4},
}



@book {Hempel2004,
    AUTHOR = {Hempel, John},
     TITLE = {3-manifolds},
      NOTE = {Reprint of the 1976 original},
 PUBLISHER = {AMS Chelsea Publishing, Providence, RI},
      YEAR = {2004},
     PAGES = {xii+195},
      ISBN = {0-8218-3695-1},
   MRCLASS = {57N10},
  MRNUMBER = {MR2098385 (2005e:57053)},
}


@article {Haglund2002,
    AUTHOR = {Haglund, Fr{\'e}d{\'e}ric},
     TITLE = {Existence, unicit\'e et homog\'en\'eit\'e de certains
              immeubles hyperboliques},
   JOURNAL = {Math. Z.},
  FJOURNAL = {Mathematische Zeitschrift},
    VOLUME = {242},
      YEAR = {2002},
    NUMBER = {1},
     PAGES = {97--148},
      ISSN = {0025-5874},
     CODEN = {MAZEAX},
   MRCLASS = {51E24 (20E42 57M20)},
  MRNUMBER = {MR1985452 (2004f:51028)},
MRREVIEWER = {Nadia Benakli},
}



@article {Bourdon97,
    AUTHOR = {Bourdon, M.},
     TITLE = {Immeubles hyperboliques, dimension conforme et rigidit\'e de
              {M}ostow},
   JOURNAL = {Geom. Funct. Anal.},
  FJOURNAL = {Geometric and Functional Analysis},
    VOLUME = {7},
      YEAR = {1997},
    NUMBER = {2},
     PAGES = {245--268},
      ISSN = {1016-443X},
     CODEN = {GFANFB},
   MRCLASS = {20E42 (20F32 51E24 57M50)},
  MRNUMBER = {MR1445387 (98c:20056)},
MRREVIEWER = {Michel Coornaert},
}
		

@article {Haglund2006,
    AUTHOR = {Haglund, Fr{\'e}d{\'e}ric},
     TITLE = {Commensurability and separability of quasiconvex subgroups},
   JOURNAL = {Algebr. Geom. Topol.},
  FJOURNAL = {Algebraic \& Geometric Topology},
    VOLUME = {6},
      YEAR = {2006},
     PAGES = {949--1024 (electronic)},
      ISSN = {1472-2747},
   MRCLASS = {20F67 (20F55 20F65 51E24)},
  MRNUMBER = {MR2240922 (2007k:20092)},
MRREVIEWER = {Michel Coornaert},
}


@article {CooperLongReid97b,
    AUTHOR = {Cooper, D. and Long, D. D. and Reid, A. W.},
     TITLE = {Finite foliations and similarity interval exchange maps},
   JOURNAL = {Topology},
  FJOURNAL = {Topology. An International Journal of Mathematics},
    VOLUME = {36},
      YEAR = {1997},
    NUMBER = {1},
     PAGES = {209--227},
      ISSN = {0040-9383},
     CODEN = {TPLGAF},
   MRCLASS = {57R30 (57N10 57N35)},
  MRNUMBER = {MR1410472 (97j:57032)},
MRREVIEWER = {Athanase Papadopoulos},
}


@article {Fenley99,
    AUTHOR = {Fenley, S{\'e}rgio R.},
     TITLE = {Surfaces transverse to pseudo-{A}nosov flows and virtual
              fibers in {$3$}-manifolds},
   JOURNAL = {Topology},
  FJOURNAL = {Topology. An International Journal of Mathematics},
    VOLUME = {38},
      YEAR = {1999},
    NUMBER = {4},
     PAGES = {823--859},
      ISSN = {0040-9383},
     CODEN = {TPLGAF},
   MRCLASS = {57R30 (57N10)},
  MRNUMBER = {MR1679801 (2001a:57041)},
MRREVIEWER = {Darren D. Long},
}


@article {Mangum98,
    AUTHOR = {Mangum, Brian S.},
     TITLE = {Incompressible surfaces and pseudo-{A}nosov flows},
   JOURNAL = {Topology Appl.},
  FJOURNAL = {Topology and its Applications},
    VOLUME = {87},
      YEAR = {1998},
    NUMBER = {1},
     PAGES = {29--51},
      ISSN = {0166-8641},
     CODEN = {TIAPD9},
   MRCLASS = {57M50 (57R30 58F18)},
  MRNUMBER = {MR1626072 (99e:57024)},
MRREVIEWER = {Darren D. Long},
}


@article {Masters2006,
    AUTHOR = {Masters, Joseph D.},
     TITLE = {Thick surfaces in hyperbolic 3-manifolds},
   JOURNAL = {Geom. Dedicata},
  FJOURNAL = {Geometriae Dedicata},
    VOLUME = {119},
      YEAR = {2006},
     PAGES = {17--33},
      ISSN = {0046-5755},
     CODEN = {GEMDAT},
   MRCLASS = {57M50 (57N10)},
  MRNUMBER = {MR2247645 (2007f:57031)},
MRREVIEWER = {Sungbok Hong},
}



@article {CooperLongReid94,
    AUTHOR = {Cooper, D. and Long, D. D. and Reid, A. W.},
     TITLE = {Bundles and finite foliations},
   JOURNAL = {Invent. Math.},
  FJOURNAL = {Inventiones Mathematicae},
    VOLUME = {118},
      YEAR = {1994},
    NUMBER = {2},
     PAGES = {255--283},
      ISSN = {0020-9910},
     CODEN = {INVMBH},
   MRCLASS = {57N10 (55R10 57M50 57R30)},
  MRNUMBER = {MR1292113 (96h:57013)},
}

@article {JanzenWise09,
    AUTHOR = {Janzen, David and Wise, Daniel},
     TITLE = {Cubulating rhombus groups},
   JOURNAL = {Groups Geom. Dyn.},
  FJOURNAL = {Groups, Geometry, and Dynamics},
    VOLUME = {7},
      YEAR = {2013},
    NUMBER = {2},
     PAGES = {419--442},
      ISSN = {1661-7207},
   MRCLASS = {Preliminary Data},
  MRNUMBER = {3054576},
       DOI = {10.4171/GGD/188},
       URL = {http://dx.doi.org/10.4171/GGD/188},
}
		


@article {Sela2003,
    AUTHOR = {Sela, Z.},
     TITLE = {Diophantine geometry over groups. {II}. {C}ompletions,
              closures and formal solutions},
   JOURNAL = {Israel J. Math.},
  FJOURNAL = {Israel Journal of Mathematics},
    VOLUME = {134},
      YEAR = {2003},
     PAGES = {173--254},
      ISSN = {0021-2172},
     CODEN = {ISJMAP},
   MRCLASS = {20F65 (03B25 20E05 20F10)},
  MRNUMBER = {MR1972179 (2004g:20061)},
MRREVIEWER = {Jos{\'e} Burillo},
}
	


@article{KozakovaSapirGeneric,
author={Iva Koz{\'a}kov{\'a} and Mark Sapir},
title={Almost all one-relator groups with at least three generators are residually finite},
year={2008},
}

@article {Wilton2008,
    AUTHOR = {Wilton, Henry},
     TITLE = {Hall's theorem for limit groups},
   JOURNAL = {Geom. Funct. Anal.},
  FJOURNAL = {Geometric and Functional Analysis},
    VOLUME = {18},
      YEAR = {2008},
    NUMBER = {1},
     PAGES = {271--303},
      ISSN = {1016-443X},
     CODEN = {GFANFB},
   MRCLASS = {20F65 (20E05 20E26)},
  MRNUMBER = {MR2399104 (2009d:20101)},
MRREVIEWER = {Vassilis Metaftsis},
}

@article{DelzantPapasoglu,
author={Thomas Delzant and Panos Papasoglu},
title={Codimension one subgroups and boundaries of hyperbolic groups},
year={2008},
}

@article{SelaRetractiveTowers,
    author={Zlil Sela},
    title={What is the correct reference?},
    }

@article {KharlampovichMyasnikov98b,
    AUTHOR = {Kharlampovich, O. and Myasnikov, A.},
     TITLE = {Irreducible affine varieties over a free group. {II}.
              {S}ystems in triangular quasi-quadratic form and description
              of residually free groups},
   JOURNAL = {J. Algebra},
  FJOURNAL = {Journal of Algebra},
    VOLUME = {200},
      YEAR = {1998},
    NUMBER = {2},
     PAGES = {517--570},
      ISSN = {0021-8693},
     CODEN = {JALGA4},
   MRCLASS = {20E10 (20E26)},
  MRNUMBER = {MR1610664 (2000b:20032b)},
}

@article {GrovesManning2008,
    AUTHOR = {Groves, Daniel and Manning, Jason Fox},
     TITLE = {Dehn filling in relatively hyperbolic groups},
   JOURNAL = {Israel J. Math.},
  FJOURNAL = {Israel Journal of Mathematics},
    VOLUME = {168},
      YEAR = {2008},
     PAGES = {317--429},
      ISSN = {0021-2172},
     CODEN = {ISJMAP},
   MRCLASS = {57M50},
  MRNUMBER = {MR2448064},
MRREVIEWER = {Colin C. Adams},
}

@article {Osin2007,
    AUTHOR = {Osin, Denis V.},
     TITLE = {Peripheral fillings of relatively hyperbolic groups},
   JOURNAL = {Invent. Math.},
  FJOURNAL = {Inventiones Mathematicae},
    VOLUME = {167},
      YEAR = {2007},
    NUMBER = {2},
     PAGES = {295--326},
      ISSN = {0020-9910},
     CODEN = {INVMBH},
   MRCLASS = {20F67 (20E26 20F06 20F65 57M27)},
  MRNUMBER = {MR2270456 (2008d:20080)},
MRREVIEWER = {Ilya Kapovich},
}


@article {McCammond2000,
    AUTHOR = {McCammond, Jonathan P.},
     TITLE = {A general small cancellation theory},
   JOURNAL = {Internat. J. Algebra Comput.},
  FJOURNAL = {International Journal of Algebra and Computation},
    VOLUME = {10},
      YEAR = {2000},
    NUMBER = {1},
     PAGES = {1--172},
      ISSN = {0218-1967},
   MRCLASS = {20F06 (20F65 57M07)},
  MRNUMBER = {MR1752738 (2001f:20064)},
MRREVIEWER = {Martin Edjvet},
}


@article{OlshanskiiReference,
author={Yu Olshanskii},
title={What is the correct reference?},
}


@MISC{WiseIsraelHierarchyOLD,
    author={Wise, Daniel T.},
    title={The structure of groups with a quasiconvex hierarchy},
NOTE={pp. 1--189. Submitted},
howpublished = {Available at \url{http://www.math.mcgill.ca/wise/papers}},
    }

@book{WiseIsraelHierarchy,
    author={Wise, Daniel T.},
    title={The structure of groups with a quasiconvex hierarchy},
   note = {Annals of Mathematics Studies, to appear},
pages = {iv + 310}},
    }


@article{SageevWiseCores,
     AUTHOR = {Sageev, Michah and Wise, Daniel T.},
     TITLE = {Cores for quasiconvex actions},
   JOURNAL = {Proc. Amer. Math. Soc.},
  FJOURNAL = {Proceedings of the American Mathematical Society},
    VOLUME = {143},
      YEAR = {2015},
    NUMBER = {7},
     PAGES = {2731--2741},
      ISSN = {0002-9939},
   MRCLASS = {20F67},
  MRNUMBER = {3336599},
       DOI = {10.1090/S0002-9939-2015-12297-6},
       URL = {http://dx.doi.org/10.1090/S0002-9939-2015-12297-6},
}


@article {BestvinaKleinerSageev,
    AUTHOR = {Bestvina, Mladen and Kleiner, Bruce and Sageev, Michah},
     TITLE = {The asymptotic geometry of right-angled {A}rtin groups. {I}},
   JOURNAL = {Geom. Topol.},
  FJOURNAL = {Geometry \& Topology},
    VOLUME = {12},
      YEAR = {2008},
    NUMBER = {3},
     PAGES = {1653--1699},
      ISSN = {1465-3060},
   MRCLASS = {20F65 (05C25)},
  MRNUMBER = {MR2421136 (2009f:20061)},
MRREVIEWER = {Kim E. Ruane},
       DOI = {10.2140/gt.2008.12.1653},
       URL = {http://dx.doi.org/10.2140/gt.2008.12.1653},
}
	


@article {Masters2008,
    AUTHOR = {Masters, Joseph D.},
     TITLE = {Kleinian groups with ubiquitous surface subgroups},
   JOURNAL = {Groups Geom. Dyn.},
  FJOURNAL = {Groups, Geometry, and Dynamics},
    VOLUME = {2},
      YEAR = {2008},
    NUMBER = {2},
     PAGES = {263--269},
      ISSN = {1661-7207},
   MRCLASS = {57M50 (20H10)},
  MRNUMBER = {MR2393182 (2009b:57040)},
MRREVIEWER = {John G. Ratcliffe},
}


@article {MastersZhang2008,
    AUTHOR = {Masters, Joseph D. and Zhang, Xingru},
     TITLE = {Closed quasi-{F}uchsian surfaces in hyperbolic knot
              complements},
   JOURNAL = {Geom. Topol.},
  FJOURNAL = {Geometry \& Topology},
    VOLUME = {12},
      YEAR = {2008},
    NUMBER = {4},
     PAGES = {2095--2171},
   MRCLASS = {57M50 (20E26 57M25 57N35)},
  MRNUMBER = {MR2431017 (2009g:57029)},
MRREVIEWER = {John G. Ratcliffe},
}


@article {CooperWalsh2006,
    AUTHOR = {Cooper, Daryl and Walsh, Genevieve S.},
     TITLE = {Three-manifolds, virtual homology, and group determinants},
   JOURNAL = {Geom. Topol.},
  FJOURNAL = {Geometry and Topology},
    VOLUME = {10},
      YEAR = {2006},
     PAGES = {2247--2269 (electronic)},
      ISSN = {1465-3060},
   MRCLASS = {57N10 (20C10 57M25)},
  MRNUMBER = {MR2284057 (2008m:57049)},
MRREVIEWER = {J. S. Birman},
}
		

@article {CooperLong2001,
    AUTHOR = {Cooper, D. and Long, D. D.},
     TITLE = {Some surface subgroups survive surgery},
   JOURNAL = {Geom. Topol.},
  FJOURNAL = {Geometry and Topology},
    VOLUME = {5},
      YEAR = {2001},
     PAGES = {347--367 (electronic)},
      ISSN = {1465-3060},
   MRCLASS = {57M50 (57N10)},
  MRNUMBER = {MR1825666 (2002g:57031)},
MRREVIEWER = {Sergej V. Matveev},
}
		

@article {BakerCooper2000,
    AUTHOR = {Baker, M. and Cooper, D.},
     TITLE = {Immersed, virtually-embedded, boundary slopes},
   JOURNAL = {Topology Appl.},
  FJOURNAL = {Topology and its Applications},
    VOLUME = {102},
      YEAR = {2000},
    NUMBER = {3},
     PAGES = {239--252},
      ISSN = {0166-8641},
     CODEN = {TIAPD9},
   MRCLASS = {57M25 (57M50 57N10)},
  MRNUMBER = {MR1745446 (2000m:57006)},
MRREVIEWER = {Andrei Yu. Vesnin},
}

@article {CooperLong99,
    AUTHOR = {Cooper, D. and Long, D. D.},
     TITLE = {Virtually {H}aken {D}ehn-filling},
   JOURNAL = {J. Differential Geom.},
  FJOURNAL = {Journal of Differential Geometry},
    VOLUME = {52},
      YEAR = {1999},
    NUMBER = {1},
     PAGES = {173--187},
      ISSN = {0022-040X},
     CODEN = {JDGEAS},
   MRCLASS = {57M50 (57N10)},
  MRNUMBER = {MR1743462 (2001a:57025)},
MRREVIEWER = {Danny C. Calegari},
}
		

@article {Li2002,
    AUTHOR = {Li, Tao},
     TITLE = {Boundary curves of surfaces with the 4-plane property},
   JOURNAL = {Geom. Topol.},
  FJOURNAL = {Geometry and Topology},
    VOLUME = {6},
      YEAR = {2002},
     PAGES = {609--647 (electronic)},
      ISSN = {1465-3060},
   MRCLASS = {57M50 (57M07 57M25 57N10)},
  MRNUMBER = {MR1941725 (2003m:57039)},
MRREVIEWER = {William Dunbar},
}


@article {MyasnikovRemeslennikov96,
    AUTHOR = {Myasnikov, A. G. and Remeslennikov, V. N.},
     TITLE = {Exponential groups. {II}. {E}xtensions of centralizers and
              tensor completion of {CSA}-groups},
   JOURNAL = {Internat. J. Algebra Comput.},
  FJOURNAL = {International Journal of Algebra and Computation},
    VOLUME = {6},
      YEAR = {1996},
    NUMBER = {6},
     PAGES = {687--711},
      ISSN = {0218-1967},
   MRCLASS = {20F99 (20F06)},
  MRNUMBER = {MR1421886 (97j:20039)},
MRREVIEWER = {Alla S. Detinko},
}


@article {OsinBook06,
    AUTHOR = {Osin, Denis V.},
     TITLE = {Relatively hyperbolic groups: intrinsic geometry, algebraic
              properties, and algorithmic problems},
   JOURNAL = {Mem. Amer. Math. Soc.},
  FJOURNAL = {Memoirs of the American Mathematical Society},
    VOLUME = {179},
      YEAR = {2006},
    NUMBER = {843},
     PAGES = {vi+100},
      ISSN = {0065-9266},
     CODEN = {MAMCAU},
   MRCLASS = {20F67},
  MRNUMBER = {MR2182268 (2006i:20047)},
MRREVIEWER = {Ilya Kapovich},
}
		

@article {Agol08,
    AUTHOR = {Agol, Ian},
     TITLE = {Criteria for virtual fibering},
   JOURNAL = {J. Topol.},
  FJOURNAL = {Journal of Topology},
    VOLUME = {1},
      YEAR = {2008},
    NUMBER = {2},
     PAGES = {269--284},
      ISSN = {1753-8416},
   MRCLASS = {57M50 (57N10)},
  MRNUMBER = {MR2399130 (2009b:57033)},
MRREVIEWER = {Darren D. Long},
}


@article {CalegariGabai06,
    AUTHOR = {Calegari, Danny and Gabai, David},
     TITLE = {Shrinkwrapping and the taming of hyperbolic 3-manifolds},
   JOURNAL = {J. Amer. Math. Soc.},
  FJOURNAL = {Journal of the American Mathematical Society},
    VOLUME = {19},
      YEAR = {2006},
    NUMBER = {2},
     PAGES = {385--446 (electronic)},
      ISSN = {0894-0347},
   MRCLASS = {57M50 (30F40 57N10)},
  MRNUMBER = {MR2188131 (2006g:57030)},
MRREVIEWER = {Bruno Zimmermann},
}



@PHDTHESIS{DromsPhD83,
   AUTHOR = {Droms, Carl},
  TITLE =        "Graph Groups",
  SCHOOL =       "Syracuse University",
  YEAR =         "1983",
}



@MastersThesis{LauerMSc07,
  author =   {Joseph Lauer},
  title =    {Cubulating One Relator Groups With Torsion},
  school =   {McGill University},
  year =     {2007},
}


@article{HsuWiseCubulatingMalnormal,
   AUTHOR = {Hsu, Tim and Wise, Daniel T.},
   title = {Cubulating Malnormal Amalgams},
   JOURNAL = {Invent. Math.},
  FJOURNAL = {Inventiones Mathematicae},
  VOLUME = {199},
  ISSUE = {2},
   YEAR = {2015},
   PAGES = {293-331},
   }

@article {RipsSegev87,
    AUTHOR = {Rips, Eliyahu and Segev, Yoav},
     TITLE = {Torsion-free group without unique product property},
   JOURNAL = {J. Algebra},
  FJOURNAL = {Journal of Algebra},
    VOLUME = {108},
      YEAR = {1987},
    NUMBER = {1},
     PAGES = {116--126},
      ISSN = {0021-8693},
     CODEN = {JALGA4},
   MRCLASS = {20F06 (20C07)},
  MRNUMBER = {MR887195 (88g:20071)},
MRREVIEWER = {Stephen J. Pride},
}


@misc{HaglundHabillitation,
    AUTHOR = {Haglund, Fr{\'e}d{\'e}ric},
title = {Aspects combinatoires de la th{\'e}orie g{\'e}om{\'e}trique des groupes},
year = {2007},
howpublished = {Universit{\'e} Paris Sud, Orsay},
note = {Habilitation},
}



@article {BuyaloSchroeder2005,
   AUTHOR = {Buyalo, Sergei and Schroeder, Viktor},
     TITLE = {Embedding of hyperbolic spaces in the product of trees},
   JOURNAL = {Geom. Dedicata},
  FJOURNAL = {Geometriae Dedicata},
    VOLUME = {113},
      YEAR = {2005},
     PAGES = {75--93},
      ISSN = {0046-5755},
     CODEN = {GEMDAT},
   MRCLASS = {53C23},
  MRNUMBER = {MR2171299 (2006f:53055)},
MRREVIEWER = {Joseph E. Borzellino},
}


@article {BonkSchrmm2000,
    AUTHOR = {Bonk, M. and Schramm, O.},
     TITLE = {Embeddings of {G}romov hyperbolic spaces},
   JOURNAL = {Geom. Funct. Anal.},
 FJOURNAL = {Geometric and Functional Analysis},
   VOLUME = {10},
     YEAR = {2000},
   NUMBER = {2},
    PAGES = {266--306},
     ISSN = {1016-443X},
    CODEN = {GFANFB},
  MRCLASS = {53C23 (54E40 57M07)},
 MRNUMBER = {MR1771428 (2001g:53077)},
MRREVIEWER = {Michel Coornaert},
}

@article {Arzhantseva2001,
    AUTHOR = {Arzhantseva, G. N.},
     TITLE = {On quasiconvex subgroups of word hyperbolic groups},
   JOURNAL = {Geom. Dedicata},
  FJOURNAL = {Geometriae Dedicata},
    VOLUME = {87},
      YEAR = {2001},
    NUMBER = {1-3},
     PAGES = {191--208},
      ISSN = {0046-5755},
     CODEN = {GEMDAT},
   MRCLASS = {20F67 (57M07)},
  MRNUMBER = {MR1866849 (2003h:20076)},
}
		

@article {KapovichShort96,
    AUTHOR = {Kapovich, Ilya and Short, Hamish},
     TITLE = {Greenberg's theorem for quasiconvex subgroups of word
              hyperbolic groups},
   JOURNAL = {Canad. J. Math.},
  FJOURNAL = {Canadian Journal of Mathematics. Journal Canadien de
              Math\'ematiques},
    VOLUME = {48},
      YEAR = {1996},
    NUMBER = {6},
     PAGES = {1224--1244},
      ISSN = {0008-414X},
     CODEN = {CJMAAB},
   MRCLASS = {20F32 (57M07)},
  MRNUMBER = {MR1426902 (98g:20060)},
MRREVIEWER = {Tadeusz Januszkiewicz},
}
	


@unpublished {Roller98,
    AUTHOR = {Roller, Martin A.},
     TITLE = {Poc-sets, median algebras and group actions. An extended study of
Dunwoodyís construction and Sageevís theorem},
}

@article{HsuLeary08,
    AUTHOR = {Hsu, T. and Leary, I. J.},
     TITLE = {Artin {HNN}-extensions virtually embed in {A}rtin groups},
   JOURNAL = {Bull. Lond. Math. Soc.},
  FJOURNAL = {Bulletin of the London Mathematical Society},
    VOLUME = {40},
      YEAR = {2008},
    NUMBER = {4},
     PAGES = {715--719},
      ISSN = {0024-6093},
   MRCLASS = {20F36 (20F55 20F65)},
  MRNUMBER = {MR2441144 (2009j:20047)},
MRREVIEWER = {Valerij G. Bardakov},
       DOI = {10.1112/blms/bdn055},
       URL = {http://dx.doi.org/10.1112/blms/bdn055},
}
		


@article{HaglundWiseAmalgams,
     AUTHOR = {Haglund, Fr{\'e}d{\'e}ric and Wise, Daniel T.},
     TITLE = {A combination theorem for special cube complexes},
   JOURNAL = {Ann. of Math. (2)},
  FJOURNAL = {Annals of Mathematics. Second Series},
    VOLUME = {176},
      YEAR = {2012},
    NUMBER = {3},
     PAGES = {1427--1482},
      ISSN = {0003-486X},
     CODEN = {ANMAAH},
   MRCLASS = {20F65},
  MRNUMBER = {2979855},
       DOI = {10.4007/annals.2012.176.3.2},
       URL = {http://dx.doi.org/10.4007/annals.2012.176.3.2},
}


@article{WiseLauer07,
    AUTHOR = {Lauer, Joseph and Wise, Daniel T.},
     TITLE = {Cubulating one-relator groups with torsion},
   JOURNAL = {Math. Proc. Cambridge Philos. Soc.},
  FJOURNAL = {Mathematical Proceedings of the Cambridge Philosophical
              Society},
    VOLUME = {155},
      YEAR = {2013},
    NUMBER = {3},
     PAGES = {411--429},
      ISSN = {0305-0041},
   MRCLASS = {20F65},
  MRNUMBER = {3118410},
       DOI = {10.1017/S0305004113000285},
       URL = {http://dx.doi.org/10.1017/S0305004113000285},
}

@article {DromsLewinServatius91,
    AUTHOR = {Droms, Carl and Lewin, Jacques and Servatius, Herman},
     TITLE = {Tree groups and the {$4$}-string pure braid group},
   JOURNAL = {J. Pure Appl. Algebra},
  FJOURNAL = {Journal of Pure and Applied Algebra},
    VOLUME = {70},
      YEAR = {1991},
    NUMBER = {3},
     PAGES = {251--261},
      ISSN = {0022-4049},
     CODEN = {JPAAA2},
   MRCLASS = {20F36 (20E06 20F32 57M07)},
  MRNUMBER = {MR1104843 (92b:20040)},
MRREVIEWER = {Darren D. Long},
}


@PHDTHESIS{Williams99,
  AUTHOR =       "B. T. Williams",
  TITLE =        "Two topics in geometric group theory",
  SCHOOL =       "University of Southampton",
  YEAR =         "1999",
}

@ARTICLE{CapraceParallelWall06,
    AUTHOR = {Caprace, Pierre-Emmanuel},
     TITLE = {Conjugacy of 2-spherical subgroups of {C}oxeter groups and
              parallel walls},
   JOURNAL = {Algebr. Geom. Topol.},
  FJOURNAL = {Algebraic \& Geometric Topology},
    VOLUME = {6},
      YEAR = {2006},
     PAGES = {1987--2029 (electronic)},
      ISSN = {1472-2747},
   MRCLASS = {20F65 (20F55 20F67 57M07)},
  MRNUMBER = {MR2263057},
}


@ARTICLE{Davis83,
  AUTHOR =       "Davis, Michael W.",
  TITLE =        "Groups generated by reflections and aspherical manifolds not covered by Euclidean space.",
  JOURNAL =      "Ann. of Math. (2)",
  volume =       "117",
  YEAR =         "1983",
  number =       "2",
  pages =        "293--324",
}


@PHDTHESIS{Moussong88,
  AUTHOR =       "Moussong, G{\'a}bor",
  TITLE =        "Hyperbolic Coxeter Groups",
  SCHOOL =       "Ohio State University",
  YEAR =         "1988",
}


@incollection {CharneyDavis94,
    AUTHOR = {Charney, Ruth and Davis, Michael W.},
     TITLE = {Finite {$K(\pi, 1)$}s for {A}rtin groups},
 BOOKTITLE = {Prospects in topology (Princeton, NJ, 1994)},
    SERIES = {Ann. of Math. Stud.},
    VOLUME = {138},
     PAGES = {110--124},
 PUBLISHER = {Princeton Univ. Press},
   ADDRESS = {Princeton, NJ},
      YEAR = {1995},
   MRCLASS = {57M07 (20F36 55P20)},
  MRNUMBER = {MR1368655 (97a:57001)},
MRREVIEWER = {Darryl McCullough},
}


@ARTICLE{DavisJan00,
   AUTHOR = {Davis, Michael W. and Januszkiewicz, Tadeusz},
    TITLE = {Right-angled {A}rtin groups are commensurable with right-angled {C}oxeter groups},
  JOURNAL = {J. Pure Appl. Algebra},
   VOLUME = {153},
     YEAR = {2000},
   NUMBER = {3},
    PAGES = {229--235},
}


@article{HaglundWiseCoxeter,
    AUTHOR = {Haglund, Fr{\'e}d{\'e}ric and Wise, Daniel T.},
     TITLE = {Coxeter groups are virtually special},
   JOURNAL = {Adv. Math.},
  FJOURNAL = {Advances in Mathematics},
    VOLUME = {224},
      YEAR = {2010},
    NUMBER = {5},
     PAGES = {1890--1903},
      ISSN = {0001-8708},
     CODEN = {ADMTA4},
   MRCLASS = {20Fxx},
  MRNUMBER = {2646113},
       DOI = {10.1016/j.aim.2010.01.011},
       URL = {http://dx.doi.org/10.1016/j.aim.2010.01.011},
}


@unpublished{HaglundWiseSimple,
   author = {Fr\'ed\'eric Haglund and Daniel T. Wise},
   title = {Arithmetic Hyperbolic lattices of simple type
   are Virtually Special},
   note = {2006}
}

@article{BergeronHaglundWiseSimple,
    AUTHOR = {Bergeron, Nicolas and Haglund, Fr{\'e}d{\'e}ric and Wise,
              Daniel T.},
     TITLE = {Hyperplane sections in arithmetic hyperbolic manifolds},
   JOURNAL = {J. Lond. Math. Soc. (2)},
  FJOURNAL = {Journal of the London Mathematical Society. Second Series},
    VOLUME = {83},
      YEAR = {2011},
    NUMBER = {2},
     PAGES = {431--448},
      ISSN = {0024-6107},
   MRCLASS = {57M50 (11F75 20Fxx 53Cxx)},
  MRNUMBER = {2776645},
       DOI = {10.1112/jlms/jdq082},
       URL = {http://dx.doi.org/10.1112/jlms/jdq082},
}



@article {Mozes95,
    AUTHOR = {Mozes, Shahar},
     TITLE = {Actions of {C}artan subgroups},
   JOURNAL = {Israel J. Math.},
  FJOURNAL = {Israel Journal of Mathematics},
    VOLUME = {90},
      YEAR = {1995},
    NUMBER = {1-3},
     PAGES = {253--294},
      ISSN = {0021-2172},
     CODEN = {ISJMAP},
   MRCLASS = {22E50 (20E42 54H20)},
  MRNUMBER = {MR1336326 (97b:22022)},
}

@PhDThesis{RattagiThesis04,
Author = { Diego Rattaggi},
Title = {Computations on groups acting on a
product of trees: normal subgroup structures and quaternion
lattices},
school={ETH Zurich},
year ={2004},
}

@article {MosherSageevWhyte2003,
    AUTHOR = {Mosher, Lee and Sageev, Michah and Whyte, Kevin},
     TITLE = {Quasi-actions on trees. {I}. {B}ounded valence},
   JOURNAL = {Ann. of Math. (2)},
  FJOURNAL = {Annals of Mathematics. Second Series},
    VOLUME = {158},
      YEAR = {2003},
    NUMBER = {1},
     PAGES = {115--164},
      ISSN = {0003-486X},
     CODEN = {ANMAAH},
   MRCLASS = {20F65 (20E08 57M07)},
  MRNUMBER = {MR1998479 (2004h:20055)},
MRREVIEWER = {Gilbert Levitt},
}


@article {KleinerLeeb97,
    AUTHOR = {Kleiner, Bruce and Leeb, Bernhard},
     TITLE = {Rigidity of quasi-isometries for symmetric spaces and
              {E}uclidean buildings},
   JOURNAL = {Inst. Hautes \'Etudes Sci. Publ. Math.},
  FJOURNAL = {Institut des Hautes \'Etudes Scientifiques. Publications
              Math\'ematiques},
    NUMBER = {86},
      YEAR = {1997},
     PAGES = {115--197 (1998)},
      ISSN = {0073-8301},
     CODEN = {PMIHA6},
   MRCLASS = {53C35 (20E42 20F32 53C23 57M07)},
  MRNUMBER = {MR1608566 (98m:53068)},
MRREVIEWER = {Lee Mosher},
}


@article{Ahlin2002,
    AUTHOR = {Ahlin, A. Reiter},
     TITLE = {The large scale geometry of products of trees},
      NOTE = {Dedicated to John Stallings on the occasion of his 65th
              birthday},
   JOURNAL = {Geom. Dedicata},
  FJOURNAL = {Geometriae Dedicata},
    VOLUME = {92},
      YEAR = {2002},
     PAGES = {179--184},
      ISSN = {0046-5755},
     CODEN = {GEMDAT},
   MRCLASS = {20E08 (20F65)},
  MRNUMBER = {MR1934017 (2003j:20041)},
}

@article {KapovichKleinerLeeb98,
    AUTHOR = {Kapovich, Michael and Kleiner, Bruce and Leeb, Bernhard},
     TITLE = {Quasi-isometries and the de {R}ham decomposition},
   JOURNAL = {Topology},
  FJOURNAL = {Topology. An International Journal of Mathematics},
    VOLUME = {37},
      YEAR = {1998},
    NUMBER = {6},
     PAGES = {1193--1211},
      ISSN = {0040-9383},
     CODEN = {TPLGAF},
   MRCLASS = {53C23 (53C21 53C22)},
  MRNUMBER = {MR1632904 (99g:53048)},
MRREVIEWER = {Raul Quiroga},
}


@article {Rattaggi05,
    AUTHOR = {Rattaggi, Diego},
     TITLE = {Anti-tori in square complex groups},
   JOURNAL = {Geom. Dedicata},
  FJOURNAL = {Geometriae Dedicata},
    VOLUME = {114},
      YEAR = {2005},
     PAGES = {189--207},
      ISSN = {0046-5755},
     CODEN = {GEMDAT},
   MRCLASS = {20E05 (11R52 20F67)},
  MRNUMBER = {MR2174099 (2006h:20030)},
MRREVIEWER = {Olivier Guichard},
}

@article {RattaggiRobertson05,
    AUTHOR = {Rattaggi, Diego and Robertson, Guyan},
     TITLE = {Abelian subgroup structure of square complex groups and
              arithmetic of quaternions},
   JOURNAL = {J. Algebra},
  FJOURNAL = {Journal of Algebra},
    VOLUME = {286},
      YEAR = {2005},
    NUMBER = {1},
     PAGES = {57--68},
      ISSN = {0021-8693},
     CODEN = {JALGA4},
   MRCLASS = {22E40 (20E42)},
  MRNUMBER = {MR2124808 (2005i:22010)},
MRREVIEWER = {Lucy Lifschitz},
}

@article{CherixMartinValette04,
    AUTHOR = {Cherix, Pierre-Alain and Martin, Florian and Valette, Alain},
     TITLE = {Spaces with measured walls, the {H}aagerup property and
              property ({T})},
   JOURNAL = {Ergodic Theory Dynam. Systems},
  FJOURNAL = {Ergodic Theory and Dynamical Systems},
    VOLUME = {24},
      YEAR = {2004},
    NUMBER = {6},
     PAGES = {1895--1908},
      ISSN = {0143-3857},
}

@article{Ghys03,
    AUTHOR = {Ghys, {\'E}tienne},
     TITLE = {Groupes al\'eatoires (d'apr\`es {M}isha {G}romov,{$\dots$})},
   JOURNAL = {Ast\'erisque},
  FJOURNAL = {Ast\'erisque},
    NUMBER = {294},
      YEAR = {2004},
     PAGES = {173--204},
      ISSN = {0303-1179},
      NOTE = {S\'eminaire Bourbaki, Vol. 2003/2004, Exp.~916},
}

@book{Ollivier05invitation,
    AUTHOR = {Ollivier, Yann},
     TITLE = {A {J}anuary 2005 invitation to random groups},
    SERIES = {Ensaios Matem\'aticos [Mathematical Surveys]},
    VOLUME = {10},
 PUBLISHER = {Sociedade Brasileira de Matem\'atica},
   ADDRESS = {Rio de Janeiro},
      YEAR = {2005},
     PAGES = {ii+100},
      ISBN = {85-85818-30-1},
}

@UNPUBLISHED{Ollivierglobalisoperimetry,
    author={Y. Ollivier},
    title={Some small cancellation properties of random groups},
    note={To appear in Internat. J. Algebra Comput., ArXiv {\tt math.GR/0409226}},
}

@article{Olliviercogrowth05,
    AUTHOR = {Ollivier, Yann},
     TITLE = {Cogrowth and spectral gap of generic groups},
   JOURNAL = {Ann. Inst. Fourier (Grenoble)},
  FJOURNAL = {Universit\'e de Grenoble. Annales de l'Institut Fourier},
    VOLUME = {55},
      YEAR = {2005},
    NUMBER = {1},
     PAGES = {289--317},
      ISSN = {0373-0956},
     CODEN = {AIFUA7},
}

@book {BekkaHarpeValette,
    AUTHOR = {Bekka, Bachir and de la Harpe, Pierre and Valette, Alain},
     TITLE = {Kazhdan's property ({T})},
    SERIES = {New Mathematical Monographs},
    VOLUME = {11},
 PUBLISHER = {Cambridge University Press, Cambridge},
      YEAR = {2008},
     PAGES = {xiv+472},
      ISBN = {978-0-521-88720-5},
   MRCLASS = {22-02 (22E40 28D15 37A15 43A07 43A35)},
  MRNUMBER = {2415834 (2009i:22001)},
MRREVIEWER = {Markus Neuhauser},
       DOI = {10.1017/CBO9780511542749},
       URL = {http://dx.doi.org/10.1017/CBO9780511542749},
}

--------------------------------------------------------------------------------
@book{MorrisWitteBook,
title ={Introduction to Arithmetic Groups},
author = {Dave Morris Witte},
year={2008},
note={arXiv:math/0106063v3},
}

@article{HruskaWisePacking,
    AUTHOR = {Hruska, G. Christopher and Wise, Daniel T.},
     TITLE = {Packing subgroups in relatively hyperbolic groups},
   JOURNAL = {Geom. Topol.},
  FJOURNAL = {Geometry \& Topology},
    VOLUME = {13},
      YEAR = {2009},
    NUMBER = {4},
     PAGES = {1945--1988},
      ISSN = {1465-3060},
   MRCLASS = {20F67 (20F65 20F69)},
  MRNUMBER = {MR2497315 (2010c:20053)},
MRREVIEWER = {Fran{\c{c}}ois Dahmani},
       DOI = {10.2140/gt.2009.13.1945},
       URL = {http://dx.doi.org/10.2140/gt.2009.13.1945},
}

@article{HruskaWise09,
    AUTHOR = {Hruska, G. Christopher and Wise, Daniel T.},
     TITLE = {Packing subgroups in relatively hyperbolic groups},
   JOURNAL = {Geom. Topol.},
  FJOURNAL = {Geometry \& Topology},
    VOLUME = {13},
      YEAR = {2009},
    NUMBER = {4},
     PAGES = {1945--1988},
      ISSN = {1465-3060},
   MRCLASS = {20F67 (20F65 20F69)},
  MRNUMBER = {MR2497315 (2010c:20053)},
MRREVIEWER = {Fran{\c{c}}ois Dahmani},
       DOI = {10.2140/gt.2009.13.1945},
       URL = {http://dx.doi.org/10.2140/gt.2009.13.1945},
}


@article{Agol06,
    title = {{Untitled}},
    author = {Ian Agol},
    Year = {2006},
    Note = {in preparation},
}


@article {KariPapasoglu99,
    AUTHOR = {Kari, J. and Papasoglu, P.},
     TITLE = {Deterministic aperiodic tile sets},
   JOURNAL = {Geom. Funct. Anal.},
  FJOURNAL = {Geometric and Functional Analysis},
    VOLUME = {9},
      YEAR = {1999},
    NUMBER = {2},
     PAGES = {353--369},
      ISSN = {1016-443X},
     CODEN = {GFANFB},
   MRCLASS = {52C23 (05B40 20F67 57M50)},
  MRNUMBER = {MR1692474 (2001b:52037)},
MRREVIEWER = {Mihail N. Kolountzakis},
}




@book {KapovichMisha2001,
    AUTHOR = {Kapovich, Michael},
     TITLE = {Hyperbolic manifolds and discrete groups},
    SERIES = {Progress in Mathematics},
    VOLUME = {183},
 PUBLISHER = {Birkh\"auser Boston Inc.},
   ADDRESS = {Boston, MA},
      YEAR = {2001},
     PAGES = {xxvi+467},
      ISBN = {0-8176-3904-7},
   MRCLASS = {57M50 (20F65 20H10 30F40 30F60 32G15)},
  MRNUMBER = {MR1792613 (2002m:57018)},
MRREVIEWER = {Michel Coornaert},
}


@PhdThesis{HaglundThesis,
  author =   {Haglund, Fr{\'e}d{\'e}ric},
  title =    {Les Polyedres de Gromov},
  school =   {Universit{\'e} de Lyon 1},
  year =     1992
}



@MISC{BestvinaProblemList,
   author = {Mladen Bestvina},
   title = {Questions in Geometric Group Theory},
   howpublished = {http://www.math.utah.edu/~bestvina/eprints/questions-updated.pdf},
   key = {Bestvina},
}

@incollection {Atiyah76,
    AUTHOR = {Atiyah, M. F.},
     TITLE = {Elliptic operators, discrete groups and von {N}eumann
              algebras},
 BOOKTITLE = {Colloque ``Analyse et Topologie'' en l'Honneur de Henri Cartan
              (Orsay, 1974)},
     PAGES = {43--72. Ast\'erisque, No. 32-33},
 PUBLISHER = {Soc. Math. France},
   ADDRESS = {Paris},
      YEAR = {1976},
   MRCLASS = {58G10 (46L10 22E45)},
  MRNUMBER = {MR0420729 (54 \#8741)},
MRREVIEWER = {R. D. Moyer},
}


@article {Dodziuk77,
    AUTHOR = {Dodziuk, Jozef},
     TITLE = {de {R}ham-{H}odge theory for {$L\sp{2}$}-cohomology of
              infinite coverings},
   JOURNAL = {Topology},
  FJOURNAL = {Topology. An International Journal of Mathematics},
    VOLUME = {16},
      YEAR = {1977},
    NUMBER = {2},
     PAGES = {157--165},
      ISSN = {0040-9383},
   MRCLASS = {58G10},
  MRNUMBER = {MR0445560 (56 \#3898)},
MRREVIEWER = {M. F. Atiyah},
}


@preamble{
   "\def\cprime{$'$} "
}
@article {Kazhdan67,
    AUTHOR = {Ka{\v{z}}dan, D. A.},
     TITLE = {On the connection of the dual space of a group with the
              structure of its closed subgroups},
   JOURNAL = {Funkcional. Anal. i Prilo\v zen.},
  FJOURNAL = {Akademija Nauk SSSR. Funkcional\cprime nyi Analiz i ego
              Prilo\v zenija},
    VOLUME = {1},
      YEAR = {1967},
     PAGES = {71--74},
      ISSN = {0374-1990},
   MRCLASS = {22.20},
  MRNUMBER = {MR0209390 (35 \#288)},
MRREVIEWER = {K. Strambach},
}


@article {Gromov81,
    AUTHOR = {Gromov, Mikhael},
     TITLE = {Groups of polynomial growth and expanding maps},
   JOURNAL = {Inst. Hautes \'Etudes Sci. Publ. Math.},
  FJOURNAL = {Institut des Hautes \'Etudes Scientifiques. Publications
              Math\'ematiques},
    NUMBER = {53},
      YEAR = {1981},
     PAGES = {53--73},
      ISSN = {0073-8301},
     CODEN = {PMIHA6},
   MRCLASS = {53C20 (22E40 58F15)},
  MRNUMBER = {MR623534 (83b:53041)},
MRREVIEWER = {J. A. Wolf},
}


@inproceedings {Gromov84,
    AUTHOR = {Gromov, Mikhael},
     TITLE = {Infinite groups as geometric objects},
 BOOKTITLE = {Proceedings of the International Congress of Mathematicians,
              Vol.\ 1, 2 (Warsaw, 1983)},
     PAGES = {385--392},
 PUBLISHER = {PWN},
   ADDRESS = {Warsaw},
      YEAR = {1984},
   MRCLASS = {57S30 (20F32 53C99)},
  MRNUMBER = {MR804694 (87c:57033)},
MRREVIEWER = {J{\'o}zef Dodziuk},
}


@article {GromovCheeger86,
    AUTHOR = {Cheeger, Jeff and Gromov, Mikhael},
     TITLE = {{$L\sb 2$}-cohomology and group cohomology},
   JOURNAL = {Topology},
  FJOURNAL = {Topology. An International Journal of Mathematics},
    VOLUME = {25},
      YEAR = {1986},
    NUMBER = {2},
     PAGES = {189--215},
      ISSN = {0040-9383},
     CODEN = {TPLGAF},
   MRCLASS = {58G12 (20J05 22E41 53C20 58A14)},
  MRNUMBER = {MR837621 (87i:58161)},
MRREVIEWER = {Avner Ash},
}



@incollection {Davis02,
    AUTHOR = {Davis, Michael W.},
     TITLE = {Nonpositive curvature and reflection groups},
 BOOKTITLE = {Handbook of geometric topology},
     PAGES = {373--422},
 PUBLISHER = {North-Holland},
   ADDRESS = {Amsterdam},
      YEAR = {2002},
   MRCLASS = {53C23 (20F36 20F55 20F65 57M60)},
  MRNUMBER = {MR1886674 (2002m:53061)},
MRREVIEWER = {Athanase Papadopoulos},
}



@incollection {KharlampovichMyasnikov99,
    AUTHOR = {Kharlampovich, O. and Myasnikov, A.},
     TITLE = {Description of fully residually free groups and irreducible
              affine varieties over a free group},
 BOOKTITLE = {Summer School in Group Theory in Banff, 1996},
    SERIES = {CRM Proc. Lecture Notes},
    VOLUME = {17},
     PAGES = {71--80},
 PUBLISHER = {Amer. Math. Soc.},
   ADDRESS = {Providence, RI},
      YEAR = {1999},
   MRCLASS = {20E05 (20E26 20F10)},
  MRNUMBER = {MR1653685 (99j:20032)},
MRREVIEWER = {Dennis Spellman},
}


@article {Sela01,
    AUTHOR = {Sela, Zlil},
     TITLE = {Diophantine geometry over groups. {I}. {M}akanin-{R}azborov
              diagrams},
   JOURNAL = {Publ. Math. Inst. Hautes \'Etudes Sci.},
  FJOURNAL = {Publications Math\'ematiques. Institut de Hautes \'Etudes
              Scientifiques},
    NUMBER = {93},
      YEAR = {2001},
     PAGES = {31--105},
      ISSN = {0073-8301},
   MRCLASS = {20F65 (20E05 20E18 20E26)},
  MRNUMBER = {MR1863735 (2002h:20061)},
MRREVIEWER = {Jos{\'e} Burillo},
}



@article {Szczepanski98,
    AUTHOR = {Szczepa{\'n}ski, Andrzej},
     TITLE = {Relatively hyperbolic groups},
   JOURNAL = {Michigan Math. J.},
  FJOURNAL = {The Michigan Mathematical Journal},
    VOLUME = {45},
      YEAR = {1998},
    NUMBER = {3},
     PAGES = {611--618},
      ISSN = {0026-2285},
   MRCLASS = {20F32 (57M07)},
  MRNUMBER = {MR1653287 (99i:20051)},
MRREVIEWER = {Athanase Papadopoulos},
}



@article {Farb98,
    AUTHOR = {Farb, B.},
     TITLE = {Relatively hyperbolic groups},
   JOURNAL = {Geom. Funct. Anal.},
  FJOURNAL = {Geometric and Functional Analysis},
    VOLUME = {8},
      YEAR = {1998},
    NUMBER = {5},
     PAGES = {810--840},
      ISSN = {1016-443X},
     CODEN = {GFANFB},
   MRCLASS = {20F32 (20F10 57M07)},
  MRNUMBER = {MR1650094 (99j:20043)},
MRREVIEWER = {Michel Coornaert},
}



@MastersThesis{Richer05,
  author =   {Emily Richer},
  title =    {Relative Hyperbolicity of Graphs of Free Groups with
Cyclic Edge Groups},
  school =   {McGill University},
  year =     2005},
  }

@article {Dahmani03,
    AUTHOR = {Dahmani, Fran{\c{c}}ois},
     TITLE = {Combination of convergence groups},
   JOURNAL = {Geom. Topol.},
  FJOURNAL = {Geometry and Topology},
    VOLUME = {7},
      YEAR = {2003},
     PAGES = {933--963 (electronic)},
      ISSN = {1465-3060},
   MRCLASS = {20F67 (20E06)},
  MRNUMBER = {MR2026551 (2005g:20063)},
}


@article {Alibegovic05,
    AUTHOR = {Alibegovi{\'c}, Emina},
     TITLE = {A combination theorem for relatively hyperbolic groups},
   JOURNAL = {Bull. London Math. Soc.},
  FJOURNAL = {The Bulletin of the London Mathematical Society},
    VOLUME = {37},
      YEAR = {2005},
    NUMBER = {3},
     PAGES = {459--466},
      ISSN = {0024-6093},
     CODEN = {LMSBBT},
   MRCLASS = {20F65 (57M07)},
  MRNUMBER = {MR2131400},
MRREVIEWER = {Ilya Kapovich},
}


@unpublished {KapovichExample94,
    AUTHOR = {Kapovich, Michael},
     TITLE = {An example of 2-dimensional hyperbolic group which {canít} act
on 2-dimensional negatively curved complexes},
      NOTE={Preprint, Utah},
      YEAR = {1994}
}


@article {BallmannBrin94,
    AUTHOR = {Ballmann, W. and Brin, M.},
     TITLE = {Polygonal complexes and combinatorial group theory},
   JOURNAL = {Geom. Dedicata},
  FJOURNAL = {Geometriae Dedicata},
    VOLUME = {50},
      YEAR = {1994},
    NUMBER = {2},
     PAGES = {165--191},
      ISSN = {0046-5755},
     CODEN = {GEMDAT},
   MRCLASS = {57M20 (20F05 20F10 57M07)},
  MRNUMBER = {MR1279883 (95e:57004)},
MRREVIEWER = {Michel Coornaert},
}



@unpublished{Minasyan04,
Author={Ashot Minasyan},
Title={Separable Subsets of GFERF Negatively Curved Groups},
Note={Preprint},
Year = {2004},
}

@unpublished {CalegariGabai04,
Author = {Danny Calegari and David Gabai},
Title={Shrinkwrapping and the taming of hyperbolic 3-manifolds},
Year={2004}
}

@article {BradyCrisp07,
    AUTHOR = {Brady, Noel and Crisp, John},
     TITLE = {{$\rm CAT(0)$} and {$\rm CAT(-1)$} dimensions of torsion free
              hyperbolic groups},
   JOURNAL = {Comment. Math. Helv.},
  FJOURNAL = {Commentarii Mathematici Helvetici. A Journal of the Swiss
              Mathematical Society},
    VOLUME = {82},
      YEAR = {2007},
    NUMBER = {1},
     PAGES = {61--85},
      ISSN = {0010-2571},
   MRCLASS = {20F65 (57M20)},
  MRNUMBER = {MR2296058 (2008k:20097)},
}
		

@unpublished {DromsMagnus,
   AUTHOR = {Droms, Carl},
     TITLE = {Residual Nilpotence of Graph Groups},
      NOTE = {Unpublished},
}


@article {DuchampThibon92,
    AUTHOR = {Duchamp, G{\'e}rard and Thibon, Jean-Yves},
     TITLE = {Simple orderings for free partially commutative groups},
   JOURNAL = {Internat. J. Algebra Comput.},
  FJOURNAL = {International Journal of Algebra and Computation},
    VOLUME = {2},
      YEAR = {1992},
    NUMBER = {3},
     PAGES = {351--355},
      ISSN = {0218-1967},
   MRCLASS = {06F15 (20F60)},
  MRNUMBER = {MR1189240 (93j:06017)},
MRREVIEWER = {N. Ya. Medvedev},
}


@article{GhristPeterson05,
    AUTHOR = {Ghrist, R. and Peterson, V.},
     TITLE = {The geometry and topology of reconfiguration},
   JOURNAL = {Adv. in Appl. Math.},
  FJOURNAL = {Advances in Applied Mathematics},
    VOLUME = {38},
      YEAR = {2007},
    NUMBER = {3},
     PAGES = {302--323},
      ISSN = {0196-8858},
   MRCLASS = {68Q85 (57Q05 68Q80)},
  MRNUMBER = {2301699 (2008f:68104)},
MRREVIEWER = {Nigel Martin},
       DOI = {10.1016/j.aam.2005.08.009},
       URL = {http://dx.doi.org/10.1016/j.aam.2005.08.009},
}


@misc{Agol04,
    title = {{Tameness of hyperbolic 3-manifolds}},
    AUTHOR = {Agol, Ian},
    Year = {2004},
    Note = {Preprint},
    eprint = {arXiv:math.GT/0405568}}


@article {Chepoi2000,
    AUTHOR = {Chepoi, Victor},
     TITLE = {Graphs of some {${\rm CAT}(0)$} complexes},
   JOURNAL = {Adv. in Appl. Math.},
  FJOURNAL = {Advances in Applied Mathematics},
    VOLUME = {24},
      YEAR = {2000},
    NUMBER = {2},
     PAGES = {125--179},
      ISSN = {0196-8858},
   MRCLASS = {57M07 (05C10 20F67)},
  MRNUMBER = {MR1748966 (2001a:57004)},
}


@article {Gitik99,
    AUTHOR = {Gitik, Rita},
     TITLE = {Ping-pong on negatively curved groups},
   JOURNAL = {J. Algebra},
  FJOURNAL = {Journal of Algebra},
    VOLUME = {217},
      YEAR = {1999},
    NUMBER = {1},
     PAGES = {65--72},
      ISSN = {0021-8693},
     CODEN = {JALGA4},
   MRCLASS = {20F65 (20E06 20E26 57M07)},
  MRNUMBER = {MR1700476 (2000e:20070)},
MRREVIEWER = {Michel Coornaert},
}


@article {Niblo92,
    AUTHOR = {Niblo, G. A.},
     TITLE = {Separability properties of free groups and surface groups},
   JOURNAL = {J. Pure Appl. Algebra},
  FJOURNAL = {Journal of Pure and Applied Algebra},
    VOLUME = {78},
      YEAR = {1992},
    NUMBER = {1},
     PAGES = {77--84},
      ISSN = {0022-4049},
     CODEN = {JPAAA2},
   MRCLASS = {20E05 (20F34 20H10 57M05)},
  MRNUMBER = {MR1154898 (92m:20019)},
}


@BOOK{Valette02BaumConnes,
    AUTHOR = {Valette, Alain},
     TITLE = {Introduction to the {B}aum-{C}onnes conjecture},
    SERIES = {Lectures in Mathematics ETH Z\"urich},
      NOTE = {From notes taken by Indira Chatterji,
              With an appendix by Guido Mislin},
 PUBLISHER = {Birkh\"auser Verlag},
   ADDRESS = {Basel},
      YEAR = {2002},
     PAGES = {x+104},
      ISBN = {3-7643-6706-7},
   MRCLASS = {58J22 (19K35 22D25 46L80 46L87)},
  MRNUMBER = {MR1907596 (2003f:58047)},
MRREVIEWER = {Paul D. Mitchener},
}

@book{Valette04T,
    AUTHOR = {Valette, Alain},
     TITLE = {Nouvelles approches de la propri\'et\'e {$(T)$} de {K}azhdan},
      NOTE = {S\'eminaire Bourbaki. Vol. 2003/2004},
   SERIES = {Ast\'erisque},
    NUMBER = {294},
      YEAR = {2004},
     PAGES = {Exp. No. 913, 97--124},
}

@article{HigsonLafforgueSkandalis02,
    AUTHOR = {Higson, N. and Lafforgue, V. and Skandalis, G.},
     TITLE = {Counterexamples to the {B}aum-{C}onnes conjecture},
   JOURNAL = {Geom. Funct. Anal.},
  FJOURNAL = {Geometric and Functional Analysis},
    VOLUME = {12},
      YEAR = {2002},
    NUMBER = {2},
     PAGES = {330--354},
      ISSN = {1016-443X},
     CODEN = {GFANFB},
   MRCLASS = {19K56 (22A22 46L80 46L85 58J22)},
  MRNUMBER = {MR1911663 (2003g:19007)},
MRREVIEWER = {Alain Valette},
}

@article{ArzhOls96,
    AUTHOR = {Arzhantseva, G. N. and Ol{'}shanski{\u\i}, A. Yu.},
     TITLE = {Generality of the class of groups in which subgroups with a
              lesser number of generators are free},
   JOURNAL = {Mat. Zametki},
  FJOURNAL = {Rossi\u\i skaya Akademiya Nauk. Matematicheskie Zametki},
    VOLUME = {59},
      YEAR = {1996},
    NUMBER = {4},
     PAGES = {489--496, 638},
      ISSN = {0025-567X},
   MRCLASS = {20F05 (05C25 20F06)},
  MRNUMBER = {MR1445193 (98k:20040)},
MRREVIEWER = {David I. Moldavanski{\u\i}},
}

@article{Ols93,
    AUTHOR = {Ol{'}shanski{\u\i}, A. Yu.},
     TITLE = {Almost every group is hyperbolic},
   JOURNAL = {Internat. J. Algebra Comput.},
  FJOURNAL = {International Journal of Algebra and Computation},
    VOLUME = {2},
      YEAR = {1992},
    NUMBER = {1},
     PAGES = {1--17},
      ISSN = {0218-1967},
   MRCLASS = {20F06 (20F32)},
  MRNUMBER = {MR1167524 (93j:20068)},
MRREVIEWER = {Christopher W. Stark},
}

@article{Arzh98,
    AUTHOR = {Arzhantseva, G. N.},
     TITLE = {Generic properties of finitely presented groups and {H}owson's
              theorem},
   JOURNAL = {Comm. Algebra},
  FJOURNAL = {Communications in Algebra},
    VOLUME = {26},
      YEAR = {1998},
    NUMBER = {11},
     PAGES = {3783--3792},
      ISSN = {0092-7872},
     CODEN = {COALDM},
   MRCLASS = {20F05 (05C25 20F06 20F32)},
  MRNUMBER = {MR1647075 (99j:20036)},
MRREVIEWER = {Richard M. Thomas},
}

@article{Champetier00,
    AUTHOR = {Champetier, Christophe},
     TITLE = {L'espace des groupes de type fini},
   JOURNAL = {Topology},
  FJOURNAL = {Topology. An International Journal of Mathematics},
    VOLUME = {39},
      YEAR = {2000},
    NUMBER = {4},
     PAGES = {657--680},
      ISSN = {0040-9383},
     CODEN = {TPLGAF},
   MRCLASS = {20F67 (20F05 20F06 20F65 57M07)},
  MRNUMBER = {MR1760424 (2001i:20084)},
MRREVIEWER = {Michel Coornaert},
}

@article{Champetier95,
    AUTHOR = {Champetier, Christophe},
     TITLE = {Propri\'et\'es statistiques des groupes de pr\'esentation
              finie},
   JOURNAL = {Adv. Math.},
  FJOURNAL = {Advances in Mathematics},
    VOLUME = {116},
      YEAR = {1995},
    NUMBER = {2},
     PAGES = {197--262},
      ISSN = {0001-8708},
     CODEN = {ADMTA4},
   MRCLASS = {20F32 (20F05 20F06 57M07)},
  MRNUMBER = {MR1363765 (96m:20056)},
MRREVIEWER = {Michel Coornaert},
}

@article{ArzhCherix04,
    AUTHOR={Arzhantseva, G. N. and Cherix, P.-A.},
    TITLE={On the Cayley graph of a generic finitely presented group},
    journal={Bull. Soc. Math. Belg.},
    volume={11},
    number={4},
    pages={589--601},
    year={2004}
}

@article{KapovichSchuppShpilrain,
    author={Kapovich, I. and Schupp, P. and Shpilrain, V.},
    title={Generic properties of {W}hitehead's Algorithm and
    isomorphism rigidity of random one-relator groups},
    journal={Pacific J. Math.},
    note={to appear}
}

@article{KapovichSchupp05,
    author={Kapovich, I. and Schupp, P.},
    title={Genericity, the {A}rzhantseva-{O}l{'}shanski{\u\i} method and the
    isomorphism problem for one-relator groups},
    journal={Mathematische Annalen},
    volume={331},
    number={1},
    pages={1--19},
    year={2005}
}




@UNPUBLISHED{Olliviergrowth04,
    AUTHOR={Y. Ollivier},
    TITLE={Growth exponent of generic groups},
    note={Preprint, submitted, ArXiV:math.GR/0401050},
    year={2004},
    }

@incollection {Tits69,
    AUTHOR = {Tits, Jacques},
     TITLE = {Le probl\`eme des mots dans les groupes de {C}oxeter},
 BOOKTITLE = {Symposia Mathematica (INDAM, Rome, 1967/68), Vol. 1},
     PAGES = {175--185},
 PUBLISHER = {Academic Press},
   ADDRESS = {London},
      YEAR = {1969},
   MRCLASS = {20.10},
  MRNUMBER = {MR0254129 (40 \#7339)},
MRREVIEWER = {J. E. Humphreys},
}


@book {Bourbaki68,
    AUTHOR = {Bourbaki, N.},
     TITLE = {\'{E}l\'ements de math\'ematique. {F}asc. {XXXIV}. {G}roupes
              et alg\`ebres de {L}ie. {C}hapitre {IV}: {G}roupes de
              {C}oxeter et syst\`emes de {T}its. {C}hapitre {V}: {G}roupes
              engendr\'es par des r\'eflexions. {C}hapitre {VI}: syst\`emes
              de racines},
    SERIES = {Actualit\'es Scientifiques et Industrielles, No. 1337},
 PUBLISHER = {Hermann},
   ADDRESS = {Paris},
      YEAR = {1968},
     PAGES = {288 pp. (loose errata)},
   MRCLASS = {22.50 (17.00)},
  MRNUMBER = {MR0240238 (39 \#1590)},
MRREVIEWER = {G. B. Seligman},
}


@article{SageevWiseTits,
    AUTHOR = {Sageev, Michah and Wise, Daniel T.},
     TITLE = {The {T}its alternative for {${\rm CAT}(0)$} cubical complexes},
   JOURNAL = {Bull. London Math. Soc.},
  FJOURNAL = {The Bulletin of the London Mathematical Society},
    VOLUME = {37},
      YEAR = {2005},
    NUMBER = {5},
     PAGES = {706--710},
      ISSN = {0024-6093},
     CODEN = {LMSBBT},
   MRCLASS = {20F67 (20E08)},
  MRNUMBER = {MR2164832 (2006f:20052)},
MRREVIEWER = {Hanspeter Fischer},
       DOI = {10.1112/S002460930500456X},
       URL = {http://dx.doi.org/10.1112/S002460930500456X},
}


@unpublished {HaglundSimplicialComplex03,
    AUTHOR = {Haglund, Fr\'{e}d\'{e}ric},
     TITLE = {Complexes simpliciaux hyperboliques de grande dimension},
      NOTE = {Preprint},
      YEAR = {2003}
}

@unpublished {HaglundHighDimHyper04,
    AUTHOR = {Haglund, Fr\'{e}d\'{e}ric},
     TITLE = {Groupes hyperboliques de grande dimension},
      NOTE = {in preparation},
      YEAR = {2004}
}


@article {HaglundGraphProduct,
    AUTHOR = {Haglund, Fr{\'e}d{\'e}ric},
     TITLE = {Finite index subgroups of graph products},
   JOURNAL = {Geom. Dedicata},
  FJOURNAL = {Geometriae Dedicata},
    VOLUME = {135},
      YEAR = {2008},
     PAGES = {167--209},
      ISSN = {0046-5755},
     CODEN = {GEMDAT},
   MRCLASS = {20F65 (20E26 20F36 20F55 20F67 51E24)},
  MRNUMBER = {MR2413337},
MRREVIEWER = {Henry Wilton},
}
		
@PHDTHESIS{AlJanabiThesis77,
 author = {Al-Janabi, Mohammed Abdul-Razzak. },
 title = {The SQ-universailty of some small cancellation groups},
 school = {Queen Mary College},
 year = {1977},
}


@article{ChatterjiNiblo04,
    AUTHOR = {Chatterji, Indira and Niblo, Graham},
     TITLE = {From wall spaces to {$\rm CAT(0)$} cube complexes},
   JOURNAL = {Internat. J. Algebra Comput.},
  FJOURNAL = {International Journal of Algebra and Computation},
    VOLUME = {15},
      YEAR = {2005},
    NUMBER = {5-6},
     PAGES = {875--885},
      ISSN = {0218-1967},
   MRCLASS = {20F65 (20F38 20F69)},
  MRNUMBER = {MR2197811 (2006m:20064)},
MRREVIEWER = {Robert W. Bell},
}
	

@article {JanuszkiewiczSwiatkowskiCoxeter03,
    AUTHOR = {Januszkiewicz, Tadeusz and {\'S}wi{\c{a}}tkowski, Jacek},
     TITLE = {Hyperbolic {C}oxeter groups of large dimension},
   JOURNAL = {Comment. Math. Helv.},
  FJOURNAL = {Commentarii Mathematici Helvetici},
    VOLUME = {78},
      YEAR = {2003},
    NUMBER = {3},
     PAGES = {555--583},
      ISSN = {0010-2571},
     CODEN = {COMHAX},
   MRCLASS = {20F67 (20F55 20F65 51F15 57M07 57P10)},
  MRNUMBER = {2004h:20058},
MRREVIEWER = {Jonathan P. McCammond},
}

@unpublished {HaglundCoxeter,
    AUTHOR = {Frederic Haglund},
     TITLE = {},
            YEAR = {2004}
}


@article{KapovichMishaPolgons03,
    AUTHOR = {Kapovich, Michael},
     TITLE = {Representations of polygons of finite groups},
   JOURNAL = {Geom. Topol.},
  FJOURNAL = {Geometry and Topology},
    VOLUME = {9},
      YEAR = {2005},
     PAGES = {1915--1951 (electronic)},
      ISSN = {1465-3060},
   MRCLASS = {20F69 (20G05)},
  MRNUMBER = {MR2175160 (2006g:20069)},
MRREVIEWER = {Stephen G. Brick},
}




@UNPUBLISHED{WiseCoherenceSurvey,
   author = {Wise, Daniel T.},
   title = {A Survey on Coherent Groups},
   note = {Preprint},
   year = {2004},
}


@article{OllivierWiseDensity,
    AUTHOR = {Ollivier, Yann and Wise, Daniel T.},
     TITLE = {Cubulating random groups at density less than {$1/6$}},
   JOURNAL = {Trans. Amer. Math. Soc.},
  FJOURNAL = {Transactions of the American Mathematical Society},
    VOLUME = {363},
      YEAR = {2011},
    NUMBER = {9},
     PAGES = {4701--4733},
      ISSN = {0002-9947},
     CODEN = {TAMTAM},
   MRCLASS = {20Fxx (20P05)},
  MRNUMBER = {2806688},
       DOI = {10.1090/S0002-9947-2011-05197-4},
       URL = {http://dx.doi.org/10.1090/S0002-9947-2011-05197-4},
}


@book {HarpeValette89,
    AUTHOR = {de la Harpe, Pierre and Valette, Alain},
     TITLE = {La propri\'et\'e {$(T)$} de {K}azhdan pour les groupes
              localement compacts},
      NOTE = {With an appendix by M. Burger},
   SERIES = {Ast\'erisque},
    NUMBER = {175},
      YEAR = {1989},
     PAGES = {158},
      ISSN = {0303-1179},
   MRCLASS = {22-02 (05C99 22D10 22E99 28C10)},
  MRNUMBER = {90m:22001},
MRREVIEWER = {Michael Cowling},
}

@book {Munkres75,
    AUTHOR = {Munkres, James R.},
     TITLE = {Topology: a first course},
 PUBLISHER = {Prentice-Hall Inc.},
   ADDRESS = {Englewood Cliffs, N.J.},
      YEAR = {1975},
     PAGES = {xvi+413},
   MRCLASS = {54-01},
  MRNUMBER = {57 \#4063},
}


@book {Hatcher2002,
    AUTHOR = {Hatcher, Allen},
     TITLE = {Algebraic topology},
 PUBLISHER = {Cambridge University Press},
   ADDRESS = {Cambridge},
      YEAR = {2002},
     PAGES = {xii+544},
      ISBN = {0-521-79160-X; 0-521-79540-0},
   MRCLASS = {55-01 (55-00)},
  MRNUMBER = {2002k:55001},
MRREVIEWER = {Donald W. Kahn},
}



@article{Ollivier04,
    AUTHOR={Y. Ollivier},
    TITLE={Sharp phase transition theorems for hyperbolicity of
    random groups},
    JOURNAL={GAFA, Geom. Funct. Anal.},
    VOLUME={14},
    YEAR={2004},
    NUMBER={3},
    PAGES={595--679},
    }

@article{Silberman03,
    AUTHOR={L. Silberman},
    TITLE={Addendum to ``{R}andom walk in random groups'' by {M}.~{G}romov},
    JOURNAL={GAFA, Geom. Funct. Anal.},
    VOLUME={13},
    YEAR={2003},
    NUMBER={1},
    PAGES={147--177},
    }


@unpublished{Ollivier03expanders,
    AUTHOR={Y. Ollivier},
    TITLE={Cayley graphs containing expanders, after {G}romov},
    NOTE={Expository manuscript},
    YEAR={2003},
    }

@article {Kesten59,
    AUTHOR = {Kesten, Harry},
     TITLE = {Symmetric random walks on groups},
   JOURNAL = {Trans. Amer. Math. Soc.},
    VOLUME = {92},
      YEAR = {1959},
     PAGES = {336--354},
   MRCLASS = {60.00 (20.00)},
  MRNUMBER = {22 \#253},
MRREVIEWER = {H. Bergstr{\"o}m},
}

@book {DavidoffSarnackValette03,
    AUTHOR = {Davidoff, Giuliana and Sarnak, Peter and Valette, Alain},
    TITLE = {Elementary number theory, group theory, and {R}amanujan
        graphs},
    SERIES = {London Mathematical Society Student
        Texts},
    VOLUME = {55},
    PUBLISHER = {Cambridge University Press},
    ADDRESS = {Cambridge},
    YEAR = {2003},
    PAGES = {x+144},
    ISBN = {0-521-82426-5; 0-521-53143-8},
    MRCLASS = {11-01 (05C75 11E25 20G05 20G40)},
    MRNUMBER = {2004f:11001},
    MRREVIEWER = {Thomas R.  Shemanske},
}


@article {Guba93,
    AUTHOR = {Guba, V. S.},
     TITLE = {The word problem for the relatively free semigroup satisfying
              {$T\sp m=T\sp {m+n}$} with {$m\geq 3$}},
   JOURNAL = {Internat. J. Algebra Comput.},
  FJOURNAL = {International Journal of Algebra and Computation},
    VOLUME = {3},
      YEAR = {1993},
    NUMBER = {3},
     PAGES = {335--347},
      ISSN = {0218-1967},
   MRCLASS = {20M05 (03D40 68Q45)},
  MRNUMBER = {94m:20116},
MRREVIEWER = {Yuji Kobayashi},
}



@article {IKapovich97,
    AUTHOR = {Kapovich, Ilya},
     TITLE = {Quasiconvexity and amalgams},
   JOURNAL = {Internat. J. Algebra Comput.},
  FJOURNAL = {International Journal of Algebra and Computation},
    VOLUME = {7},
      YEAR = {1997},
    NUMBER = {6},
     PAGES = {771--811},
      ISSN = {0218-1967},
   MRCLASS = {20F32 (20E06 57M07)},
  MRNUMBER = {98k:20057},
MRREVIEWER = {Athanase Papadopoulos},
}


@article {GitikDoubleHyperbolicLERF,
    AUTHOR = {Gitik, Rita},
     TITLE = {Doubles of groups and hyperbolic {LERF} 3-manifolds},
   JOURNAL = {Ann. of Math. (2)},
  FJOURNAL = {Annals of Mathematics. Second Series},
    VOLUME = {150},
      YEAR = {1999},
    NUMBER = {3},
     PAGES = {775--806},
      ISSN = {0003-486X},
     CODEN = {ANMAAH},
   MRCLASS = {20E26 (20F67 57M07)},
  MRNUMBER = {2001a:20044},
MRREVIEWER = {Lee Mosher},
}


@article {Zuk03,
    AUTHOR = {{\.Z}uk, A.},
     TITLE = {Property ({T}) and {K}azhdan constants for discrete groups},
   JOURNAL = {Geom. Funct. Anal.},
  FJOURNAL = {Geometric and Functional Analysis},
    VOLUME = {13},
      YEAR = {2003},
    NUMBER = {3},
     PAGES = {643--670},
      ISSN = {1016-443X},
     CODEN = {GFANFB},
   MRCLASS = {20F65},
  MRNUMBER = {1 995 802},
}


@article {BJS88,
    AUTHOR = {Bo{\.z}ejko, M. and Januszkiewicz, T. and Spatzier, R. J.},
     TITLE = {Infinite {C}oxeter groups do not have {K}azhdan's property},
   JOURNAL = {J. Operator Theory},
  FJOURNAL = {Journal of Operator Theory},
    VOLUME = {19},
      YEAR = {1988},
    NUMBER = {1},
     PAGES = {63--67},
      ISSN = {0379-4024},
   MRCLASS = {22E46 (20G15 22E30 51F15)},
  MRNUMBER = {89i:22025},
MRREVIEWER = {K. A. Ross},
}


@incollection {Paulin91b,
    AUTHOR = {Paulin, Fr{\'e}d{\'e}ric},
     TITLE = {Outer automorphisms of hyperbolic groups and small actions on
              {${\bf R}$}-trees},
 BOOKTITLE = {Arboreal group theory (Berkeley, CA, 1988)},
    SERIES = {Math. Sci. Res. Inst. Publ.},
    VOLUME = {19},
     PAGES = {331--343},
 PUBLISHER = {Springer},
   ADDRESS = {New York},
      YEAR = {1991},
   MRCLASS = {57M07 (20E08 20F28)},
  MRNUMBER = {92g:57003},
MRREVIEWER = {Alain Valette},
}



@book {Lubotzky94,
    AUTHOR = {Lubotzky, Alexander},
     TITLE = {Discrete groups, expanding graphs and invariant measures},
    SERIES = {Progress in Mathematics},
    VOLUME = {125},
      NOTE = {With an appendix by Jonathan D. Rogawski},
 PUBLISHER = {Birkh\"auser Verlag},
   ADDRESS = {Basel},
      YEAR = {1994},
     PAGES = {xii+195},
      ISBN = {3-7643-5075-X},
   MRCLASS = {22E40 (05C25 11F70 28C10 43A07)},
  MRNUMBER = {96g:22018},
MRREVIEWER = {Wolfgang Woess},
}





@article {NibloReeves03,
    AUTHOR = {Niblo, G. A. and Reeves, L. D.},
     TITLE = {Coxeter groups act on {${\rm CAT}(0)$} cube complexes},
   JOURNAL = {J. Group Theory},
  FJOURNAL = {Journal of Group Theory},
    VOLUME = {6},
      YEAR = {2003},
    NUMBER = {3},
     PAGES = {399--413},
      ISSN = {1433-5883},
     CODEN = {JGTHFQ},
   MRCLASS = {20F65 (20F55 20F67)},
  MRNUMBER = {2004e:20072},
MRREVIEWER = {Nadia Benakli},
}



@article {Hruska2004,
    AUTHOR = {Hruska, G. Christopher},
     TITLE = {Nonpositively curved 2-complexes with isolated flats},
   JOURNAL = {Geom. Topol.},
  FJOURNAL = {Geometry and Topology},
    VOLUME = {8},
      YEAR = {2004},
     PAGES = {205--275 (electronic)},
      ISSN = {1465-3060},
   MRCLASS = {20F67 (20F06 57M20)},
  MRNUMBER = {2 033 482},
}



@article {AgolLongReid2001,
    AUTHOR = {Agol, I. and Long, D. D. and Reid, A. W.},
     TITLE = {The {B}ianchi groups are separable on geometrically finite
              subgroups},
   JOURNAL = {Ann. of Math. (2)},
  FJOURNAL = {Annals of Mathematics. Second Series},
    VOLUME = {153},
      YEAR = {2001},
    NUMBER = {3},
     PAGES = {599--621},
      ISSN = {0003-486X},
     CODEN = {ANMAAH},
   MRCLASS = {20H10 (11F06)},
  MRNUMBER = {2002e:20099},
MRREVIEWER = {Leonid Vulakh},
}



@article {LongReid2001b,
    AUTHOR = {Long, D. D. and Reid, A. W.},
     TITLE = {The fundamental group of the double of the figure-eight knot
              exterior is {GFERF}},
   JOURNAL = {Bull. London Math. Soc.},
  FJOURNAL = {The Bulletin of the London Mathematical Society},
    VOLUME = {33},
      YEAR = {2001},
    NUMBER = {4},
     PAGES = {391--396},
      ISSN = {0024-6093},
     CODEN = {LMSBBT},
   MRCLASS = {57M50 (20F65 20H10)},
  MRNUMBER = {2002c:57029},
MRREVIEWER = {Bruno Zimmermann},
}



@article {LongReid2001,
    AUTHOR = {Long, D. D. and Reid, A. W.},
     TITLE = {On subgroup separability in hyperbolic {C}oxeter groups},
   JOURNAL = {Geom. Dedicata},
  FJOURNAL = {Geometriae Dedicata},
    VOLUME = {87},
      YEAR = {2001},
    NUMBER = {1-3},
     PAGES = {245--260},
      ISSN = {0046-5755},
     CODEN = {GEMDAT},
   MRCLASS = {20F65 (20H10)},
  MRNUMBER = {2002j:20073},
MRREVIEWER = {Andrei Yu. Vesnin},
}



@preamble{
   "\def\polhk#1{\setbox0=\hbox{#1}{\ooalign{\hidewidth
    \lower1.5ex\hbox{`}\hidewidth\crcr\unhbox0}}} "
}
@article {BallmannSwiatkowski99,
    AUTHOR = {Ballmann, Werner and {\'S}wi{\polhk{a}}tkowski, Jacek},
     TITLE = {On groups acting on nonpositively curved cubical complexes},
   JOURNAL = {Enseign. Math. (2)},
  FJOURNAL = {L'Enseignement Math\'ematique. Revue Internationale. IIe
              S\'erie},
    VOLUME = {45},
      YEAR = {1999},
    NUMBER = {1-2},
     PAGES = {51--81},
      ISSN = {0013-8584},
     CODEN = {ENMAAR},
   MRCLASS = {20E08 (20E05)},
  MRNUMBER = {2000m:20036},
MRREVIEWER = {Philip L. Bowers},
}

@article {Xiangdong05,
    AUTHOR = {Xie, Xiangdong},
     TITLE = {Groups acting on {CAT}(0) square complexes},
    Note={Preprint 2003},
}

@article {Bowditch98bc,
    AUTHOR = {Bowditch, Brian H.},
     TITLE = {Cut points and canonical splittings of hyperbolic groups},
   JOURNAL = {Acta Math.},
  FJOURNAL = {Acta Mathematica},
    VOLUME = {180},
      YEAR = {1998},
    NUMBER = {2},
     PAGES = {145--186},
      ISSN = {0001-5962},
     CODEN = {ACMAA8},
   MRCLASS = {20F32 (20E06 20E08 57M07)},
  MRNUMBER = {99g:20069},
MRREVIEWER = {Eric M. Freden},
}

@article {BallmannBrin95,
    AUTHOR = {Ballmann, Werner and Brin, Michael},
     TITLE = {Orbihedra of nonpositive curvature},
   JOURNAL = {Inst. Hautes \'Etudes Sci. Publ. Math.},
  FJOURNAL = {Institut des Hautes \'Etudes Scientifiques. Publications
              Math\'ematiques},
    NUMBER = {82},
      YEAR = {1995},
     PAGES = {169--209 (1996)},
      ISSN = {0073-8301},
     CODEN = {PMIHA6},
   MRCLASS = {53C23 (53C20 57M20)},
  MRNUMBER = {97i:53049},
MRREVIEWER = {Ralf J. Spatzier},
}

@article {Xiangdong2004,
    AUTHOR = {Xie, Xiangdong},
     TITLE = {Tits alternative for closed real analytic 4-manifolds of
              nonpositive curvature},
   JOURNAL = {Topology Appl.},
  FJOURNAL = {Topology and its Applications},
    VOLUME = {136},
      YEAR = {2004},
    NUMBER = {1-3},
     PAGES = {87--121},
      ISSN = {0166-8641},
     CODEN = {TIAPD9},
   MRCLASS = {53C20 (20F67 57M05)},
  MRNUMBER = {2 023 412},
}

@article {BrinSquier85,
    AUTHOR = {Brin, Matthew G. and Squier, Craig C.},
     TITLE = {Groups of piecewise linear homeomorphisms of the real line},
   JOURNAL = {Invent. Math.},
  FJOURNAL = {Inventiones Mathematicae},
    VOLUME = {79},
      YEAR = {1985},
    NUMBER = {3},
     PAGES = {485--498},
      ISSN = {0020-9910},
     CODEN = {INVMBH},
   MRCLASS = {57S05 (20F32 57S25)},
  MRNUMBER = {86h:57033},
MRREVIEWER = {Bruno Zimmermann},
}

@article {Tits72,
    AUTHOR = {Tits, J.},
     TITLE = {Free subgroups in linear groups},
   JOURNAL = {J. Algebra},
    VOLUME = {20},
      YEAR = {1972},
     PAGES = {250--270},
   MRCLASS = {20.75},
  MRNUMBER = {44 \#4105},
MRREVIEWER = {B. A. F. Wehrfritz},
}

@article {BestvinaFeighnHandel2000,
    AUTHOR = {Bestvina, Mladen and Feighn, Mark and Handel, Michael},
     TITLE = {The {T}its alternative for {${\rm Out}(F\sb n)$}. {I}.
              {D}ynamics of exponentially-growing automorphisms},
   JOURNAL = {Ann. of Math. (2)},
  FJOURNAL = {Annals of Mathematics. Second Series},
    VOLUME = {151},
      YEAR = {2000},
    NUMBER = {2},
     PAGES = {517--623},
      ISSN = {0003-486X},
     CODEN = {ANMAAH},
   MRCLASS = {20E36 (20E05 57M07)},
  MRNUMBER = {2002a:20034},
MRREVIEWER = {K. Vogtmann},
}

@article {ElMosalamy86,
    AUTHOR = {El-Mosalamy, Mohamed S.},
     TITLE = {Free subgroups of small cancellation groups},
   JOURNAL = {Israel J. Math.},
  FJOURNAL = {Israel Journal of Mathematics},
    VOLUME = {56},
      YEAR = {1986},
    NUMBER = {3},
     PAGES = {345--348},
      ISSN = {0021-2172},
     CODEN = {ISJMAP},
   MRCLASS = {20F06},
  MRNUMBER = {88b:20053},
MRREVIEWER = {D. E. Cohen},
}

@article {EdjvetHowie88,
    AUTHOR = {Edjvet, Martin and Howie, James},
     TITLE = {Star graphs, projective planes and free subgroups in small
              cancellation groups},
   JOURNAL = {Proc. London Math. Soc. (3)},
  FJOURNAL = {Proceedings of the London Mathematical Society. Third Series},
    VOLUME = {57},
      YEAR = {1988},
    NUMBER = {2},
     PAGES = {301--328},
      ISSN = {0024-6115},
     CODEN = {PLMTAL},
   MRCLASS = {20F05 (05C25 20F06)},
  MRNUMBER = {89m:20034},
MRREVIEWER = {A. H. M. Hoare},
}


@article {Collins73,
    AUTHOR = {Collins, Donald J.},
     TITLE = {Free subgroups of small cancellation groups},
   JOURNAL = {Proc. London Math. Soc. (3)},
    VOLUME = {26},
      YEAR = {1973},
     PAGES = {193--206},
   MRCLASS = {20F05},
  MRNUMBER = {47 \#6870},
MRREVIEWER = {R. C. Lyndon},
}

@article {Bowditch98,
    AUTHOR = {Bowditch, B. H.},
     TITLE = {Group actions on trees and dendrons},
   JOURNAL = {Topology},
  FJOURNAL = {Topology. An International Journal of Mathematics},
    VOLUME = {37},
      YEAR = {1998},
    NUMBER = {6},
     PAGES = {1275--1298},
      ISSN = {0040-9383},
     CODEN = {TPLGAF},
   MRCLASS = {20E08 (20F32 57M07)},
  MRNUMBER = {99i:20039},
MRREVIEWER = {William A. Bogley},
}

@article {Bowditch98(2),
    AUTHOR = {Bowditch, B. H.},
     TITLE = {Cut points and canonical splittings of hyperbolic groups},
   JOURNAL = {Acta Math.},
  FJOURNAL = {Acta Mathematica},
    VOLUME = {180},
      YEAR = {1998},
    NUMBER = {2},
     PAGES = {145--186},
      ISSN = {0001-5692},
     CODEN = {ACMAA8},
   MRCLASS = {20F32 (20E06 20E08 57M07)},
  MRNUMBER = {99g:20069},
MRREVIEWER = {Eric M. Freden},
}

@article {ScottSwarup2000,
    AUTHOR = {Scott, G. P. and Swarup, G. A.},
     TITLE = {An algebraic annulus theorem},
   JOURNAL = {Pacific J. Math.},
  FJOURNAL = {Pacific Journal of Mathematics},
    VOLUME = {196},
      YEAR = {2000},
    NUMBER = {2},
     PAGES = {461--506},
      ISSN = {0030-8730},
     CODEN = {PJMAAI},
   MRCLASS = {20F65 (20F67)},
  MRNUMBER = {2001k:20090},
MRREVIEWER = {Athanase Papadopoulos},
}

@article {CorsonTrace96,
    AUTHOR = {Corson, J. M. and Trace, B.},
     TITLE = {Geometry and algebra of nonspherical {$2$}-complexes},
   JOURNAL = {J. London Math. Soc. (2)},
  FJOURNAL = {Journal of the London Mathematical Society. Second Series},
    VOLUME = {54},
      YEAR = {1996},
    NUMBER = {1},
     PAGES = {180--198},
      ISSN = {0024-6107},
     CODEN = {JLMSAK},
   MRCLASS = {57M20 (20F05 20F06)},
  MRNUMBER = {98b:57007},
MRREVIEWER = {Stephen J. Pride},
}

@article {Farley2003,
    AUTHOR = {Farley, Daniel S.},
     TITLE = {Finiteness and {$\rm CAT(0)$} properties of diagram groups},
   JOURNAL = {Topology},
  FJOURNAL = {Topology. An International Journal of Mathematics},
    VOLUME = {42},
      YEAR = {2003},
    NUMBER = {5},
     PAGES = {1065--1082},
      ISSN = {0040-9383},
     CODEN = {TPLGAF},
   MRCLASS = {20F65 (20F06 20F67 57M07)},
  MRNUMBER = {2004b:20057},
MRREVIEWER = {Hanspeter Fischer},
}

@article {Bridson99,
    AUTHOR = {Bridson, Martin R.},
     TITLE = {On the semisimplicity of polyhedral isometries},
   JOURNAL = {Proc. Amer. Math. Soc.},
  FJOURNAL = {Proceedings of the American Mathematical Society},
    VOLUME = {127},
      YEAR = {1999},
    NUMBER = {7},
     PAGES = {2143--2146},
      ISSN = {0002-9939},
     CODEN = {PAMYAR},
   MRCLASS = {53C23 (20F32)},
  MRNUMBER = {99m:53086},
}


@article {DunwoodySwenson2000,
    AUTHOR = {Dunwoody, M. J. and Swenson, E. L.},
     TITLE = {The algebraic torus theorem},
   JOURNAL = {Invent. Math.},
  FJOURNAL = {Inventiones Mathematicae},
    VOLUME = {140},
      YEAR = {2000},
    NUMBER = {3},
     PAGES = {605--637},
      ISSN = {0020-9910},
     CODEN = {INVMBH},
   MRCLASS = {20F65},
  MRNUMBER = {2001d:20039},
MRREVIEWER = {Ilya Kapovich},
}

@article {Hillman2000,
    AUTHOR = {Hillman, Jonathan A.},
     TITLE = {Complex surfaces which are fibre bundles},
   JOURNAL = {Topology Appl.},
  FJOURNAL = {Topology and its Applications},
    VOLUME = {100},
      YEAR = {2000},
    NUMBER = {2-3},
     PAGES = {187--191},
      ISSN = {0166-8641},
     CODEN = {TIAPD9},
   MRCLASS = {32J15 (57N13)},
  MRNUMBER = {2000i:32031},
MRREVIEWER = {Ivan Smith},
}

@article{WisePQRcomplexes,
    AUTHOR = {Wise, Daniel T.},
     TITLE = {Nonpositive sectional curvature for {$(p,q,r)$}-complexes},
   JOURNAL = {Proc. Amer. Math. Soc.},
  FJOURNAL = {Proceedings of the American Mathematical Society},
    VOLUME = {136},
      YEAR = {2008},
    NUMBER = {1},
     PAGES = {41--48 (electronic)},
      ISSN = {0002-9939},
     CODEN = {PAMYAR},
   MRCLASS = {20F67},
  MRNUMBER = {MR2350386 (2009h:20046)},
}
		

@article {Shalen79,
    AUTHOR = {Shalen, Peter B.},
     TITLE = {Linear representations of certain amalgamated products},
   JOURNAL = {J. Pure Appl. Algebra},
  FJOURNAL = {Journal of Pure and Applied Algebra},
    VOLUME = {15},
      YEAR = {1979},
    NUMBER = {2},
     PAGES = {187--197},
      ISSN = {0022-4049},
   MRCLASS = {20C15 (57M05)},
  MRNUMBER = {80e:20011},
MRREVIEWER = {L. G. Mikha\u{\i} lov},
}

@article {Wehrfritz73,
    AUTHOR = {Wehrfritz, B. A. F.},
     TITLE = {Generalized free products of linear groups},
   JOURNAL = {Proc. London Math. Soc. (3)},
    VOLUME = {27},
      YEAR = {1973},
     PAGES = {402--424},
   MRCLASS = {20G15},
  MRNUMBER = {51 \#3322},
MRREVIEWER = {R. C. Lyndon},
}

@article {Adams1955,
    AUTHOR = {Adams, J. F.},
     TITLE = {A new proof of a theorem of {W}. {H}. {C}ockcroft},
   JOURNAL = {J. London Math. Soc.},
    VOLUME = {30},
      YEAR = {1955},
     PAGES = {482--488},
   MRCLASS = {55.0X},
  MRNUMBER = {17,883d},
MRREVIEWER = {J. Adem},
}

@article {GarnickKwongLazebnik93,
    AUTHOR = {Garnick, David K. and Kwong, Y. H. Harris and Lazebnik, Felix},
     TITLE = {Extremal graphs without three-cycles or four-cycles},
   JOURNAL = {J. Graph Theory},
  FJOURNAL = {Journal of Graph Theory},
    VOLUME = {17},
      YEAR = {1993},
    NUMBER = {5},
     PAGES = {633--645},
      ISSN = {0364-9024},
     CODEN = {JGTHDO},
   MRCLASS = {05C35},
  MRNUMBER = {94j:05068},
MRREVIEWER = {Kathryn Fraughnaugh},
}


@book {BollobasBook78,
    AUTHOR = {Bollob{\'a}s, B{\'e}la},
     TITLE = {Extremal graph theory},
    SERIES = {London Mathematical Society Monographs},
    VOLUME = {11},
 PUBLISHER = {Academic Press Inc. [Harcourt Brace Jovanovich Publishers]},
   ADDRESS = {London},
      YEAR = {1978},
     PAGES = {xx+488},
      ISBN = {0-12-111750-2},
   MRCLASS = {05C35 (05-02)},
  MRNUMBER = {80a:05120},
MRREVIEWER = {Michael O. Albertson},
}

@article {DongKoh96,
    AUTHOR = {Dong, F. M. and Koh, K. M.},
     TITLE = {The sizes of graphs with small girth},
   JOURNAL = {Bull. Inst. Combin. Appl.},
  FJOURNAL = {Bulletin of the Institute of Combinatorics and its
              Applications},
    VOLUME = {18},
      YEAR = {1996},
     PAGES = {33--44},
      ISSN = {1183-1278},
   MRCLASS = {05C35},
  MRNUMBER = {97f:05091},
}

@article {DuttonBrigham91,
    AUTHOR = {Dutton, R. D. and Brigham, R. C.},
     TITLE = {Edges in graphs with large girth},
   JOURNAL = {Graphs Combin.},
  FJOURNAL = {Graphs and Combinatorics},
    VOLUME = {7},
      YEAR = {1991},
    NUMBER = {4},
     PAGES = {315--321},
      ISSN = {0911-0119},
     CODEN = {GRCOE5},
   MRCLASS = {05C35 (05C75)},
  MRNUMBER = {93b:05075},
MRREVIEWER = {Samuel Stueckle},
}

@unpublished {KapovichMishaIncoherent98,
    AUTHOR = {Kapovich, Michael},
     TITLE = {On normal subgroups in the fundamental groups of complex
     surfaces},
      NOTE={Preprint},
      YEAR = {1998}
}

@article {RipsGeneralized82,
    AUTHOR = {Rips, E.},
     TITLE = {Generalized small cancellation theory and applications. {I}.
              {T}he word problem},
   JOURNAL = {Israel J. Math.},
  FJOURNAL = {Israel Journal of Mathematics},
    VOLUME = {41},
      YEAR = {1982},
    NUMBER = {1-2},
     PAGES = {1--146},
      ISSN = {0021-2172},
     CODEN = {ISJMAP},
   MRCLASS = {20F06},
  MRNUMBER = {83m:20047},
MRREVIEWER = {D. E. Cohen},
}

@preamble{
   "\def\cprime{$'$} "
}
@book {OlshanskiiBook91,
    AUTHOR = {Ol{\cprime}shanski\u{\i}, A. Yu.},
     TITLE = {Geometry of defining relations in groups},
    SERIES = {Mathematics and its Applications (Soviet Series)},
    VOLUME = {70},
      NOTE = {Translated from the 1989 Russian original by Yu.\ A.
              Bakhturin},
 PUBLISHER = {Kluwer Academic Publishers Group},
   ADDRESS = {Dordrecht},
      YEAR = {1991},
     PAGES = {xxvi+505},
      ISBN = {0-7923-1394-1},
   MRCLASS = {20F32 (20E10 57M07)},
  MRNUMBER = {93g:20071},
}

@article {Schupp03,
    AUTHOR = {Schupp, Paul E.},
     TITLE = {Coxeter groups, 2-completion, perimeter reduction and subgroup
              separability},
   JOURNAL = {Geom. Dedicata},
  FJOURNAL = {Geometriae Dedicata},
    VOLUME = {96},
      YEAR = {2003},
     PAGES = {179--198},
      ISSN = {0046-5755},
     CODEN = {GEMDAT},
   MRCLASS = {20F55 (20F06)},
  MRNUMBER = {2003m:20052},
MRREVIEWER = {Andrew R. Francis},
}


@article {BaumslagShalen90,
    AUTHOR = {Baumslag, Gilbert and Shalen, Peter B.},
     TITLE = {Amalgamated products and finitely presented groups},
   JOURNAL = {Comment. Math. Helv.},
  FJOURNAL = {Commentarii Mathematici Helvetici},
    VOLUME = {65},
      YEAR = {1990},
    NUMBER = {2},
     PAGES = {243--254},
      ISSN = {0010-2571},
     CODEN = {COMHAX},
   MRCLASS = {20E06},
  MRNUMBER = {91j:20071},
MRREVIEWER = {Stephen J. Pride},
}

@article {BieriStrebel78,
    AUTHOR = {Bieri, Robert and Strebel, Ralph},
     TITLE = {Almost finitely presented soluble groups},
   JOURNAL = {Comment. Math. Helv.},
    VOLUME = {53},
      YEAR = {1978},
    NUMBER = {2},
     PAGES = {258--278},
   MRCLASS = {20F05},
  MRNUMBER = {58 \#16890},
MRREVIEWER = {B. Hartley},
}

@incollection {MorganUniformization84,
    AUTHOR = {Morgan, John W.},
     TITLE = {On {T}hurston's uniformization theorem for three-dimensional
              manifolds},
 BOOKTITLE = {The Smith conjecture (New York, 1979)},
    SERIES = {Pure Appl. Math.},
    VOLUME = {112},
     PAGES = {37--125},
 PUBLISHER = {Academic Press},
   ADDRESS = {Orlando, FL},
      YEAR = {1984},
   MRCLASS = {57N10 (30F10)},
  MRNUMBER = {758 464},
}

@book {Luck02,
    AUTHOR = {L{\"u}ck, Wolfgang},
     TITLE = {{$L\sp 2$}-invariants: theory and applications to geometry and
              {$K$}-theory},
  PUBLISHER = {Springer-Verlag},
   ADDRESS = {Berlin},
      YEAR = {2002},
     PAGES = {xvi+595},
      ISBN = {3-540-43566-2},
   MRCLASS = {58J22 (19K56 46L80 57Q10 57R20 58J52)},
  MRNUMBER = {2003m:58033},
MRREVIEWER = {Thomas Schick},
}

@article{KapovichWeidmann03,
    AUTHOR = {Kapovich, Ilya and Weidmann, Richard},
     TITLE = {Freely indecomposable groups acting on hyperbolic spaces},
   JOURNAL = {Internat. J. Algebra Comput.},
  FJOURNAL = {International Journal of Algebra and Computation},
    VOLUME = {14},
      YEAR = {2004},
    NUMBER = {2},
     PAGES = {115--171},
      ISSN = {0218-1967},
   MRCLASS = {20F67 (57M07)},
  MRNUMBER = {2058318},
MRREVIEWER = {Rafael Oswaldo Ruggiero},
       DOI = {10.1142/S0218196704001682},
       URL = {https://doi-org.proxy3.library.mcgill.ca/10.1142/S0218196704001682},
}


@book {HaagerupBook01,
    AUTHOR = {Cherix, Pierre-Alain and Cowling, Michael and Jolissaint, Paul
              and Julg, Pierre and Valette, Alain},
     TITLE = {Groups with the {H}aagerup property},
    SERIES = {Progress in Mathematics},
    VOLUME = {197},
      NOTE = {Gromov's a-T-menability},
 PUBLISHER = {Birkh\"auser Verlag},
   ADDRESS = {Basel},
      YEAR = {2001},
     PAGES = {viii+126},
      ISBN = {3-7643-6598-6},
   MRCLASS = {22D10 (22-02 22D25 22E30 43A07 46Lxx)},
  MRNUMBER = {2002h:22007},
MRREVIEWER = {Tullio G. Ceccherini-Silberstein},
}

@article {Short01,
    AUTHOR = {Short, Hamish},
     TITLE = {Finitely presented subgroups of a product of two free groups},
   JOURNAL = {Q. J. Math.},
  FJOURNAL = {The Quarterly Journal of Mathematics},
    VOLUME = {52},
      YEAR = {2001},
    NUMBER = {1},
     PAGES = {127--131},
      ISSN = {0033-5606},
   MRCLASS = {20F06 (20E05 57M07)},
  MRNUMBER = {2001m:20048},
}
@preamble{
   "\def\cprime{$'$} "
}
@inproceedings {Olshanskii84,
    AUTHOR = {Ol{\cprime}{\v{s}}anski\u{\i}, A. Yu.},
     TITLE = {On a geometric method in the combinatorial group theory},
 BOOKTITLE = {Proceedings of the International Congress of Mathematicians,
              Vol.\ 1, 2 (Warsaw, 1983)},
     PAGES = {415--424},
 PUBLISHER = {PWN},
   ADDRESS = {Warsaw},
      YEAR = {1984},
   MRCLASS = {20F05 (20F06)},
  MRNUMBER = {86j:20031},
MRREVIEWER = {Andrew Vince},
}

@article {Miller02,
    AUTHOR = {Miller, III, Charles F.},
     TITLE = {Subgroups of direct products with a free group},
   JOURNAL = {Q. J. Math.},
  FJOURNAL = {The Quarterly Journal of Mathematics},
    VOLUME = {53},
      YEAR = {2002},
    NUMBER = {4},
     PAGES = {503--506},
      ISSN = {0033-5606},
   MRCLASS = {20E05 (20F05)},
  MRNUMBER = {2003m:20026},
}


@article {BridsonHowieMillerShort02,
    AUTHOR = {Bridson, Martin R. and Howie, James and Miller, III, Charles
              F. and Short, Hamish},
     TITLE = {The subgroups of direct products of surface groups},
      NOTE = {Dedicated to John Stallings on the occasion of his 65th
              birthday},
   JOURNAL = {Geom. Dedicata},
  FJOURNAL = {Geometriae Dedicata},
    VOLUME = {92},
      YEAR = {2002},
     PAGES = {95--103},
      ISSN = {0046-5755},
     CODEN = {GEMDAT},
   MRCLASS = {20Fxx (20Jxx 57Mxx)},
  MRNUMBER = {1 934 013},
}

@incollection {Strebel90,
    AUTHOR = {Strebel, Ralph},
     TITLE = {Appendix. {S}mall cancellation groups},
 BOOKTITLE = {Sur les groupes hyperboliques d'apr\`es Mikhael Gromov (Bern,
              1988)},
    SERIES = {Progr. Math.},
    VOLUME = {83},
     PAGES = {227--273},
 PUBLISHER = {Birkh\"auser Boston},
   ADDRESS = {Boston, MA},
      YEAR = {1990},
   MRCLASS = {57M05 (20F06 53C23)},
  MRNUMBER = {1 086 661},
}

@incollection {Stallings77,
    AUTHOR = {Stallings, John},
     TITLE = {Coherence of {$3$}-manifold fundamental groups},
 BOOKTITLE = {S\'eminaire Bourbaki, Vol. 1975/76, 28 \`eme ann\'ee, Exp. No.
              481},
     PAGES = {167--173. Lecture Notes in Math., Vol. 567},
 PUBLISHER = {Springer},
   ADDRESS = {Berlin},
      YEAR = {1977},
   MRCLASS = {55A05 (20E40)},
  MRNUMBER = {56 \#1290},
MRREVIEWER = {G. Peter Scott},
}

@article {Swarup73,
    AUTHOR = {Swarup, G. Ananda},
     TITLE = {Finding incompressible surfaces in {$3$}-manifolds},
   JOURNAL = {J. London Math. Soc. (2)},
    VOLUME = {6},
      YEAR = {1973},
     PAGES = {441--452},
   MRCLASS = {55A05},
  MRNUMBER = {52 \#1661},
MRREVIEWER = {J. S. Birman},
}


@article {BaumslagMorganShalen87,
    AUTHOR = {Baumslag, Gilbert and Morgan, John W. and Shalen, Peter B.},
     TITLE = {Generalized triangle groups},
   JOURNAL = {Math. Proc. Cambridge Philos. Soc.},
  FJOURNAL = {Mathematical Proceedings of the Cambridge Philosophical
              Society},
    VOLUME = {102},
      YEAR = {1987},
    NUMBER = {1},
     PAGES = {25--31},
      ISSN = {0305-0041},
     CODEN = {MPCPCO},
   MRCLASS = {20F05},
  MRNUMBER = {88g:20062},
MRREVIEWER = {Stephen J. Pride},
}

@article {Howie85,
    AUTHOR = {Howie, James},
     TITLE = {On the asphericity of ribbon disc complements},
   JOURNAL = {Trans. Amer. Math. Soc.},
  FJOURNAL = {Transactions of the American Mathematical Society},
    VOLUME = {289},
      YEAR = {1985},
    NUMBER = {1},
     PAGES = {281--302},
      ISSN = {0002-9947},
     CODEN = {TAMTAM},
   MRCLASS = {57M20 (20F05 57Q45)},
  MRNUMBER = {87a:57007},
MRREVIEWER = {Michel Boileau},
}

@incollection {Bogley93,
    AUTHOR = {Bogley, William A.},
     TITLE = {J. {H}. {C}. {W}hitehead's asphericity question},
 BOOKTITLE = {Two-dimensional homotopy and combinatorial group theory},
    SERIES = {London Math. Soc. Lecture Note Ser.},
    VOLUME = {197},
     PAGES = {309--334},
 PUBLISHER = {Cambridge Univ. Press},
   ADDRESS = {Cambridge},
      YEAR = {1993},
   MRCLASS = {57M20 (55Q52)},
  MRNUMBER = {1 279 184},
}

@article {Whitehead41,
    AUTHOR = {Whitehead, J. H. C.},
     TITLE = {On adding relations to homotopy groups},
   JOURNAL = {Ann. of Math. (2)},
    VOLUME = {42},
      YEAR = {1941},
     PAGES = {409--428},
   MRCLASS = {56.0X},
  MRNUMBER = {2,323c},
MRREVIEWER = {R. H. Fox},
}

@article {Kapovich2002,
    AUTHOR = {Kapovich, Ilya},
     TITLE = {Subgroup properties of fully residually free groups},
   JOURNAL = {Trans. Amer. Math. Soc.},
  FJOURNAL = {Transactions of the American Mathematical Society},
    VOLUME = {354},
      YEAR = {2002},
    NUMBER = {1},
     PAGES = {335--362 (electronic)},
      ISSN = {0002-9947},
     CODEN = {TAMTAM},
   MRCLASS = {20F65 (20E26 57M07)},
  MRNUMBER = {2002h:20058},
MRREVIEWER = {Dimitrios Varsos},
}


@article {PotyagailoKapovich91,
    AUTHOR = {Kapovich, M. {\`E}. and Potyaga\u{\i}lo, L. D.},
     TITLE = {On the absence of finiteness theorems of {A}hlfors and
              {S}ullivan for {K}leinian groups in higher dimensions},
   JOURNAL = {Sibirsk. Mat. Zh.},
  FJOURNAL = {Akademiya Nauk SSSR. Sibirskoe Otdelenie. Sibirski\u\i\
              Matematicheski\u\i\ Zhurnal},
    VOLUME = {32},
      YEAR = {1991},
    NUMBER = {2},
     PAGES = {61--73, 212},
      ISSN = {0037-4474},
   MRCLASS = {30F40 (20F34 20H10 53A30 57S30)},
  MRNUMBER = {93g:30064},
MRREVIEWER = {V. V. Chueshev},
}

@article {Potyagailo94,
    AUTHOR = {Potyaga\u{\i}lo, L.},
     TITLE = {Finitely generated {K}leinian groups in {$3$}-space and
              {$3$}-manifolds of infinite homotopy type},
   JOURNAL = {Trans. Amer. Math. Soc.},
  FJOURNAL = {Transactions of the American Mathematical Society},
    VOLUME = {344},
      YEAR = {1994},
    NUMBER = {1},
     PAGES = {57--77},
      ISSN = {0002-9947},
     CODEN = {TAMTAM},
   MRCLASS = {57M50 (20H10 30F40 57N10 57S30)},
  MRNUMBER = {94m:57030},
MRREVIEWER = {Darryl McCullough},
}

@article {BowditchMess94,
    AUTHOR = {Bowditch, B. H. and Mess, G.},
     TITLE = {A {$4$}-dimensional {K}leinian group},
   JOURNAL = {Trans. Amer. Math. Soc.},
  FJOURNAL = {Transactions of the American Mathematical Society},
    VOLUME = {344},
      YEAR = {1994},
    NUMBER = {1},
     PAGES = {391--405},
      ISSN = {0002-9947},
     CODEN = {TAMTAM},
   MRCLASS = {57S30 (20H10 30F40 57M50)},
  MRNUMBER = {95f:57057},
MRREVIEWER = {Darryl McCullough},
}

@article {BorelSerre73,
    AUTHOR = {Borel, A. and Serre, J.-P.},
     TITLE = {Corners and arithmetic groups},
      NOTE = {Avec un appendice: Arrondissement des vari\'et\'es \`a coins,
              par A. Douady et L. H\'erault},
   JOURNAL = {Comment. Math. Helv.},
    VOLUME = {48},
      YEAR = {1973},
     PAGES = {436--491},
   MRCLASS = {22E40},
  MRNUMBER = {52 \#8337},
MRREVIEWER = {M. S. Raghunathan},
}


@article{NicaCubulating04,
    AUTHOR = {Nica, Bogdan},
     TITLE = {Cubulating spaces with walls},
   JOURNAL = {Algebr. Geom. Topol.},
  FJOURNAL = {Algebraic \& Geometric Topology},
    VOLUME = {4},
      YEAR = {2004},
     PAGES = {297--309 (electronic)},
      ISSN = {1472-2747},
   MRCLASS = {20F65},
  MRNUMBER = {2 059 193},
}


@UNPUBLISHED{WiseSixtolic,
   author = {Wise, Daniel T.},
   title = {Sixtolic complexes and their fundamental groups},
   note = {Preprint},
    year = {2003},
}

@UNPUBLISHED{SageevWisePeriodic,
   author = {Michah Sageev and Daniel T. Wise},
   title = {Periodic flats in cube complexes},
 note = {Preprint},
 year = {2004},
}

@article{BumaginWiseOut,
   author = {Inna Bumagin and Daniel T. Wise},
   title = {Every group is an outer automorphism group of a finitely generated
   group},
   JOURNAL = {J. Pure Appl. Algebra},
  FJOURNAL = {Journal of Pure and Applied Algebra},
   note = {To appear},
}

@article{HruskaWiseAxioms,
    AUTHOR = {Hruska, G. C. and Wise, Daniel T.},
     TITLE = {Finiteness properties of cubulated groups},
   JOURNAL = {Compos. Math.},
  FJOURNAL = {Compositio Mathematica},
    VOLUME = {150},
      YEAR = {2014},
    NUMBER = {3},
     PAGES = {453--506},
      ISSN = {0010-437X},
   MRCLASS = {20F65 (20E08 20F67)},
  MRNUMBER = {3187627},
MRREVIEWER = {Michael L. Mihalik},
       DOI = {10.1112/S0010437X13007112},
       URL = {http://dx.doi.org/10.1112/S0010437X13007112},
}


@article{HsuWiseCubulating,
    AUTHOR = {Hsu, Tim and Wise, Daniel T.},
     TITLE = {Cubulating graphs of free groups with cyclic edge groups},
   JOURNAL = {Amer. J. Math.},
  FJOURNAL = {American Journal of Mathematics},
    VOLUME = {132},
      YEAR = {2010},
    NUMBER = {5},
     PAGES = {1153--1188},
      ISSN = {0002-9327},
     CODEN = {AJMAAN},
   MRCLASS = {20F05 (05C25 20F67)},
  MRNUMBER = {2732342 (2011j:20080)},
MRREVIEWER = {Goulnara N. Arzhantseva},
       DOI = {10.1353/ajm.2010.0004},
       URL = {http://dx.doi.org/10.1353/ajm.2010.0004},
}

@UNPUBLISHED{WiseEventuallyInjective,
   author = {Daniel T. Wise},
   title = {On Eventually Injective Endomorphisms},
   note = {Preprint},
}



@article {HaglundWiseSpecial,
    AUTHOR = {Haglund, Fr{\'e}d{\'e}ric and Wise, Daniel T.},
     TITLE = {Special cube complexes},
   JOURNAL = {Geom. Funct. Anal.},
  FJOURNAL = {Geometric and Functional Analysis},
    VOLUME = {17},
      YEAR = {2008},
    NUMBER = {5},
     PAGES = {1
     551--1620},
      ISSN = {1016-443X},
     CODEN = {GFANFB},
   MRCLASS = {20F36 (20F55 20F67)},
  MRNUMBER = {MR2377497},
}
		



@UNPUBLISHED{BumaginWiseCoherence,
   author = {Inna Bumagin and Daniel T. Wise},
   title = {Coherence of Word-hyperbolic by cyclic groups},
   note = {Preprint},
   year = {2003},
}

@MISC{WiseEnergy,
   author = {Daniel T. Wise},
   title = {On the vanishing of the 2nd {$L^2$} betti number},
howpublished = {Available at \url{http://www.math.mcgill.ca/wise/papers}},
   note = {pp. 1-21. Submitted},
 }

@article{WiseHNCoherence,
     AUTHOR = {Wise, Daniel T.},
     TITLE = {The coherence of one-relator groups with torsion and the
              {H}anna {N}eumann conjecture},
   JOURNAL = {Bull. London Math. Soc.},
  FJOURNAL = {The Bulletin of the London Mathematical Society},
    VOLUME = {37},
      YEAR = {2005},
    NUMBER = {5},
     PAGES = {697--705},
      ISSN = {0024-6093},
     CODEN = {LMSBBT},
   MRCLASS = {20F05 (05C25 05C38 20E05)},
  MRNUMBER = {2164831 (2006f:20037)},
MRREVIEWER = {Jon McCammond},
       DOI = {10.1112/S0024609305004376},
       URL = {http://dx.doi.org/10.1112/S0024609305004376},
}

@article {WiseAnnouncement03,
    AUTHOR = {Wise, Daniel T.},
     TITLE = {Nonpositive immersions, sectional curvature, and subgroup
              properties},
   JOURNAL = {Electron. Res. Announc. Amer. Math. Soc.},
  FJOURNAL = {Electronic Research Announcements of the American Mathematical
              Society},
    VOLUME = {9},
      YEAR = {2003},
     PAGES = {1--9 (electronic)},
      ISSN = {1079-6762},
   MRCLASS = {57M07 (20F67 57M20)},
  MRNUMBER = {1 988 866},
}

@article{McCammondWiseLQCSC,
    AUTHOR = {McCammond, Jonathan P. and Wise, Daniel T.},
     TITLE = {Locally quasiconvex small-cancellation groups},
   JOURNAL = {Trans. Amer. Math. Soc.},
  FJOURNAL = {Transactions of the American Mathematical Society},
    VOLUME = {360},
      YEAR = {2008},
    NUMBER = {1},
     PAGES = {237--271 (electronic)},
      ISSN = {0002-9947},
     CODEN = {TAMTAM},
   MRCLASS = {20F06 (20F67 57M07)},
  MRNUMBER = {MR2342002 (2009a:20053)},
MRREVIEWER = {Brent Everitt},
       DOI = {10.1090/S0002-9947-07-04206-7},
       URL = {http://dx.doi.org/10.1090/S0002-9947-07-04206-7},
}

@ARTICLE{HsuWiseFixed,
    AUTHOR = {Hsu, Tim and Wise, Daniel T.},
     TITLE = {Groups with infinitely many types of fixed subgroups},
   JOURNAL = {Israel J. Math.},
  FJOURNAL = {Israel Journal of Mathematics},
    VOLUME = {144},
      YEAR = {2004},
     PAGES = {93--107},
      ISSN = {0021-2172},
     CODEN = {ISJMAP},
   MRCLASS = {20F65 (20E08 20E36 20F28 20F67)},
  MRNUMBER = {MR2121535 (2006a:20079)},
MRREVIEWER = {Jos{\'e} Burillo},
}


@unpublished{Rattaggi2001,
   author = {Diego Rattaggi},
   title = {Three remarkable amalgams {$F_9*_{F_{81}}{F_9}$}},
   note = {Preprint, 2001},
}

@article {BurgerMozes2000,
    AUTHOR = {Burger, Marc and Mozes, Shahar},
     TITLE = {Lattices in product of trees},
   JOURNAL = {Inst. Hautes \'Etudes Sci. Publ. Math.},
  FJOURNAL = {Institut des Hautes \'Etudes Scientifiques. Publications
              Math\'ematiques},
    NUMBER = {92},
      YEAR = {2000},
     PAGES = {151--194 (2001)},
      ISSN = {0073-8301},
     CODEN = {PMIHA6},
   MRCLASS = {20E08 (22E40)},
  MRNUMBER = {2002i:20042},
MRREVIEWER = {Alexander Lubotzky},
}

@article {BurgerMozes97,
    AUTHOR = {Burger, Marc and Mozes, Shahar},
     TITLE = {Finitely presented simple groups and products of trees},
   JOURNAL = {C. R. Acad. Sci. Paris S\'er. I Math.},
  FJOURNAL = {Comptes Rendus de l'Acad\'emie des Sciences. S\'erie I.
              Math\'ematique},
    VOLUME = {324},
      YEAR = {1997},
    NUMBER = {7},
     PAGES = {747--752},
      ISSN = {0764-4442},
     CODEN = {CASMEI},
   MRCLASS = {20E08 (20E32)},
  MRNUMBER = {98g:20041},
MRREVIEWER = {Olympia Talelli},
}

@article {Malcev40NOENG,
    AUTHOR = {Malcev, A.},
     TITLE = {On isomorphic matrix representations of infinite groups},
   JOURNAL = {Rec. Math. [Mat. Sbornik] N.S.},
    VOLUME = {8 (50)},
      YEAR = {1940},
     PAGES = {405--422},
   MRCLASS = {20.0X},
  MRNUMBER = {2,216d},
MRREVIEWER = {L. Zippin},
}



@article {Dunwoody85,
    AUTHOR = {Dunwoody, M. J.},
     TITLE = {The accessibility of finitely presented groups},
   JOURNAL = {Invent. Math.},
  FJOURNAL = {Inventiones Mathematicae},
    VOLUME = {81},
      YEAR = {1985},
    NUMBER = {3},
     PAGES = {449--457},
      ISSN = {0020-9910},
     CODEN = {INVMBH},
   MRCLASS = {20E06 (54H99 57M99)},
  MRNUMBER = {87d:20037},
MRREVIEWER = {D. E. Cohen},
}

@article {Gromov2003,
    AUTHOR = {Gromov, M.},
     TITLE = {Random walk in random groups},
   JOURNAL = {Geom. Funct. Anal.},
  FJOURNAL = {Geometric and Functional Analysis},
    VOLUME = {13},
      YEAR = {2003},
    NUMBER = {1},
     PAGES = {73--146},
      ISSN = {1016-443X},
     CODEN = {GFANFB},
   MRCLASS = {20F65 (20P05 60G50)},
  MRNUMBER = {1 978 492},
}

@incollection {Ventura02,
    AUTHOR = {Ventura, E.},
     TITLE = {Fixed subgroups in free groups: a survey},
 BOOKTITLE = {Combinatorial and geometric group theory (New York,
              2000/Hoboken, NJ, 2001)},
    SERIES = {Contemp. Math.},
    VOLUME = {296},
     PAGES = {231--255},
 PUBLISHER = {Amer. Math. Soc.},
   ADDRESS = {Providence, RI},
      YEAR = {2002},
   MRCLASS = {20E05},
  MRNUMBER = {2003f:20037},
MRREVIEWER = {Gilbert Levitt},
}

@article {BestvinaHandel92,
    AUTHOR = {Bestvina, Mladen and Handel, Michael},
     TITLE = {Train tracks and automorphisms of free groups},
   JOURNAL = {Ann. of Math. (2)},
  FJOURNAL = {Annals of Mathematics. Second Series},
    VOLUME = {135},
      YEAR = {1992},
    NUMBER = {1},
     PAGES = {1--51},
      ISSN = {0003-486X},
     CODEN = {ANMAAH},
   MRCLASS = {20E05 (20F28 20F32 20F34 57M07 57M15)},
  MRNUMBER = {92m:20017},
MRREVIEWER = {Darryl McCullough},
}

@PHDTHESIS{ShorThesis99,
 author = {Jeremy Andrew Shor},
 title = {On fixed subgroups of automorphisms in hyperbolic groups},
 school = {Columbia University},
 year = {1999},
}


@article {Weinbaum72,
    AUTHOR = {Weinbaum, C. M.},
     TITLE = {On relators and diagrams for groups with one defining
              relation},
   JOURNAL = {Illinois J. Math.},
    VOLUME = {16},
      YEAR = {1972},
     PAGES = {308--322},
   MRCLASS = {20F05},
  MRNUMBER = {45 \#6901},
MRREVIEWER = {I. Chiswell},
}

@article {Howie00,
    AUTHOR = {Howie, James},
     TITLE = {A short proof of a theorem of {B}rodski\u\i},
   JOURNAL = {Publ. Mat.},
  FJOURNAL = {Publicacions Matem\`atiques},
    VOLUME = {44},
      YEAR = {2000},
    NUMBER = {2},
     PAGES = {641--647},
      ISSN = {0214-1493},
   MRCLASS = {20F05 (57M07)},
  MRNUMBER = {2001i:20066},
}

@inproceedings {MeakinWeil02,
    AUTHOR = {Meakin, J. and Weil, P.},
     TITLE = {Subgroups of free groups: a contribution to the {H}anna
              {N}eumann conjecture},
 BOOKTITLE = {Proceedings of the Conference on Geometric and Combinatorial
              Group Theory, Part I (Haifa, 2000)},
   JOURNAL = {Geom. Dedicata},
  FJOURNAL = {Geometriae Dedicata},
    VOLUME = {94},
      YEAR = {2002},
     PAGES = {33--43},
      ISSN = {0046-5755},
     CODEN = {GEMDAT},
   MRCLASS = {20E05},
  MRNUMBER = {1 950 872},
}

@incollection {Khan02,
    AUTHOR = {Khan, Bilal},
     TITLE = {Positively generated subgroups of free groups and the {H}anna
              {N}eumann conjecture},
 BOOKTITLE = {Combinatorial and geometric group theory (New York,
              2000/Hoboken, NJ, 2001)},
    SERIES = {Contemp. Math.},
    VOLUME = {296},
     PAGES = {155--170},
 PUBLISHER = {Amer. Math. Soc.},
   ADDRESS = {Providence, RI},
      YEAR = {2002},
   MRCLASS = {20E05 (20F10)},
  MRNUMBER = {2003e:20027},
MRREVIEWER = {Waldemar M. Ho{\l}ubowski},
}

@UNPUBLISHED{JS03,
   author = {Tadeusz Januszkiewicz and Jacek Swiatkowski},
   title = {},
   note = {In preparation},
}

@article {Ollivier06,
    AUTHOR = {Ollivier, Yann},
     TITLE = {On a small cancellation theorem of {G}romov},
   JOURNAL = {Bull. Belg. Math. Soc. Simon Stevin},
  FJOURNAL = {Bulletin of the Belgian Mathematical Society. Simon Stevin},
    VOLUME = {13},
      YEAR = {2006},
    NUMBER = {1},
     PAGES = {75--89},
      ISSN = {1370-1444},
   MRCLASS = {20F06 (20F65)},
  MRNUMBER = {MR2245980 (2007e:20066)},
MRREVIEWER = {Armando Martino},
}
		
@UNPUBLISHED{Gromov02,
   author = {M. Gromov},
   title = {Random Walk in Random Groups},
   note = {IH{\'{E}}S Preprint 2003},
}

@UNPUBLISHED{OllivierThesis03,
   author = {Y. Ollivier},
   title = {Sharp phase transition theorems for hyperbolicity of random groups},
   note = {Preprint},
   YEAR={2003},
}

@article {LawsonYau72,
    AUTHOR = {Lawson, Jr., H. Blaine and Yau, Shing Tung},
     TITLE = {Compact manifolds of nonpositive curvature},
   JOURNAL = {J. Differential Geometry},
    VOLUME = {7},
      YEAR = {1972},
     PAGES = {211--228},
   MRCLASS = {53C20},
  MRNUMBER = {48 \#12402},
MRREVIEWER = {F. Brickell},
}

@article {GromollWolf71,
    AUTHOR = {Gromoll, Detlef and Wolf, Joseph A.},
     TITLE = {Some relations between the metric structure and the algebraic
              structure of the fundamental group in manifolds of nonpositive
              curvature},
   JOURNAL = {Bull. Amer. Math. Soc.},
    VOLUME = {77},
      YEAR = {1971},
     PAGES = {545--552},
   MRCLASS = {53.72},
  MRNUMBER = {43 \#6841},
MRREVIEWER = {F. Brickell},
}

@article {Brady99,
    AUTHOR = {Brady, Noel},
     TITLE = {Branched coverings of cubical complexes and subgroups of
              hyperbolic groups},
   JOURNAL = {J. London Math. Soc. (2)},
  FJOURNAL = {Journal of the London Mathematical Society. Second Series},
    VOLUME = {60},
      YEAR = {1999},
    NUMBER = {2},
     PAGES = {461--480},
      ISSN = {0024-6107},
     CODEN = {JLMSAK},
   MRCLASS = {20F67 (20F05 20F65 57M07)},
  MRNUMBER = {2000j:20076},
MRREVIEWER = {Michel Coornaert},
}

@article {WiseNonApproximable03,
    AUTHOR = {Wise, Daniel T.},
     TITLE = {A flat plane that is not the limit of periodic flat planes},
        JOURNAL = {Algebr. Geom. Topol.},
  FJOURNAL = {Algebraic \& Geometric Topology},
    VOLUME = {3},
      YEAR = {2003},
     PAGES = {147--154 (electronic)},
}



@article {Berger1966,
    AUTHOR = {Berger, Robert},
     TITLE = {The undecidability of the domino problem},
   JOURNAL = {Mem. Amer. Math. Soc. No.},
    VOLUME = {66},
      YEAR = {1966},
     PAGES = {72},
   MRCLASS = {02.74},
  MRNUMBER = {36 \#49},
MRREVIEWER = {J. R. B{\"u}chi},
}

@article{WiseCSC,
    AUTHOR = {Wise, Daniel T.},
     TITLE = {Complete square complexes},
   JOURNAL = {Comment. Math. Helv.},
  FJOURNAL = {Commentarii Mathematici Helvetici. A Journal of the Swiss
              Mathematical Society},
    VOLUME = {82},
      YEAR = {2007},
    NUMBER = {4},
     PAGES = {683--724},
      ISSN = {0010-2571},
   MRCLASS = {20F67 (20F06)},
  MRNUMBER = {MR2341837 (2009c:20078)},
MRREVIEWER = {Richard Weidmann},
}



@article {WiseVHtori,
    AUTHOR = {Wise, Daniel T.},
     TITLE = {Approximating flats by periodic flats in {CAT}(0) square
              complexes},
   JOURNAL = {Canad. J. Math.},
  FJOURNAL = {Canadian Journal of Mathematics. Journal Canadien de
              Math\'ematiques},
    VOLUME = {57},
      YEAR = {2005},
    NUMBER = {2},
     PAGES = {416--448},
      ISSN = {0008-414X},
     CODEN = {CJMAAB},
   MRCLASS = {20F67 (20F06 52C23 57M05 57M40)},
  MRNUMBER = {MR2124924 (2006c:20090)},
MRREVIEWER = {Andrzej Szczepa{\'n}ski},
}



@book {Epstein92,
    AUTHOR = {Epstein, David B. A. and Cannon, James W. and Holt, Derek F.
              and Levy, Silvio V. F. and Paterson, Michael S. and Thurston,
              William P.},
     TITLE = {Word processing in groups},
 PUBLISHER = {Jones and Bartlett Publishers},
   ADDRESS = {Boston, MA},
      YEAR = {1992},
     PAGES = {xii+330},
      ISBN = {0-86720-244-0},
   MRCLASS = {20F10 (03D40 20-02 68Q70)},
  MRNUMBER = {93i:20036},
MRREVIEWER = {Richard M. Thomas},
}

@incollection {Hu95,
    AUTHOR = {Hu, B.},
     TITLE = {Retractions of closed manifolds with nonpositive curvature},
 BOOKTITLE = {Geometric group theory (Columbus, OH, 1992)},
    SERIES = {Ohio State Univ. Math. Res. Inst. Publ.},
    VOLUME = {3},
     PAGES = {135--147},
 PUBLISHER = {de Gruyter},
   ADDRESS = {Berlin},
      YEAR = {1995},
   MRCLASS = {57Q99},
  MRNUMBER = {96h:57023},
MRREVIEWER = {Fr{\'e}d{\'e}ric Paulin},
}



@incollection {Tucker90,
    AUTHOR = {Tucker, Thomas W.},
     TITLE = {Some topological graph theory for topologists: a sampler of
              covering space constructions},
 BOOKTITLE = {Topology and combinatorial group theory (Hanover, NH,
              1986/1987; Enfield, NH, 1988)},
    SERIES = {Lecture Notes in Math.},
    VOLUME = {1440},
     PAGES = {192--207},
 PUBLISHER = {Springer},
   ADDRESS = {Berlin},
      YEAR = {1990},
   MRCLASS = {57M10 (05C10 57M15)},
  MRNUMBER = {92i:57002},
}



@book {GrunbaumShephard87,
    AUTHOR = {Gr{\"u}nbaum, Branko and Shephard, G. C.},
     TITLE = {Tilings and patterns},
 PUBLISHER = {W. H. Freeman and Company},
   ADDRESS = {New York},
      YEAR = {1987},
     PAGES = {xii+700},
      ISBN = {0-7167-1193-1},
   MRCLASS = {52A45 (03B25 03D20 05B45 20H15)},
  MRNUMBER = {88k:52018},
MRREVIEWER = {H. S. M. Coxeter},
}



@unpublished{Wise95,
   author = {Wise, Daniel T.},
   title = {A non-positively curved squared complex with no finite covers},
   note = {Preprint, 1995},
}

@article {Eberlein72,
    AUTHOR = {Eberlein, Patrick},
     TITLE = {Geodesic flow in certain manifolds without conjugate points},
   JOURNAL = {Trans. Amer. Math. Soc.},
    VOLUME = {167},
      YEAR = {1972},
     PAGES = {151--170},
   MRCLASS = {58E10 (53C20)},
  MRNUMBER = {45 \#4453},
MRREVIEWER = {W. Klingenberg},
}



@unpublished {KapovichMisha98,
    AUTHOR = {Kapovich, Michael},
     TITLE = {Flats in $3$-manifolds},
 NOTE={Preprint},
      YEAR = {1998},
     PAGES = {1--32},
}


@article {Buyalo88,
    AUTHOR = {Buyalo, S. V.},
     TITLE = {Euclidean planes in three-dimensional manifolds of nonpositive
              curvature},
   JOURNAL = {Mat. Zametki},
  FJOURNAL = {Akademiya Nauk SSSR. Matematicheskie Zametki},
    VOLUME = {43},
      YEAR = {1988},
    NUMBER = {1},
     PAGES = {103--114, 155},
      ISSN = {0025-567X},
   MRCLASS = {53C20},
  MRNUMBER = {89d:53082},
MRREVIEWER = {V. V. Glazyrin},
}

@article {Schroeder88,
    AUTHOR = {Schroeder, Viktor},
     TITLE = {Existence of immersed tori in manifolds of nonpositive
              curvature},
   JOURNAL = {J. Reine Angew. Math.},
  FJOURNAL = {Journal f\"ur die Reine und Angewandte Mathematik},
    VOLUME = {390},
      YEAR = {1988},
     PAGES = {32--46},
      ISSN = {0075-4102},
     CODEN = {JRMAA8},
   MRCLASS = {53C20},
  MRNUMBER = {89i:53032},
MRREVIEWER = {Werner Ballmann},
}

@article {Schroeder90,
    AUTHOR = {Schroeder, Viktor},
     TITLE = {Codimension one tori in manifolds of nonpositive curvature},
   JOURNAL = {Geom. Dedicata},
  FJOURNAL = {Geometriae Dedicata},
    VOLUME = {33},
      YEAR = {1990},
    NUMBER = {3},
     PAGES = {251--263},
      ISSN = {0046-5755},
     CODEN = {GEMDAT},
   MRCLASS = {53C21},
  MRNUMBER = {91k:53049},
MRREVIEWER = {Ji-Ping Sha},
}



@book {Ballmann95,
    AUTHOR = {Ballmann, Werner},
     TITLE = {Lectures on spaces of nonpositive curvature},
    SERIES = {DMV Seminar},
    VOLUME = {25},
      NOTE = {With an appendix by Misha Brin},
 PUBLISHER = {Birkh\"auser Verlag},
   ADDRESS = {Basel},
      YEAR = {1995},
     PAGES = {viii+112},
      ISBN = {3-7643-5242-6},
   MRCLASS = {53C21 (58F17)},
  MRNUMBER = {97a:53053},
MRREVIEWER = {Boris Hasselblatt},
}


@unpublished{Schlenker2002,
    AUTHOR = {Schlenker, Jean-Marc},
   title = {Ideal triangulations of finite volume hyperbolic 3-manifolds},
   note = {Preprint 2002},
}



@article {Shentizer55,
    AUTHOR = {Shenitzer, Abe},
     TITLE = {Decomposition of a group with a single defining relation into
              a free product},
   JOURNAL = {Proc. Amer. Math. Soc.},
    VOLUME = {6},
      YEAR = {1955},
     PAGES = {273--279},
   MRCLASS = {20.0X},
  MRNUMBER = {16,995c},
MRREVIEWER = {A. Kert{\'e}sz},
}



@incollection {FineGaglioneRosenbergerSpellman95,
    AUTHOR = {Fine, Benjamin and Gaglione, Anthony M. and Rosenberger,
              Gerhard and Spellman, Dennis},
     TITLE = {{$n$}-free groups and questions about universally free groups},
 BOOKTITLE = {Groups '93 Galway/St.\ Andrews, Vol.\ 1 (Galway, 1993)},
    SERIES = {London Math. Soc. Lecture Note Ser.},
    VOLUME = {211},
     PAGES = {191--204},
 PUBLISHER = {Cambridge Univ. Press},
   ADDRESS = {Cambridge},
      YEAR = {1995},
   MRCLASS = {20E06 (20F32)},
  MRNUMBER = {96h:20052},
MRREVIEWER = {Gary L. Walls},
}

@article {ArzhantsevaOlshanskii96,
    AUTHOR = {Arzhantseva, G. N. and Ol{'s}hanski{\u\i}, A. Yu.},
     TITLE = {Generality of the class of groups in which subgroups with a
              lesser number of generators are free},
   JOURNAL = {Mat. Zametki},
  FJOURNAL = {Rossi\u\i skaya Akademiya Nauk. Matematicheskie Zametki},
    VOLUME = {59},
      YEAR = {1996},
    NUMBER = {4},
     PAGES = {489--496, 638},
      ISSN = {0025-567X},
   MRCLASS = {20F05 (05C25 20F06)},
  MRNUMBER = {98k:20040},
MRREVIEWER = {David I. Moldavanski{\u\i}},
}


@article {Bumagin2001,
    AUTHOR = {Bumagin, Inna},
     TITLE = {On small cancellation {$k$}-generated groups with
              {$(k-1)$}-generated subgroups all free},
   JOURNAL = {Internat. J. Algebra Comput.},
  FJOURNAL = {International Journal of Algebra and Computation},
    VOLUME = {11},
      YEAR = {2001},
    NUMBER = {5},
     PAGES = {507--524},
      ISSN = {0218-1967},
   MRCLASS = {20F06 (05C25)},
  MRNUMBER = {1 869 228},
}


@article {BaumslagShalen89,
    AUTHOR = {Baumslag, Gilbert and Shalen, Peter B.},
     TITLE = {Groups whose three-generator subgroups are free},
   JOURNAL = {Bull. Austral. Math. Soc.},
  FJOURNAL = {Bulletin of the Australian Mathematical Society},
    VOLUME = {40},
      YEAR = {1989},
    NUMBER = {2},
     PAGES = {163--174},
      ISSN = {0004-9727},
     CODEN = {ALNBAB},
   MRCLASS = {20F05 (20E06)},
  MRNUMBER = {90h:20041},
MRREVIEWER = {Maziar Shirvani},
}


@article {FischerKarrassSolitar72,
    AUTHOR = {Fischer, J. and Karrass, A. and Solitar, D.},
     TITLE = {On one-relator groups having elements of finite order},
   JOURNAL = {Proc. Amer. Math. Soc.},
    VOLUME = {33},
      YEAR = {1972},
     PAGES = {297--301},
   MRCLASS = {20F05},
  MRNUMBER = {47 \#342},
MRREVIEWER = {C. F. Miller, III},
}


@article {WiseRFTorsion,
    AUTHOR = {Wise, Daniel T.},
     TITLE = {Residual finiteness of quasi-positive one-relator groups},
   JOURNAL = {J. London Math. Soc. (2)},
  FJOURNAL = {Journal of the London Mathematical Society. Second Series},
    VOLUME = {66},
      YEAR = {2002},
    NUMBER = {2},
     PAGES = {334--350},
      ISSN = {0024-6107},
     CODEN = {JLMSAK},
   MRCLASS = {20E26 (20F05)},
  MRNUMBER = {1 920 406},
}




@article {BurnsHale72,
    AUTHOR = {Burns, R. G. and Hale, V. W. D.},
     TITLE = {A note on group rings of certain torsion-free groups},
   JOURNAL = {Canad. Math. Bull.},
    VOLUME = {15},
      YEAR = {1972},
     PAGES = {441--445},
   MRCLASS = {20C05},
  MRNUMBER = {46 \#9149},
MRREVIEWER = {Donald S. Passman},
}


@article {MR83e:20066,
    AUTHOR = {Sarkisyan, O. A.},
     TITLE = {Word and divisibility problems in semigroups and groups
              without cycles},
   JOURNAL = {Izv. Akad. Nauk SSSR Ser. Mat.},
  FJOURNAL = {Izvestiya Akademii Nauk SSSR. Seriya Matematicheskaya},
    VOLUME = {45},
      YEAR = {1981},
    NUMBER = {6},
     PAGES = {1424--1440},
      ISSN = {0373-2436},
   MRCLASS = {20M05 (03B25 03D40 20F05 20F10)},
  MRNUMBER = {83e:20066},
MRREVIEWER = {O. V. Belegradek},
}


@book {MR36:1520,
    AUTHOR = {Adjan, S. I.},
     TITLE = {Defining relations and algorithmic problems for groups and
              semigroups},
    SERIES = {Proceedings of the Steklov Institute of Mathematics, No. 85
              (1966). Translated from the Russian by M. Greendlinger},
 PUBLISHER = {American Mathematical Society},
   ADDRESS = {Providence, R.I.},
      YEAR = {1966},
     PAGES = {iii+152},
   MRCLASS = {20.10},
  MRNUMBER = {36 \#1520},
}



@article {Truffault74,
    AUTHOR = {Truffault, Bernard},
     TITLE = {Centralisateurs des \'el\'ements dans les groupes de
              {G}reendlinger},
   JOURNAL = {C. R. Acad. Sci. Paris. S\'er. A},
    VOLUME = {279},
      YEAR = {1974},
     PAGES = {317--319},
   MRCLASS = {20F05},
  MRNUMBER = {52 \#5813},
MRREVIEWER = {Leo P. Comerford},
}


@PHDTHESIS {Seymour74,
 author = {J.~E.~Seymour},
 title = {Conjugate powers and unique roots in certain small cancellation groups},
 school = {University of Illinois},
 year = {1974},
}



@article {Greendlinger62,
    AUTHOR = {Greendlinger, Martin},
     TITLE = {A class of groups all of whose elements have trivial
              centralizers},
   JOURNAL = {Math. Z.},
    VOLUME = {78},
      YEAR = {1962},
     PAGES = {91--96},
   MRCLASS = {20.10},
  MRNUMBER = {25 \#1200},
MRREVIEWER = {K. A. Hirsch},
}


@article {Lipschutz62,
    AUTHOR = {Lipschutz, Seymour},
     TITLE = {On powers of elements in {$S$}-groups},
   JOURNAL = {Proc. Amer. Math. Soc.},
    VOLUME = {13},
      YEAR = {1962},
     PAGES = {181--186},
   MRCLASS = {20.10},
  MRNUMBER = {26 \#3760},
MRREVIEWER = {M. Greendlinger},
}


@article {DugasGobel93,
    AUTHOR = {Dugas, Manfred and G{\"o}bel, R{\"u}diger},
     TITLE = {On locally finite {$p$}-groups and a problem of {P}hilip
              {H}all's},
   JOURNAL = {J. Algebra},
  FJOURNAL = {Journal of Algebra},
    VOLUME = {159},
      YEAR = {1993},
    NUMBER = {1},
     PAGES = {115--138},
      ISSN = {0021-8693},
     CODEN = {JALGA4},
   MRCLASS = {20F50 (20F28)},
  MRNUMBER = {94g:20054},
MRREVIEWER = {Zhi Rang Zhang},
}



@article {GobelParas2000,
    AUTHOR = {G{\"o}bel, R{\"u}diger and Paras, Agnes T.},
     TITLE = {Outer automorphism groups of metabelian groups},
   JOURNAL = {J. Pure Appl. Algebra},
  FJOURNAL = {Journal of Pure and Applied Algebra},
    VOLUME = {149},
      YEAR = {2000},
    NUMBER = {3},
     PAGES = {251--266},
      ISSN = {0022-4049},
     CODEN = {JPAAA2},
   MRCLASS = {20F29 (20K20)},
  MRNUMBER = {2001d:20034},
MRREVIEWER = {Andreas Caranti},
}



@article {Kojima88,
    AUTHOR = {Kojima, Sadayoshi},
     TITLE = {Isometry transformations of hyperbolic {$3$}-manifolds},
   JOURNAL = {Topology Appl.},
  FJOURNAL = {Topology and its Applications},
    VOLUME = {29},
      YEAR = {1988},
    NUMBER = {3},
     PAGES = {297--307},
      ISSN = {0166-8641},
     CODEN = {TIAPD9},
   MRCLASS = {57S17 (22E40 57M99 57S30)},
  MRNUMBER = {90c:57033},
MRREVIEWER = {Andrey V. Tetenov},
}


@article {Matumoto89,
    AUTHOR = {Matumoto, Takao},
     TITLE = {Any group is represented by an outerautomorphism group},
   JOURNAL = {Hiroshima Math. J.},
  FJOURNAL = {Hiroshima Mathematical Journal},
    VOLUME = {19},
      YEAR = {1989},
    NUMBER = {1},
     PAGES = {209--219},
      ISSN = {0018-2079},
     CODEN = {HMTJAD},
   MRCLASS = {20F28 (20E06)},
  MRNUMBER = {90g:20051},
MRREVIEWER = {Stephen J. Pride},
}



@article {DrosteGiraudetGobel2001,
    AUTHOR = {Droste, Manfred and Giraudet, Mich{\`e}le and G{\"o}bel,
              R{\"u}diger},
     TITLE = {All groups are outer automorphism groups of simple groups},
   JOURNAL = {J. London Math. Soc. (2)},
  FJOURNAL = {Journal of the London Mathematical Society. Second Series},
    VOLUME = {64},
      YEAR = {2001},
    NUMBER = {3},
     PAGES = {565--575},
      ISSN = {0024-6107},
     CODEN = {JLMSAK},
   MRCLASS = {20F28 (20F29)},
  MRNUMBER = {2002h:20050},
MRREVIEWER = {Martyn R. Dixon},
}




@article {GerstenhaberRothaus62,
    AUTHOR = {Gerstenhaber, Murray and Rothaus, Oscar S.},
     TITLE = {The solution of sets of equations in groups},
   JOURNAL = {Proc. Nat. Acad. Sci. U.S.A.},
    VOLUME = {48},
      YEAR = {1962},
     PAGES = {1531--1533},
   MRCLASS = {22.50},
  MRNUMBER = {29 \#3573},
MRREVIEWER = {Hanna Neumann},
}


@article {Baumslag60,
    AUTHOR = {Baumslag, Gilbert},
     TITLE = {Wreath products and finitely presented groups},
   JOURNAL = {Math. Z.},
    VOLUME = {75},
      YEAR = {1960/1961},
     PAGES = {22--28},
   MRCLASS = {20.00},
  MRNUMBER = {22 \#11026},
MRREVIEWER = {B. H. Neumann},
}



@article {Gersten83,
    AUTHOR = {Gersten, S. M.},
     TITLE = {Conservative groups, indicability, and a conjecture of
              {H}owie},
   JOURNAL = {J. Pure Appl. Algebra},
  FJOURNAL = {Journal of Pure and Applied Algebra},
    VOLUME = {29},
      YEAR = {1983},
    NUMBER = {1},
     PAGES = {59--74},
      ISSN = {0022-4049},
     CODEN = {JPAAA},
   MRCLASS = {20E25 (57M05)},
  MRNUMBER = {84m:20035},
MRREVIEWER = {James Howie},
}




@article {Krstic85,
    AUTHOR = {Krsti{\'c}, Sava},
     TITLE = {Systems of equations over locally {$p$}-indicable groups},
   JOURNAL = {Invent. Math.},
  FJOURNAL = {Inventiones Mathematicae},
    VOLUME = {81},
      YEAR = {1985},
    NUMBER = {2},
     PAGES = {373--378},
      ISSN = {0020-9910},
     CODEN = {INVMBH},
   MRCLASS = {20F05 (20F99)},
  MRNUMBER = {87a:20033},
MRREVIEWER = {F. Levin},
}




@article {FennRourke96,
    AUTHOR = {Fenn, Roger and Rourke, Colin},
     TITLE = {Klyachko's methods and the solution of equations over
              torsion-free groups},
   JOURNAL = {Enseign. Math. (2)},
  FJOURNAL = {L'Enseignement Math\'ematique. Revue Internationale. IIe
              S\'erie},
    VOLUME = {42},
      YEAR = {1996},
    NUMBER = {1-2},
     PAGES = {49--74},
      ISSN = {0013-8584},
     CODEN = {ENMAAR},
   MRCLASS = {20E06},
  MRNUMBER = {97k:20044},
MRREVIEWER = {Martin Edjvet},
}


@article {CliffordGoldstein95,
    AUTHOR = {Clifford, A. and Goldstein, R. Z.},
     TITLE = {Tesselations of {$S\sp 2$} and equations over torsion-free
              groups},
   JOURNAL = {Proc. Edinburgh Math. Soc. (2)},
  FJOURNAL = {Proceedings of the Edinburgh Mathematical Society. Series II},
    VOLUME = {38},
      YEAR = {1995},
    NUMBER = {3},
     PAGES = {485--493},
      ISSN = {0013-0915},
     CODEN = {PRMSA3},
   MRCLASS = {20E99 (57M07)},
  MRNUMBER = {97b:20042},
MRREVIEWER = {Martin Edjvet},
}




@article {Klyachko93,
    AUTHOR = {Klyachko, Anton A.},
     TITLE = {A funny property of sphere and equations over groups},
   JOURNAL = {Comm. Algebra},
  FJOURNAL = {Communications in Algebra},
    VOLUME = {21},
      YEAR = {1993},
    NUMBER = {7},
     PAGES = {2555--2575},
      ISSN = {0092-7872},
     CODEN = {COALDM},
   MRCLASS = {20F32},
  MRNUMBER = {94c:20070},
MRREVIEWER = {Martin Edjvet},
}




@article {Howie2002,
    AUTHOR = {Howie, James},
     TITLE = {A proof of the {S}cott-{W}iegold conjecture on free products
              of cyclic groups},
   JOURNAL = {J. Pure Appl. Algebra},
  FJOURNAL = {Journal of Pure and Applied Algebra},
    VOLUME = {173},
      YEAR = {2002},
    NUMBER = {2},
     PAGES = {167--176},
      ISSN = {0022-4049},
     CODEN = {JPAAA2},
   MRCLASS = {20E06 (20Fxx)},
  MRNUMBER = {1 915 093},
}




@article {Boyer89,
    AUTHOR = {Boyer, Steven},
     TITLE = {On proper powers in free products and {D}ehn surgery},
   JOURNAL = {J. Pure Appl. Algebra},
  FJOURNAL = {Journal of Pure and Applied Algebra},
    VOLUME = {51},
      YEAR = {1988},
    NUMBER = {3},
     PAGES = {217--229},
      ISSN = {0022-4049},
     CODEN = {JPAAA2},
   MRCLASS = {57M25},
  MRNUMBER = {89m:57003},
MRREVIEWER = {Charles Livingston},
}


@article {Huebschmann81,
    AUTHOR = {Huebschmann, Johannes},
     TITLE = {Aspherical $2$-complexes and an unsettled problem of {J}. {H}.
              {C}. {W}hitehead},
   JOURNAL = {Math. Ann.},
  FJOURNAL = {Mathematische Annalen},
    VOLUME = {258},
      YEAR = {1981/82},
    NUMBER = {1},
     PAGES = {17--37},
      ISSN = {0025-5831},
     CODEN = {MAANA3},
   MRCLASS = {57M20 (20F05 57M05)},
  MRNUMBER = {83e:57004},
MRREVIEWER = {Ronald Brown},
}


@article{WiseSectional02,
    AUTHOR = {Wise, D. T.},
     TITLE = {Sectional curvature, compact cores, and local quasiconvexity},
   JOURNAL = {Geom. Funct. Anal.},
  FJOURNAL = {Geometric and Functional Analysis},
    VOLUME = {14},
      YEAR = {2004},
    NUMBER = {2},
     PAGES = {433--468},
      ISSN = {1016-443X},
     CODEN = {GFANFB},
   MRCLASS = {53C21 (57M20)},
  MRNUMBER = {2 062 762},
}


@MISC{WisePositiveRelatorCoherence02,
   author = {Wise, Daniel T.},
   title = {Positive one-relator groups are coherent},
   note = {pp. 1-19},
howpublished = {Available at \url{http://www.math.mcgill.ca/wise/papers}},
}



@article{WiseNonPositiveCoherence,
   author = {Wise, Daniel T.},
   title = {Coherence, Local-indicability, and Nonpositive Immersions},
   year=2018,
   note = {Submitted},
}

@MISC{WiseNonPositiveCoherence02old,
   author = {Wise, Daniel T.},
   title = {Coherence, Local-indicability, and Nonpositive Immersions},
   note = {Preprint},
howpublished = {Available at \url{http://www.math.mcgill.ca/wise/papers}},
}


@article {Brodskii84,
    AUTHOR = {Brodski{\u\i}, S. D.},
     TITLE = {Equations over groups, and groups with one defining relation},
   JOURNAL = {Sibirsk. Mat. Zh.},
  FJOURNAL = {Akademiya Nauk SSSR. Sibirskoe Otdelenie. Sibirski\u\i\
              Matematicheski\u\i\ Zhurnal},
    VOLUME = {25},
      YEAR = {1984},
    NUMBER = {2},
     PAGES = {84--103},
      ISSN = {0037-4474},
   MRCLASS = {20E06 (20E25)},
  MRNUMBER = {86e:20026},
MRREVIEWER = {James Howie},
}


@article {Brodskii80,
    AUTHOR = {Brodski{\u\i}, S. D.},
     TITLE = {Equations over groups and groups with one defining relation},
   JOURNAL = {Uspekhi Mat. Nauk},
  FJOURNAL = {Akademiya Nauk SSSR i Moskovskoe Matematicheskoe Obshchestvo.
              Uspekhi Matematicheskikh Nauk},
    VOLUME = {35},
      YEAR = {1980},
    NUMBER = {4(214)},
     PAGES = {183},
      ISSN = {0042-1316},
   MRCLASS = {20F05},
  MRNUMBER = {82a:20041},
MRREVIEWER = {F. Haimo},
}


@incollection {Paulin91,
    AUTHOR = {Paulin, Fr{\'e}d{\'e}ric},
     TITLE = {Constructions of hyperbolic groups via hyperbolizations of
              polyhedra},
 BOOKTITLE = {Group theory from a geometrical viewpoint (Trieste, 1990)},
     PAGES = {313--372},
 PUBLISHER = {World Sci. Publishing},
   ADDRESS = {River Edge, NJ},
      YEAR = {1991},
   MRCLASS = {57M07 (20F32)},
  MRNUMBER = {93d:57005},
}



@article {EpsteinPenner88,
    AUTHOR = {Epstein, D. B. A. and Penner, R. C.},
     TITLE = {Euclidean decompositions of noncompact hyperbolic manifolds},
   JOURNAL = {J. Differential Geom.},
  FJOURNAL = {Journal of Differential Geometry},
    VOLUME = {27},
      YEAR = {1988},
    NUMBER = {1},
     PAGES = {67--80},
      ISSN = {0022-040X},
     CODEN = {JDGEAS},
   MRCLASS = {57N15 (20H10 22E40 51M10)},
  MRNUMBER = {89a:57020},
MRREVIEWER = {N. V. Ivanov},
}


@incollection {Stallings87,
    AUTHOR = {Stallings, John R.},
     TITLE = {Adian groups and pregroups},
 BOOKTITLE = {Essays in group theory},
     PAGES = {321--342},
 PUBLISHER = {Springer},
   ADDRESS = {New York},
      YEAR = {1987},
   MRCLASS = {20F06},
  MRNUMBER = {88m:20075},
MRREVIEWER = {Roger C. Alperin},
}




@preamble{
   "\def\polhk#1{\setbox0=\hbox{#1}{\ooalign{\hidewidth
    \lower1.5ex\hbox{`}\hidewidth\crcr\unhbox0}}} "
}
@article {BallmannSwiatkowski97,
    AUTHOR = {Ballmann, W. and {\'S}wi{\polhk{a}}tkowski, J.},
     TITLE = {On ${L}\sp 2$-cohomology and property ({T}) for automorphism
              groups of polyhedral cell complexes},
   JOURNAL = {Geom. Funct. Anal.},
  FJOURNAL = {Geometric and Functional Analysis},
    VOLUME = {7},
      YEAR = {1997},
    NUMBER = {4},
     PAGES = {615--645},
      ISSN = {1016-443X},
     CODEN = {GFANFB},
   MRCLASS = {20F32 (20J05 22D10 53C23 57M07)},
  MRNUMBER = {98m:20043},
MRREVIEWER = {Alain Valette},
}


@article {Shalom2000,
    AUTHOR = {Shalom, Yehuda},
     TITLE = {Rigidity of commensurators and irreducible lattices},
   JOURNAL = {Invent. Math.},
  FJOURNAL = {Inventiones Mathematicae},
    VOLUME = {141},
      YEAR = {2000},
    NUMBER = {1},
     PAGES = {1--54},
      ISSN = {0020-9910},
     CODEN = {INVMBH},
   MRCLASS = {22E40 (20E08 20F65 20G10)},
  MRNUMBER = {2001k:22022},
MRREVIEWER = {Alain Valette},
}


@article {Greendlinger60,
    AUTHOR = {Greendlinger, Martin},
     TITLE = {On {D}ehn's algorithms for the conjugacy and word problems,
              with applications},
   JOURNAL = {Comm. Pure Appl. Math.},
    VOLUME = {13},
      YEAR = {1960},
     PAGES = {641--677},
   MRCLASS = {02.54},
  MRNUMBER = {23 \#A2327},
MRREVIEWER = {R. C. Lyndon},
}


@article {Greendlinger66,
    AUTHOR = {Grindlinger, M.},
     TITLE = {The problem of conjugacy and coincidence with an anticenter in
              the theory of groups},
   JOURNAL = {Sibirsk. Mat. \u Z.},
    VOLUME = {7},
      YEAR = {1966},
     PAGES = {785--803},
   MRCLASS = {20.10},
  MRNUMBER = {33 \#7406},
MRREVIEWER = {P. M. Cohn},
}



@article {vanKampen33,
   AUTHOR = {van Kampen, E. R.},
    TITLE = {On some lemmas in the theory of groups},
  JOURNAL = {Amer. J. Math.},
   VOLUME = {55},
     YEAR = {1933},
    PAGES = {268--273},
}

@article {Howie82,
    AUTHOR = {Howie, James},
     TITLE = {On locally indicable groups},
   JOURNAL = {Math. Z.},
  FJOURNAL = {Mathematische Zeitschrift},
    VOLUME = {180},
      YEAR = {1982},
    NUMBER = {4},
     PAGES = {445--461},
      ISSN = {0025-5874},
     CODEN = {MAZEAX},
   MRCLASS = {20F05 (57M20)},
  MRNUMBER = {84b:20036},
MRREVIEWER = {Johannes Huebschmann},
}


@article {CorsonTrace2000,
    AUTHOR = {Corson, J. M. and Trace, B.},
     TITLE = {Diagrammatically reducible complexes and {H}aken manifolds},
   JOURNAL = {J. Austral. Math. Soc. Ser. A},
  FJOURNAL = {Australian Mathematical Society. Journal. Series A. Pure
              Mathematics and Statistics},
    VOLUME = {69},
      YEAR = {2000},
    NUMBER = {1},
     PAGES = {116--126},
      ISSN = {0263-6115},
     CODEN = {JAMADS},
   MRCLASS = {57M20 (57M50 57N10)},
  MRNUMBER = {2001f:57005},
MRREVIEWER = {Charles Livingston},
}

@article {WiseStaggeredCoherence,
    AUTHOR = {Wise, Daniel T.},
     TITLE = {Positive one-relator groups are coherent},
NOTE={Preprint 2002},
}

@article {Dicks94,
    AUTHOR = {Dicks, Warren},
     TITLE = {Equivalence of the strengthened {H}anna {N}eumann conjecture
              and the amalgamated graph conjecture},
   JOURNAL = {Invent. Math.},
  FJOURNAL = {Inventiones Mathematicae},
    VOLUME = {117},
      YEAR = {1994},
    NUMBER = {3},
     PAGES = {373--389},
      ISSN = {0020-9910},
     CODEN = {INVMBH},
   MRCLASS = {20E07 (05C25 20E05)},
  MRNUMBER = {95c:20034},
MRREVIEWER = {Dimitrios Varsos},
}


@incollection {Gerasimov97,
    AUTHOR = {Gerasimov, V. N.},
     TITLE = {Semi-splittings of groups and actions on cubings},
 BOOKTITLE = {Algebra, geometry, analysis and mathematical physics (Russian)
              (Novosibirsk, 1996)},
     PAGES = {91--109, 190},
 PUBLISHER = {Izdat. Ross. Akad. Nauk Sib. Otd. Inst. Mat., Novosibirsk},
      YEAR = {1997},
   MRCLASS = {20F32 (57M07)},
  MRNUMBER = {99c:20049},
MRREVIEWER = {Igor Belegradek},
}

@article {Scott77,
    AUTHOR = {Scott, Peter},
     TITLE = {Ends of pairs of groups},
   JOURNAL = {J. Pure Appl. Algebra},
  FJOURNAL = {Journal of Pure and Applied Algebra},
    VOLUME = {11},
      YEAR = {1977/78},
    NUMBER = {1-3},
     PAGES = {179--198},
      ISSN = {0022-4049},
   MRCLASS = {20F99},
  MRNUMBER = {81h:20047},
MRREVIEWER = {Ross Geoghegan},
}


@article {WiseQuasiPositive,
    AUTHOR = {Wise, Daniel T.},
     TITLE = {The residual finiteness of qausi-positive one-relator groups},
   JOURNAL = {Jour. London Math. Soc. (3)},
  FJOURNAL = {Journal of the London Mathematical Society. Third Series},
NOTE={to appear},
}

   JOURNAL = {Comment. Math. Helv.},
  FJOURNAL = {Commentarii Mathematici Helvetici},
    VOLUME = {76},
      YEAR = {2001},
    NUMBER = {2},
     PAGES = {314--338},
      ISSN = {0010-2571},
     CODEN = {COMHAX},
   MRCLASS = {20Exx (20Fxx)},
  MRNUMBER = {1 839 349},
}


@article {NibloReeves97,
    AUTHOR = {Niblo, Graham and Reeves, Lawrence},
     TITLE = {Groups acting on ${{\rm CAT}(0)}$ cube complexes},
   JOURNAL = {Geom. Topol.},
  FJOURNAL = {Geometry and Topology},
    VOLUME = {1},
      YEAR = {1997},
     PAGES = {approx.\ 7 pp.\ (electronic)},
      ISSN = {1465-3060},
   MRCLASS = {57M07 (20F32)},
  MRNUMBER = {98d:57005},
MRREVIEWER = {Philip L. Bowers},
}



@article {Sageev97,
    AUTHOR = {Sageev, Michah},
     TITLE = {Codimension-$1$ subgroups and splittings of groups},
   JOURNAL = {J. Algebra},
  FJOURNAL = {Journal of Algebra},
    VOLUME = {189},
      YEAR = {1997},
    NUMBER = {2},
     PAGES = {377--389},
      ISSN = {0021-8693},
     CODEN = {JALGA4},
   MRCLASS = {20F32 (57M07)},
  MRNUMBER = {98c:20071},
MRREVIEWER = {G. Peter Scott},
}


@article {Houghton74,
    AUTHOR = {Houghton, C. H.},
     TITLE = {Ends of locally compact groups and their coset spaces},
      NOTE = {Collection of articles dedicated to the memory of Hanna
              Neumann, VII},
   JOURNAL = {J. Austral. Math. Soc.},
    VOLUME = {17},
      YEAR = {1974},
     PAGES = {274--284},
   MRCLASS = {22D05},
  MRNUMBER = {50 \#10147},
MRREVIEWER = {Herbert Abels},
}



@article {Sageev95,
    AUTHOR = {Sageev, Michah},
     TITLE = {Ends of group pairs and non-positively curved cube complexes},
   JOURNAL = {Proc. London Math. Soc. (3)},
  FJOURNAL = {Proceedings of the London Mathematical Society. Third Series},
    VOLUME = {71},
      YEAR = {1995},
    NUMBER = {3},
     PAGES = {585--617},
      ISSN = {0024-6115},
     CODEN = {PLMTAL},
   MRCLASS = {20F32 (20E08)},
  MRNUMBER = {97a:20062},
MRREVIEWER = {G. Peter Scott},
}



@article {Pride83,
    AUTHOR = {Pride, Stephen J.},
     TITLE = {Some finitely presented groups of cohomological dimension two
              with property ({F}{A})},
   JOURNAL = {J. Pure Appl. Algebra},
  FJOURNAL = {Journal of Pure and Applied Algebra},
    VOLUME = {29},
      YEAR = {1983},
    NUMBER = {2},
     PAGES = {167--168},
      ISSN = {0022-4049},
     CODEN = {JPAAA2},
   MRCLASS = {20J05},
  MRNUMBER = {85c:20042},
MRREVIEWER = {Johannes Huebschmann},
}




@article {Stallings63,
    AUTHOR = {Stallings, John},
     TITLE = {A finitely presented group whose 3-dimensional integral
              homology is not finitely generated},
   JOURNAL = {Amer. J. Math.},
    VOLUME = {85},
      YEAR = {1963},
     PAGES = {541--543},
   MRCLASS = {18.20},
  MRNUMBER = {28 \#2139},
MRREVIEWER = {J. F. Adams},
}


@article {Hall59,
    AUTHOR = {Hall, P.},
     TITLE = {On the finiteness of cetain soluble groups},
   JOURNAL = {Proc. London Math. Soc. (3)},
    VOLUME = {9},
      YEAR = {1959},
     PAGES = {595--622},
   MRCLASS = {20.00},
  MRNUMBER = {22 \#1618},
MRREVIEWER = {K. Gruenberg},
}


@book {MillerStudy71,
   AUTHOR = {Miller, III, Charles F.},
    TITLE = {On group-theoretic decision problems and their classification},
     NOTE = {Annals of Mathematics Studies, No. 68},
PUBLISHER = {Princeton University Press},
  ADDRESS = {Princeton, N.J.},
     YEAR = {1971},
    PAGES = {viii+106},
}


@article {DiaconisGraham99,
    AUTHOR = {Diaconis, Persi and Graham, Ronald},
     TITLE = {The graph of generating sets of an abelian group},
   JOURNAL = {Colloq. Math.},
  FJOURNAL = {Colloquium Mathematicum},
    VOLUME = {80},
      YEAR = {1999},
    NUMBER = {1},
     PAGES = {31--38},
      ISSN = {0010-1354},
     CODEN = {CQMAAQ},
   MRCLASS = {20P05 (20F65 20K01 60C05)},
  MRNUMBER = {2000f:20124},
MRREVIEWER = {Sarah E. Rees},
}



@article {HruskaWise-Torsion,
    AUTHOR = {Hruska, G. Christopher and Wise, Daniel T.},
     TITLE = {Towers, ladders and the {B}. {B}. {N}ewman spelling theorem},
   JOURNAL = {J. Aust. Math. Soc.},
  FJOURNAL = {Journal of the Australian Mathematical Society},
    VOLUME = {71},
      YEAR = {2001},
    NUMBER = {1},
     PAGES = {53--69},
      ISSN = {0263-6115},
   MRCLASS = {20F06 (20F67 57M07)},
  MRNUMBER = {1 840 493},
}

@article {WisePositive,
    AUTHOR = {Wise, Daniel T.},
     TITLE = {The residual finiteness of positive one-relator groups},
   JOURNAL = {Comment. Math. Helv.},
  FJOURNAL = {Commentarii Mathematici Helvetici},
    VOLUME = {76},
      YEAR = {2001},
    NUMBER = {2},
     PAGES = {314--338},
      ISSN = {0010-2571},
     CODEN = {COMHAX},
   MRCLASS = {20Exx (20Fxx)},
  MRNUMBER = {1 839 349},
}
@article {KapovichWisecoHopf,
AUTHOR = {Kapovich, Ilya and Wise, Daniel T.},
     TITLE = {On the failure of the co-{H}opf property for subgroups of
              word-hyperbolic groups},
   JOURNAL = {Israel J. Math.},
  FJOURNAL = {Israel Journal of Mathematics},
    VOLUME = {122},
      YEAR = {2001},
     PAGES = {125--147},
      ISSN = {0021-2172},
     CODEN = {ISJMAP},
   MRCLASS = {20Fxx (57M07)},
  MRNUMBER = {1 826 495},
}



@unpublished{Sapir98lecture,
Author={Mark Sapir},
Title={Residually finite hyperbolic groups and dynamics of polynomial maps over {$Z_p$}},
Note={Lecture in:
International Conference on Non-Positive Curvature in Group Theory,
Topology, and Geometry, May 1998,
Vanderbilt University}
}

 @Book{BaumslagNilpotent71,
  author =       {Baumslag, Gilbert},
  title =        {Lecture notes on nilpotent groups},
  publisher =    {American Mathematical Society},
  year =         1971,
  number =       2,
  series =       {CBMS Regional Conference Series in Mathematics},
  address =      {Providence, RI}
}


@article {Groves80,
    AUTHOR = {Groves, J. R. J.},
     TITLE = {Soluble groups in which every finitely generated subgroup is
              finitely presented},
   JOURNAL = {J. Austral. Math. Soc. Ser. A},
  FJOURNAL = {Australian Mathematical Society. Journal. Series A},
    VOLUME = {26},
      YEAR = {1978},
    NUMBER = {1},
     PAGES = {115--125},
      ISSN = {0263-6115},
     CODEN = {JAMADS},
   MRCLASS = {20F05},
  MRNUMBER = {80a:20037},
MRREVIEWER = {E. F. Robertson},
}

@article {NibloWiseGraphmanifolds,
    AUTHOR = {Niblo, Graham A. and Wise, Daniel T.},
     TITLE = {Subgroup separability, knot groups and graph manifolds},
   JOURNAL = {Proc. Amer. Math. Soc.},
  FJOURNAL = {Proceedings of the American Mathematical Society},
    VOLUME = {129},
      YEAR = {2001},
    NUMBER = {3},
     PAGES = {685--693},
      ISSN = {0002-9939},
     CODEN = {PAMYAR},
   MRCLASS = {20F34 (20E26 57M05 57M25)},
  MRNUMBER = {1 707 529},
}


@article {Jones1974,
    AUTHOR = {Jones, J. M. Tyrer},
     TITLE = {Direct products and the {H}opf property},
      NOTE = {Collection of articles dedicated to the memory of Hanna
              Neumann, VI},
   JOURNAL = {J. Austral. Math. Soc.},
    VOLUME = {17},
      YEAR = {1974},
     PAGES = {174--196},
  MRCLASS = {20F25},
  MRNUMBER = {50 \#2348},
MRREVIEWER = {J. Wiegold},
}


@article {Pride76,
    AUTHOR = {Pride, Stephen J.},
     TITLE = {On the {H}opficity and related properties of small
              cancellation groups},
   JOURNAL = {J. London Math. Soc. (2)},
    VOLUME = {14},
      YEAR = {1976},
    NUMBER = {2},
     PAGES = {269--276},
   MRCLASS = {20F05},
  MRNUMBER = {55 \#10570},
MRREVIEWER = {A. M. Brunner},
}

@article {WiegoldWilson78,
    AUTHOR = {Wiegold, James and Wilson, John S.},
     TITLE = {Growth sequences of finitely generated groups},
   JOURNAL = {Arch. Math. (Basel)},
  FJOURNAL = {Archiv der Mathematik. Archives of Mathematics. Archives
              Math\'ematiques},
    VOLUME = {30},
      YEAR = {1978},
    NUMBER = {4},
     PAGES = {337--343},
      ISSN = {0003-889X},
     CODEN = {ACVMAL},
   MRCLASS = {20F05},
  MRNUMBER = {80k:20038},
MRREVIEWER = {Benjamin Fine},
}


@article {Erfanian95,
    AUTHOR = {Erfanian, A.},
     TITLE = {A problem on growth sequences of groups},
   JOURNAL = {J. Austral. Math. Soc. Ser. A},
  FJOURNAL = {Australian Mathematical Society. Journal. Series A. Pure
              Mathematics and Statistics},
    VOLUME = {59},
      YEAR = {1995},
    NUMBER = {2},
     PAGES = {283--286},
      ISSN = {0263-6115},
     CODEN = {JAMADS},
   MRCLASS = {20D60},
  MRNUMBER = {96f:20032},
MRREVIEWER = {J. Wiegold},
}


@article {Wiegold78,
    AUTHOR = {Wiegold, James},
     TITLE = {Growth sequences of finite groups. {I}{I}{I}},
   JOURNAL = {J. Austral. Math. Soc. Ser. A},
  FJOURNAL = {Australian Mathematical Society. Journal. Series A},
    VOLUME = {25},
      YEAR = {1978},
    NUMBER = {2},
     PAGES = {142--144},
      ISSN = {0263-6115},
     CODEN = {JAMADS},
   MRCLASS = {20D30},
  MRNUMBER = {80c:20028},
MRREVIEWER = {F. Levin},
}

@article {Hall36,
   AUTHOR = {Hall, Phillip},
    TITLE = {The Eulerian Function of a Group},
    JOURNAL = {Quart. J. Math., Oxford Ser.},
 FJOURNAL = {The Quarterly Journal of Mathematics. Oxford. Second Series},
   VOLUME = {7},
     YEAR = {1936},
   NUMBER = {133},
    PAGES = {97--106},
}


@book {BaumslagBook93,
   AUTHOR = {Baumslag, Gilbert},
    TITLE = {Topics in combinatorial group theory},
PUBLISHER = {Birkh\"auser Verlag},
  ADDRESS = {Basel},
     YEAR = {1993},
    PAGES = {viii+164},
     ISBN = {3-7643-2921-1},
}



@book {Adian79,
   AUTHOR = {Adian, S. I.},
    TITLE = {The {B}urnside problem and identities in groups},
     NOTE = {Translated from the Russian by John Lennox and James Wiegold},
PUBLISHER = {Springer-Verlag},
  ADDRESS = {Berlin},
     YEAR = {1979},
    PAGES = {xi+311},
     ISBN = {3-540-08728-1},
}

@book {BieriBook81,
   AUTHOR = {Bieri, Robert},
    TITLE = {Homological dimension of discrete groups},
  EDITION = {Second},
PUBLISHER = {Queen Mary College Department of Pure Mathematics},
  ADDRESS = {London},
     YEAR = {1981},
    PAGES = {iv+198},
}

@article {BaumslagBooneNeumann59,
   AUTHOR = {Baumslag, Gilbert and Boone, W. W. and Neumann, B. H.},
    TITLE = {Some unsolvable problems about elements and subgroups of
             groups},
  JOURNAL = {Math. Scand.},
   VOLUME = {7},
     YEAR = {1959},
    PAGES = {191--201},
}

@article {Bergman68,
   AUTHOR = {Bergman, George M.},
    TITLE = {On groups acting on locally finite graphs},
  JOURNAL = {Ann. of Math. (2)},
   VOLUME = {88},
     YEAR = {1968},
    PAGES = {335--340},
}



@article {Fischer77,
   AUTHOR = {Fischer, Jerrold},
    TITLE = {Torsion-free subgroups of finite index in one-relator groups},
  JOURNAL = {Comm. Algebra},
   VOLUME = {5},
     YEAR = {1977},
   NUMBER = {11},
    PAGES = {1211--1222},
}

@book {Kourovka95,
    TITLE = {Unsolved problems in group theory. {T}he {K}ourovka notebook},
  EDITION = {augmented},
   EDITOR = {Mazurov, V. D. and Khukhro, E. I.},
PUBLISHER = {Russian Academy of Sciences Siberian Division Institute of
             Mathematics},
  ADDRESS = {Novosibirsk},
     YEAR = {1995},
    PAGES = {120},
}

@book {StallingsMonograph71,
   AUTHOR = {Stallings, John},
    TITLE = {Group theory and three-dimensional manifolds},
     NOTE = {A James K. Whittemore Lecture in Mathematics given at Yale
             University, 1969,
             Yale Mathematical Monographs, 4},
PUBLISHER = {Yale University Press},
  ADDRESS = {New Haven, Conn.},
     YEAR = {1971},
    PAGES = {v+65},
}



@article {Stallings68,
   AUTHOR = {Stallings, John R.},
    TITLE = {On torsion-free groups with infinitely many ends},
  JOURNAL = {Ann. of Math. (2)},
   VOLUME = {88},
     YEAR = {1968},
    PAGES = {312--334},
}



@incollection {Stallings70,
   AUTHOR = {Stallings, John},
    TITLE = {Groups of cohomological dimension one},
BOOKTITLE = {Applications of Categorical Algebra (Proc. Sympos. Pure Math.,
             Vol. XVIII, New York, 1968)},
    PAGES = {124--128},
PUBLISHER = {Amer. Math. Soc.},
  ADDRESS = {Providence, R.I.},
     YEAR = {1970},
}



@article {BrownGeoghegan85,
   AUTHOR = {Brown, Kenneth S. and Geoghegan, Ross},
    TITLE = {Cohomology with free coefficients of the fundamental group of a
             graph of groups},
  JOURNAL = {Comment. Math. Helv.},
 FJOURNAL = {Commentarii Mathematici Helvetici},
   VOLUME = {60},
     YEAR = {1985},
   NUMBER = {1},
    PAGES = {31--45},
     ISSN = {0010-2571},
    CODEN = {COMHAX},
}


@book {Ronan89,
   AUTHOR = {Ronan, Mark},
    TITLE = {Lectures on buildings},
PUBLISHER = {Academic Press Inc.},
  ADDRESS = {Boston, MA},
     YEAR = {1989},
    PAGES = {xiv+201},
     ISBN = {0-12-594750-X},
  MRCLASS = {20-02 (11E57 51-02 51B25 57M05)},
 MRNUMBER = {90j:20001},
   MRREVR = {Guy Rousseau},
}
@book {Brown89,
   AUTHOR = {Brown, Kenneth S.},
    TITLE = {Buildings},
PUBLISHER = {Springer-Verlag},
  ADDRESS = {New York},
     YEAR = {1989},
    PAGES = {viii+215},
     ISBN = {0-387-96876-8},
  MRCLASS = {20-02 (20E32 20G15 22E99 51B25)},
 MRNUMBER = {90e:20001},
   MRREVR = {W. M. Kantor},
}


@book {BrownBook82and94,
   AUTHOR = {Brown, Kenneth S.},
    TITLE = {Cohomology of groups},
     NOTE = {Corrected reprint of the 1982 original},
PUBLISHER = {Springer-Verlag},
  ADDRESS = {New York},
     YEAR = {1994},
    PAGES = {x+306},
     ISBN = {0-387-90688-6},
}


@article {Mihalik85,
   AUTHOR = {Mihalik, Michael L.},
    TITLE = {Ends of groups with the integers as quotient},
  JOURNAL = {J. Pure Appl. Algebra},
 FJOURNAL = {Journal of Pure and Applied Algebra},
   VOLUME = {35},
     YEAR = {1985},
   NUMBER = {3},
    PAGES = {305--320},
     ISSN = {0022-4049},
    CODEN = {JPAAA2},
}

@MISC{MagnusProblemList,
   author = {New York Group Theory Cooperative at CCNY},
   title = {Open problems in combinatorial group theory},
   howpublished = {http://zebra.sci.ccny.cuny.edu/web/html/magnushome.html},
   key = {Magnus},
}

@article {Magnus69,
    AUTHOR = {Magnus, W.},
     TITLE = {Residually finite groups},
   JOURNAL = {Bull. Amer. Math. Soc.},
    VOLUME = {75},
      YEAR = {1969},
     PAGES = {305--316},
   MRCLASS = {},
  MRNUMBER = {39 \#2865},
MRREVIEWER = {R. H. Fox},
}




@ARTICLE{AitchisonMatsumotoRubinstein97,
   author = {Aitchison, I. R. and Matsumoto, S. and Rubinstein, J. H.},
   title = {Immersed surfaces in cubed manifolds},
   journal = {Asian J. Math.},
   year = {1997},
   volume = {1},
   number = {1},
   pages = {85--95},
}



@book {GhysBook90,
     TITLE = {Sur les groupes hyperboliques d'apr\`es {M}ikhael {G}romov},
    SERIES = {Progress in Mathematics},
    VOLUME = {83},
    EDITOR = {Ghys, {\'E}. and de la Harpe, P.},
      NOTE = {Papers from the Swiss Seminar on Hyperbolic Groups held in
              Bern, 1988},
 PUBLISHER = {Birkh\"auser Boston Inc.},
   ADDRESS = {Boston, MA},
      YEAR = {1990},
     PAGES = {xii+285},
      ISBN = {0-8176-3508-4},
   MRCLASS = {53C23 (20F32 57M05 57S30)},
  MRNUMBER = {92f:53050},
MRREVIEWER = {Viktor Schroeder},
}


@article {Grossman74,
   AUTHOR = {Grossman, Edna K.},
    TITLE = {On the residual finiteness of certain mapping class groups},
  JOURNAL = {J. London Math. Soc. (2)},
   VOLUME = {9},
     YEAR = {1974/75},
    PAGES = {160--164},
}


@article{BurgerMozes99,
   AUTHOR = {Burger, Marc and Mozes, Shahar},
    TITLE = {Lattices in product of trees},
   JOURNAL = {Inst. Hautes \'Etudes Sci. Publ. Math.},
  FJOURNAL = {Institut des Hautes \'Etudes Scientifiques. Publications
              Math\'ematiques},
   Note = {To appear},
}

@article {BurgerMozes,
   AUTHOR = {Burger, Marc and Mozes, Shahar},
    TITLE = {Finitely presented simple groups and products of trees},
  JOURNAL = {C. R. Acad. Sci. Paris S\'er. I Math.},
 FJOURNAL = {Comptes Rendus de l'Acad\'emie des Sciences. S\'erie I.
             Math\'ematique},
   VOLUME = {324},
     YEAR = {1997},
   NUMBER = {7},
    PAGES = {747--752},
     ISSN = {0764-4442},
    CODEN = {CASMEI},
}

@ARTICLE{Baumslag67,
   author = {Baumslag, Gilbert},
   title = {Residually finite one-relator groups},
   journal = {Bull. Amer. Math. Soc.},
   year = {1967},
   volume = {73},
   pages = {618--620},
}



@incollection {Egorov81,
   AUTHOR = {Egorov, V.},
    TITLE = {The residual finiteness of certain one-relator groups},
BOOKTITLE = {Algebraic systems},
    PAGES = {100--121},
PUBLISHER = {Ivanov. Gos. Univ.},
  ADDRESS = {Ivanovo},
     YEAR = {1981},
}


@article{Moldavanskii92,
   AUTHOR = {Moldavanski{\u\i}, D. I.},
    TITLE = {Residual finiteness of descending {H}{N}{N}-extensions of
             groups},
  JOURNAL = {Ukra{\"\i}n. Mat. Zh.},
 FJOURNAL = {Akadem{\=\i}ya Nauk Ukra\"\i ni. \=Institut Matematiki. Ukra\"\i
             ns\cprime ki\u\i\ Matematichni\u\i\ Zhurnal},
   VOLUME = {44},
     YEAR = {1992},
   NUMBER = {6},
    PAGES = {842--845},
     ISSN = {0041-6053},
}


@article {BaumslagRoseblade84,
   AUTHOR = {Baumslag, Gilbert and Roseblade, James E.},
    TITLE = {Subgroups of direct products of free groups},
  JOURNAL = {J. London Math. Soc. (2)},
 FJOURNAL = {The Journal of the London Mathematical Society. Second Series},
   VOLUME = {30},
     YEAR = {1984},
   NUMBER = {1},
    PAGES = {44--52},
     ISSN = {0024-6107},
    CODEN = {JLMSAK},
}



@article {Hirshon77,
   AUTHOR = {Hirshon, Ronald},
    TITLE = {Some properties of endomorphisms in residually finite groups},
  JOURNAL = {J. Austral. Math. Soc. Ser. A},
   VOLUME = {24},
     YEAR = {1977},
   NUMBER = {1},
    PAGES = {117--120},
}


@article {Mosher95,
   AUTHOR = {Mosher, Lee},
    TITLE = {Geometry of cubulated $3$-manifolds},
  JOURNAL = {Topology},
 FJOURNAL = {Topology. An International Journal of Mathematics},
   VOLUME = {34},
     YEAR = {1995},
   NUMBER = {4},
    PAGES = {789--814},
     ISSN = {0040-9383},
    CODEN = {TPLGAF},
}

@article {BaumslagMiller88,
    AUTHOR = {Baumslag, Gilbert and Miller, III, Charles F.},
     TITLE = {Some odd finitely presented groups},
   JOURNAL = {Bull. London Math. Soc.},
  FJOURNAL = {The Bulletin of the London Mathematical Society},
    VOLUME = {20},
      YEAR = {1988},
    NUMBER = {3},
     PAGES = {239--244},
      ISSN = {0024-6093},
     CODEN = {LMSBBT},
   MRCLASS = {20F05 (20E06)},
  MRNUMBER = {89e:20059},
MRREVIEWER = {Leo P. Comerford, Jr.},
}



@article {BaumslagMillerShort94,
   AUTHOR = {Baumslag, G. and Miller, III, Charles F. and Short, H.},
    TITLE = {Unsolvable problems about small cancellation and word
             hyperbolic groups},
  JOURNAL = {Bull. London Math. Soc.},
 FJOURNAL = {The Bulletin of the London Mathematical Society},
   VOLUME = {26},
     YEAR = {1994},
   NUMBER = {1},
    PAGES = {97--101},
     ISSN = {0024-6093},
    CODEN = {LMSBBT},
}


@article {Grindlinger66,
    AUTHOR = {Grindlinger, M.},
     TITLE = {The problem of conjugacy and coincidence with an anticenter in
              the theory of groups},
   JOURNAL = {Sibirsk. Mat. \u Z.},
    VOLUME = {7},
      YEAR = {1966},
     PAGES = {785--803},
   MRCLASS = {20.10},
  MRNUMBER = {33 \#7406},
MRREVIEWER = {P. M. Cohn},
}


@article {GreendlingerWord60,
   AUTHOR = {Greendlinger, Martin},
    TITLE = {Dehn's algorithm for the word problem},
  JOURNAL = {Comm. Pure Appl. Math.},
   VOLUME = {13},
     YEAR = {1960},
    PAGES = {67--83},
}



@article {GreendlingerConjugacy60,
   AUTHOR = {Greendlinger, Martin},
    TITLE = {On {D}ehn's algorithms for the conjugacy and word problems,
             with applications},
  JOURNAL = {Comm. Pure Appl. Math.},
   VOLUME = {13},
     YEAR = {1960},
    PAGES = {641--677},
}

@article {Rips82,
   AUTHOR = {Rips, E.},
    TITLE = {Subgroups of small cancellation groups},
  JOURNAL = {Bull. Lond. Math. Soc.},
 FJOURNAL = {The Bulletin of the London Mathematical Society},
   VOLUME = {14},
     YEAR = {1982},
   NUMBER = {1},
    PAGES = {45--47},
     ISSN = {0024-6093},
    CODEN = {LMSBBT},
}


@article {CullerShalen84,
   AUTHOR = {Culler, M. and Shalen, P. B.},
    TITLE = {Bounded, separating, incompressible surfaces in knot manifolds},
  JOURNAL = {Invent. Math.},
 FJOURNAL = {Inventiones Mathematicae},
   VOLUME = {75},
     YEAR = {1984},
   NUMBER = {3},
    PAGES = {537--545},
     ISSN = {0020-9910},
    CODEN = {INVMBH},
}



@article {RibesZalesskii93,
   AUTHOR = {Ribes, Luis and Zalesskii, Pavel A.},
    TITLE = {On the profinite topology on a free group},
  JOURNAL = {Bull. London Math. Soc.},
 FJOURNAL = {The Bulletin of the London Mathematical Society},
   VOLUME = {25},
     YEAR = {1993},
   NUMBER = {1},
    PAGES = {37--43},
     ISSN = {0024-6093},
    CODEN = {LMSBBT},
}




@article {MeierVanWyk95,
   AUTHOR = {Meier, John and VanWyk, Leonard},
    TITLE = {The {B}ieri-{N}eumann-{S}trebel invariants for graph groups},
  JOURNAL = {Proc. London Math. Soc. (3)},
 FJOURNAL = {Proceedings of the London Mathematical Society. Third Series},
   VOLUME = {71},
     YEAR = {1995},
   NUMBER = {2},
    PAGES = {263--280},
     ISSN = {0024-6115},
    CODEN = {PLMTAL},
}



@article {BieriNeumannStrebel87,
   AUTHOR = {Bieri, Robert and Neumann, Walter D. and Strebel, Ralph},
    TITLE = {A geometric invariant of discrete groups},
  JOURNAL = {Invent. Math.},
 FJOURNAL = {Inventiones Mathematicae},
   VOLUME = {90},
     YEAR = {1987},
   NUMBER = {3},
    PAGES = {451--477},
     ISSN = {0020-9910},
    CODEN = {INVMBH},
}



@INCOLLECTION {BaumslagProblems74,
   AUTHOR = {Baumslag, Gilbert},
    TITLE = {Some problems on one-relator groups},
BOOKTITLE = {Proceedings of the Second International Conference on the
             Theory of Groups (Australian Nat. Univ., Canberra, 1973)},
PUBLISHER = {Springer},
     YEAR = {1974},
    volume = {372},
    Series = {Lecture Notes in Math.},
    PAGES = {75--81},
  ADDRESS = {Berlin},
}



@incollection {BieriStrebelCoherentSolvable79,
   AUTHOR = {Bieri, Robert and Strebel, Ralph},
    TITLE = {Soluble groups with coherent group rings},
BOOKTITLE = {Homological group theory (Proc. Sympos., Durham, 1977)},
    PAGES = {235--240},
PUBLISHER = {Cambridge Univ. Press},
  ADDRESS = {Cambridge},
     YEAR = {1979},
}

@article {MR48:6252,
   AUTHOR = {Baumslag, Gilbert},
    TITLE = {A finitely presented solvable group that is not residually
             finite},
  JOURNAL = {Math. Z.},
   VOLUME = {133},
     YEAR = {1973},
    PAGES = {125--127},
}
@article {BaumslagFreebyZ72,
   AUTHOR = {Baumslag, Gilbert},
    TITLE = {A non-cyclic, locally free, free-by-cyclic group all of whose
             finite factor groups are cyclic},
  JOURNAL = {Bull. Austral. Math. Soc.},
   VOLUME = {6},
     YEAR = {1972},
    PAGES = {313--314},
}

@article {Baumslag71b,
   AUTHOR = {Baumslag, Gilbert},
    TITLE = {Finitely generated cyclic extensions of free groups are
             residually finite},
  JOURNAL = {Bull. Austral. Math. Soc.},
   VOLUME = {5},
     YEAR = {1971},
    PAGES = {87--94},
}

@article {Baumslag71,
   AUTHOR = {Baumslag, Gilbert},
    TITLE = {Positive one-relator groups},
  JOURNAL = {Trans. Amer. Math. Soc.},
   VOLUME = {156},
     YEAR = {1971},
    PAGES = {165--183},
}

@article {Baumslag69,
   AUTHOR = {Baumslag, Gilbert},
    TITLE = {A non-cyclic one-relator group all of whose finite quotients
             are cyclic},
  JOURNAL = {J. Austral. Math. Soc.},
   VOLUME = {10},
     YEAR = {1969},
    PAGES = {497--498},
}



@article {Baumslag63b,
   AUTHOR = {Baumslag, Gilbert},
    TITLE = {On the residual finiteness of generalised free products of
             nilpotent groups},
  JOURNAL = {Trans. Amer. Math. Soc.},
   VOLUME = {106},
     YEAR = {1963},
    PAGES = {193--209},
  MRCLASS = {20.52},
 MRNUMBER = {26 #2489},
   MRREVR = {Hanna Neumann},
}

@Article{Humphries94,
  author =   {S. P. Humphries},
  title =    {On Representations of {Artin} Groups and the {Tits}
                  Conjecture},
  journal =      {J. Algebra},
  year =     {1994},
  volume =   {169},
  pages =    {847--862}
}

@ARTICLE{AlonsoBridson95,
   author = {Alonso, Juan M. and Bridson, Martin R.},
   title = {Semihyperbolic groups},
   journal = {Proc. London Math. Soc. (3)},
   year = {1995},
   volume = {70},
   pages = {56--114},
}


@article {BallmannBuyalo96,
   AUTHOR = {Ballmann, W. and Buyalo, S.},
    TITLE = {Nonpositively curved metrics on $2$-polyhedra},
  JOURNAL = {Math. Z.},
 FJOURNAL = {Mathematische Zeitschrift},
   VOLUME = {222},
     YEAR = {1996},
   NUMBER = {1},
    PAGES = {97--134},
     ISSN = {0025-5874},
    CODEN = {MAZEAX},
  MRCLASS = {53C23 (20F32 53C45 57S25)},
 MRNUMBER = {97c:53063},
   MRREVR = {Athanase Papadopoulos},
}

@article {HillPrideVella84,
   AUTHOR = {Hill, Pat and Pride, Stephen J. and Vella, Alfred D.},
    TITLE = {Subgroups of small cancellation groups},
  JOURNAL = {J. Reine Angew. Math.},
 FJOURNAL = {Journal f\"ur die Reine und Angewandte Mathematik},
   VOLUME = {349},
     YEAR = {1984},
    PAGES = {24--54},
     ISSN = {0075-4102},
    CODEN = {JRMAA8},
  MRCLASS = {20F06},
 MRNUMBER = {85m:20052},
   MRREVR = {J. S. Birman},
}

@article {Zuk96,
   AUTHOR = {{\.Z}uk, Andrzej},
    TITLE = {La propri\'et\'e ({T}) de {K}azhdan pour les groupes agissant
             sur les poly\`edres},
  JOURNAL = {C. R. Acad. Sci. Paris S\'er. I Math.},
 FJOURNAL = {Comptes Rendus de l'Acad\'emie des Sciences. S\'erie I.
             Math\'ematique},
   VOLUME = {323},
     YEAR = {1996},
   NUMBER = {5},
    PAGES = {453--458},
     ISSN = {0764-4442},
    CODEN = {CASMEI},
  MRCLASS = {22D10 (15A18 57M07)},
 MRNUMBER = {97i:22001},
   MRREVR = {Alain Valette},
}



@article {CartwrightMotkowskiSteger94,
   AUTHOR = {Cartwright, D. I. and M{\l}otkowski, W. and Steger, T.},
    TITLE = {Property ({T}) and $\tilde{{A}\sb 2}$ groups},
  JOURNAL = {Ann. Inst. Fourier (Grenoble)},
 FJOURNAL = {Universit\'e de Grenoble. Annales de l'Institut Fourier},
   VOLUME = {44},
     YEAR = {1994},
   NUMBER = {1},
    PAGES = {213--248},
     ISSN = {0373-0956},
    CODEN = {AIFUA7},
  MRCLASS = {20E42 (22D10 22E40 43A99 51E24)},
 MRNUMBER = {95j:20024},
   MRREVR = {Alain Valette},
}

@article {HillPrideVella85,
   AUTHOR = {Hill, P. and Pride, S.~J. and Vella, A.~D.},
    TITLE = {On the ${T}(q)$-conditions of small cancellation theory},
  JOURNAL = {Israel J. Math.},
 FJOURNAL = {Israel Journal of Mathematics},
   VOLUME = {52},
     YEAR = {1985},
   NUMBER = {4},
    PAGES = {293--304},
     ISSN = {0021-2172},
    CODEN = {ISJMAP},
  MRCLASS = {20F06 (05C25 20F32)},
 MRNUMBER = {88a:20045},
   MRREVR = {Ian M. Chiswell},
}


@article {Juhasz89,
   AUTHOR = {Juh{\'a}sz, A.},
    TITLE = {Small cancellation theory with a unified small cancellation
             condition. {I}},
  JOURNAL = {J. London Math. Soc. (2)},
 FJOURNAL = {The Journal of the London Mathematical Society. Second Series},
   VOLUME = {40},
     YEAR = {1989},
   NUMBER = {1},
    PAGES = {57--80},
     ISSN = {0024-6107},
    CODEN = {JLMSAK},
  MRCLASS = {20F06},
 MRNUMBER = {90j:20072},
   MRREVR = {Martin Edjvet},
}

@article {NeumannBNeumannH53,
   AUTHOR = {Neumann, B. H. and Neumann, Hanna},
    TITLE = {A contribution to the embedding theory of group amalgams},
  JOURNAL = {Proc. London Math. Soc. (3)},
   VOLUME = {3},
     YEAR = {1953},
    PAGES = {243--256},
  MRCLASS = {20.0X},
 MRNUMBER = {15,286f},
   MRREVR = {D. G. Higman},
}

@ARTICLE{BF92,
   author = {Bestvina, M. and Feighn, M.},
   title = {A combination theorem for negatively curved groups},
   journal = {J. Differential Geom.},
   year = {1992},
   volume = {35},
   number = {1},
   pages = {85--101},
}



@article {KarrassSolitar70,
   AUTHOR = {Karrass, A. and Solitar, D.},
    TITLE = {The subgroups of a free product of two groups with an
             amalgamated subgroup},
  JOURNAL = {Trans. Amer. Math. Soc.},
   VOLUME = {150},
     YEAR = {1970},
    PAGES = {227--255},
}

@article {KarrassSolitar71,
   AUTHOR = {Karrass, A. and Solitar, D.},
    TITLE = {The free product of two groups with a malnormal amalgamated
             subgroup},
  JOURNAL = {Canad. J. Math.},
   VOLUME = {23},
     YEAR = {1971},
    PAGES = {933--959},
}



@ARTICLE{BKS87,
   author = {Burns, R. G. and Karrass, A. and Solitar, D.},
   title = {A note on groups with separable finitely generated subgroups},
   journal = {Bull. Austral. Math. Soc.},
   year = {1987},
   volume = {36},
   number = {1},
   pages = {153--160},
}

@ARTICLE{Bonahon86,
   author = {Bonahon, Francis},
   title = {Bouts des vari\'et\'es hyperboliques de dimension $3$},
   journal = {Ann. of Math. (2)},
   year = {1986},
   volume = {124},
   number = {1},
   pages = {71--158},
}

@ARTICLE{Bridson95,
   author = {Bridson, Martin R.},
   title = {On the existence of flat planes in spaces of nonpositive
             curvature},
   journal = {Proc. Amer. Math. Soc.},
   year = {1995},
   volume = {123},
   number = {1},
   pages = {223--235},
}

@ARTICLE{BridsonWise,
   AUTHOR = {Bridson, Martin R. and Wise, Daniel T.},
    TITLE = {{$\mathcal{V}\mathcal {H}$} complexes, towers and subgroups of
             {${F}\times {F}$}},
  JOURNAL = {Math. Proc. Cambridge Philos. Soc.},
 FJOURNAL = {Mathematical Proceedings of the Cambridge Philosophical
             Society},
   VOLUME = {126},
     YEAR = {1999},
   NUMBER = {3},
    PAGES = {481--497},
     ISSN = {0305-0041},
    CODEN = {MPCPCO},
  MRCLASS = {20F05},
 MRNUMBER = {2000c:20050},
   MRREVR = {Eric Lewis Swenson},
}



@ARTICLE{BS62,
   author = {Baumslag, Gilbert and Solitar, Donald},
   title = {Some two-generator one-relator non-{H}opfian groups},
   journal = {Bull. Amer. Math. Soc.},
   year = {1962},
   volume = {68},
   pages = {199--201},
}

@ARTICLE{Canary96,
   author = {Canary, Richard D.},
   title = {A covering theorem for hyperbolic $3$-manifolds and its
             applications},
   journal = {Topology},
   year = {1996},
   volume = {35},
   number = {3},
   pages = {751--778},
}

@ARTICLE{CooperLongReid97,
   author = {Cooper, D. and Long, D. D. and Reid, A. W.},
   title = {Essential closed surfaces in bounded $3$-manifolds},
   journal = {J. Amer. Math. Soc.},
   year = {1997},
   volume = {10},
   number = {3},
   pages = {553--563},
}

@ARTICLE{Delzant96,
   author = {Delzant, Thomas},
   title = {Sous-groupes distingu\'es et quotients des groupes
             hyperboliques},
   journal = {Duke Math. J.},
   year = {1996},
   volume = {83},
   number = {3},
   pages = {661--682},
}

@ARTICLE{Gersten81,
   author = {Gersten, S. M.},
   title = {Coherence in doubled groups},
   journal = {Comm. Algebra},
   year = {1981},
   volume = {9},
   number = {18},
   pages = {1893--1900},
}



@ARTICLE{Gitik97,
   author = {Gitik, Rita},
   title = {Graphs and separability properties of groups},
   journal = {J. Algebra},
   year = {1997},
   volume = {188},
   number = {1},
   pages = {125--143},
}

@ARTICLE{GitikRips95,
   author = {Gitik, Rita and Rips, Eliyahu},
   title = {On separability properties of groups},
   journal = {Internat. J. Algebra Comput.},
   year = {1995},
   volume = {5},
   number = {6},
   pages = {703--717},
}

@ARTICLE{Hall49,
   author = {Hall, Jr., Marshall},
   title = {Coset representations in free groups},
   journal = {Trans. Amer. Math. Soc.},
   year = {1949},
   volume = {67},
   pages = {421--432},
}



@ARTICLE{HsuWiseGraphProducts,
   AUTHOR = {Hsu, Tim and Wise, Daniel T.},
    TITLE = {On linear and residual properties of graph products},
  JOURNAL = {Michigan Math. J.},
 FJOURNAL = {The Michigan Mathematical Journal},
   VOLUME = {46},
     YEAR = {1999},
   NUMBER = {2},
    PAGES = {251--259},
     ISSN = {0026-2285},
  MRCLASS = {20Fxx (05C25)},
 MRNUMBER = {1 704 150},
}

@ARTICLE{HW98,
   author = {Hsu, Tim and Wise, Daniel T.},
   title = {Embedding theorems for non-positively curved polygons of finite
             groups},
   journal = {J. Pure Appl. Algebra},
   year = {1998},
   volume = {123},
   number = {1-3},
   pages = {201--221},
}

@article {NibloRoller98,
    AUTHOR = {Niblo, Graham A. and Roller, Martin A.},
     TITLE = {Groups acting on cubes and {K}azhdan's property ({T})},
   JOURNAL = {Proc. Amer. Math. Soc.},
  FJOURNAL = {Proceedings of the American Mathematical Society},
    VOLUME = {126},
      YEAR = {1998},
    NUMBER = {3},
     PAGES = {693--699},
      ISSN = {0002-9939},
     CODEN = {PAMYAR},
   MRCLASS = {20F32 (05C25 22D10 57M07)},
  MRNUMBER = {98k:20058},
MRREVIEWER = {Alain Valette},
}



@ARTICLE{LN91,
   author = {Long, D. D. and Niblo, G. A.},
   title = {Subgroup separability and $3$-manifold groups},
   journal = {Math. Z.},
   year = {1991},
   volume = {207},
   number = {2},
   pages = {209--215},
}

@article {NibloReeves98,
   AUTHOR = {Niblo, G. A. and Reeves, L. D.},
    TITLE = {The geometry of cube complexes and the complexity of their
             fundamental groups},
  JOURNAL = {Topology},
 FJOURNAL = {Topology. An International Journal of Mathematics},
   VOLUME = {37},
     YEAR = {1998},
   NUMBER = {3},
    PAGES = {621--633},
     ISSN = {0040-9383},
    CODEN = {TPLGAF},
}


@ARTICLE{Long87,
   author = {Long, D. D.},
   title = {Immersions and embeddings of totally geodesic surfaces},
   journal = {Bull. London Math. Soc.},
   year = {1987},
   volume = {19},
   number = {5},
   pages = {481--484},
}

@ARTICLE{Long88,
   author = {Long, D. D.},
   title = {Engulfing and subgroup separability for hyperbolic groups},
   journal = {Trans. Amer. Math. Soc.},
   year = {1988},
   volume = {308},
   number = {2},
   pages = {849--859},
}




@article {Malcev40,
   AUTHOR = {Malcev, A.},
    TITLE = {On isomorphic matrix representations of infinite groups},
  JOURNAL = {Rec. Math. [Mat. Sbornik] N.S.},
   VOLUME = {8 (50)},
     YEAR = {1940},
    PAGES = {405--422},
    NOTE = {English transl. in: Amer. Math. Soc. Transl. (2) {\bf{45}}, 1--18 (1965) },
}


@article {Malcev83,
   AUTHOR = {Malc{'}ev, A. I.},
    TITLE = {On homomorphisms onto finite groups},
  JOURNAL = {Uchen. Zap. Ivanov Gos. Ped. Inst.},
   VOLUME = {18},
     YEAR = {1956},
    PAGES = {49--60},
    NOTE = {English transl. in: Amer. Math. Soc. Transl. (2) {\bf{119}}, 67--79 (1983) },
}



@ARTICLE{Menasco84,
   author = {Menasco, W.},
   title = {Closed incompressible surfaces in alternating knot and link
             complements},
   journal = {Topology},
   year = {1984},
   volume = {23},
   number = {1},
   pages = {37--44},
}

@ARTICLE{Meskin72,
   author = {Meskin, Stephen},
   title = {Nonresidually finite one-relator groups},
   journal = {Trans. Amer. Math. Soc.},
   year = {1972},
   volume = {164},
   pages = {105--114},
}

@ARTICLE{MR50:10082,
   author = {Scott, G. P.},
   title = {An embedding theorem for groups with a free subgroup of finite
             index},
   journal = {Bull. London Math. Soc.},
   year = {1974},
   volume = {6},
   pages = {304--306},
}

@ARTICLE{Niblo90,
   author = {Niblo, Graham A.},
   title = {H.{N}.{N}.\ extensions of a free group by ${\bf {Z}}$ which are
             subgroup separable},
   journal = {Proc. London Math. Soc. (3)},
   year = {1990},
   volume = {61},
   number = {1},
   pages = {18--32},
}




@article {Olshanskii92,
   AUTHOR = {Ol{'s}hanski{\u\i}, A. Yu.},
    TITLE = {Almost every group is hyperbolic},
  JOURNAL = {Internat. J. Algebra Comput.},
 FJOURNAL = {International Journal of Algebra and Computation},
   VOLUME = {2},
     YEAR = {1992},
   NUMBER = {1},
    PAGES = {1--17},
     ISSN = {0218-1967},
  MRCLASS = {20F06 (20F32)},
 MRNUMBER = {93j:20068},
   MRREVR = {Christopher W. Stark},
}



@ARTICLE{Olshanskii93,
   author = {Ol{'}shanski{\u\i}, A. Yu.},
   title = {On residualing homomorphisms and ${G}$-subgroups of hyperbolic
             groups},
   journal = {Internat. J. Algebra Comput.},
   year = {1993},
   volume = {3},
   number = {4},
   pages = {365--409},
}




@article {RubinsteinWang,
   AUTHOR = {Rubinstein, J. Hyam and Wang, Shicheng},
    TITLE = {$\pi\sb 1$-injective surfaces in graph manifolds},
  JOURNAL = {Comment. Math. Helv.},
 FJOURNAL = {Commentarii Mathematici Helvetici},
   VOLUME = {73},
     YEAR = {1998},
   NUMBER = {4},
    PAGES = {499--515},
     ISSN = {0010-2571},
    CODEN = {COMHAX},
}

@article {RubinsteinWang98,
   AUTHOR = {Rubinstein, J. Hyam and Wang, Shicheng},
    TITLE = {$\pi\sb 1$-injective surfaces in graph manifolds},
  JOURNAL = {Comment. Math. Helv.},
 FJOURNAL = {Commentarii Mathematici Helvetici},
   VOLUME = {73},
     YEAR = {1998},
   NUMBER = {4},
    PAGES = {499--515},
     ISSN = {0010-2571},
    CODEN = {COMHAX},
}



@article {Schupp73,
   AUTHOR = {Schupp, Paul E.},
    TITLE = {A survey of small cancellation theory},
BOOKTITLE = {Word problems: decision problems and the Burnside problem in
             group theory (Conf. on Decision Problems in Group Theory, Univ.
             California, Irvine, Calif. 1969; dedicated to Hanna Neumann)},
    PAGES = {569--589. Studies in Logic and the Foundations of Math., Vol.
             71},
PUBLISHER = {North-Holland},
  ADDRESS = {Amsterdam},
     YEAR = {1973},
  MRCLASS = {20F10},
 MRNUMBER = {54 #415},
   MRREVR = {Robert G. Burns},
}


@article {GMRS98,
   AUTHOR = {Gitik, Rita and Mitra, Mahan and Rips, Eliyahu and Sageev,
             Michah},
    TITLE = {Widths of subgroups},
  JOURNAL = {Trans. Amer. Math. Soc.},
 FJOURNAL = {Transactions of the American Mathematical Society},
   VOLUME = {350},
     YEAR = {1998},
   NUMBER = {1},
    PAGES = {321--329},
     ISSN = {0002-9947},
    CODEN = {TAMTAM},
}




@ARTICLE{Scott73,
   author = {Scott, G. P.},
   title = {Finitely generated $3$-manifold groups are finitely presented},
   journal = {J. London Math. Soc. (2)},
   year = {1973},
   volume = {6},
   pages = {437--440},
}

@ARTICLE{Scott78,
   author = {Scott, Peter},
   title = {Subgroups of surface groups are almost geometric},
   journal = {J. London Math. Soc. (2)},
   year = {1978},
   volume = {17},
   number = {3},
   pages = {555--565},
}

@ARTICLE{Scott85,
   author = {Scott, Peter},
   title = {Correction to: ``{S}ubgroups of surface groups are almost
             geometric'' [{J}. {L}ondon {M}ath. {S}oc. (2) {\bf 17} (1978),
             no. 3, 555--565; {M}{R} {\bf 58} \#12996]},
   journal = {J. London Math. Soc. (2)},
   year = {1985},
   volume = {32},
   number = {2},
   pages = {217--220},
}


@article {SelaHopfian,
   AUTHOR = {Sela, Zlil},
    TITLE = {Endomorphisms of hyperbolic groups. {I}. {T}he {H}opf property},
  JOURNAL = {Topology},
 FJOURNAL = {Topology. An International Journal of Mathematics},
   VOLUME = {38},
     YEAR = {1999},
   NUMBER = {2},
    PAGES = {301--321},
     ISSN = {0040-9383},
    CODEN = {TPLGAF},
}

@article {Sela99Hopf,
   AUTHOR = {Sela, Zlil},
    TITLE = {Endomorphisms of hyperbolic groups. {I}. {T}he {H}opf property},
  JOURNAL = {Topology},
 FJOURNAL = {Topology. An International Journal of Mathematics},
   VOLUME = {38},
     YEAR = {1999},
   NUMBER = {2},
    PAGES = {301--321},
     ISSN = {0040-9383},
    CODEN = {TPLGAF},
}



@article {MihalikTamePairs,
   AUTHOR = {Mihalik, Michael L.},
    TITLE = {Group extensions and tame pairs},
  JOURNAL = {Trans. Amer. Math. Soc.},
 FJOURNAL = {Transactions of the American Mathematical Society},
     ISSN = {0002-9947},
    CODEN = {TAMTAM},
    note = {To appear},
}



@incollection {Gromov93,
   AUTHOR = {Gromov, M.},
    TITLE = {Asymptotic invariants of infinite groups},
BOOKTITLE = {Geometric group theory, Vol.\ 2 (Sussex, 1991)},
    PAGES = {1--295},
PUBLISHER = {Cambridge Univ. Press},
  ADDRESS = {Cambridge},
     YEAR = {1993},
}

@ARTICLE{ScottCore73,
   author = {Scott, G. P.},
   title = {Compact submanifolds of $3$-manifolds},
   journal = {J. London Math. Soc. (2)},
   year = {1973},
   volume = {7},
   pages = {246--250},
}



@incollection {Stallings91,
   AUTHOR = {Stallings, John R.},
    TITLE = {Non-positively curved triangles of groups},
BOOKTITLE = {Group theory from a geometrical viewpoint (Trieste, 1990)},
    EDITOR = {Ghys, {\'E}. and Haefliger, A. and Verjovsky, A.},
    PAGES = {491--503},
PUBLISHER = {World Sci. Publishing},
  ADDRESS = {River Edge, NJ},
     YEAR = {1991},
}

@ARTICLE{Stallings83,
   author = {Stallings, John R.},
   title = {Topology of finite graphs},
   journal = {Invent. Math.},
   year = {1983},
   volume = {71},
   number = {3},
   pages = {551--565},
}

@ARTICLE{Stebe71,
   author = {Stebe, Peter F.},
   title = {Conjugacy separability of certain free products with
             amalgamation},
   journal = {Trans. Amer. Math. Soc.},
   year = {1971},
   volume = {156},
   pages = {119--129},
}



@article {Swarup93,
   AUTHOR = {Swarup, G. A.},
    TITLE = {Geometric finiteness and rationality},
  JOURNAL = {J. Pure Appl. Algebra},
 FJOURNAL = {Journal of Pure and Applied Algebra},
   VOLUME = {86},
     YEAR = {1993},
   NUMBER = {3},
    PAGES = {327--333},
     ISSN = {0022-4049},
    CODEN = {JPAAA2},
}

@ARTICLE{SusskindSwarup92,
   author = {Susskind, Perry and Swarup, Gadde A.},
   title = {Limit sets of geometrically finite hyperbolic groups},
   journal = {Amer. J. Math.},
   year = {1992},
   volume = {114},
   number = {2},
   pages = {233--250},
}

@ARTICLE{Thurston82,
   author = {Thurston, William P.},
   title = {Three-dimensional manifolds, {K}leinian groups and hyperbolic
             geometry},
   journal = {Bull. Amer. Math. Soc. (N.S.)},
   year = {1982},
   volume = {6},
   number = {3},
   pages = {357--381},
}

@ARTICLE{Weinbaum71,
   author = {Weinbaum, C. M.},
   title = {The word and conjugacy problems for the knot group of any tame,
             prime, alternating knot},
   journal = {Proc. Amer. Math. Soc.},
   year = {1971},
   volume = {30},
   pages = {22--26},
}



@article {Weinbaum90,
   AUTHOR = {Weinbaum, C. M.},
    TITLE = {Unique subwords in nonperiodic words},
  JOURNAL = {Proc. Amer. Math. Soc.},
 FJOURNAL = {Proceedings of the American Mathematical Society},
   VOLUME = {109},
     YEAR = {1990},
   NUMBER = {3},
    PAGES = {615--619},
     ISSN = {0002-9939},
    CODEN = {PAMYAR},
  MRCLASS = {20M05 (05A05 20F05)},
 MRNUMBER = {90k:20097},
   MRREVR = {Ian M. Chiswell},
}


@article {DuncanHowie92,
   AUTHOR = {Duncan, Andrew J. and Howie, James},
    TITLE = {Weinbaum's conjecture on unique subwords of nonperiodic words},
  JOURNAL = {Proc. Amer. Math. Soc.},
 FJOURNAL = {Proceedings of the American Mathematical Society},
   VOLUME = {115},
     YEAR = {1992},
   NUMBER = {4},
    PAGES = {947--954},
     ISSN = {0002-9939},
    CODEN = {PAMYAR},
  MRCLASS = {20F05 (20F10)},
 MRNUMBER = {92j:20027},
   MRREVR = {Martin Edjvet},
}


@article {Baumslag63,
   AUTHOR = {Baumslag, Gilbert},
    TITLE = {Automorphism groups of residually finite groups},
  JOURNAL = {J. London Math. Soc.},
   VOLUME = {38},
     YEAR = {1963},
    PAGES = {117--118},
}

@ARTICLE{Wise96,
   author = {Wise, Daniel T.},
   title = {A non-{H}opfian automatic group},
   journal = {J. Algebra},
   year = {1996},
   volume = {180},
   number = {3},
   pages = {845--847},
}




@ARTICLE{Wise98,
   author = {Wise, Daniel T.},
   title = {Incoherent negatively curved groups},
   journal = {Proc. Amer. Math. Soc.},
   year = {1998},
   volume = {126},
   number = {4},
   pages = {957--964},
}



@article {WiseDescending,
   AUTHOR = {Wise, Daniel T.},
    TITLE = {A continually descending endomorphism of a finitely generated
             residually finite group},
  JOURNAL = {Bull. London Math. Soc.},
 FJOURNAL = {The Bulletin of the London Mathematical Society},
   VOLUME = {31},
     YEAR = {1999},
   NUMBER = {1},
    PAGES = {45--49},
     ISSN = {0024-6093},
    CODEN = {LMSBBT},
}


@article {WiseDescending99,
   AUTHOR = {Wise, Daniel T.},
    TITLE = {A continually descending endomorphism of a finitely generated
             residually finite group},
  JOURNAL = {Bull. London Math. Soc.},
 FJOURNAL = {The Bulletin of the London Mathematical Society},
   VOLUME = {31},
     YEAR = {1999},
   NUMBER = {1},
    PAGES = {45--49},
     ISSN = {0024-6093},
    CODEN = {LMSBBT},
}



@BOOK{BridsonHaefliger,
   AUTHOR = {Bridson, Martin R. and Haefliger, Andr{\'e}},
    TITLE = {Metric spaces of non-positive curvature},
PUBLISHER = {Springer-Verlag},
  ADDRESS = {Berlin},
     YEAR = {1999},
    PAGES = {xxii+643},
     ISBN = {3-540-64324-9},
  MRCLASS = {53C23 (57Mxx)},
 MRNUMBER = {1 744 486},
}

@BOOK{LS77,
   author = {Lyndon, Roger C. and Schupp, Paul E.},
   title = {Combinatorial group theory},
   publisher = {Springer-Verlag},
   year = {1977},
   address = {Berlin},
   note = {Ergebnisse der Mathematik und ihrer Grenz\-gebiete, Band 89},
}

@BOOK{MaxDehnBook,
   author = {Dehn, Max},
   title = {Papers on group theory and topology},
   publisher = {Springer-Verlag, New York-Berlin},
   year = {1987},
   note = {Translated from the German and with introductions and an
             appendix by John Stillwell,
             With an appendix by Otto Schreier},
}

@BOOK{MKS66,
   author = {Magnus, Wilhelm and Karrass, Abraham and Solitar, Donald},
   title = {Combinatorial group theory: {P}resentations of groups in terms
             of generators and relations},
   publisher = {Interscience Publishers [John Wiley \& Sons, Inc.], New
             York-London-Sydney},
   year = {1966},
}



@article {Lyndon50,
   AUTHOR = {Lyndon, Roger C.},
    TITLE = {Cohomology theory of groups with a single defining relation},
  JOURNAL = {Ann. of Math. (2)},
   VOLUME = {52},
     YEAR = {1950},
    PAGES = {650--665},
  MRCLASS = {20.0X},
 MRNUMBER = {13,819b},
   MRREVR = {B. Eckmann},
}



@article {Magnus30,
   AUTHOR = {Magnus, Wilhelm},
    TITLE = {\"{U}ber diskontinuierliche {G}ruppen mit einer definierenden {R}elation
             ({D}er {F}reiheitssatz)},
  JOURNAL = {J. Reine Angew. Math.},
   VOLUME = {163},
     YEAR = {1930},
    PAGES = {141--165},
}

@article {Swan69,
   AUTHOR = {Swan, Richard G.},
    TITLE = {Groups of cohomological dimension one},
  JOURNAL = {J. Algebra},
   VOLUME = {12},
     YEAR = {1969},
    PAGES = {585--610},
}



@BOOK{Neuwirth65,
   author = {Neuwirth, L. P.},
   title = {Knot groups},
   publisher = {Princeton University Press},
   year = {1965},
   address = {Princeton, N.J.},
   note = {Annals of Mathematics Studies, No. 56},
}

@BOOK{RatcliffeBook,
   author = {Ratcliffe, John G.},
   title = {Foundations of hyperbolic manifolds},
   publisher = {Springer-Verlag},
   year = {1994},
   volume = {149},
   series = {Graduate Texts in Mathematics},
   address = {New York},
}

@BOOK{Robinson96,
   author = {Robinson, Derek J. S.},
   title = {A course in the theory of groups},
   publisher = {Springer-Verlag},
   year = {1996},
   volume = {80},
   series = {Graduate Texts in Mathematics},
   address = {New York},
   edition = {Second},
}

@BOOK{RolfsenBook,
   author = {Rolfsen, Dale},
   title = {Knots and links},
   publisher = {Publish or Perish Inc.},
   year = {1990},
   volume = {7},
   series = {Mathematics Lecture Series},
   address = {Houston, TX},
   note = {Corrected reprint of the 1976 original},
}

@BOOK{Serre80,
   author = {Serre, Jean-Pierre},
   title = {Trees},
   publisher = {Springer-Verlag},
   year = {1980},
   address = {Berlin},
   note = {Translated from the French by John Stillwell},
}

@BOOK{ThurstonBook,
   author = {Thurston, William P.},
   title = {Three-dimensional geometry and topology. {V}ol. 1},
   publisher = {Princeton University Press},
   year = {1997},
   volume = {35},
   series = {Princeton Mathematical Series},
   address = {Princeton, NJ},
   note = {Edited by Silvio Levy},
}




@article {Bogley91,
   AUTHOR = {Bogley, William A.},
    TITLE = {An identity theorem for multi-relator groups},
  JOURNAL = {Math. Proc. Cambridge Philos. Soc.},
 FJOURNAL = {Mathematical Proceedings of the Cambridge Philosophical
             Society},
   VOLUME = {109},
     YEAR = {1991},
   NUMBER = {2},
    PAGES = {313--321},
     ISSN = {0305-0041},
    CODEN = {MPCPCO},
  MRCLASS = {20F05 (20F32 57M20)},
 MRNUMBER = {92c:20056},
   MRREVR = {Ian M. Chiswell},
}

@incollection {BogleyPride93,
   AUTHOR = {Bogley, W. A. and Pride, S. J.},
    TITLE = {Calculating generators of $\Pi\sb 2$},
BOOKTITLE = {Two-dimensional homotopy and combinatorial group theory},
    EDITOR = {Hog-Angeloni, Cynthia and Metzler, Wolfgang and Sieradski, Allen J.},
    PAGES = {157--188},
PUBLISHER = {Cambridge Univ. Press},
  ADDRESS = {Cambridge},
     YEAR = {1993},
  MRCLASS = {57M20 (55Q52)},
 MRNUMBER = {1 279 179},
}


@incollection { refkey,
author = "author",
title = "title",
booktitle = "booktitle",
publisher = "publisher",
year = "year",
editor = "optional",
chapter = "optional",
pages = "optional",
address = "optional",
month = "optional",
note = "optional",
key = "optional",
}


@book {MR95g:57006,
     TITLE = {Two-dimensional homotopy and combinatorial group theory},
    EDITOR = {Hog-Angeloni, Cynthia and Metzler, Wolfgang and Sieradski, Allen J.},
 PUBLISHER = {Cambridge University Press},
   ADDRESS = {Cambridge},
      YEAR = {1993},
     PAGES = {xii+412},
      ISBN = {0-521-44700-3},
   MRCLASS = {57M20 (19J10 20F06 20F10 20F32 55P15 55Q52 57-06)},
  MRNUMBER = {95g:57006},
MRREVIEWER = {John G. Ratcliffe},
}

@article {ChiswellCollinsHuebschmann81,
   AUTHOR = {Chiswell, Ian M. and Collins, Donald J. and Huebschmann,
             Johannes},
    TITLE = {Aspherical group presentations},
  JOURNAL = {Math. Z.},
 FJOURNAL = {Mathematische Zeitschrift},
   VOLUME = {178},
     YEAR = {1981},
   NUMBER = {1},
    PAGES = {1--36},
     ISSN = {0025-5874},
    CODEN = {MAZEAX},
  MRCLASS = {20F05 (57M05)},
 MRNUMBER = {83a:20046},
   MRREVR = {M. J. Dunwoody},
}


@incollection {Short91,
   AUTHOR = {Short, Hamish},
    TITLE = {Quasiconvexity and a theorem of {H}owson's},
BOOKTITLE = {Group theory from a geometrical viewpoint (Trieste, 1990)},
    EDITOR = {Ghys, {\'E}. and Haefliger, A. and Verjovsky, A.},
    PAGES = {168--176},
PUBLISHER = {World Sci. Publishing},
  ADDRESS = {River Edge, NJ},
     YEAR = {1991},
}

@article {GerstenShort91,
   AUTHOR = {Gersten, S. M. and Short, H.},
    TITLE = {Small cancellation theory and automatic groups. {I}{I}},
  JOURNAL = {Invent. Math.},
 FJOURNAL = {Inventiones Mathematicae},
   VOLUME = {105},
     YEAR = {1991},
   NUMBER = {3},
    PAGES = {641--662},
     ISSN = {0020-9910},
    CODEN = {INVMBH},
}

@incollection {GerstenReducible87,
   AUTHOR = {Gersten, S. M.},
    TITLE = {Reducible diagrams and equations over groups},
BOOKTITLE = {Essays in group theory},
    PAGES = {15--73},
PUBLISHER = {Springer, New York-Berlin},
     YEAR = {1987},
}

@article {Sieradski84,
   AUTHOR = {Sieradski, Allan J.},
    TITLE = {A coloring test for asphericity},
  JOURNAL = {Quart. J. Math. Oxford Ser. (2)},
 FJOURNAL = {The Quarterly Journal of Mathematics. Oxford. Second Series},
   VOLUME = {34},
     YEAR = {1983},
   NUMBER = {133},
    PAGES = {97--106},
     ISSN = {0033-5606},
    CODEN = {QJMAAT},
  MRCLASS = {57M20},
 MRNUMBER = {84g:57004},
   MRREVR = {Johannes Huebschmann},
}

@article {TakahasiChains51,
   AUTHOR = {Takahasi, Mutuo},
    TITLE = {Note on chain conditions in free groups},
  JOURNAL = {Osaka Math. J.},
   VOLUME = {3},
     YEAR = {1951},
    PAGES = {221--225},
  MRCLASS = {20.0X},
 MRNUMBER = {13,721e},
   MRREVR = {Marshall Hall},
}

@article {TakahasiLocallyFree50,
   AUTHOR = {Takahasi, Mutuo},
    TITLE = {Note on locally free groups},
  JOURNAL = {J. Inst. Polytech. Osaka City Univ. Ser. A. Math.},
   VOLUME = {1},
     YEAR = {1950},
    PAGES = {65--70},
  MRCLASS = {20.0X},
 MRNUMBER = {13,9h},
   MRREVR = {F. W. Levi},
}

@article {PrideHyperbolicComplexes88,
   AUTHOR = {Pride, Stephen J.},
    TITLE = {Star-complexes, and the dependence problems for hyperbolic
             complexes},
  JOURNAL = {Glasgow Math. J.},
 FJOURNAL = {Glasgow Mathematical Journal},
   VOLUME = {30},
     YEAR = {1988},
   NUMBER = {2},
    PAGES = {155--170},
     ISSN = {0017-0895},
    CODEN = {GLMJAS},
  MRCLASS = {20F10 (05C10 20F06 20F32 57M99)},
 MRNUMBER = {89k:20049},
   MRREVR = {James Howie},
}

@article {GerstenShort90,
   AUTHOR = {Gersten, S. M. and Short, H. B.},
    TITLE = {Small cancellation theory and automatic groups},
  JOURNAL = {Invent. Math.},
 FJOURNAL = {Inventiones Mathematicae},
   VOLUME = {102},
     YEAR = {1990},
   NUMBER = {2},
    PAGES = {305--334},
     ISSN = {0020-9910},
    CODEN = {INVMBH},
}



@article {OshikaPotyagailo98,
   AUTHOR = {Ohshika, Ken'ichi and Potyagailo, Leonid},
    TITLE = {Self-embeddings of {K}leinian groups},
  JOURNAL = {Ann. Sci. \'Ecole Norm. Sup. (4)},
 FJOURNAL = {Annales Scientifiques de l'\'Ecole Normale Sup\'erieure.
             Quatri\`eme S\'erie},
   VOLUME = {31},
     YEAR = {1998},
   NUMBER = {3},
    PAGES = {329--343},
     ISSN = {0012-9593},
    CODEN = {ASENAH},
}



@article {BBaumslag66,
   AUTHOR = {Baumslag, Benjamin},
    TITLE = {Intersections of finitely generated subgroups in free products},
  JOURNAL = {J. London Math. Soc.},
   VOLUME = {41},
     YEAR = {1966},
    PAGES = {673--679},
}


@proceedings {MR93a:20001,
     TITLE = {Group theory from a geometrical viewpoint},
 BOOKTITLE = {Proceedings of the workshop held in Trieste, March 26--April
              6, 1990},
    EDITOR = {Ghys, {\'E}. and Haefliger, A. and Verjovsky, A.},
 PUBLISHER = {World Scientific Publishing Co. Inc.},
   ADDRESS = {River Edge, NJ},
      YEAR = {1991},
     PAGES = {viii+733},
      ISBN = {981-02-0442-6},
   MRCLASS = {20-06 (00B25 57-06)},
  MRNUMBER = {93a:20001},
}

@INCOLLECTION{AitchisonRubinstein90,
   author = {Aitchison, I. R. and Rubinstein, J. H.},
   title = {An introduction to polyhedral metrics of nonpositive curvature
             on $3$-manifolds},
   booktitle = {Geometry of low-dimensional manifolds, 2 (Durham, 1989)},
   publisher = {Cambridge Univ. Press},
   year = {1990},
   pages = {127--161},
   address = {Cambridge},
}

@INCOLLECTION{BBS84,
   author = {Brunner, A. M. and Burns, R. G. and Solitar, D.},
   title = {The subgroup separability of free products of two free groups
             with cyclic amalgamation},
   booktitle = {Contributions to group theory},
   publisher = {Amer. Math. Soc.},
   year = {1984},
   volume = {33},
   series = {Contemp. Math.},
   pages = {90--115},
   address = {Providence, R.I.},
}

@INCOLLECTION{Canary94,
   author = {Canary, Richard D.},
   title = {Covering theorems for hyperbolic $3$-manifolds},
   booktitle = {Low-dimensional topology (Knoxville, TN, 1992)},
   publisher = {Internat. Press},
   year = {1994},
   series = {Conf. Proc. Lecture Notes Geom. Topology, III},
   pages = {21--30},
   address = {Cambridge, MA},
}

@INCOLLECTION{FoxProblems61,
   author = {Fox, R. H.},
   title = {Some problems in knot theory},
   booktitle = {Topology of 3-manifolds and related topics (Proc. The Univ. of
             Georgia Institute, 1961)},
   publisher = {Prentice-Hall},
   year = {1962},
   pages = {168--176},
   address = {Englewood Cliffs, N.J.},
}



@article {RipsSela94,
   AUTHOR = {Rips, E. and Sela, Z.},
    TITLE = {Structure and rigidity in hyperbolic groups. {I}},
  JOURNAL = {Geom. Funct. Anal.},
 FJOURNAL = {Geometric and Functional Analysis},
   VOLUME = {4},
     YEAR = {1994},
   NUMBER = {3},
    PAGES = {337--371},
     ISSN = {1016-443X},
}



@article {KharlampovichMyasnikov98,
   AUTHOR = {Kharlampovich, O. and Myasnikov, A.},
    TITLE = {Hyperbolic groups and free constructions},
  JOURNAL = {Trans. Amer. Math. Soc.},
 FJOURNAL = {Transactions of the American Mathematical Society},
   VOLUME = {350},
     YEAR = {1998},
   NUMBER = {2},
    PAGES = {571--613},
     ISSN = {0002-9947},
    CODEN = {TAMTAM},
}


@INCOLLECTION{Gromov87,
   author = {Gromov, M.},
   title = {Hyperbolic groups},
   booktitle = {Essays in group theory},
   publisher = {Springer},
   year = {1987},
   volume = {8},
   series = {Math. Sci. Res. Inst. Publ.},
   pages = {75--263},
   address = {New York},
}

@INCOLLECTION{Hempel84,
   author = {Hempel, John},
   title = {Residual finiteness for $3$-manifolds},
   booktitle = {Combinatorial group theory and topology (Alta,
Utah, 1984)},
   publisher = {Princeton Univ. Press, Princeton, NJ},
   year = {1987},
   pages = {379--396},
}




@incollection {NibloWiseNonEngulfing,
   AUTHOR = {Niblo, Graham A. and Wise, Daniel T.},
    TITLE = {The engulfing property for $3$-manifolds},
BOOKTITLE = {The Epstein birthday schrift},
    PAGES = {413--418 (electronic)},
PUBLISHER = {Geom. Topol., Coventry},
     YEAR = {1998},
}

@article {Corson92,
   AUTHOR = {Corson, Jon Michael},
    TITLE = {Complexes of groups},
  JOURNAL = {Proc. London Math. Soc. (3)},
 FJOURNAL = {Proceedings of the London Mathematical Society. Third Series},
   VOLUME = {65},
     YEAR = {1992},
   NUMBER = {1},
    PAGES = {199--224},
     ISSN = {0024-6115},
    CODEN = {PLMTAL},
}





@INCOLLECTION{Pride90,
   author = {Pride, Stephen J.},
   title = {Some problems in combinatorial group theory},
   booktitle = {Groups---Korea 1988 (Pusan, 1988)},
   publisher = {Springer},
   year = {1989},
   volume = {1398},
   series = {Lecture Notes in Math.},
   pages = {146--155},
   address = {Berlin},
}




@article {Gersten96Subgroups,
   AUTHOR = {Gersten, S. M.},
    TITLE = {Subgroups of word hyperbolic groups in dimension $2$},
  JOURNAL = {J. London Math. Soc. (2)},
 FJOURNAL = {The Journal of the London Mathematical Society. Second Series},
   VOLUME = {54},
     YEAR = {1996},
   NUMBER = {2},
    PAGES = {261--283},
     ISSN = {0024-6107},
    CODEN = {JLMSAK},
}





@incollection {GerstenProblems92,
   AUTHOR = {Gersten, S. M.},
    TITLE = {Problems on automatic groups},
BOOKTITLE = {Algorithms and classification in combinatorial group theory
             (Berkeley, CA, 1989)},
    PAGES = {225--232},
PUBLISHER = {Springer},
  ADDRESS = {New York},
     YEAR = {1992},
}

@proceedings {MR564417,
     TITLE = {Homological group theory},
    SERIES = {London Mathematical Society Lecture Note Series},
    VOLUME = {36},
 BOOKTITLE = {Proceedings of a {S}ymposium on {H}omological and
              {C}ombinational {T}echniques in {G}roup {T}heory held at
              {D}urham, {S}eptember, 1977},
    EDITOR = {Wall, C. T. C.},
 PUBLISHER = {Cambridge University Press, Cambridge-New York},
      YEAR = {1979},
     PAGES = {ix+394},
      ISBN = {0-521-22729-1},
   MRCLASS = {20-06 (22-06)},
  MRNUMBER = {564417},
}

@incollection {Wall79,
    TITLE = {List of problems},
BOOKTITLE = {Homological group theory (Proc. Sympos., Durham, 1977)},
    PAGES = {369--394},
   EDITOR = {Wall, C. T. C.},
PUBLISHER = {Cambridge Univ. Press},
  ADDRESS = {Cambridge},
     YEAR = {1979},
}

@INCOLLECTION{ScottWall79,
   author = {Scott, Peter and Wall, Terry},
   title = {Topological methods in group theory},
   booktitle = {Homological group theory (Proc. Sympos., Durham, 1977)},
   publisher = {Cambridge Univ. Press},
   year = {1979},
   volume = {36},
   series = {London Math. Soc. Lecture Note Ser.},
   pages = {137--203},
   address = {Cambridge},
}

@INCOLLECTION{Tretkoff91,
   author = {Tretkoff, M.},
   title = {Covering spaces, subgroup separability, and the generalized
             {M}. {H}all property},
   booktitle = {Combinatorial group theory (College Park, MD, 1988)},
   publisher = {Amer. Math. Soc.},
   year = {1990},
   volume = {109},
   series = {Contemp. Math.},
   pages = {179--191},
   address = {Providence, RI},
}

@incollection {HsuWiseSquare2,
   AUTHOR = {Hsu, Tim and Wise, Dani},
    TITLE = {A non-residually finite square of finite groups},
BOOKTITLE = {Groups St. Andrews 1997 in Bath, I},
    PAGES = {368--378},
PUBLISHER = {Cambridge Univ. Press},
  ADDRESS = {Cambridge},
     YEAR = {1999},
  MRCLASS = {20Fxx},
 MRNUMBER = {1 676 633},
}

@incollection {LearyNibloWise,
   AUTHOR = {Leary, Ian J. and Niblo, Graham A. and Wise, Daniel T.},
    TITLE = {Some free-by-cyclic groups},
BOOKTITLE = {Groups St. Andrews 1997 in Bath, II},
    PAGES = {512--516},
PUBLISHER = {Cambridge Univ. Press},
  ADDRESS = {Cambridge},
     YEAR = {1999},
  MRCLASS = {20Exx},
 MRNUMBER = {1 676 647},
}



@article {Meier94,
   AUTHOR = {Meier, John},
    TITLE = {Hopfnicity of negatively curved polygonal amalgams of finite
             groups},
  JOURNAL = {J. Pure Appl. Algebra},
 FJOURNAL = {Journal of Pure and Applied Algebra},
   VOLUME = {94},
     YEAR = {1994},
   NUMBER = {3},
    PAGES = {331--340},
     ISSN = {0022-4049},
    CODEN = {JPAAA2},
}



@incollection {Haefliger91,
   AUTHOR = {Haefliger, Andr{\'e}},
    TITLE = {Complexes of groups and orbihedra},
BOOKTITLE = {Group theory from a geometrical viewpoint (Trieste, 1990)},
    EDITOR = {Ghys, {\'E}. and Haefliger, A. and Verjovsky, A.},
    PAGES = {504--540},
PUBLISHER = {World Sci. Publishing},
  ADDRESS = {River Edge, NJ},
     YEAR = {1991},
}

@article {Meier93,
   AUTHOR = {Meier, John},
    TITLE = {Endomorphisms of discrete groups acting chamber transitively on
             affine buildings},
  JOURNAL = {Internat. J. Algebra Comput.},
 FJOURNAL = {International Journal of Algebra and Computation},
   VOLUME = {3},
     YEAR = {1993},
   NUMBER = {3},
    PAGES = {357--364},
     ISSN = {0218-1967},
}



@incollection {Brown92,
   AUTHOR = {Brown, Kenneth S.},
    TITLE = {The geometry of finitely presented infinite simple groups},
BOOKTITLE = {Algorithms and classification in combinatorial group theory
             (Berkeley, CA, 1989)},
    PAGES = {121--136},
PUBLISHER = {Springer},
  ADDRESS = {New York},
     YEAR = {1992},
}

@PHDTHESIS{GreenThesis90,
 author = {Elisabeth R. Green},
 title = {Graph Products of Groups},
 school = {University of Leeds},
 year = {1990},
}

@PHDTHESIS{Wise96Thesis,
   author = {Wise, Daniel T.},
   title = {Non-positively curved squared complexes, aperiodic tilings, and non-residually finite groups},
   school = {Princeton University},
   year = {1996},
}

@PROCEEDINGS{KirbyGabaiList,
   title = {Geometric topology},
   year = {1997},
   editor = {Kazez, William H.},
   volume = {2},
   series = {AMS/IP Studies in Advanced Mathematics},
   publisher = {American Mathematical Society},
   address = {Providence, RI},
}



@article {SelaCoHopf97,
   AUTHOR = {Sela, Zlil},
    TITLE = {Structure and rigidity in ({G}romov) hyperbolic groups and
             discrete groups in rank $1$ {L}ie groups. {I}{I}},
  JOURNAL = {Geom. Funct. Anal.},
 FJOURNAL = {Geometric and Functional Analysis},
   VOLUME = {7},
     YEAR = {1997},
   NUMBER = {3},
    PAGES = {561--593},
     ISSN = {1016-443X},
    CODEN = {GFANFB},
}




@article {BestvinaFeighn95,
   AUTHOR = {Bestvina, Mladen and Feighn, Mark},
    TITLE = {Stable actions of groups on real trees},
  JOURNAL = {Invent. Math.},
 FJOURNAL = {Inventiones Mathematicae},
   VOLUME = {121},
     YEAR = {1995},
   NUMBER = {2},
    PAGES = {287--321},
     ISSN = {0020-9910},
    CODEN = {INVMBH},
}



@incollection {Potyagailo97,
   AUTHOR = {Potyaga{\u\i}lo, L. D.},
    TITLE = {The co-{H}opf property and the embedding of {K}leinian groups
             into themselves},
BOOKTITLE = {Algebra, geometry, analysis and mathematical physics (Russian)
             (Novosibirsk, 1996)},
    PAGES = {180},
PUBLISHER = {Izdat. Ross. Akad. Nauk Sibirsk. Otdel. Inst. Mat.},
  ADDRESS = {Novosibirsk},
     YEAR = {1997},
}



@UNPUBLISHED{NBradyNotHyperbolic,
   author = {Brady, Noel},
   title = {Branched coverings of cubical complexes and subgroups of
        hyperbolic groups},
   note = {Univ. of Utah, Preprint},
   year = {1995},
}



@UNPUBLISHED{BaumslagMyasnikovRemeslenikov,
   author = {Gilbert Baumslag and Alexei Myasnikov and Vladimir Remeslennikov},
   title = {Malnormality is decidable in free groups},
   note = {preprint 1997}
   }



@article {KapovichWise,
   AUTHOR = {Kapovich, Ilya and Wise, Daniel T.},
    TITLE = {The equivalence of some residual properties of word-hyperbolic
             groups},
  JOURNAL = {J. Algebra},
 FJOURNAL = {Journal of Algebra},
   VOLUME = {223},
     YEAR = {2000},
   NUMBER = {2},
    PAGES = {562--583},
     ISSN = {0021-8693},
    CODEN = {JALGA4},
  MRCLASS = {20Fxx},
 MRNUMBER = {1 735 163},
}


@article {BridsonWiseMalnormal,
   AUTHOR = {Bridson, Martin R. and Wise, Daniel T.},
       TITLE = {Malnormality is undecidable in hyperbolic groups},
     JOURNAL = {Israel J. Math.},
 FJOURNAL = {Israel Journal of Mathematics},
 Note = {To appear},
}






@unpublished{DelzantPotyagailo,
    author={Delzant, Thomas and Potyagailo, Leonid},
      title={Small splittings of Kleinian groups and embedding properties},
      note ={preprint},
      year ={1998},
}

@UNPUBLISHED{IKapovichAscending,
   author = {Ilya Kapovich},
   title = {On mapping tori of endomorphisms of free groups},
   note = {Preprint},
   year = {1999},
}

@UNPUBLISHED{LongReid,
   author = {D.D. Long and A.W. Reid},
   title = {Separating geometrically finite subgroups of {K}leinian groups},
   note = {preprint},
}

@article {FeighnHandelCoherence,
   AUTHOR = {Feighn, Mark and Handel, Michael},
    TITLE = {Mapping tori of free group automorphisms are coherent},
  JOURNAL = {Ann. of Math. (2)},
 FJOURNAL = {Annals of Mathematics. Second Series},
   VOLUME = {149},
     YEAR = {1999},
   NUMBER = {3},
    PAGES = {1061--1077},
     ISSN = {0003-486X},
    CODEN = {ANMAAH},
  MRCLASS = {20Fxx (57-XX)},
 MRNUMBER = {1 709 311},
}

@UNPUBLISHED{McCammondWiseCoherenceold,
   author = {Jonathan P. McCammond and Daniel T. Wise},
   title = {Coherent groups and the perimeter of {$2$}-complexes},
   note = {Preprint},
   year = {1997},
}



@manual{GAP4,
  key          = "GAP",
  organization = "The GAP~Group",
  title        = "{GAP -- Groups, Algorithms, and Programming, Version 4.2}",
  year         = 1999,
  address      = "Aachen, St~Andrews",
  note         = "\verb+(http://www-gap.dcs.st-and.ac.uk/~gap)+",
  keywords     = "groups; *; gap; manual"
}


@article{McCammondWiseCoherence,
    AUTHOR = {McCammond, J. P. and Wise, D. T.},
     TITLE = {Coherence, local quasiconvexity, and the perimeter of
              2-complexes},
   JOURNAL = {Geom. Funct. Anal.},
  FJOURNAL = {Geometric and Functional Analysis},
    VOLUME = {15},
      YEAR = {2005},
    NUMBER = {4},
     PAGES = {859--927},
      ISSN = {1016-443X},
     CODEN = {GFANFB},
   MRCLASS = {20Fxx},
  MRNUMBER = {MR2221153},
}


@article {McCammondWiseFanLadder,
    AUTHOR = {McCammond, Jonathan P. and Wise, Daniel T.},
     TITLE = {Fans and ladders in small cancellation theory},
   JOURNAL = {Proc. London Math. Soc. (3)},
  FJOURNAL = {Proceedings of the London Mathematical Society. Third Series},
    VOLUME = {84},
      YEAR = {2002},
    NUMBER = {3},
     PAGES = {599--644},
      ISSN = {0024-6115},
     CODEN = {PLMTAL},
   MRCLASS = {20F06},
  MRNUMBER = {1 888 425},
}


@UNPUBLISHED{McCammondWiseCoherenceI,
   author = {Jonathan P. McCammond and Daniel T. Wise},
   title = {The perimeter of {$2$}-complexes {I}: Coherence},
   note = {Preprint},
   year = {1998},
}

@UNPUBLISHED{McCammondWiseCoherenceII,
   author = {Jonathan P. McCammond and Daniel T. Wise},
   title = {The perimeter of {$2$}-complexes {II}: Local quasiconvexity},
   note = {In preparation},
}

@article{McCammondWiseOneRelator,
    AUTHOR = {McCammond, Jon and Wise, Daniel},
     TITLE = {Windmills and extreme 2-cells},
   JOURNAL = {Illinois J. Math.},
  FJOURNAL = {Illinois Journal of Mathematics},
    VOLUME = {54},
      YEAR = {2010},
    NUMBER = {1},
     PAGES = {69--87},
      ISSN = {0019-2082},
   MRCLASS = {20F67 (57M07)},
  MRNUMBER = {2776985},
MRREVIEWER = {Robert W. Bell},
       URL = {http://projecteuclid.org.proxy3.library.mcgill.ca/euclid.ijm/1299679738},
}



@article {Shalen98,
    AUTHOR = {Shalen, Peter B.},
     TITLE = {Three-manifolds and {B}aumslag-{S}olitar groups},
      NOTE = {Geometric topology and geometric group theory (Milwaukee, WI,
              1997)},
   JOURNAL = {Topology Appl.},
  FJOURNAL = {Topology and its Applications},
    VOLUME = {110},
      YEAR = {2001},
    NUMBER = {1},
     PAGES = {113--118},
      ISSN = {0166-8641},
     CODEN = {TIAPD9},
   MRCLASS = {57M05 (20F05 57N10)},
  MRNUMBER = {2001j:57002},
MRREVIEWER = {Stephen J. Pride},
}


@UNPUBLISHED{ThurstonNotes,
   author = {Thurston, William P.},
   title = {The geometry and topology of $3$-manifolds},
   note = {Lecture Notes},
}

@article{WiseCycHNN,
   AUTHOR = {Wise, Daniel T.},
    TITLE = {Subgroup separability of graphs of free groups with cyclic edge
             groups},
  JOURNAL = {Q. J. Math.},
 FJOURNAL = {The Quarterly Journal of Mathematics},
   VOLUME = {51},
     YEAR = {2000},
   NUMBER = {1},
    PAGES = {107--129},
     ISSN = {0033-5606},
  MRCLASS = {20Exx (57Mxx)},
 MRNUMBER = {1 760 573},
}


@article{WiseFigure8,
    AUTHOR = {Wise, Daniel T.},
     TITLE = {Subgroup separability of the figure 8 knot group},
   JOURNAL = {Topology},
  FJOURNAL = {Topology. An International Journal of Mathematics},
    VOLUME = {45},
      YEAR = {2006},
    NUMBER = {3},
     PAGES = {421--463},
      ISSN = {0040-9383},
     CODEN = {TPLGAF},
   MRCLASS = {57M25 (20E26 20F67 57M07)},
  MRNUMBER = {MR2218750},
MRREVIEWER = {Daan Krammer},
}


@article{WiseNoCore,
   author = {Wise, Daniel T.},
   title = {A covering space with no compact core},
   JOURNAL = {Geom. Ded.},
   FJOURNAL = {Geometriae Dedicata},
      VOLUME = {92},
     YEAR = {2002},
   NUMBER = {1},
    PAGES = {59--62},
}

@article{WiseProductRank,
   author = {Wise, Daniel T.},
   title = {The rank of a direct power of a small-cancellation group},
   JOURNAL = {Geom. Ded.},
   FJOURNAL = {Geometriae Dedicata},
   NOTE= {To appear},
}


@unpublished{HsuWiseAscendingPolycyclic,
   author = {Tim Hsu and Daniel T. Wise},
   title = {The residual finiteness of ascending {HNN} extensions of polycyclic groups},
   note = {Preprint 2001},
}

@article{HsuWiseSeparatingGraphGroups,
    AUTHOR = {Hsu, Tim and Wise, Daniel T.},
     TITLE = {Separating quasiconvex subgroups of right-angled {A}rtin
              groups},
   JOURNAL = {Math. Z.},
  FJOURNAL = {Mathematische Zeitschrift},
    VOLUME = {240},
      YEAR = {2002},
    NUMBER = {3},
     PAGES = {521--548},
      ISSN = {0025-5874},
     CODEN = {MAZEAX},
   MRCLASS = {20F36},
  MRNUMBER = {1 924 020},
}

@article {WisePolygons,
   author = {Wise, Daniel T.},
   title = {The residual finiteness of negatively curved polygons of finite groups},
  JOURNAL = {Invent. Math.},
 FJOURNAL = {Inventiones Mathematicae},
   VOLUME = {149},
     YEAR = {2002},
   NUMBER = {3},
    PAGES = {579--617},
}


@article{WiseSmallCanCube04,
    author={Wise, Daniel T.},
    title={Cubulating small cancellation groups},
    JOURNAL={GAFA, Geom. Funct. Anal.},
    VOLUME={14},
    YEAR={2004},
    NUMBER={1},
    PAGES={150--214},
    }






@article{WiseRFRips,
    AUTHOR = {Wise, Daniel T.},
     TITLE = {A residually finite version of {R}ips's construction},
   JOURNAL = {Bull. London Math. Soc.},
  FJOURNAL = {The Bulletin of the London Mathematical Society},
    VOLUME = {35},
      YEAR = {2003},
    NUMBER = {1},
     PAGES = {23--29},
      ISSN = {0024-6093},
     CODEN = {LMSBBT},
   MRCLASS = {20E26 (20E22 20F06)},
  MRNUMBER = {2003g:20047},
MRREVIEWER = {Dennis Spellman},
}



@UNPUBLISHED{WiseSmall,
   author = {Wise, Daniel T.},
   title = {Residually finite small cancellation groups},
   note = {In preparation},
}

@UNPUBLISHED{Wise3Conjugation,
   author = {Daniel T. Wise},
   title = {Conjugating  subgroups of $3$-manifold groups},
   note = {In preparation},
}



@article{DMeier82,
   AUTHOR = {Meier, David},
    TITLE = {Non-{H}opfian groups},
  JOURNAL = {J. London Math. Soc. (2)},
 FJOURNAL = {The Journal of the London Mathematical Society. Second Series},
   VOLUME = {26},
     YEAR = {1982},
   NUMBER = {2},
    PAGES = {265--270},
     ISSN = {0024-6107},
    CODEN = {JLMSAK},
}


@article{SapirWiseAscending,
   author = {Mark Sapir and Daniel T. Wise},
   title = {Non-residually finite ascending {H}{N}{N} extensions},
   JOURNAL = {J. Pure Appl. Algebra},
   note = {To appear},
}

@UNPUBLISHED{SapirRFofFreeAscending,
   author = {Mark Sapir},
   title = {Topological dynamics of polynomial maps over p-adic numbers and
residual finiteness of ascending {HNN} extensions},
   note = {In preparation},
}

@article{GeogheganMihalikSapirWise99,
    AUTHOR = {Geoghegan, Ross and Mihalik, Michael L. and Sapir, Mark and
              Wise, Daniel T.},
     TITLE = {Ascending {H}{N}{N} extensions of finitely generated free
              groups are {H}opfian},
   JOURNAL = {Bull. London Math. Soc.},
  FJOURNAL = {The Bulletin of the London Mathematical Society},
    VOLUME = {33},
      YEAR = {2001},
    NUMBER = {3},
     PAGES = {292--298},
      ISSN = {0024-6093},
     CODEN = {LMSBBT},
   MRCLASS = {20E06},
  MRNUMBER = {1 817 768},
}



@UNPUBLISHED{WiseNonHopfAscending,
   author = {Daniel T. Wise},
   title = {A non-{H}opfian ascending {H}{N}{N} extension of a residually finite group},
   note = {Preprint},
}

@UNPUBLISHED{GMT96,
   author = {D.~Gabai and G.R.Meryhoff and N.Thurston},
   title = {Homotopy hyperbolic $3$-manifolds are hyperbolic},
   year = {1996},
   note = {Preprint},
}



@article {Grigorchuk98,
   AUTHOR = {Grigorchuk, R. I.},
    TITLE = {An example of a finitely presented amenable group that does not
             belong to the class {E}{G}},
  JOURNAL = {Mat. Sb.},
 FJOURNAL = {Rossi\u\i skaya Akademiya Nauk. Matematicheski\u\i\ Sbornik},
   VOLUME = {189},
     YEAR = {1998},
   NUMBER = {1},
    PAGES = {79--100},
     ISSN = {0368-8666},
}
@article {Grigorchuk80,
   AUTHOR = {Grigor{\v{c}}uk, R. I.},
    TITLE = {On {B}urnside's problem on periodic groups},
  JOURNAL = {Funktsional. Anal. i Prilozhen.},
 FJOURNAL = {Akademiya Nauk SSSR. Funktsional\cprime ny\u \i \ Analiz i ego
             Prilozheniya},
   VOLUME = {14},
     YEAR = {1980},
   NUMBER = {1},
    PAGES = {53--54},
     ISSN = {0374-1990},
}



@article {Lysenok85,
   AUTHOR = {Lysenok, I. G.},
    TITLE = {A set of defining relations for the {G}rigorchuk group},
  JOURNAL = {Mat. Zametki},
 FJOURNAL = {Akademiya Nauk Soyuza SSR. Matematicheskie Zametki},
   VOLUME = {38},
     YEAR = {1985},
   NUMBER = {4},
    PAGES = {503--516, 634},
     ISSN = {0025-567X},
}



@article {BestvinaBrady97,
   AUTHOR = {Bestvina, Mladen and Brady, Noel},
    TITLE = {Morse theory and finiteness properties of groups},
  JOURNAL = {Invent. Math.},
 FJOURNAL = {Inventiones Mathematicae},
   VOLUME = {129},
     YEAR = {1997},
   NUMBER = {3},
    PAGES = {445--470},
     ISSN = {0020-9910},
    CODEN = {INVMBH},
}



@article {Aumann56,
   AUTHOR = {Aumann, Robert J.},
    TITLE = {Asphericity of alternating knots},
  JOURNAL = {Ann. of Math. (2)},
   VOLUME = {64},
     YEAR = {1956},
    PAGES = {374--392},
}




@article {Baudisch81,
   AUTHOR = {Baudisch, A.},
    TITLE = {Subgroups of semifree groups},
  JOURNAL = {Acta Math. Acad. Sci. Hungar.},
 FJOURNAL = {Acta Mathematica Academiae Scientiarum Hungaricae},
   VOLUME = {38},
     YEAR = {1981},
   NUMBER = {1-4},
    PAGES = {19--28},
     ISSN = {0001-5954},
    CODEN = {ACMTAV},
}



@article {Servatius89,
   AUTHOR = {Servatius, Herman},
    TITLE = {Automorphisms of graph groups},
  JOURNAL = {J. Algebra},
 FJOURNAL = {Journal of Algebra},
   VOLUME = {126},
     YEAR = {1989},
   NUMBER = {1},
    PAGES = {34--60},
     ISSN = {0021-8693},
    CODEN = {JALGA4},
}



@article {Laurence95,
   AUTHOR = {Laurence, Michael R.},
    TITLE = {A generating set for the automorphism group of a graph group},
  JOURNAL = {J. London Math. Soc. (2)},
 FJOURNAL = {The Journal of the London Mathematical Society. Second Series},
   VOLUME = {52},
     YEAR = {1995},
   NUMBER = {2},
    PAGES = {318--334},
     ISSN = {0024-6107},
    CODEN = {JLMSAK},
}



@article {DromsSubgroups87,
   AUTHOR = {Droms, Carl},
    TITLE = {Subgroups of graph groups},
  JOURNAL = {J. Algebra},
 FJOURNAL = {Journal of Algebra},
   VOLUME = {110},
     YEAR = {1987},
   NUMBER = {2},
    PAGES = {519--522},
     ISSN = {0021-8693},
    CODEN = {JALGA4},
}



@article {DromsCoherence87,
   AUTHOR = {Droms, Carl},
    TITLE = {Graph groups, coherence, and three-manifolds},
  JOURNAL = {J. Algebra},
 FJOURNAL = {Journal of Algebra},
   VOLUME = {106},
     YEAR = {1987},
   NUMBER = {2},
    PAGES = {484--489},
     ISSN = {0021-8693},
    CODEN = {JALGA4},
  MRCLASS = {57M15 (05C25 20F05 20F32 57N10)},
 MRNUMBER = {88e:57003},
   MRREVR = {R. Z. Goldstein},
}


@article {DromsIsomorphisms87,
   AUTHOR = {Droms, Carl},
    TITLE = {Isomorphisms of graph groups},
  JOURNAL = {Proc. Amer. Math. Soc.},
 FJOURNAL = {Proceedings of the American Mathematical Society},
   VOLUME = {100},
     YEAR = {1987},
   NUMBER = {3},
    PAGES = {407--408},
     ISSN = {0002-9939},
    CODEN = {PAMYAR},
}



@article {HermillerMeier95,
   AUTHOR = {Hermiller, Susan and Meier, John},
    TITLE = {Algorithms and geometry for graph products of groups},
  JOURNAL = {J. Algebra},
 FJOURNAL = {Journal of Algebra},
   VOLUME = {171},
     YEAR = {1995},
   NUMBER = {1},
    PAGES = {230--257},
     ISSN = {0021-8693},
    CODEN = {JALGA4},
}



@article {VanWyk94,
   AUTHOR = {Van Wyk, Leonard},
    TITLE = {Graph groups are biautomatic},
  JOURNAL = {J. Pure Appl. Algebra},
 FJOURNAL = {Journal of Pure and Applied Algebra},
   VOLUME = {94},
     YEAR = {1994},
   NUMBER = {3},
    PAGES = {341--352},
     ISSN = {0022-4049},
    CODEN = {JPAAA2},
}



@article {BNeumann50,
   AUTHOR = {Neumann, B. H.},
    TITLE = {A two-generator group isomorphic to a proper factor group},
  JOURNAL = {J. London Math. Soc.},
   VOLUME = {25},
     YEAR = {1950},
    PAGES = {247--248},
}



@article {Higman51,
   AUTHOR = {Higman, Graham},
    TITLE = {A finitely related group with an isomorphic proper factor
             group},
  JOURNAL = {J. London Math. Soc.},
   VOLUME = {26},
     YEAR = {1951},
    PAGES = {59--61},
}



@article {Higman51simple,
   AUTHOR = {Higman, Graham},
    TITLE = {A finitely generated infinite simple group},
  JOURNAL = {J. London Math. Soc.},
   VOLUME = {26},
     YEAR = {1951},
    PAGES = {61--64},
}


@article {BlassNeumann74,
   AUTHOR = {Blass, Andreas and Neumann, Peter M.},
    TITLE = {An application of universal algebra in group theory},
  JOURNAL = {Michigan Math. J.},
   VOLUME = {21},
     YEAR = {1974},
    PAGES = {167--169},
}



@article {BBaumslagLevin79,
   AUTHOR = {Baumslag, Benjamin and Levin, Frank},
    TITLE = {A class of one-relator groups with torsion},
  JOURNAL = {Arch. Math. (Basel)},
 FJOURNAL = {Archiv der Mathematik. Archives of Mathematics. Archives
             Math\'ematiques},
   VOLUME = {33},
     YEAR = {1979/80},
   NUMBER = {3},
    PAGES = {209--215},
     ISSN = {0003-889X},
    CODEN = {ACVMAL},
}




@article {AllenbyTang81four,
   AUTHOR = {Allenby, R. B. J. T. and Tang, C. Y.},
    TITLE = {Residually finite one-relator groups with torsion},
  JOURNAL = {Arch. Math. (Basel)},
 FJOURNAL = {Archiv der Mathematik. Archives of Mathematics. Archives
             Math\'ematiques},
   VOLUME = {37},
     YEAR = {1981},
   NUMBER = {2},
    PAGES = {97--105},
     ISSN = {0003-889X},
    CODEN = {ACVMAL},
}

@article {AllenbyTang81commutators,
   AUTHOR = {Allenby, R. B. J. T. and Tang, C. Y.},
    TITLE = {The residual finiteness of some one-relator groups with
             torsion},
  JOURNAL = {J. Algebra},
 FJOURNAL = {Journal of Algebra},
   VOLUME = {71},
     YEAR = {1981},
   NUMBER = {1},
    PAGES = {132--140},
     ISSN = {0021-8693},
    CODEN = {JALGA4},
}



@article {AllenbyTang85,
   AUTHOR = {Allenby, R. B. J. T. and Tang, C. Y.},
    TITLE = {Residual finiteness of certain $1$-relator groups: extensions
             of results of {G}ilbert {B}aumslag},
  JOURNAL = {Math. Proc. Cambridge Philos. Soc.},
 FJOURNAL = {Mathematical Proceedings of the Cambridge Philosophical
             Society},
   VOLUME = {97},
     YEAR = {1985},
   NUMBER = {2},
    PAGES = {225--230},
     ISSN = {0305-0041},
    CODEN = {MPCPCO},
}



@incollection {Baumslag96Problems,
   AUTHOR = {Baumslag, Gilbert},
    TITLE = {Some open problems},
BOOKTITLE = {Summer School in Group Theory in Banff, 1996},
   EDITOR = {Kharlampovich, Olga},
    PAGES = {1--9},
PUBLISHER = {Amer. Math. Soc.},
  ADDRESS = {Providence, RI},
     YEAR = {1999},
}



@inproceedings {Howie87,
   AUTHOR = {Howie, James},
    TITLE = {How to generalize one-relator group theory},
BOOKTITLE = {Combinatorial group theory and topology},
    EDITOR = {Gersten, S. M. and Stallings, John R.},
    PAGES = {53--78},
PUBLISHER = {Princeton Univ. Press},
  ADDRESS = {Princeton, N.J.},
     YEAR = {1987},
}

@book {GerstenStallings87,
     TITLE = {Combinatorial group theory and topology},
    EDITOR = {Gersten, S. M. and Stallings, John R.},
      NOTE = {Papers from the conference held in Alta, Utah, July 15--18,
              1984},
 PUBLISHER = {Princeton University Press},
   ADDRESS = {Princeton, N.J.},
      YEAR = {1987},
     PAGES = {viii+552},
      ISBN = {0-691-08409-2; 0-691-08410-6},
   MRCLASS = {20-06 (57-06)},
  MRNUMBER = {88c:20005},
}


@article {HowiePride84,
   AUTHOR = {Howie, J. and Pride, S. J.},
    TITLE = {A spelling theorem for staggered generalized $2$-complexes,
             with applications},
  JOURNAL = {Invent. Math.},
 FJOURNAL = {Inventiones Mathematicae},
   VOLUME = {76},
     YEAR = {1984},
   NUMBER = {1},
    PAGES = {55--74},
     ISSN = {0020-9910},
    CODEN = {INVMBH},
}
@article {Howie81,
   AUTHOR = {Howie, James},
    TITLE = {On pairs of $2$-complexes and systems of equations over groups},
  JOURNAL = {J. Reine Angew. Math.},
 FJOURNAL = {Journal f\"ur die Reine und Angewandte Mathematik},
   VOLUME = {324},
     YEAR = {1981},
    PAGES = {165--174},
     ISSN = {0075-4102},
    CODEN = {JRMAA8},
}



@article {Newman68,
   AUTHOR = {Newman, B. B.},
    TITLE = {Some results on one-relator groups},
  JOURNAL = {Bull. Amer. Math. Soc.},
   VOLUME = {74},
     YEAR = {1968},
    PAGES = {568--571},
}



@incollection {WNeumann89,
   AUTHOR = {Neumann, Walter D.},
    TITLE = {On intersections of finitely generated subgroups of free
             groups},
BOOKTITLE = {Groups---Canberra 1989},
    PAGES = {161--170},
PUBLISHER = {Springer},
  ADDRESS = {Berlin},
     YEAR = {1990},
}



@article {Gersten87,
   AUTHOR = {Gersten, S. M.},
    TITLE = {Fixed points of automorphisms of free groups},
  JOURNAL = {Adv. in Math.},
 FJOURNAL = {Advances in Mathematics},
   VOLUME = {64},
     YEAR = {1987},
   NUMBER = {1},
    PAGES = {51--85},
     ISSN = {0001-8708},
    CODEN = {ADMTA4},
}



@article {MR92m:20017,
   AUTHOR = {Bestvina, Mladen and Handel, Michael},
    TITLE = {Train tracks and automorphisms of free groups},
  JOURNAL = {Ann. of Math. (2)},
 FJOURNAL = {Annals of Mathematics. Second Series},
   VOLUME = {135},
     YEAR = {1992},
   NUMBER = {1},
    PAGES = {1--51},
     ISSN = {0003-486X},
    CODEN = {ANMAAH},
}



@article {Golod64,
   AUTHOR = {Golod, E. S.},
    TITLE = {On nil-algebras and finitely approximable $p$-groups},
  JOURNAL = {Izv. Akad. Nauk SSSR Ser. Mat.},
   VOLUME = {28},
     YEAR = {1964},
    PAGES = {273--276},
    NOTE = {English transl. in: Amer. Math. Soc. Transl. (2) {\bf {48}}, 103--106 (1965) },
}

@article {GolodShafarevich64,
   AUTHOR = {Golod, E. S. and {\v{S}}afarevi{\v{c}}, I. R.},
    TITLE = {On the class field tower},
  JOURNAL = {Izv. Akad. Nauk SSSR Ser. Mat.},
   VOLUME = {28},
     YEAR = {1964},
    PAGES = {261--272},
    NOTE = {English transl. in: Amer. Math. Soc. Transl. (2) {\bf{48}}, 91--102 (1965) },
}




@article {Gruenberg57,
   AUTHOR = {Gruenberg, K. W.},
    TITLE = {Residual properties of infinite soluble groups},
  JOURNAL = {Proc. London Math. Soc. (3)},
   VOLUME = {7},
     YEAR = {1957},
    PAGES = {29--62},
}



@article {Stallings86,
   AUTHOR = {Stallings, John R.},
    TITLE = {Finiteness properties of matrix representations},
  JOURNAL = {Ann. of Math. (2)},
 FJOURNAL = {Annals of Mathematics. Second Series},
   VOLUME = {124},
     YEAR = {1986},
   NUMBER = {2},
    PAGES = {337--346},
     ISSN = {0003-486X},
    CODEN = {ANMAAH},
}



@article {Howson54,
   AUTHOR = {Howson, A. G.},
    TITLE = {On the intersection of finitely generated free groups},
  JOURNAL = {J. London Math. Soc.},
   VOLUME = {29},
     YEAR = {1954},
    PAGES = {428--434},
}

@article {Magnus32,
   AUTHOR = {Magnus, Wilhelm},
    TITLE = {Das {I}dentit{\"{a}}tsproblem f{\"{u}}r {G}ruppen mit einer
            definierenden {R}elation},
  JOURNAL = {Math. Ann.},
   VOLUME = {106},
     YEAR = {1932},
    PAGES = {295--307},
}

@article {Papakyriakopoulos57,
   AUTHOR = {Papakyriakopoulos, C. D.},
    TITLE = {On {D}ehn's lemma and the asphericity of knots},
  JOURNAL = {Ann. of Math. (2)},
   VOLUME = {66},
     YEAR = {1957},
    PAGES = {1--26},
  MRCLASS = {55.0X},
 MRNUMBER = {19,761a},
   MRREVR = {R. H. Fox},
}




@article {McKinsey43,
   AUTHOR = {McKinsey, J. C. C.},
    TITLE = {The decision problem for some classes of sentences without
             quantifiers},
  JOURNAL = {J. Symbolic Logic},
   VOLUME = {8},
     YEAR = {1943},
    PAGES = {61--76},
}



@incollection {HaglundPaulin98,
   AUTHOR = {Haglund, Fr{\'e}d{\'e}ric and Paulin, Fr{\'e}d{\'e}ric},
    TITLE = {Simplicit\'e de groupes d'automorphismes d'espaces \`a courbure
             n\'egative},
BOOKTITLE = {The Epstein birthday schrift},
    PAGES = {181--248 (electronic)},
PUBLISHER = {Geom. Topol., Coventry},
     YEAR = {1998},
  MRCLASS = {20E32 (20F55 20F65 51E24 57M07)},
 MRNUMBER = {2000b:20034},
   MRREVR = {Michel Coornaert},
}

@article {Yaman,
    AUTHOR = {Yaman, Asli},
     TITLE = {A topological characterisation of relatively hyperbolic
              groups},
   JOURNAL = {J. Reine Angew. Math.},
  FJOURNAL = {Journal f\"ur die Reine und Angewandte Mathematik},
    VOLUME = {566},
      YEAR = {2004},
     PAGES = {41--89},
      ISSN = {0075-4102},
     CODEN = {JRMAA8},
   MRCLASS = {20F67 (54H11)},
  MRNUMBER = {MR2039323 (2005e:20064)},
MRREVIEWER = {Jane Gilman},
}

@article {Bowditch99RH,
    AUTHOR = {Bowditch, Brian},
     TITLE = {Relatively hyperbolic
              groups},
   Year={1999},
Journal={Preprint},
Pages={1-63},
     }
	

